On the Linear Regime of the Characteristic formulation of General relativity in the Minkowski and Schwarzschild's Backgrounds

We present here the linear regime of the Einstein's field equations in the characteristic formulation. Through a simple decomposition of the metric variables in spin-weighted spherical harmonics, the field equations are expressed as a system of coupled ordinary differential equations. The process for decoupling them leads to a simple equation for $J$ - one of the Bondi-Sachs metric variables - known in the literature as the master equation. Then, this last equation is solved in terms of Bessel's functions of the first kind for the Minkowski's background, and in terms of the Heun's function in the Schwarzschild's case. In addition, when a matter source is considered, the boundary conditions across the time-like world tubes bounding the source are taken into account. These boundary conditions are computed for all multipole modes. Some examples as the point particle binaries in circular and eccentric orbits, in the Minkowski's background are shown as particular cases of this formalism.

==> docs/ADM.tex <==
\section{Arnowitt-Desser-Misner Formulations (ADM)}
In this section will be presented some of the ADM based formulations, which are the formalisms most commonly used in the numerical relativity applications. The equations and derivations needed to obtain them are presented in some detail in order to understand the differences between those ADM based formulations and the outgoing characteristic formalism. The ADM formalism are in reality a Hamiltonian formulation of the general relativity which at the end 
\graphicspath{{./Figuras/ADM/}}
\input{./docs/ADM_Formalism}
\input{./docs/BSSN_Formalism}


==> docs/ADM_Formalism.tex <==
\subsection{Arnowitt-Deser-Misner ({\it ADM}) formalism}
It is supposed that the manifold $\mathcal M$, represents the space-time, and it is associated with the metric $g_{\mu\nu}$, which is foliated into 3-dimensional space-like hypersurfaces labelled by $\Sigma$. They are orthogonal to the vector $\Omega^\mu$ (locally almost), and the intersections between them are forbidden. $\Omega^\mu$ is defined as tangent to a central time-like geodesic in the form  
\begin{equation}\label{ADM1}
\Omega_\mu= t_{;\mu}.
\end{equation}
$t$ can be interpreted as a {\it global time}. Also, this time $u$, corresponds to an affine parameter to the arc length described by the central geodesic \cite{A08_book,BS10_Book}. See the figure \ref{FADM1}
%\newpage
\graphicspath{{./Figuras/ADM/}}
\begin{figure}[h!]
	\begin{center}
		%\includegraphics[height=6cm]{./Figuras/ADM/ADM_1}
		\input{./Figuras/ADM/ADM_1.eps_tex}
		\caption{Space-time $\mathcal M$ foliated in 3D - hypersurfaces $\Sigma$.}
		\label{FADM1}
	\end{center}
\end{figure}
\\From \eqref{ADM1}, is computed the norm $\|\Omega_\mu\|$, where it is used the $g_{\mu\nu}$ 
\begin{equation}\label{ADM2}
\|\Omega_\mu\|^2= g^{\mu\nu} t_{;\mu} t_{;\nu}.
\end{equation}
It is defined a scalar function $\alpha$, namely {\it lapse function}, such that
\begin{equation}\label{ADM3}
\alpha^ 2=-\frac{1}{\|\Omega_\mu\|^2}.
\end{equation}
Thus, $\alpha > 0$, means that $\Omega^\mu$ is a time-like vector, then almost locally the hypersurfaces $\Sigma$ shall be space-like, if on other hand $\alpha < 0$, then $\Omega^\mu$ is space-like and almost locally, the hypersurfaces $\Sigma$ will be time-like. This function return the lapse of proper time $d\tau$ between two successive hypersurfaces when are measured by an {\it Eulerian observer}\footnote{Namely too {\it Normal observer}}, which are observers that are moving in normal direction to these hypersurfaces.
\\In this manner it is build a normalised and irrotational one-form $\omega_\mu=\alpha\Omega_\mu$, i.e.,
\begin{equation}\label{ADM4}
\omega_{[\nu}\omega_{\mu;\delta]}=0.
\end{equation}
%Aqui usamos a conven\c c\~ao de antissimetriza\c c\~ao
%\begin{equation}\label{ADM5}
%A_{[\alpha_{1} \cdots \alpha_{n}]}=\frac{1}{n!}\sum_{\gamma_1\cdots\gamma_n}\text{Sgn}(\gamma_1\cdots\gamma_n)\delta_{\alpha_1}^{~~\gamma_1}\cdots \delta_{\alpha_n}^{~~\gamma_n} A_{\gamma_{1} \cdots \gamma_{n}},
%\end{equation}
%onde a fun\c c\~ao Sgn \'e tal que 
%\begin{equation}\label{ADM6}
%\text{Sgn}(\gamma_1\cdots\gamma_n)=
%\begin{cases}
%1 \text{ para permuta\c c\~oes c\'iclicas dos \'indices } \gamma_1\cdots\gamma_n \\
%-1 \text{ para permuta\c c\~oes n\~ao c\'iclicas dos \'indices } \gamma_1\cdots\gamma_n.
%\end{cases}
%\end{equation}
From the 1-forms $\omega_\mu$ the normal vectors to the hypersurfaces $\Sigma$ can be build in the form,
\begin{equation}\label{ADM7}
n^\nu=-g^{\mu\nu}\omega_\mu,
\end{equation}
where the minus indicates that the vectors are appointed to the future, i.e., the sense in which $t$ increases.Also, the one-forms $\omega_\mu$ and the vectors $n^\nu$ satisfy 
\begin{equation}\label{ADM8}
n^\nu\omega_\nu=-g^{\mu\nu}\omega_\mu\omega_\nu=-1, \hspace{0.5cm} n^\nu n_\nu=1.
\end{equation}
The metric $\gamma_{\mu\nu}$ corresponding to the hypersurfaces $\Sigma$, is said as the spacial part of $g_{\mu\nu}$. Thus, 
\begin{equation}\label{ADM9}
\gamma_{\mu\nu}=g_{\mu\nu}+n_\mu n_\nu.
\end{equation}
Observe that $n^{\mu}\gamma_{\mu\nu}=0$, indicates that $n^{\mu}$ is a vector that has no components on the hypersurfaces $\Sigma$\footnote{Or, that are normal vectors to $\Sigma$.}. The inverse metric $\gamma^{\mu\nu}$ is computed raising the indices of $\gamma_{\mu\nu}$, using for this $g^{\mu\nu}$ i.e.,
\begin{equation}\label{ADM10}
\gamma^{\mu\nu}=g^{\mu\nu}+n^\mu n^\nu.
\end{equation}
When only one of the indices in \eqref{ADM9} is raised, is obtained the following projection tensor 
\begin{equation}\label{ADM11}
\gamma^{\mu}_{~\nu}=\delta^{\mu}_{~\nu}+n^\mu n_\nu.
\end{equation}
Then, the tensor that projects in the normal direction to the hypersurfaces is given by 
\begin{equation}\label{ADM12}
N^{\mu}_{~\nu}=-n^\mu n_\nu.
\end{equation}
The covariant derivative compatible\footnote{Compatible means $^3\nabla_\delta \gamma_{\mu\nu}=0$.} with $\gamma_{\mu\nu}$, are obtained from the projection of $\nabla_\mu$ on the hypersurfaces 
\begin{equation}\label{ADM13}
^3\nabla_\nu=-\gamma^\mu_{~\nu} \nabla_\mu.
\end{equation}
These three-dimensional covariant derivatives are expressed in terms of the connection coefficients %\footnote{Estes coeficientes s\~ao s\'imbolos de Christoffel associados \`a m\'etrica $\gamma_{\mu\nu}$ destes subespa\c cos.} 
associated with the hypersurfaces $\Sigma$, 
\begin{equation}\label{ADM14}
^3\Gamma^\mu_{~\nu\delta}=\frac{1}{2}\gamma^{\mu\theta}(\gamma_{\theta\nu,\delta}+\gamma_{\theta\delta,\nu}-\gamma_{\nu\delta,\theta}).
\end{equation}
On the other hand, the Riemann tensor $^3R^{\gamma}_{~\delta\nu\mu}$ associated to the metric $\gamma_{\mu\nu}$ is defined by,
\begin{equation}\label{ADM15}
2 \ ^3\nabla_{[\mu} \ ^3\nabla_{\nu]}v_\delta =\ ^3R^{\gamma}_{~\delta\nu\mu}v_\gamma, \hspace{0.5cm} ^3R^{\gamma}_{~\delta\nu\mu}n_\gamma=0,
\end{equation}
which must be satisfied by any space-like $v_{\gamma}$  and any time-like $n_\gamma$ 1-forms. Then, from \eqref{ADM15}, the Riemann tensor $^3R^{\gamma}_{~\delta\nu\mu}$ is defined from the Christoffel symbols $^3\Gamma^\mu_{~\nu\delta}$, as
\begin{equation}\label{ADM16}
^3R^{\gamma}_{~\delta\nu\mu}=\ ^3\Gamma^\gamma_{~\delta\mu,\nu} - \ ^3\Gamma^\gamma_{~\nu\mu,\delta} + \ ^3\Gamma^\gamma_{~\sigma\nu} \ ^3\Gamma^\sigma_{~\delta\mu} - \ ^3\Gamma^\gamma_{~\sigma\delta}\ ^3\Gamma^\sigma_{~\nu\mu}.
\end{equation}
The expressions for the Ricci's tensor $^3R_{\mu\nu}=\ ^3R^\gamma_{~\mu\gamma\nu}$ and the scaar fo curvature $^3R=\ ^3R^\mu_{~\mu}$ are obtained from here. 
\\ Given that $^3R^{\gamma}_{~\delta\nu\mu}$ contains only pure spacial information, then all quantities derived from it will contains only information about the intrinsic curvature of the hypersurfaces $\Sigma$, thus it is necessary to introduce almost one more geometric object to take account of the extrinsic curvature. It is labelled as $K_{\mu\nu}$ and can be defined from the projections of the gradients of the normal vectors to the hypersurfaces $\Sigma$.
\\Such projections can be decomposed into a symmetric and antisymmetric part, in the form
\begin{eqnarray}\label{ADM17}
\gamma^\beta_{~\delta} \gamma^\alpha_{~\nu}  n_{\alpha;\beta} &=& \gamma^\beta_{~\delta} \gamma^\alpha_{~\nu}  n_{(\alpha;\beta)} + \gamma^\beta_{~\delta} \gamma^\alpha_{~\nu}  n_{[\alpha;\beta]},\nonumber\\
&=&\Theta_{\delta\nu}+\omega_{\delta\nu},
\end{eqnarray}
where $\Theta_{\delta\nu}$ corresponds to its symmetric part and is known as the expansion tensor and $\omega_{\delta\nu}$ corresponds to its antisymmetric part and is known as the rotational 2-form. Note that, given \eqref{ADM4}, $\omega_{\delta\nu}=0$. 
%\\Aqui usamos a conven\c c\~ao de simetriza\c c\~ao
%\begin{equation}\label{ADM18}
%A_{(\alpha_1\cdots\alpha_n)}=\frac{1}{n!}\sum_{\gamma_1\cdots\gamma_n}\delta_{\alpha_1}^{~~\gamma_1}\cdots\delta_{\alpha_n}^{~~\gamma_n} A_{\gamma_n\cdots\gamma_n}.
%\end{equation}
Thus, the extrinsic curvature is defined as
\begin{eqnarray}\label{ADM19}
K_{\mu\nu}&=&-\gamma^\beta_{~\delta} \gamma^\alpha_{~\nu}  n_{\alpha;\beta}, \nonumber\\
&=&-\frac{1}{2}\mathcal L_{\mathbf n} \gamma_{\mu\nu},
\end{eqnarray}
where $\mathcal L_{\mathbf n} \gamma_{\mu\nu}$ is the Lie derivative of $\gamma_{\mu\nu}$ along the vector field $\mathbf n=n^\alpha \mathbf e_\alpha$. Here, $\mathbf e_\alpha$ is any base. When a local coordinate basis is selected $\mathbf e_\alpha=\partial_\alpha$.
\\Thus, the extrinsic curvature is symmetric and only spacial, furnishing information on how many the normal vectors in $\Sigma$ change their directions. In the figure \ref{FADM2} is shown the change of the normal vectors to the hypersurfaces $\Sigma$. These normal vectors are referred to two distinct and nearly hypersurfaces $\Sigma_{i+1}$ and $\Sigma_{i+2}$. 
\begin{figure}[h!]\label{figADM1}
	\begin{center}
		\input{./Figuras/ADM/ADM_2.eps_tex}
		\caption{Change of the normal vectors to $\Sigma$. The difference $\delta n^a$ only provides information about the changes only on the direction of the vectors, because they are normalised.}
		\label{FADM2}
	\end{center}
\end{figure}
\\Both the extrinsic curvature and the metric $\gamma_{\mu\nu}$ provide information about the instantaneous state do gravitational field. In this manner, it is possible to do the analogy with the classical mechanics in which the first is analogue to the velocities and the second is analogue to the positions in a given set of particles.
\\The projection of the Riemann's tensor completely covariant $R_{\alpha\beta\xi\varphi}$ associated with $g_{\mu\nu}$ on $\Sigma$, are related with the extrinsic $K_{\mu\nu}$ and the intrinsic $^3R_{\mu\nu\eta\delta}$ curvatures, through 
%associado ao espa\c co-tempo, sobre as hipersuperf\'icies $\Sigma$, encontram-se relacionadas com a curvatura extr\'inseca $K_{\mu\nu}$ e o tensor de curvatura intr\'inseca $^3R_{\mu\nu\eta\delta}$, na forma
\begin{equation}\label{ADM20}
^3R_{\mu\nu\eta\delta}+K_{\mu\eta}K_{\nu\delta}-K_{\mu\delta}K_{\eta\nu}=\gamma^\alpha_{~\mu} \gamma^\beta_{~\nu} \gamma^\xi_{~\eta} \gamma^\varphi_{~\delta} R_{\alpha\beta\xi\varphi}.
\end{equation}
which is known as the {\it Gauss equation}.
\\In addition the projection of the first tree components of the Riemann's tensor $R_{\alpha\beta\xi\varphi}$ on $\Sigma$ and of the its four component on the normal vector to the hypersurfaces $\Sigma$ depends only on the derivatives of the extrinsic curvature tensor. 
These quantities are functions only of the spacial part of the metric $\gamma_{\mu\nu}$ and its derivatives, thus
\begin{equation}\label{ADM21}
^3\nabla_\eta K_{\mu\nu}-\ ^3\nabla_\mu K_{\eta\nu}=\gamma^\alpha_{~\mu} \gamma^\beta_{~\eta} \gamma^\xi_{~\nu} n^\varphi R_{\alpha\beta\xi\varphi}.
\end{equation}
The last equations in known as {\it Codazzi equation}.
%Esta \'e conhecida como a {\it equa\c c\~ao de Codazzi}.
\\Both equations \eqref{ADM20} and \eqref{ADM21}, lead to the constraint equations, because them provide the integrability conditions which allow to put the hypersurfaces $\Sigma$, which carry the information about $K_{\mu\nu}$ and $\gamma_{\mu\nu}$, to the four-dimensional space-time.
\\On the other hand, when is computed the Lie derivative of the extrinsic curvature $K_{\mu\nu}$ along $n^\alpha$, it is obtained 
\begin{equation}\label{ADM22}
\mathcal L_{\mathbf n}K_{\mu\nu}=n^\alpha n^\beta\gamma_{~\mu}^\sigma\gamma_{~\nu}^\varphi R_{\alpha\beta\sigma\varphi} -\frac{1}{\alpha}\ ^3\nabla_\mu \ ^3\nabla_\nu \alpha -K_{~\nu}^\sigma K_{\mu\sigma}.
\end{equation}
This is known as the {\it Ricci equation}. It express that temporal changes in the extrinsic curvature are related with the Riemann's tensor $R_{\alpha\beta\sigma\varphi}$, when only two of their indices are projected in the direction of the time.
\\Now, contracting the Gauss equation \eqref{ADM20} it is obtained \cite{ADM59}
\begin{equation}\label{ADM23}
\gamma^{\alpha\nu} \gamma^{\beta\mu} R_{\alpha\beta\nu\mu}=\ ^3R+K^2-K_{\sigma\varphi}K^{\sigma\varphi},
\end{equation}
where the trace of the extrinsic curvature was defined $K=\gamma^{\alpha\beta}K_{\alpha\beta}$. From the Einstein's tensor definition
\begin{equation}\label{ADM24}
G_{\mu\nu}=R_{\mu\nu}-\frac{1}{2}g_{\mu\nu}R,
\end{equation}
results
\begin{equation}\label{ADM25}
2n^\mu n^\nu G_{\mu\nu}=\gamma^{\alpha\mu} \gamma^{\beta\nu} R_{\alpha\beta\mu\nu}.
\end{equation}
Therefore \eqref{ADM23} becomes
\begin{equation}\label{ADM26}
2n^\mu n^\nu G_{\mu\nu}=\ ^3R+K^2-K_{\sigma\varphi}K^{\sigma\varphi}.
\end{equation}
If is defined the energy density $\rho$ as the total energy density as measured by an Eulerian observed i.e., 
%como a densidade total de energia medida por um observador Euleriano, i.e.,
\begin{equation}\label{ADM27}
\rho=n_\mu n_\nu T^{\mu\nu}.
\end{equation}
Then, the projection of the Einstein's field equations \eqref{eq2.24} on the normal vectors to the hypersurfaces $\Sigma$ is
\begin{equation}\label{ADM28}
^3R+K^2 -K_{\mu\nu}K^{\mu\nu}=16\pi\rho,
\end{equation}
which is a {\it hamiltonian constrain equation}.
\\Now, contracting the Codazzi equation it is obtained
\begin{equation}\label{ADM29}
^3\nabla_{\varphi} K_\sigma^{~\varphi}  -\ ^3\nabla_{\sigma} K=\gamma^{\alpha}_{~\sigma} \gamma^{\beta\mu}n^\nu R_{\alpha\beta\mu\nu}.
\end{equation}
However from the Einstein's tensor it is obtained 
\begin{equation}\label{ADM30}
\gamma^{\mu}_{~\sigma} n^{\nu}G_{\mu\nu}=\gamma^{\mu}_{~\sigma} n^{\nu}R_{\mu\nu}.
\end{equation}
In this manner, the Codazzi equation take the form
\begin{equation}\label{ADM31}
^3\nabla_{\varphi} K_\sigma^{~\varphi}  -\ ^3\nabla_{\sigma} K=8\pi S_\sigma,
\end{equation}
where 
\begin{equation}\label{ADM32}
S_\sigma=-\gamma^\mu_{~\sigma} n^\nu T_{\mu\nu}
\end{equation}
which corresponds to the momentum density as measured by an Eulerian observed. The equation \eqref{ADM31} is commonly referred as  {\it the momentum constrain}.
\\Now it is defined a vector $t^\mu$ as
\begin{equation}\label{ADM33}
t^\mu=\alpha n^\mu + \beta^\mu,
\end{equation}
where $\beta^\alpha$ is the {\it displacement vector}. This vector indicates the displacement of the Eulerian observes between two successive hypersurfaces, as sketched in the figure \ref{FADM3}. 
\begin{figure}[h!]
	\begin{center}
		\input{./Figuras/ADM/ADM_3.eps_tex}
		\caption{Representation of two sucessives hypersurfaces and the displacement vector $\beta^\mu$ in red. This represent the displacement of the normal observers between these two succesive hypersurfaces.}
		\label{FADM3}
	\end{center}	
\end{figure}
\\With this, the vector $t^\alpha$ is the dual to the one-form $\Omega_\alpha$. Thus, from the extrinsic curvature  $K_{\mu\nu}$ it is obtained
\begin{equation}\label{ADM34}
\mathcal L_{\mathbf t}\gamma_{\mu\nu}=-2\alpha K_{\mu\nu}+\mathcal L_\beta \gamma_{\mu\nu}.
\end{equation}
This is the {\it evolution equation for the metric} $\gamma_{\mu\nu}$ associated with the hypersurfaces $\Sigma$. 
\\The evolution equation of the extrinsic curvature is obtained taken its Lie derivative along $t^a$, as
\begin{equation}\label{ADM35}
\mathcal L_{\mathbf t}K_{\mu\nu}=\alpha\mathcal L_{\mathbf n}K_{\mu\nu}+\mathcal L_{\beta}K_{\mu\nu}.
\end{equation}
However, from the Ricci's equation \eqref{ADM22} and from the Einstein's field equations \eqref{eq2.24} it is obtained that
\begin{equation}\label{ADM36}
n^\alpha n^\delta\gamma_{~\mu}^\varepsilon\gamma_{~\nu}^\beta R_{\alpha\beta\delta\varepsilon}=\ ^3R_{\mu\nu}+KK_{\mu\nu}-K_{\mu\sigma}K^\sigma_{~\nu}-8\pi \gamma_{~\mu}^\sigma\gamma_{~\nu}^\varphi \left(T_{\sigma\varphi}-\frac{1}{2}g_{\sigma\varphi}T\right),
\end{equation}
where $T$ is the trace of the stress-energy tensor $T=g^{\mu\nu}T_{\mu\nu}$. Defining the spacial part of $T_{\mu\nu}$ and its trace from  
\begin{equation}\label{ADM37}
S_{\mu\nu}=\gamma_{~\mu}^\sigma\gamma_{~\nu}^\varepsilon T_{\sigma\varepsilon}, \hspace{1cm}S=S_{~\mu}^\mu,
\end{equation}
and substituting into \eqref{ADM35} it is obtained
\begin{eqnarray}\label{ADM38}
\mathcal L_{\mathbf t}K_{\mu\nu}&=&-\ ^3\nabla_\mu \ ^3\nabla_\nu \alpha + \alpha(\ ^3R_{\mu\nu}-2K_{\mu\sigma}K_{~\nu}^\sigma+KK_{\mu\nu})\nonumber\\&& -8\pi\alpha\left(S_{\mu\nu}-\frac{1}{2}\gamma_{\mu\nu}(S-\rho)\right) +\mathcal L_{\beta}K_{\mu\nu}.
\end{eqnarray}
In this evolution equation for the extrinsic curvature all the differential operators and the Ricci's tensor are associated to $\gamma_{\mu}$. The evolution equations for the metric of the hypersurfaces and for the extrinsic curvature \eqref{ADM34} and \eqref{ADM38} are coupled. They determine the evolution of the gravitational field specified by $\gamma_{\mu\nu}$ and $K_{\mu\nu}$. They and the Hamiltonian constrain equations and the momentum constrain \eqref{ADM28} and \eqref{ADM31} contain the same information that the field equations\eqref{eq2.24}. Furthermore, it is possible to observe that the differential equations that govern the matter and the space-time dynamics are from here, differential equations of first order in time, which is different to the original field equations. As in any initial value problem, the evolution equations must conserve the constrain equations, in this form, if $\gamma_{\mu\nu}$ and $K_{\mu\nu}$ satisfy the constrain equations, in some hypersurface $\Sigma_i$, then the same constrains must be satisfy along the all temporal evolution, i.e. this conditions must be satisfied for all the hypersurfaces $\Sigma$ in which the space-time is foliated.
\\At last, specifying the vector $t^\mu$ as $t^\mu=(1,0,0,0)$, and introducing a 3-dimensional vectorial base $e^\mu_{~(i)}$, where $i$ indicates each of three vectors and taking into account that $\Omega_\mu e^\mu_{~(i)}=0$, then it is possible to make the choice that the spatial components of $n_i=0$, in this form the displacement vector becomes with only spacial components $\beta^\mu=(0,\beta^i)$, and therefore the normal vectors to the hypersurfaces result as $n^\mu=\alpha^{-1}(1,\beta^i)$ in this form the metric of the space-time can be represented by the matrix
\begin{equation}\label{ADM39}
g_{\mu\nu}=\begin{pmatrix}
-\alpha^2+\beta_k\beta^k & \beta_i \\
\beta_j & \gamma_{ij}
\end{pmatrix},
\end{equation}
or in the form of line element 
\begin{equation}\label{ADM40}
ds^2=-\alpha^2dt^2+\gamma_{ij}(dx^i+\beta^idt)(dx^j+\beta^jdt).
\end{equation}
The last form is usually known as the {\it line element in the 3+1 form}. 

==> docs/BSSN_Formalism.tex <==
\subsection{The Baumgarte-Shibata-Shapiro-Nakamura ({\it BSSN}) Equations}
A variation of the ADM formalism is the Baumgarte-Shibata-Shapiro-Nakamura (BSSN) formalism \cite{BS99,SN95}. In this, the metric $\gamma_{ij}$ associated with the hypersurfaces $\Sigma$ is conformal to other denoted by $\tilde{\gamma}_{ij}$ and the conformal factor is given by  $e^{i\phi}$, i.e.,
\begin{equation}\label{BSSN1}
	\gamma_{ij}=e^{i\phi}\tilde{\gamma}_{ij},\hspace{1cm}\|\tilde{\gamma}_{ij}\|=1.
\end{equation} 
The fundamental idea is to introduce this conformal factor and evolve both, separately, the conformal factor and the metric. This simplifies the Ricci's tensor and simplifies the numerical codes. In order to obtain the evolution equations, the extrinsic curvature $K_{ij}$ is decomposed into its trace $K$ and the trace-free part $A_{ij}$ 
\begin{equation}\label{BSSN2}
	K_{ij}=A_{ij}+\frac{1}{3}\gamma_{ij}K.
\end{equation}
In addition $A_{ij}$ is expressed in terms of a trace-free conformal curvature, i.e., 
\begin{equation}\label{BSSN3}
	A_{ij}=e^{i\phi}\tilde{A}_{ij}.
\end{equation}
Contracting the evolution equation for the metric $\gamma_{ij}$ \eqref{ADM35}, it is obtained 
\begin{equation}\label{BSSN4}
	\partial_t \ln \gamma^{1/2}=\alpha K +\ ^3\nabla_i\beta^i,
\end{equation}
and using \eqref{BSSN1} here, it is obtained an evolution equation for $\phi$
\begin{equation}\label{BSSN5}
	\partial_t \phi=-\frac{1}{6}\alpha K + \partial_i\beta^i +\beta^i\partial_i \phi.
\end{equation}
Also, contracting the evolution equation for the extrinsic curvature \eqref{ADM38} it is obtained 
\begin{equation}\label{BSSN6}
	\partial_t K=-\ ^3\nabla^2\alpha+\alpha(K_{ij}K^{ij}+4\pi(\rho+S))+\beta^i\ ^3\nabla_iK,
\end{equation}
where 
$$^3\nabla^2 =\gamma^{ij} \ ^3\nabla_i\ ^3\nabla_j,$$ 
such that, substituting \eqref{BSSN2} and using \eqref{BSSN3}
\begin{equation}\label{BSSN7}
	\partial_t K=-\ ^3\nabla^2\alpha+\alpha\left(\tilde A_{ij}\tilde A^{ij}+\frac{1}{3}K^2\right)+4\pi\alpha(\rho+S)+\beta^i\partial_i K.
\end{equation}
Subtracting \eqref{BSSN5} from \eqref{ADM35} it is obtained the evolution equation for $\tilde \gamma_{ij}$
\begin{equation}\label{BSSN8}
	\partial_t\tilde \gamma_{ij}=-2\alpha \tilde A_{ij}+\beta^k\partial_k\tilde\gamma_{ij}+\tilde \gamma_{kj}\partial_i\beta^k-\frac{2}{3}\tilde \gamma_{ij}\partial_k\beta^k,
\end{equation}
also, subtracting \eqref{BSSN7} from \eqref{ADM38} it is obtained the evolution equation for $\tilde A_{ij}$
\begin{eqnarray}\label{BSSN9}
	\partial_t \tilde A_{ij}&=&e^{4\phi}\left(-(\ ^3\nabla_i \ ^3\nabla_j\alpha)^{\text{TF}}+\alpha(R_{ij}^{\text{TF}}-8\pi S_{ij}^{\text{TF}})\right)+\alpha(K\tilde A_{ij}-2\tilde A_{in}\tilde A^n_{~j})\nonumber\\
	&&+\beta^k\partial_k\tilde A_{ij}+\tilde A_{ik}\partial_j B^k+\tilde A_{kj}\partial_i B^k -\frac{2}{3}\tilde A_{ij}\partial_k\beta^k,
\end{eqnarray}
where the superscript TF indicates trace-free, i.e,
\begin{equation}
	^3R_{ij}^{\text{TF}}=\ ^3R_{ij}-\frac{1}{3}\gamma_{ij}\ ^3R,\hspace{0.5cm} S_{ij}^{\text{TF}}=S_{ij}-\frac{1}{3}\gamma_{ij}\ ^3R,
\end{equation}
and
\begin{equation}
	(\ ^3\nabla_i \ ^3\nabla_j\alpha)^{\text{TF}}=(\ ^3\nabla_i \ ^3\nabla_j\alpha)-\frac{1}{3}\gamma_{ij}(\ ^3\nabla^2\alpha).
\end{equation}
Now, in terms of these variables, the momentum constrain becomes 
\begin{eqnarray}\label{BSSN10}
	0=\gamma^{ij}\ ^3\tilde\nabla_i\ ^ 3\tilde\nabla_j e^\phi-\frac{1}{8}e^\phi \ ^3\tilde R+\frac{1}{8}e^{5\phi}\tilde A_{ij}\tilde A^{ij}-\frac{1}{12}e^{5\phi}K^2+2\pi e^{5\phi}\rho,
\end{eqnarray}
where the operator $^3\tilde\nabla_i=e^{i\phi}\ ^3\nabla_i$, is the hamiltonian constrain 
\begin{eqnarray}\label{BSSN10}
	0=\ ^3\tilde\nabla_j \left(\tilde A^{ji}e^{6\phi}\right)-\frac{2}{3}e^{6\phi} \ ^3\tilde \nabla^i K-8\pi e^{6\phi}S^i.
\end{eqnarray}

==> docs/Bondi_Sachs.tex <==
\subsection{The Bondi-Sachs Metric}
\citeonline{B_VII,B_VIII} in their remarkable work describe in detail the radiation coordinates construction. Here, these details are reviewed in order to understand the metric and its metric functions. Thus, it is supposed that the manifold $\mathcal{M}$ is doted of a metric tensor such that $g_{\mu\nu}:=g_{\mu\nu}(x^\alpha)$ and having a signature $+2$. It is supposed a generic scalar function that depend on these unknown and arbitrary coordinates $u:=u(x^\mu)$, such that obeys 
\begin{equation}
u_{,\mu}u^{,\mu}=0.
\label{bs1}
\end{equation}
Thus, denoting by $k^\mu=u_{,\nu}g^{\nu\mu}$,
\begin{equation}
k_\mu k^\mu=0.
\label{bs2}
\end{equation} 
The hypersurfaces for $u$ constant are null; and its normal vectors $k^\mu$ also satisfy
\begin{equation}
k_{;\mu} k^\mu=0.
\label{bs3}
\end{equation} 
Thus, the lines whose tangent is described by $k^\mu$ are called as rays, see Figure \ref{FADM1}. 
\begin{figure}[h!]
	\begin{center}
		\input{./Figuras/Characteristic/foliation_11.eps_tex}
		\caption{Null coordinates construction. Tangent and normal vectors to the null hypersurfaces emanated from a time-like world tube $\Gamma$.}
		\label{FADM1}
	\end{center}
\end{figure}
\\From \eqref{bs3}, the congruence of rays of null geodesic are too normal to the hypersurfaces for $u$ constant, thus these rays lie in the hypersurfaces and in the normal plane to the null hypersurfaces. The parameter $u$ must be such that the expansion $\xi$ and the shear $\sigma$ of the congruences, formed by these rays (the null cones)
\begin{equation}
\xi=\dfrac{k^\alpha_{~;\alpha}}{2}\ne 0,\hspace{1cm}|\sigma|^2=\dfrac{k_{\alpha;\beta}k^{\alpha;\beta}}{2}-\rho^2\ne\rho^2.
\end{equation}
It is assumed that $u$ satisfies these conditions for any coordinate system. The parameter $u$ will be selected as the retarded time. The scalar functions $\theta:=\theta(x^\alpha)$, $\phi:=\phi(x^\alpha)$ can be selected such that
\begin{equation}
\theta_{,\alpha}k^\alpha=\phi_{,\alpha}k^\alpha=0,\hspace{0.5cm}\theta_{,\alpha}\theta_{,\beta}\theta_{,\gamma}\theta_{,\delta}g^{\alpha\beta}g^{\gamma\delta}-\left(\theta_{,\alpha}\theta_{,\beta}g^{\alpha\beta}\right)^2=D\ne 0,
\end{equation}
where $D>0$. Thus $\theta$ and $\phi$ are constant along each ray, and for this, can be identified as optical angles. In addition, it is possible to choose the scalar function $r:=r(x^\alpha)$, such that
\begin{equation}
r^4=\dfrac{1}{D\sin^2\theta},
\end{equation}
in which case $r$ is the luminosity distance, defining hypersurfaces for $u,r$ constants such that its area is exactly $4\pi r^ 2$. Defining $x^\mu=(u,r,\theta,\phi)$ as coordinates with $\mu=1,2,3,4$, and $x^A=(\theta,\phi)$ with $A=3,4$ then the line element such that the above conditions being satisfied is
\begin{align}
ds^2=&-\left(\frac{Ve^{2\beta}}{r}-r^2h_{AB}U^AU^B\right)du^2-2e^{2\beta}dudr-2r^2h_{AB}U^Bdudx^A\nonumber\\
&+r^2h_{AB}dx^Adx^B.
\label{BS1}
\end{align}
That can be written conveniently as
\begin{align}
ds^2=&-\left(\frac{Ve^{2\beta}}{r}\right)du^2-2e^{2\beta}dudr+r^2h_{AB}\left(U^Adu -dx^A\right)\left(U^Bdu-dx^B\right),
\label{BS2}
\end{align}
where
\begin{align}
2h_{AB}dx^Adx^B&=\left(e^{2\gamma}+e^{2\delta}\right)d\theta^2+4\sin\theta\sinh(\gamma-\delta)d\theta d\phi \nonumber\\
&+ \sin^2\theta\left(e^{-2\gamma}+e^{-2\delta}\right)d\phi^2.
\end{align}
Then, $\|h_{AB}\|=\sin\theta$, that is just the determinant of the unitary sphere, if $\theta$ and $\phi$ can be identified as the usual spherical angles. The form \eqref{BS2} allows us to identify $Ve^{2\beta}/r$ as the square of the lapse function, $U^\mu$ the shift displacement between two successive hypersurfaces , $\beta$ the red-shift 

==> docs/CEFE.tex <==
\subsection{The Einstein's Field Equations}
The Einstein's field equation in this formalism can be decomposed into hypersurface, evolution and constrain equations. 
\begin{subequations}
	\begin{align}
& R_{22}=0,\hspace{0.5cm}R_{2A}=0,\hspace{0.5cm}h^{AB}R_{AB}=0,\\
& R_{AB}-\frac{1}{2}h_{AB}h^{CD}R_{CD}=0,\\
& R^2_{~A}=0,\hspace{0.5cm}R^2_{~u}=0.
\end{align}
\label{CEFE}
\end{subequations}
The first set of equations read 
\begin{align}
\beta_{,r}&=\frac{1}{16}rh^{AC}h^{BD}h_{AB,r}h_{CD,r},\\
\left(r^4e^{2\beta}h_{AB}U^B_{~,r}\right)_{,r}&=2r^4\left(r^{-2}\beta_{,A}\right)_{,r}-r^2h^{BC}h_{AB,r:C},\\
2V_{,r}&=e^{2\beta}\mathcal{R}-2e^{2\beta}\beta_{:A}^{~~A}-2e^{2\beta}\beta^{:A}\beta_{:A}+r^{-2}\left(r^4U^A\right)_{,r:A}\nonumber\\
&\hspace{0.5cm}-\frac{r^4e^{-2\beta}}{2}h_{AB}U^A_{~~,r}U^B_{~~,r},
\label{fe1}
\end{align}
for which $u$ is constant, the colon indicates covariant derivative associated to $h_{AB}$ and $\mathcal{R}$ is the Ricci's scalar associated to $h_{AB}$. The evolution equations take the form
\begin{align}
&%m^Am^B
\left(r h_{AB,u}\right)_{,r}-\frac{%m^Am^B
	\left(rVh_{AB,r}\right)_{,r}}{2r}-\frac{2e^{\beta}e^{\beta}_{~~:AB}%m^Am^B
	}{r}\nonumber\\
&+rh_{AC:B}U^C_{~,r}%m^Am^B
-\frac{r^3e^{-2\beta}h_{AC}h_{BD}U^C_{~,r}U^D_{~,r}}{2}+2U_{B:A}%m^Am^B
\nonumber\\
&+\frac{rh_{AB,r}U^C_{~:C}%m^Am^B
	+rU^Ch_{AB,r:C}%m^Am^B
	}{2}+rh_{AD,r}h^{CD}\left(U_{C:B}-U_{B:C}\right)%m^Am^B
	\nonumber\\
&=0,
\end{align}
in which are involved time derivatives of the $J$ function, and the third set, the constrain equations, must be satisfied for all null cones in wich is foliated the space-time, or conversely for all time in the evolution.  

==> docs/CEFE_QSA.tex <==
\section{The Einstein's field equations in the quasi-spherical approximation}
\begin{equation}
\Omega^C_{~AB}=\dfrac{h^{CD}\left(h_{DB|A}+h_{AD|B}-h_{AB|D}\right)}{2},
\end{equation}
\begin{equation}
Q_{A}=r^2e^{-2\beta}h_{AB}U^B_{~,r},
\end{equation}
\begin{align}
\left(r^2Q_{A}\right)_{,r}&=2r^4\left(r^{-2}\beta_{,A}\right)_{,r}-r^2h^{BC}h_{AB,r:C},\\
U^A_{~,r}&=r^{-2}e^{2\beta}h^{AB}Q_{B},
\end{align}
\begin{subequations}
\begin{align}
\beta_{,r}&=N_\beta,\\
\left(r^2Q\right)_{,r}&=-r^2q^Aq^{BC}h_{AB:C}+2r^4q^A\left(r^{-2}\beta_{,A}\right)_{,r}+N_Q,\\
U_{,r}&=r^2e^{2\beta}Q+N_U,\\
w_{,r}&=\dfrac{e^{2\beta}\mathcal{R}}{2}-1-e^{\beta}\eth\overline{\eth}e^\beta+\dfrac{r^{-2}\left(r^4\left(\eth\overline{U}+\overline{\eth}U\right)\right)_{,r}}{4}+N_w,
\end{align}
\begin{align}
2\left(rJ\right)_{,ur}-\left(r^{-1}V\left(rJ\right)_{,r}\right)_{,r}=&-r^{-1}\left(r^2\eth U\right)_{,r}+2r^{-1}e^\beta\eth^2 e^\beta\nonumber\\
& -\left(r^{-1}w\right)_{,r}J+N_J,
\end{align}
\end{subequations}
where
\begin{align}
N_\beta&=\frac{1}{16}rh^{AC}h^{BD}h_{AB,r}h_{CD,r},\\
N_Q&=q^A\left(r^2h^{BC}\left(\Omega^D_{~CA}h_{DB,r}+\Omega^D_{~CB}h_{AD,r}\right)-r^2\left(h^{BC}-q^{BC}\right)h_{AB,r|C}\right),\\
N_U&=r^{-2}e^{2\beta}q_A\left(h^{AB}-q^{AB}\right)Q_{B},\\
N_w&=-e^{\beta}\left(\left(h^{AB}-q^{AB}\right)\left(e^\beta\right)_{:B}\right)_{:A}-\dfrac{r^4e^{-2\beta}h_{AB}U^A_{~,r}U^B_{~,r}}{4},\\
N_J&=\dfrac{q^Aq^B}{r}\left(-2e^\beta\Omega^C_{~AB}\left(e^\beta\right)_{:C}-h_{AC}\Omega^C_{~DB}\left(r^2U^D\right)_{,r}\nonumber\right.\\
&\left.-\left(h_{AC}-q_{AC}\right)\left(r^2U^C\right)_{,r}+\dfrac{r^4e^{-2\beta}h_{AC}h_{DB}U^C_{~,r}U^D_{~,r}}{2}\right.\nonumber\\
&\left.-\dfrac{r^2h_{AB,r}U^C_{~:C}}{2}-r^2U^Ch_{AB,r:C}+r^2h^{CD}h_{AD,r}U_{[B:C]}+\dfrac{h_{AB}F}{2}\right),
\end{align}
\begin{align}
F=&-r^2h^{AB}_{~~~,r}\left(h_{AB,u}-\dfrac{Vh_{AB,r}}{2r}\right)-2e^\beta \left(e^\beta\right)_{:A}^{~~A}+\left(r^2U^A\right)_{,r:A}\nonumber\\
&-\dfrac{r^4e^{-2\beta}h_{AB}U^A_{~,r}U^B_{~,r}}{2},
\end{align}

==> docs/CLEFE.tex <==
\section{Einstein's Field Equations}
In the linear regime, the field equations \eqref{CEFE} are reduced to
\begin{subequations}
\begin{eqnarray}
&& 8 \pi  T_{22}=\frac{4 \beta _{,r}}{r}, \label{field_eq_1}\\
&& 8 \pi  T_{2A} q^A=\frac{\overline{\eth }J_{,r}}{2} -\eth \beta _{,r} +\frac{2 \eth \beta}{r} +\frac{\left(r^4 U_{,r}\right)_{,r}}{2r^2}, \label{field_eq_2}\\
&& 8 \pi  \left(h^{AB} T_{AB}-r^2 T\right) =-2 \eth \overline{\eth }\beta +\frac{\eth^2\overline{J} + \overline{\eth }^2 J}{2} +\frac{\left(r^4\left(\overline{\eth}U+\eth \overline{U}\right)\right)_{,r}}{2r^2}\nonumber\\
&& \hspace{4.0cm}+4 \beta -2 w_{,r}, \label{field_eq_3}\\
&& 8 \pi T_{AB}  q^A q^B=-2 \eth^2 \beta + \left(r^2\eth U \right)_{,r} - \left(r^2 J_{,r}\right)_{,r} +2 r\left(rJ\right)_{,ur},\label{field_eq_4}\\
&& 8 \pi  \left(\frac{T}{2}+T_{11}\right)=\frac{\eth \overline{\eth }w}{2 r^3} + \frac{\eth \overline {\eth }\beta }{r^2} -\frac{\left(\eth \overline{U} + \overline{\eth} U \right)_{,u}}{2} +\frac{w_{,u}}{r^2} +\frac{w_{,rr}}{2 r} -\frac{2 \beta_{,u}}{r}, \label{field_eq_5}\\ 
&& 8 \pi  \left(\frac{T}{2}+T_{12}\right)=
\frac{\eth \overline{\eth }\beta }{r^2} -\frac{\left(r^2\left(\eth \overline{U} + \overline{\eth   }U\right)\right)_{,r}}{4r^2}
+\frac{w_{,rr}}{2 r}, \label{field_eq_6}\\
&& 8 \pi  T_{1A} q^A=\frac{\overline{\eth }J_{,u}}{2} -\frac{\eth^2
	\overline{U} }{4} +\frac{\eth \overline{\eth }U}{4} +\frac{1}{2}\left(\frac{\eth w}{r}\right)_{,r} -\eth \beta _{,u} +\frac{\left(r^4U\right)_{,r}}{2r^2}\nonumber\\
&& \hspace{2cm}-\frac{r^2 U_{,ur}}{2} +U. \label{field_eq_7}
\end{eqnarray}
\label{linear_field_eqs}
\end{subequations}

==> docs/Characteristic.tex <==
\section{Outgoing Characteristic Formulation}
\graphicspath{{./Figuras/Characteristic/}}
In this section will be described one of the characteristic formalism, in which the space-time is foliated into null cones oriented to the future. In order to do so, it is described the Bondi-Sachs metric and the characteristic initial value problem, after this there are presented the non-linear filed equations in the characteristic formalism and for ending this section these equations are rewritten using the eth formalism previoulsy described.
\input{./docs/Bondi_Sachs}
\input{./docs/IVP}
\input{./docs/CEFE}
\input{./docs/CEFE_QSA}
\input{./docs/non_linear_regime_eth}
%\subsection{Caustic Formation}


==> docs/Eth.tex <==
\chapter{THE {\it eth} FORMALISM AND SPIN-WEIGHTED SPHERICAL HARMONICS }
Before introduce the outgoing characteristic formulation of the general relativity, it is convenient to expose a standard tool for regularising the angular differential operators, namely the {\it eth formalism}. It is based on a non-conformal mapping of the regular coordinate charts to make a finite coverage of the unit sphere. These kind of mapping was originally used in global weather studies \cite{W70,S72,RIP96}, and are based on the stereographic and gnomonic projections. It is worth mentioning, that these projections to make the finite coverage of the unit sphere, remove the singular points given by the fact that the sphere can not be cover by only one coordinate chart. 
\\The {\it eth formalism} \cite{NP66,GMNRS66} is a variation of the Newman-Penrose formalism. As in this last formalism, scalars and associated functions and operators related with the projections onto the null tangent vectors to the unit sphere appear; also it can be generalised to the projection onto the tangent vectors to a topological sphere (a diffeomorphism to the unit sphere). In order to present the eth formalism, the non-conformal mapping using stereographic coordinates is presented. After this, a decomposition for the unit sphere and the transformation for vectors and one-forms are shown. These transformation rules are extended to the dyads and their spin-weights are founded. It is worth mentioning that the spin-weight induced into the scalar functions comes from the transformation rules associated with the stereographic dyads, however this property is not exclusive of this kind of coordinates, and appears as a transformation associated between the coordinate maps needed to make the finite coverage to the unit sphere. Then the spin-weighted scalars are constructed from the irreducible representation for tensors of type $(0,2)$ and then it is shown the general from for a spin-weighted scalar of spin-weight $s$. The rising and lowering operators are presented from the projection of the covariant derivative associated to the unit sphere metric and the Legendrian operator is then expressed in terms of these rising and lowering operators. After this, some properties of spin-weighted scalars are shown and the orthonormality of such functions is defined. The spin-weighted spherical harmonics $_sY_{lm}$ and the action of the rising and lowering operators in them are constructed. Finally, another base of functions to decompose functions on the sphere, the spin-weighted spherical harmonics $_sZ_{lm}$, are shown as linear combinations of the $_sY_{lm}$. 
%\\It is explored in details the {\it eth} formalism as a variation of the Newman-Penrose formalism. As in this last, scalars and associated functions related with the projections onto the null tangent vectors appears. Through the transformation rules associated with the stereographic dyads, it is induced the spin-weight in the scalar functions, however this property %(the spin-weight of the scalar functions) 
%is not exclusive of this kind of coordinates, and appears as a transformation associated between the coordinate maps needed to make a finite coverage to the unit sphere. Here, the non-conformal mapping in the sphere are presented, the stereographic dyads are constructed and it is shown the spin-weighted scalars.
\section{Non-conformal Mappings in the Sphere}
There are infinite forms to make up finite coverage to the sphere. The principal aim here is to shown an atlas, with almost two coordinate charts, in which all points in $S^2$ are mapped. In the context of the global weather studies were proposed diverse  useful schemes, from the numerical point of view, to make finite coverages to the sphere \cite{SAM68,W70,S72,Thacker80, BF85,CK15}. Only two of them become important in numerical relativity, since has been used widely, the first one is the stereographic projection in two maps and the second one is the gnomonic projection in six maps or also known as cubed sphere. Both offers great numerical advantages, as the simplification of all angular derivatives, as in the case of the stereographic coordinates and simplification in the numerical calculus as in the case of the cubed sphere projection. It is worth stressing that the {\it eth} formalism is totally independent on the selection of the coordinates, as we will shown in the next sections. However, given the simplification in some of the calculations and its usability in those numerical, it is presented in  details the connection between the stereographic coordinates and the spin-weighted scalars.%The stereographic coordinates will induce also a simple transformation rule for the tangent vectors to the unitary sphere, whi    %In the first the metric for each map turns up diagonal simplifying its decomposition into 
%They minimise the overlapping zones as possible, help in avoiding the complex two dimensional interpolation algorithms necessary to pass the information from one sector to another,    .  We will show here ....
\input{./docs/stereo_coordinates}
%\section{Gnomonic Coordinates}
\input{./docs/unit_metric_decomposition}
\input{./docs/differential_operators}
\input{./docs/tangent_vectors_spin_weight}
\input{./docs/spin_weighted_scalars}
\input{./docs/ladder_operators}
\input{./docs/transforming_basis}
\input{./docs/legendrian}
\input{./docs/eth_spherical}
\input{./docs/angular_integrals}
\input{.docs/spin_weighted_Y}
\section{Spin-weighted Spherical Harmonics $_sZ_{lm}$}
There exist another base of spherical harmonics in which the functions defined on the sphere surface can be expanded, namely $_sZ_{lm}$, which is defined as
\begin{equation}
_sZ_{lm}=\begin{cases}
\dfrac{i}{\sqrt{2}}\left((-1)^m\ _sY_{lm}+\ _sY_{l\ -m}\right) &\text{for} \hspace{0.5cm} m<0 \\
_sY_{lm}&\text{for} \hspace{0.5cm} m=0 \\
\dfrac{1}{\sqrt{2}}\left(_sY_{lm}+(-1)^m\ _sY_{l\ -m}\right) &\text{for} \hspace{0.5cm} m>0
\end{cases},
\end{equation}
Since these harmonics are constructed from linear combinations of $_sY_{lm}$, then they are eigenfunctions of the $\eth\overline{\eth}$ operator, \cite{ZGHLW03}, are orthonormal
%\\Além disso, estes harmônicos também são ortogonais %pois para $m,m'<0$
\begin{align*}
\int_{\Omega} d\Omega \ _sZ_{lm} \ _s\bar{Z}_{l'm'} %&=
%\int_{\Omega} d\Omega \dfrac{i}{\sqrt{2}}\left((-1)^m\ _sY_{lm}+\ _sY_{l\ -m}\right)\left(\dfrac{-i}{\sqrt{2}}\left((-1)^{m'}\ _s\bar{Y}_{l'm'}+\ _s\bar{Y}_{l'\ -m'}\right)\right)\\
%&=
%\dfrac{1}{2} \Big((-1)^{m+m'} \int_{\Omega} d\Omega \ _sY_{lm}\ _s\bar{Y}_{l'm'}+ \int_{\Omega} d\Omega \ _sY_{l\ -m}\ _s\bar{Y}_{l'\ -m'}\Big)\\
&=\delta_{ll'}\delta_{mm'}
\label{orto_sZlm}
\end{align*}
%enquanto que para $m,m'>0$ 
and complete
\begin{equation*}
\sum_{l=0}^{\infty}\sum_{m=-l}^{l} \ _sZ_{lm}(\theta,\phi) \ _s\bar{Z}_{lm}(\theta',\phi')=\delta(\phi-\phi')\delta(\cos(\theta)-\cos(\theta')).
\label{compl_sZlm}
\end{equation*}
Therefore, any angular function $_s\Psi$ with spin-weight $s$ can be expanded in terms of $_sZ_{lm}$,
%Porém determinam uma base de funções para $\mathcal M$ e isto garante automaticamente que toda função com peso de spin $s$ na variedade angular pode ser expandida em termos destes, i.e,
\begin{equation}
_s\Psi =\sum_{l=0}^{\infty}\sum_{m=-l}^{l} \ _s\Psi_{lm}\ _sZ_{lm}.
\label{exp_sZlm}
\end{equation}
They will be important because is in term of these spherical harmonics that the Einstein's field equations are re-expressed. The reason for do that, is the $_sZ_{lm}$ decouple the $m$ mode in the equations. 

==> docs/HDBP.tex <==
\section{Harmonic Decomposition and Boundary Problem}
\begin{equation}
_sf=\sum_{l=0}^\infty \sum_{m=l}^l \Re\left(f_{lm}e^{i|m|\tilde{\phi}}\right)\ \eth^s\ Z_{lm},
\label{expansion}
\end{equation}
where $_sf=\{\beta,w,J,\overline{J},U,\overline{U}\}$, $Z_{lm}=\ _0Z_{lm}$, $\tilde{\phi}$ is a general function of the retarded time, i.e., $\tilde{\phi}:=\tilde{\phi}(u)$, $f_{lm}$ are the spectral components of the function $_sf$, $m\in \mathbb{Z}$, $m\in [-l,l]$ and $l\ge 0$ indicating the multipolar order. 
\\ Notice that in \eqref{expansion} the spin-weight of the function $_sf$ is contained in $\eth^s Z_{lm}$. Therefore, substituting \eqref{expansion} into the field equations \eqref{linear_field_eqs} one obtains ordinary differential equations for their spectral components, in which the spin-weighted factors have been eliminated, namely  
\begin{subequations}
	\begin{align}
	&\beta_{lm,r}= 2\pi \int_{\Omega}d\Omega\ \overline{Z}_{lm}\int_{0}^{2\pi}d\tilde\phi \ e^{-i|m|\tilde\phi} r T_{22} 
	\label{field_eq_s1} ,
	\end{align}
	\begin{align}
	& -\frac{(l+2)(l-1)J_{lm,r}}{2} -\beta _{lm,r} +\frac{2 \beta_{lm}}{r} +\frac{\left(r^4 U_{lm,r}\right)_{,r}}{2r^2} 
	\nonumber\\
	&
	= \frac{8 \pi}{\sqrt{l(l+1)}} \int_{\Omega} d\Omega \ \overline{Z}_{lm}\int_{0}^{2\pi} d\tilde\phi \ e^{-i|m|\tilde{\phi}} T_{2A} q^A, 
	\label{field_eq_s2}
	\end{align}
	\begin{align}
	& 2l(l+1) \beta_{lm} +(l-1)l(l+1)(l+2)J_{lm}  +\frac{l(l+1)\left(r^4\left(U_{lm}\right)\right)_{,r}}{r^2}\nonumber\\
	& + 4 \beta_{lm} -2 w_{lm,r} = 8 \pi \int_{\Omega}d\Omega \ \overline{Z}_{lm}\int_{0}^{2\pi}d\tilde\phi\ e^{-i|m|\tilde{\phi}}\left(h^{AB} T_{AB}-r^2 T\right) , \label{field_eq_s3}
	\end{align}
	\begin{align}
	&-2 \beta_{lm} + \left(r^2 U_{lm} \right)_{,r} - \left(r^2 J_{lm,r}\right)_{,r} +2 i|m| r\dot{\tilde{\phi}} \left(rJ_{lm}\right)_{,r} \nonumber\\
	&= \frac{8 \pi}{\sqrt{(l-1)l(l+1)(l+2)}} \int_{\Omega}d\Omega \ \overline{Z}_{lm} \int_{0}^{2\pi}d\tilde{\phi}\ e^{-i|m|\tilde{\phi}}T_{AB}  q^A q^B,
	\label{field_eq_s4}
	\end{align}
	\begin{align}
	& -\frac{l(l+1) w_{lm}}{2 r^3} - \frac{l(l+1)\beta_{lm} }{r^2} +i|m|l(l+1)\dot{\tilde{\phi}} U_{lm}  +\frac{i|m|\dot{\tilde{\phi}} w_{lm}}{r^2}   \nonumber\\
	&+\frac{w_{lm,rr}}{2 r} -\frac{2 i|m|\dot{\tilde{\phi}} \beta_{lm}}{r}+\frac{2\beta_{lm,r}}{r} + \beta_{lm,rr}-2\dot{\tilde{\phi}}\beta_{lm,r}\nonumber\\
	&=8 \pi \int_{\Omega}d\Omega \ \overline{Z}_{lm} \int_{0}^{2\pi}d\tilde{\phi}\ e^{-i|m|\tilde{\phi}} \left(\frac{T}{2}+T_{11}\right), \label{field_eq_s5}\\
	& -\frac{l(l+1)\beta_{lm} }{r^2} +\frac{l(l+1)\left(r^2 U_{lm} \right)_{,r}}{2r^2} +\frac{w_{lm,rr}}{2 r} \nonumber\\
	&=8 \pi \int_{\Omega}d\Omega \ \overline{Z}_{lm} \int_{0}^{2\pi}d\tilde{\phi}\ e^{-i|m|\tilde{\phi}} \left(\frac{T}{2}+T_{12}\right), \label{field_eq_s6}
	\end{align}
	\begin{align}
	& -\frac{i|m|(l+2)(l-1)J_{lm}\dot{\tilde{\phi}}}{2} +\frac{1}{2}\left(\frac{w_{lm}}{r}\right)_{,r} -i|m|\dot{\tilde{\phi}} \beta _{lm} +\frac{\left(r^4U_{lm,r}\right)_{,r}}{2r^2}\nonumber\\
	& -\frac{i|m|r^2\dot{\tilde{\phi}}}{2}U_{lm,r} +U_{lm} =\frac{8 \pi}{\sqrt{l(l+1)}}  \int_{\Omega}d\Omega \ \overline{Z}_{lm} \int_{0}^{2\pi}d\tilde{\phi}\ e^{-i|m|\tilde{\phi}} T_{1A} q^A, \label{field_eq_s7}
	\end{align}
	\label{field_eq_s}
\end{subequations}
This system of coupled ordinary equations is separable through a simple procedure, as we will show in the next section. Notice that an alternative procedure is presented by M\"adler in \cite{M13}.

==> docs/IVP.tex <==
\subsection{Characteristic Initial Value Problem}
%\def\input@path{{./Figuras/Characteristic/}}
\begin{figure}[h!]
	\begin{center}
		\input{./Figuras/Characteristic/foliation_1.eps_tex}
		\caption{Space-time $\mathcal M$ foliated in 2D - null hypersurfaces $\Sigma$.}
		\label{FADM1}
	\end{center}
\end{figure}
\begin{figure}[h!]
	\begin{center}
		\input{./Figuras/Characteristic/foliation_2.eps_tex}
		\caption{Space-time $\mathcal M$ foliated in 2D - null hypersurfaces $\Sigma$.}
		\label{FADM1}
	\end{center}
\end{figure}
\begin{figure}[h!]
	\begin{center}
		\input{./Figuras/Characteristic/foliation_3.eps_tex}
		\caption{Space-time $\mathcal M$ foliated in 2D - null hypersurfaces $\Sigma$.}
		\label{FADM1}
	\end{center}
\end{figure}


==> docs/Linear_Characteristic.tex <==
\chapter{THE LINEAR REGIME IN THE CHARACTERISTIC FORMULATION}
The linear regime of the field equations leads to different approximations according with how it is made. Here, we put the Bondi-Sachs metric in terms of the spin-weighted scalars $J,w$ and $\beta$ in stereographic-radiation coordinates
\begin{eqnarray}
\label{bs_explicit}
ds^2&=&-\left(e^{2\beta}\left(1+\frac{w}{r}\right)-r^2(J\bar{U}^2+U^2\bar{J}+2 K U \bar{U})\right)du^2  -2e^{2\beta}dudr \nonumber\\
&&-\frac{2r^2\left((K +\bar{J}) U+(J+K) \bar{U}\right)}{1+|\zeta|^2}dq du\nonumber\\
&&-\frac{2ir^2\left((K -\bar{J}) U+(J-K)	\bar{U}\right)}{1+|\zeta|^2}dpdu+\frac{2 r^2 \left(J+2K+\bar{J}\right)}{(1+|\zeta|^2)^2}dq^2\nonumber\\
&&-\frac{4 i r^2
	\left(J-\bar{J}\right)}{(1+|\zeta|^2)^2}dqdp-\frac{2 r^2 \left(J-2 K+\bar{J}\right)}{(1+|\zeta|^2)^2}dp^2.
\end{eqnarray}
\\In the weak field limit, i.e., when slight deviations from the Minkowski background $|g_{\mu\nu}|\ll|\eta_{\mu\nu}|$  are considered, and the second order terms are disregarded, the Bondi-Sachs metric is reduced to,
\begin{eqnarray}
\label{bs_lin}
ds^2&=&-\left(1-\frac{w}{r}-2\beta\right)du^2 -2(1+2\beta)dudr -2r^2\frac{(U+\overline{U})}{1+|\zeta|^2}dq du
\nonumber \\&& 
-2r^2\frac{i(U-\overline{U})}{1+|\zeta|^2}dp du+2r^2\frac{\left(2+J+\overline{J}\right)}{\left(1+|\zeta|^2\right)^2}dq^2\nonumber\\&&
-4ir^2\frac{(J-\overline{J})}{(1+|\zeta|^2)^2}dqdp-2r^2\frac{\left(-2+J+\overline{J}\right)}{\left(1+|\zeta|^2\right)^2}dp^2,
\end{eqnarray} 
which clearly can be separated as,
\begin{eqnarray}
\label{bs_lin2}
ds^2&=&-du^2-2dudr + \frac{4r^2}{\left(1+|\zeta|^2\right)^2}\left(dq^2+dp^2\right) +\left(\frac{w}{r}+2\beta\right)du^2   \nonumber\\
&&-4\beta dudr -\frac{2r^2}{1+|\zeta|^2}du\left((U+\overline{U})dq -i(U-\overline{U})dp \right)
\nonumber \\&& 
-4ir^2\frac{(J-\overline{J})}{(1+|\zeta|^2)^2}dqdp+\frac{2r^2\left(J+\overline{J}\right)}{\left(1+|\zeta|^2\right)^2}\left(dq^2-dp^2\right),
\label{bs_lin_pert}
\end{eqnarray} 
showing that it corresponds to a Minkowski background plus a perturbation. 
\input{./docs/CLEFE}
%\section{Bondi's News Functions}
%\section{Weyl tensor and $\Psi_4$}
\input{./docs/HDBP}
\input{./docs/ME}
\section{Families of Solutions to the Master Equation}
Now, the families of solutions to the master equations \eqref{field_eq_x11} and \eqref{meqsch1} associated with the linear approximation in the Minkowski and the Schwarzschild's space-times are explicitly shown. 
\\
To proceed, consider that $l$ is integer and greater than or equal to zero, i.e., $l\ge 0$, the constants of integration $C_i$ are complexes $C_i\in \mathbb{C}$, $i=1..4$, and arabic lower case letters represent real constants, i.e., $a,b,c,d,e,f,\cdots \in \mathbb{R}$
\\ It is worth stressing that the applicability of the present work has some limitations,
since in the context of the characteristic formulation the matter fields must be known a
priori throughout the space-time.
\input{./docs/Minkowski_Background}
\input{./docs/Schwarzschild_Background}
\input{.docs/Thin_Shell}
\input{.docs/Circular_Binary_System}
\input{.docs/Eccentric_Binary_System}

==> docs/ME.tex <==
\section{The Master Equation}
Making the change of variable $x=r^{-1}$, the field equations \eqref{field_eq_s1} - \eqref{field_eq_s4} become 
\begin{subequations}	
	\begin{align}
	&\beta_{lm,x}= -x^2A_{lm},  
	\label{field_eq_x1}\\
	& (l+2)(l-1)xJ_{lm,x} +2x\beta _{lm,x} +4 \beta_{lm} -2U_{lm,x}+xU_{lm,xx} = B_{lm}, 
	\label{field_eq_x2}\\
	& - 2x^3 J_{lm,xx}  -4 i|m|\dot{\tilde{\phi}} x J_{lm,x} +4i|m| \dot{\tilde{\phi}} J_{lm} +4 U_{lm} - 2xU_{lm,x}-4 x\beta_{lm} 
	\nonumber\\
	&
	= 2x D_{lm},
	\label{field_eq_x4}
	\end{align}
\end{subequations}
where the source terms $A_{lm}:=A_{lm}(x)$, $B_{lm}:=B_{lm}(x)$ and $D_{lm}:=D_{lm}(x)$ are explicitly defined,
\begin{subequations}
	\begin{align}
	& A_{lm}=2\pi \int_{\Omega}d\Omega\ \overline{Z}_{lm}\int_{0}^{2\pi}d\tilde\phi \ e^{-i|m|\tilde\phi} x T_{22},\\
	& B_{lm}=\frac{16 \pi}{\sqrt{l(l+1)}} \int_{\Omega} d\Omega \ \overline{Z}_{lm}\int_{0}^{2\pi} d\tilde\phi \ e^{-i|m|\tilde{\phi}} x T_{2A} q^A,\\
	& D_{lm}= \frac{8 \pi}{\sqrt{(l-1)l(l+1)(l+2)}} \int_{\Omega}d\Omega \ \overline{Z}_{lm} \int_{0}^{2\pi}d\tilde{\phi}\ e^{-i|m|\tilde{\phi}}T_{AB}  q^A q^B.
	\end{align}
\end{subequations}
In addition, solving \eqref{field_eq_x2} for $4x\beta_{lm}$ 
and substituting it into \eqref{field_eq_x4}, one obtains
\begin{align}
& - 2x^3 J_{lm,xx}  -4 i|m| \dot{\tilde{\phi}}xJ_{lm,x} + x^2(l+2)(l-1)J_{lm,x} +4i|m| \dot{\tilde{\phi}} J_{lm}   \nonumber \\
&  +x^2U_{lm,xx} - 4xU_{lm,x} +4 U_{lm} +2x^2\beta _{lm,x}  = x (2D_{lm}+ B_{lm}).
\label{field_eq_x5}
\end{align}
Thus, the derivative of \eqref{field_eq_x5} with respect to $x$ yields  a third order differential equation for $J_{lm}$, i.e., 
\begin{align}
& - 2x^3 J_{lm,xxx} - 6x^2 J_{lm,xx}  -4 i|m| \dot{\tilde{\phi}}xJ_{lm,xx} + x^2(l+2)(l-1)J_{lm,xx} \nonumber\\
&+ 2x(l+2)(l-1) J_{lm,x}   +x^2U_{lm,xxx}  - 2xU_{lm,xx}   \nonumber \\
&  +4x\beta _{lm,x} +2x^2\beta _{lm,xx} = (2D_{lm}+ B_{lm}) + x (2D_{lm,x}+ B_{lm,x}).
\label{field_eq_x6}
\end{align}
After this, notice that it is possible to obtain $x^2U_{lm,xxx}$ just deriving \eqref{field_eq_x2} with respect to $x$, 
\begin{align}
&  x^2U_{lm,xxx} = -x^2(l+2)(l-1)J_{lm,xx} -x(l+2)(l-1)J_{lm,x}  +xU_{lm,xx}  \nonumber\\
&  -6x\beta _{lm,x} -2x^2\beta _{lm,xx} + x B_{lm,x}.
\label{field_eq_x7}
\end{align}
Then, substituting it in \eqref{field_eq_x6} and simplifying one obtains
\begin{align}
& - 2x^3 J_{lm,xxx} - 6x^2 J_{lm,xx}  -4 i|m| \dot{\tilde{\phi}}xJ_{lm,xx} + x(l+2)(l-1) J_{lm,x} \nonumber\\
&  -xU_{lm,xx}  -2x\beta _{lm,x} = 2 x D_{lm,x}+B_{lm}+2 D_{lm}.
\label{field_eq_x8}
\end{align}
Making the derivative of \eqref{field_eq_x8} with respect to $x$, and substituting  $xU_{xxx}$ from \eqref{field_eq_x7} one  finds a fourth order differential equation for $J_{lm}$, namely
\begin{align}
&  - 2x^4 J_{lm,xxxx} - 12x^3 J_{lm,xxx} - 12x^2 J_{lm,xx}   -4i|m|  \dot{\tilde{\phi}}xJ_{lm,xx} -4i|m|  \dot{\tilde{\phi}} x^2 J_{lm,xxx} \nonumber\\
&+ 2x(l+2)(l-1) J_{lm,x} + 2x^2(l+2)(l-1) J_{lm,xx} +4x\beta _{lm,x} -2x U_{lm,xx}  \nonumber\\
&= 2 x B_{lm,x}+2 x^2 D_{lm,xx}+4 x D_{lm,x}.
\label{field_eq_x10}
\end{align}
Finally, solving \eqref{field_eq_x8} for $U_{lm,xx}$ and substituting into \eqref{field_eq_x10}, a differential equation containing only $J_{lm}$ with source terms is obtained, namely
\begin{align}
&  - 2x^4 J_{lm,xxxx} - 4x^2\left(2x  + i|m|\dot{\tilde{\phi}}\right)J_{lm,xxx} \nonumber\\ &+2x\left(2i|m|  \dot{\tilde{\phi}} + x(l+2)(l-1) \right)J_{lm,xx}  
   = H_{lm}(x),
\label{field_eq_x11}
\end{align}
where 
\begin{align}
H_{lm}(x)=2 x B_{lm,x}+2 x^2 D_{lm,xx}-8 x \beta_{lm,x}-2 B_{lm}-4 D_{lm}
\end{align}
represents the source terms.\\
In order to reduce the order of this differential equation, one  defines \\  $\tilde{J}_{lm}=J_{lm,xx}$, thus,
\begin{align}
&  - 2x^4 \tilde{J}_{lm,xx} - 4x^2\left(2x  + i|m|\dot{\tilde{\phi}}\right)\tilde{J}_{lm,x} +2x\left(2i|m|  \dot{\tilde{\phi}} + x(l+2)(l-1) \right)\tilde{J}_{lm}  
   = H_{lm}.
\label{field_eq_x12}
\end{align}
For the vacuum, this differential equation turns homogeneous, i.e.,  $H_{lm}=0$, and hence \eqref{field_eq_x12} is reduced to the master equation presented by M\"adler in \cite{M13}
\begin{align}
- x^3 \tilde{J}_{lm,xx} - 2x\left(2x  + i|m|\dot{\tilde{\phi}}\right)\tilde{J}_{lm,x} +\left(2i|m|  \dot{\tilde{\phi}} + x(l+2)(l-1) \right)\tilde{J}_{lm}  
= 0.
\label{field_eq_x13}
\end{align}
Making $l=2$, this master equation reduces to those presented previously in \cite{B05} for the Minkowski's Background i.e.,
\begin{align*}
- x^3 \tilde{J}_{lm,xx} - 2x\left(2x  + i|m|\dot{\tilde{\phi}}\right)\tilde{J}_{lm,x} +2\left(i|m|  \dot{\tilde{\phi}} + 2x \right)\tilde{J}_{lm}  = 0.
\end{align*}
The derivation of the master equation for the Schwarzschild's background follows the same scheme. In this case the master equation is given by
\begin{align}
& J_{lm,xxxx}x^4 (2 M x-1) + J_{lm,xxx} \left(2 x^3 (7 M x-2)-2 i x^2 \dot{\tilde{\phi }}
\left| m\right| \right)\nonumber\\
&+J_{lm,xx} \left(2 i x \dot{\tilde{\phi }} \left| m\right| +(l-1) (l+2) x^2+16 M
x^3\right)=G_{lm}(x),
\label{meqsch1}
\end{align}
where $M$ is the mass of the central static black-hole and $G_{lm}(x)$ represents the source term, which is given by
\begin{equation}
G_{lm}(x)=\frac{H_{lm}(x)}{2}.
\end{equation}
It is important to observe that $M=0$ effectively reduces \eqref{meqsch1} to \eqref{field_eq_x11}. 
\\
Defining $\tilde{J}_{lm}=J_{lm,xx}$, the order of the differential equation \eqref{meqsch1} is reduced, namely 
\begin{align}
& \tilde{J}_{lm,xx}x^4 (2 M x-1) + \tilde{J}_{lm,x} \left(2 x^3 (7 M x-2)-2 i x^2 \dot{\tilde{\phi }}
\left| m\right| \right)\nonumber\\
&+\tilde{J}_{lm} \left(2 i x \dot{\tilde{\phi }} \left| m\right| +(l-1) (l+2) x^2+16 M
x^3\right)=G_{lm}(x).
\label{meqsch2}
\end{align}

==> docs/Minkowski_Background.tex <==
\subsection{The Minkowski's Background}
First, let us consider the most simple case corresponding to the non-radiative, $m=0$, Minkowski's master equation without sources \eqref{field_eq_x13}. Assuming the ansatz \\ $J_{lm}=x^k$, we obtain immediately 
\begin{equation*}
(k-l+1) (k+l+2)=0,
\end{equation*}
whose roots leave us to the general family of solutions, 
\begin{equation}
\tilde{J}_{l0}(x)= C_1 x^{l-1}+C_2 x^{-(l+2)}.
\label{Msol1}
\end{equation}
Thus, integrating the last equation two times and rearranging the constants one obtains families of solutions to \eqref{field_eq_x11} of four parameters for the vacuum,
\begin{equation}
J_{l0}(x)= C_1 x^{l+1}+C_2 x^{-l}+C_3x+C_4.
\label{Msol2}
\end{equation}
When the source term is not null, we find that the non-radiative family of solutions, $m=0$, to the inhomogeneous equation \eqref{field_eq_x12} reads
\begin{align}
\tilde{J}_{l0}(x)=& C_1 x^{l-1} + C_2 x^{-(l+2)}+ x^{-(l+2)} \int_a^x dy\, \frac{H(y) y^{l-1}}{2 l+1} -x^{l-1} \int_b^x dy\, 
\frac{H(y) y^{-(l+2)}}{2 l+1}, 
\label{Msol3}
\end{align}
where $a$ and $b$ are real constants. Therefore, integrating two times with respect to $x$ and rearranging the constants we find the family of solutions to the inhomogeneous master equation \eqref{field_eq_x11}, for $m=0$,
\begin{align}
J_{l0}(x)=& C_1 x^{l+1}+ C_2 x^{-l}+ C_3x +C_4
+ \int_a^x dv\, \int_{b}^{v}dw \, w^{-(l+2)} \int_c^w dy\, \frac{H(y) y^{l-1}}{4 l+2}
\nonumber\\
&  -\int_d^xdv\, \int_{e}^{v} dw\, w^{l-1} \int_f^w dy\, \frac{H(y) y^{-(l+2)}}{4 l+2},
\label{Msol4}
\end{align}
where it is clear that the analyticity of the solutions depends on the existence and analyticity of the integrals. If the source term is disregarded, then \eqref{Msol4} is reduced immediately to \eqref{Msol2}.
\\Now, we will consider the case for a radiative family of solutions, $m\ne 0, \ |m|\le l$ for $l> 0$, without source term. In this case \eqref{field_eq_x13} becomes a Bessel's type differential equation. \citeonline{M13} previously shows that the general solutions to this master equation can be expressed as a linear combination of the first and second kind spherical Bessel's functions. We find here that the family of solutions to the master equation  \eqref{field_eq_x13} can be expressed in terms only of the first kind Bessel's functions, as
\begin{align}
\tilde{J}_{lm}&=\frac{C_1 2^{\frac{1}{2}-2 l} z^{3/2} e^{\frac{1}{2} i (\pi  l+2 z)} \Gamma \left(\frac{1}{2}-l\right) \left(K
	J_{-l-\frac{1}{2}}+L J_{\frac{1}{2}-l}\right)}{(l-1) l}\nonumber\\
&+\frac{i C_2 2^{2 l+\frac{5}{2}} z^{3/2} e^{i
		z-\frac{i \pi  l}{2}} \Gamma \left(l+\frac{3}{2}\right) \left(K J_{l+\frac{1}{2}}+L
	J_{l-\frac{1}{2}}\right)}{(l+1) (l+2)},
\label{mes2}
\end{align}
where the argument of the first kind Bessel's functions $J_{n}$ are referred to $z$, which is defined as
\begin{equation}
z=\dfrac{|m|\dot{\tilde{\phi}}}{x},
\label{zdef}
\end{equation}
and the coefficients $K$, $L$ and $S$ are,
\begin{subequations}
	\begin{align}
    K&=-i (l(l-1)+2iz) -2z(l-i z),\\
	L&=-2 z (z-i),\\
	S&=l(l-1)+2iz.
	\end{align}
\end{subequations}
Integrating two times \eqref{mes2}, and rearranging the constants we find the family of solutions that satisfies \eqref{field_eq_x11}, i.e.,
\begin{align}
J_{lm}=&-\frac{iC_1 2^{\frac{1}{2}-2 l} \dot{\tilde{\phi}} ^2 \left| m\right| ^2 z^{-1/2}e^{\frac{1}{2} i (\pi  l+2 z)} \Gamma
	\left(\frac{1}{2}-l\right) \left(-2 z J_{\frac{1}{2}-l}+\overline{S}
	J_{-l-\frac{1}{2}}\right)}{l^2 \left(l^2-1\right)}\nonumber\\
&-\frac{C_22^{2 l+\frac{5}{2}} \dot{\tilde{\phi}} ^2 \left| m\right| ^2 z^{-1/2}e^{-\frac{1}{2} i (\pi  l-2 z)} \Gamma
	\left(l+\frac{3}{2}\right) \left(2 z J_{l-\frac{1}{2}}+\overline{S}
	J_{l+\frac{1}{2}}\right)}{l (l+1)^2 (l+2) }\nonumber\\
&+C_3+C_4\frac{\dot{\tilde{\phi}} |m|}{z}.
\end{align}
When matter is considered, we found that the family of solutions to \eqref{field_eq_x13} becomes,
\begin{align}
\tilde{J}_{lm}=&\frac{2^{\frac{1}{2}-2 l} z^{3/2} \left(C_1+D_1\right) e^{\frac{i \pi  l}{2}+i z} \Gamma
	\left(\frac{1}{2}-l\right) \left(K J_{-l-\frac{1}{2}}+L J_{\frac{1}{2}-l}\right)}{(l-1) l}\nonumber\\
&+\frac{i 2^{2
		l+\frac{5}{2}} z^{3/2} \left(C_2+D_2\right) e^{i z-\frac{i \pi  l}{2}} \Gamma \left(l+\frac{3}{2}\right)
	\left(K J_{l+\frac{1}{2}}+L J_{l-\frac{1}{2}}\right)}{(l+1) (l+2)},
\label{mes3}
\end{align}
where the coefficients $K$ and $L$ were defined above, and the terms representing sources are
\begin{subequations}	
\begin{align}
D_1=-&\int_{|m|\dot{\tilde{\phi}}}^{|m|\dot{\tilde{\phi}}/z}d\tilde{z}\, \frac{2^{2 l-\frac{5}{2}} \tilde{z}^{-1/2} e^{-\frac{1}{2} i (\pi  l+2 \tilde{z})} \Gamma \left(l+\frac{1}{2}\right)  \left(K J_{l+\frac{1}{2}}-L
	J_{l-\frac{1}{2}}\right)}{(l+1) (l+2) \dot{\tilde{\phi}} ^2 \left| m\right| ^2}H\left(\frac{\dot{\tilde{\phi}}  \left| m\right| }{\tilde{z}}\right),
\end{align}
and
\begin{align}
D_2=&-i\int_{|m|\dot{\tilde{\phi}}}^{|m|\dot{\tilde{\phi}}/z}d\tilde{z}\, \frac{ 2^{-2 l-\frac{9}{2}}\tilde{z}^{-1/2} e^{\frac{1}{2} i (\pi  l-2 \tilde{z})} \Gamma \left(-l-\frac{1}{2}\right)  \left(K J_{-l-\frac{1}{2}}+L
	J_{\frac{1}{2}-l}\right)}{(l-1) l \dot{\tilde{\phi}} ^2  \left| m\right| ^2} H\left(\frac{\dot{\tilde{\phi}}  \left| m\right| }{\tilde{z}}\right),
\end{align}
\end{subequations}
where the argument of the first kind Bessel's functions $J_n$ is $z$, which is defined just in \eqref{zdef}.
It is worth noting that in this form, it is clear that \eqref{mes3} converges immediately to \eqref{mes2}, when the sources are not considered. 
\\
Integrating \eqref{mes3} two times  we obtain the general family of solutions to the master equation with sources, which reads 
\begin{align}
J_{lm}=&-\frac{iC_1 2^{\frac{1}{2}-2 l} \dot{\tilde{\phi}} ^2 \left| m\right| ^2 z^{-1/2}e^{\frac{1}{2} i (\pi  l+2 z)} \Gamma
	\left(\frac{1}{2}-l\right) \left(-2 z J_{\frac{1}{2}-l}+\overline{S}
	J_{-l-\frac{1}{2}}\right)}{l^2 \left(l^2-1\right)}\nonumber\\
&-\frac{C_22^{2 l+\frac{5}{2}} \dot{\tilde{\phi}} ^2 \left| m\right| ^2 z^{-1/2}e^{-\frac{1}{2} i (\pi  l-2 z)} \Gamma
	\left(l+\frac{3}{2}\right) \left(2 z J_{l-\frac{1}{2}}+\overline{S}
	J_{l+\frac{1}{2}}\right)}{l (l+1)^2 (l+2) }\nonumber\\
&+\int_b^{z}dy\,\int_{a}^{y}d \tilde{z}\, \left(\frac{2^{\frac{1}{2}-2 l} \tilde{z}^{3/2} D_1 e^{\frac{i \pi  l}{2}+i \tilde{z}} \Gamma
	\left(\frac{1}{2}-l\right) \left(K J_{-l-\frac{1}{2}}+L J_{\frac{1}{2}-l}\right)}{(l-1) l}\right.\nonumber\\
&\left.+\frac{i 2^{2
		l+\frac{5}{2}} \tilde{z}^{3/2} D_2 e^{i \tilde{z}-\frac{i \pi  l}{2}} \Gamma \left(l+\frac{3}{2}\right)
	\left(K J_{l+\frac{1}{2}}+L J_{l-\frac{1}{2}}\right)}{(l+1) (l+2)}\right)      \nonumber\\
&+C_3+C_4\frac{\dot{\tilde{\phi}} |m|}{z}.
\label{mes4}
\end{align}
These families of solutions are particularly interesting and useful to explore the dynamics of matter clouds immersed in a Minkowski's background.

==> docs/Schwarzschild_Background.tex <==
\subsection{The Schwarzschild's Background}
Now, we show the non-radiative families of solutions, $m=0$, for the vacuum i.e., $G(x)=0$, for equation \eqref{meqsch2}. The solution is expressed in terms of the hypergeometric functions $_2F_1(a_1,a_2;b;z)$, as
\begin{align}
\tilde{J}_{lm}=& (-2)^{-l-2} C_1  M^{-l-2} x^{-l-2} \, _2F_1(2-l,-l;-2 l;2 M x) \nonumber\\
&+ (-2)^{l-1} C_2  M^{l-1} x^{l-1} \, _2F_1(l+1,l+3;2l+2;2 M x).
\label{sch1}
\end{align}
Integrating two times, we find the family of solutions to \eqref{meqsch1}
\begin{align}
J_{lm}=& \frac{C_1 (-1)^{-l} 2^{-l-2} (M x)^{-l} \, _3F_2(-l-1,2-l,-l;1-l,-2 l;2 M x)}{l (l+1) M^2}\nonumber\\
&+\frac{C_2 (-1)^{l+1}
	2^{l-1} x (M x)^l \, _3F_2(l,l+1,l+3;l+2,2 l+2;2 M x)}{l (l+1) M} + C_3x +C_4,
\label{sch2}
\end{align}
where, $_pF_q(a_1,\cdots a_p ;b_1,\cdots, b_q;z)$ are the generalised hypergeometric functions.
\\When we consider the source terms, i.e., $H(x)\ne 0$, the non radiative solutions to \eqref{meqsch2} reads,
\begin{align}
\tilde{J}_{lm}=&(-1)^{1-l} 2^{-l-2} M^{-l-2} x^{-l-2} \left(A_2 (-1)^{2 l} 2^{2 l+1} M^{2 l+1} x^{2 l+1} \, _2F_1(l+1,l+3;2 l+2;2M x)\right.\nonumber\\
&\left.-A_1 \, _2F_1(2-l,-l;-2 l;2 M x)\right)
 +C_1 (-2)^{-l-2} M^{-l-2} x^{-l-2} \, _2F_1(2-l,-l;-2 l;2 M x)\nonumber\\
&+C_2 (-2)^{l-1} M^{l-1} x^{l-1} \, _2F_1(l+1,l+3;2 l+2;2 M x),
\label{sch3}
\end{align}
where $A_1$, $A_2$ are given by the integrals
\begin{subequations}
\begin{align}
A_1&=-\int_a^xdy\,\frac{(-2)^{l+2} H(y) M^{l+2} y^l \, _2F_1(l+1,l+3;2 (l+1);2 M y)}{B_1+B_2},\\
A_2&=\int_b^x dy\, \frac{(-2)^{1-l} H(y) M^{1-l} y^{-l-1} \, _2F_1(2-l,-l;-2 l;2 M y)}{B_1+B_2},
\end{align}
\end{subequations}
and the functions $B_1$ and $B_2$ are 
\begin{subequations}
\begin{align}
B_1=&(2 M y-1) ((l-2) \, _2F_1(3-l,-l;-2 l;2 M y)\, _2F_1(l+1,l+3;2 (l+1);2 M y),\\
B_2=&\, _2F_1(2-l,-l;-2 l;2 M y) (2 \, _2F_1(l+1,l+3;2 (l+1);2 M y)\nonumber\\
&+(l+1) \,_2F_1(l+2,l+3;2 (l+1);2 M y))).
\end{align}
\end{subequations}
For the radiative ($m\ne 0$) family of solutions to the master equation \eqref{meqsch2} for the vacuum, we find that its most general solution is given by
\begin{align}
\tilde{J}_{lm}=& C_1 L e^{\frac{2\alpha}{xM}} x^{-4}+C_2K \left(2Mx-1\right)^{4\alpha -2}x^{-2-4\alpha} e^{\frac{2\alpha}{xM}},
\label{heunc_sols}
\end{align}
with
\begin{align}
L=H_C\left(-4\alpha ,\beta;\gamma,\delta,\epsilon,\eta\right)\hspace{0.5cm} {\rm and} \hspace{0.5cm}
K=H_C\left(-4\alpha ,-\beta;\gamma,\delta,\epsilon,\eta\right),
\end{align}
where $H_C(\alpha,\beta;\gamma,\delta,\epsilon,\eta)$ are the confluent Heun's functions and their parameters are given by
\begin{subequations}
\begin{align}
\alpha &= i\dot{\tilde{\phi}}m M,\hspace{4.6cm}\beta  = 2-4\alpha,\\
\gamma &= 2, \hspace{5.6cm} \delta = 8\alpha(\alpha-1),\\
\epsilon &=-(l+2)(l-1)-8\alpha(\alpha-1),\hspace{0.8cm}\eta =\frac{2Mx-1}{2Mx}.
\end{align}
\label{heun_par}
\end{subequations}
Finally, we present the analytical family of solutions to \eqref{meqsch2} in the radiative case, $m\ne 0$,  when the source terms are considered,
\begin{align}
J_{lm} =&-8M{e^{\frac {2a}{Mx}}} \left( -LMx+{M}^{2}{x}^{2}L+L/4
\right) A_1 x^{-4} \left( 2Mx-1 \right) ^{-2}\nonumber\\
&+2M{e^{\frac {2a}{Mx}}}{x}^{2-4a} \left( 2Mx-1 \right) ^{4a}A_2 K{x}^{-4} \left( 2Mx-1 \right) ^{-2}\nonumber\\
&+C_1 L e^{\frac {2a}{Mx}} x^{-4} + C_2 K e^{\frac {2a}{Mx}} x^{-2-4a}
\left( 2Mx-1 \right)^{-2+4a},
\end{align}
where $A_1$ and $A_2$ are the integrals
\begin{subequations}
\begin{align}
A_1=&\int_a^x d\tilde{x}\, \frac{\tilde{x}^2 H(\tilde{x}) e^{-\frac{2a}{M\tilde{x}}}K}{-4\,
	LKM\tilde{x}+8\,LKaM\tilde{x}-LS+2\,LM\tilde{x}S+KR-2\,KM\tilde{x}R} \label{a1}\\
A_2=&\int_b^x d\tilde{x}\, \frac{4\tilde{x}^{4a}{e^{-\frac {2a}{M\tilde{x}}}}H(\tilde{x})
\left( M\tilde{x}-1/2 \right) ^{2} \left( 2M\tilde{x}-1 \right) ^{-4a}L}{-4
\,LKM\tilde{x}+8\,LKaM\tilde{x}-LS+2\,LM\tilde{x}S+KR-2\,KM\tilde{x}R}\label{a2} ,
\end{align}
\end{subequations}
where $S$ and $R$ are the derivative of the Heun's functions, i.e. $S=K'(x)$ and $R=L'(x)$, in which we suppress all indices except one which gives the functional dependence. 
\section{Families of Solutions for $l=2$}
Now, we show that the families of solutions found here are reduced to those previously reported in the literature for $l=2$. Thus, for this particular value of $l$ we obtain that the family of solutions to the master equation for the vacuum, \eqref{field_eq_x13} takes the explicit form
\begin{equation}
\tilde{J}_{lm}=E_1 x+\frac{E_2 e^{\frac{2 i \dot{\tilde{\phi }} \left| m\right| }{x}} \left(6 x^3 \dot{\tilde{\phi }} \left| m\right| -6 i x^2 \dot{\tilde{\phi }}^2 \left| m\right| ^2-4 x
	\dot{\tilde{\phi }}^3 \left| m\right| ^3+2 i \dot{\tilde{\phi }}^4 \left| m\right| ^4+3 i x^4\right)}{4 x^3 \dot{\tilde{\phi }}^5 \left| m\right| ^5}.
\label{fam1}
\end{equation}
Now, substituting $l=2$ in the family of solutions \eqref{mes2}, one obtains
\begin{align}
\tilde{J}_{lm}=&\frac{i C_1 \dot{\tilde{\phi}} ^3 \left| m\right| ^3 e^{\frac{2 i \dot{\tilde{\phi}}  \left| m\right| }{x}}}{6 x^3}-\frac{40 i C_2 \dot{\tilde{\phi}} ^3 \left| m\right| ^3 e^{\frac{2 i \dot{\tilde{\phi}}  \left| m\right|
		}{x}}}{x^3}-\frac{C_1 \dot{\tilde{\phi}} ^2 \left| m\right| ^2 e^{\frac{2 i \dot{\tilde{\phi}}  \left| m\right| }{x}}}{3 x^2} +\frac{80 C_2 \dot{\tilde{\phi}} ^2 \left| m\right| ^2 e^{\frac{2 i \dot{\tilde{\phi}}  \left| m\right|
	}{x}}}{x^2} \nonumber
\\&-\frac{i C_1 \dot{\tilde{\phi}}  \left| m\right|  e^{\frac{2 i \dot{\tilde{\phi}}  \left| m\right| }{x}}}{2 x}+\frac{120 i C_2 \dot{\tilde{\phi}}  \left| m\right|  e^{\frac{2 i \dot{\tilde{\phi}}  \left| m\right|
}{x}}}{x}+\frac{1}{2} C_1 e^{\frac{2 i \dot{\tilde{\phi}}  \left| m\right| }{x}} -120 C_2 e^{\frac{2 i \dot{\tilde{\phi}}  \left| m\right| }{x}}\nonumber
\\&+\frac{i C_1 x e^{\frac{2 i \dot{\tilde{\phi}}  \left| m\right| }{x}}}{4 \dot{\tilde{\phi}} 
\left| m\right| }+\frac{i C_1 x}{4 \dot{\tilde{\phi}}  \left| m\right| }-\frac{60 i C_2 x e^{\frac{2 i \dot{\tilde{\phi}}  \left| m\right| }{x}}}{\dot{\tilde{\phi}}  \left| m\right| }+\frac{60 i  x}{\dot{\tilde{\phi}}  \left|
m\right| }.
\label{fam2}
\end{align} 
Both family of solutions, \eqref{fam1} and \eqref{fam2}, are completely equivalent. Note that, the transformation between the constants, necessary to pass from \eqref{fam1} to \eqref{fam2} is given by
\begin{equation}
E_1= \frac{i \left(C_1+240 C_2\right)}{4 \dot{\tilde{\phi}}  \left| m\right| },\hspace{1cm}
E_2= \frac{1}{3} \left(C_1-240 C_2\right) \dot{\tilde{\phi}} ^4 \left| m\right| ^4.
\end{equation}
Note that for the Schwarzschild case, when no sources are present, the master equation \eqref{meqsch2}, for the vacuum and $l=2$ takes the explicit form
\begin{align}
x^2 (2 M x-1) \tilde{J}_{lm,xx}+2 x (7 M x-2) \tilde{J}_{lm,x}+ (16 M x+4)\tilde{J}_{lm}=0.
\end{align}
Its family of solutions is
\begin{equation}
\tilde{J}_{lm}=\frac{C_1}{x^4}-\frac{C_2 \left(16 M^4 x^4+32 M^3 x^3-44 M^2 x^2-4 M x+12 (1-2 M x)^2 \log (1-2 M x)+7\right)}{64
	M^5 x^4 (1-2 M x)^2}.
\end{equation}
Now, specialising the solutions \eqref{sch1} for $l=2$, we find a totally equivalent solution, i.e.,
\begin{equation}
\tilde{J}_{lm}=\frac{D_1}{16 M^4 x^4}+\frac{5 D_2 \left(2 M x \left(2 M^3 x^3+4 M^2 x^2-9 M x+3\right)+3 (1-2 M x)^2 \log (1-2 M
	x)\right)}{8 M^4 x^4 (1-2 M x)^2}.
\end{equation}
Thus, a simple Maclaurin series expansion of both solutions shows that the relationship between the constants is
\begin{align}
D_1= \frac{64 C_1 M^5-7 C_2}{4 M},\hspace{1cm} D_2 = -\frac{C_2}{10 M}.
\end{align}
Finally, given that the known family of solutions for $l=2$ is written in terms of power of series around the point $r=2M$, as shown in \cite{B05}, we expand the radiative family of solutions for the master equation \eqref{meqsch1} around the same point $r=2M$ for $l=2$. Thus, we observe that the Confluent Heun's function $H_C(-4\alpha,\beta;\gamma,\delta,\epsilon,\eta)$ is expressed as a Taylor series for the parameters \eqref{heun_par} around $\eta=0$, namely
\begin{align}
H_C(-4\alpha,\beta;\gamma,\delta,\epsilon,\eta)\simeq& 1+{\frac { \left( (4a+1)^2-5+(l-1)(l+2) \right) \eta}{-3+4\,a}}\nonumber\\
&+\frac{1}{8 (a-1) (4 a-3)}
\left( \left(256 a^4+192 a^3+32 a^2 \left(l^2+l-5\right) \right.\right.\nonumber\\
&+\left.\left. 4 a \left(4 l^2+4 l-39\right)+l^4+2 l^3-17 l^2-18 l+72\right)\eta^2\right),
\label{Heun1}
\end{align}
and for the Confluent Heun's function $H_C(-4\alpha,-\beta;\gamma,\delta,\epsilon,\eta)$, 
\begin{align}
H_C(-4\alpha,-\beta;\gamma,\delta,\epsilon,\eta)\simeq&1-\frac{\left(4 a+l^2+l\right)\eta}{4 a-1}-\frac{\left(12 a-l^4-2 l^3+l^2+2 l\right)\eta^2 }{8 a (4 a-1)}.
\label{Heun2}
\end{align}
Then, from \eqref{Heun1} and \eqref{Heun2} we obtain that around to $r=2M$, \eqref{heunc_sols} at first order for $l=2$, 
\begin{align}
\tilde{J}_{lm}=& C_1 \left(\frac{16 e^{4 \alpha } (4 \alpha +12) \eta  M^4}{4 \alpha -3}+16 e^{4 \alpha } M^4\right)
-\frac{2^{4 \alpha +2} C_2 e^{4 \alpha } \left(16 \alpha ^2+16 \alpha +2\right) \eta ^{4 \alpha -1}	\left(\frac{1}{M}\right)^{-4 \alpha -2}}{4 \alpha -1}\nonumber
\\
&+\frac{2^{4 \alpha -1} C_2 e^{4 \alpha } \left(256 \alpha^4+576 \alpha ^3+384 \alpha ^2+132 \alpha +24\right) \eta ^{4 \alpha } \left(\frac{1}{M}\right)^{-4 \alpha	-2}}{\alpha  (4 \alpha -1)}\nonumber\\
&-\frac{2^{4 \alpha +1} C_2e^{4 \alpha } \left(256 \alpha ^5+896 \alpha ^4+1056 \alpha^3+636 \alpha ^2+228 \alpha +72\right) \eta ^{4 \alpha +1} \left(\frac{1}{M}\right)^{-4 \alpha -2}}{3 \alpha(4 \alpha -1)}\nonumber\\
&+2^{4 \alpha +2} C_2 e^{4 \alpha } \eta ^{4 \alpha -2} \left(\frac{1}{M}\right)^{-4 \alpha -2},
\end{align}
that are just the family of solutions for the master equation obtained using power series around $r=2M$.

==> docs/abreviaturasesiglas.tex <==
\begin{abreviaturasesiglas}  

\\
ADM   &--&   Arnowitt-Deser-Misner formalism \\
IVP   &--&  Intial Value Problem\\
CIVP   &--&  Characteristic Intial Value Problem\\
WKB    &--&  Wentzel-Kramers-Brillouin\\
BSSN   &--&  Baumgarte-Shapiro-Shibata-Nakamura\\


\end{abreviaturasesiglas}


==> docs/angular_integrals.tex <==
\section{Integrals for the Angular Manifold}
In order to compute the inner product of the spin-weighted functions, we will need the correct expressions for the integrals involving angular variables. Thus is important to obtain these expressions when are used the $(q,p)$, $(\zeta,\overline{\zeta})$ and the $(\theta,\phi)$ coordinates. Then the quantities of the type
\begin{align}
I=\oiint\limits_{\Omega} d\Omega f(\theta,\phi),
\label{integral1}
\end{align}
where $\Omega$ is the complete solid angle, in spherical coordinates are expressed as
\begin{align}
I=\iint\limits_{\Omega} d\phi d\theta \sin\theta f(\theta,\phi).
\label{integral2}
\end{align}
These integrals can be decomposed in two parts,  involving each hemisphere in the form
\begin{align}
I&= \iint\limits_{\Omega_N} d\phi d\theta \sin\theta f(\theta,\phi) + \iint_{\Omega_S} d\phi d\theta \sin\theta f(\theta,\phi),\nonumber\\
&= \iint\limits_{\Omega_N} d\phi_N d\theta_N \sin\theta_N f(\theta_N,\phi_N) + \iint_{\Omega_S} d\phi_S d\theta_S \sin\theta_S f(\theta_S,\phi_S),
%&=\iint\limits_{\Omega_N} dq_N dp_N \sin\theta_N J(q_N,p_N) f(q_N,p_N)+\iint\limits_{\Omega_S} dq_S dp_S \sin\theta_S J(q_S,p_S) f(q_S,p_S)
\label{integral3}
\end{align}
where $\Omega_N$ and $\Omega_S$, label the north and the south regions in which was decomposed the unitary sphere. Both domains share the same boundary that is the equator line. 
\\Now, from the transformation of coordinates \eqref{stereo1}, it is possible write that
\begin{align}
q=\tan\left(\theta/2\right)\cos{\phi}, \hspace{1cm}p=\tan\left(\theta/2\right)\sin{\phi}.
\label{integral4}
\end{align}
Now, we will perform transformation of the coordinates from spherical to stereographic $(q,p)$. First, we rewrite \eqref{integral2} 
as
\begin{align}
I=&\iint\limits_{\Omega_N} dq_N dp_N \sin\theta_N J(q_N,p_N) f(q_N,p_N)\nonumber\\
&+\iint\limits_{\Omega_S} dq_S dp_S \sin\theta_S J(q_S,p_S) f(q_S,p_S),
\label{integral5}
\end{align}
where $J(q,p)$ is the Jacobian of the transformation of coordinates, (in which we suppress the index to indicate that the Jacobian has the same form for both hemispheres), which is given by
\begin{equation*}
J(q,p)=\left|\begin{matrix}
\theta_{,q} & \theta_{,p}\\
\phi_{,q} & \phi_{,p}
\end{matrix}\right|.
\end{equation*}
From \eqref{integral4}, the derivatives in the Jacobian are 
\begin{align}
\begin{array}{ll}
\theta_{,q}=\dfrac{2q(q^2+p^2)^{1/2}}{1+q^2+p^2}, & \theta_{,p}=\dfrac{2p(q^2+p^2)^{1/2}}{1+q^2+p^2},\\[0.5cm]
\phi_{,q}=-\dfrac{p}{q^2+p^2}, & \phi_{,p}=\dfrac{q}{q^2+p^2},
\end{array}
\label{integral6}
\end{align}
then,
\begin{equation}
J(q,p)=\dfrac{2(q^2+p^2)^{-1/2}}{1+q^2+p^2}.
\label{integral7}
\end{equation}
We must observe that 
\begin{align}
\sin\theta %&=\sin(2(\theta/2))\\
&=2\tan(\theta/2)\cos^2(\theta/2),\nonumber\\
&=\dfrac{2(q^2+p^2)^{1/2}}{1+q^2+p^2}.
\label{integral8}
\end{align}
Thus, the substitution of \eqref{integral7} and \eqref{integral8} into \eqref{integral3} yields us to
\begin{align}
I=\iint\limits_{\Omega_N} dq_N dp_N  \dfrac{4f(q_N,p_N)}{\left(1+q_N^2+p_N^2\right)^2}+\iint\limits_{\Omega_S} dq_S dp_S  \dfrac{4f(q_S,p_S)}{\left(1+q_S^2+p_S^2\right)^2}.
\label{integral9}
\end{align}
The last expression is particularly useful when is necessary the numerical evaluation of kind of integrals. From here, it is possible to obtain the expression of the same kind of integrals in terms of the complex stereographic coordinates $(\zeta,\overline{\zeta})$. These expressions are
\begin{align}
I=&\iint\limits_{\Omega_N} d\zeta_N d\overline{\zeta}_N J(\zeta_N,\overline{\zeta}_N)  \dfrac{4f(\zeta_N,\overline{\zeta}_N)}{\left(1+\zeta_N\overline{\zeta}_N\right)^2}\nonumber\\
&+\iint\limits_{\Omega_S} d\zeta_S d\overline{\zeta}_S  J(\zeta_S,\overline{\zeta}_S)\dfrac{4f(\zeta_S,\overline{\zeta}_S)}{\left(1+\zeta_S\overline{\zeta}_S\right)^2}
\label{integral10}
\end{align}
where, the Jacobian of the transformation of coordinates is given by
\begin{equation*}
J(\zeta,\overline{\zeta})=\left|\begin{matrix}
q_{,\zeta} & q_{,\overline{\zeta}}\\
p_{,\zeta} & p_{,\overline{\zeta}}
\end{matrix}\right|.
\end{equation*}
The derivatives in this Jacobian are
\begin{align}
\begin{array}{ll}
q_{,\zeta}=\dfrac{1}{2}, & q_{,\overline{\zeta}}=\dfrac{1}{2},\\[0.5cm]
p_{,\zeta}=-\dfrac{i}{2}, & p_{,\overline{\zeta}}=\dfrac{i}{2}.
\end{array}
\label{integral11}
\end{align}
Thus, the Jacobian of the transformation of the coordinates becomes explicitly
\begin{equation*}
J(\zeta,\overline{\zeta})=\dfrac{i}{2}.
\end{equation*}
Then the integral \eqref{integral10} in terms of $(\zeta,\overline{\zeta})$ is transformed as 
\begin{align}
I=\iint\limits_{\Omega_N} d\zeta_N d\overline{\zeta}_N   \dfrac{2if(\zeta_N,\overline{\zeta}_N)}{\left(1+\zeta_N\overline{\zeta}_N\right)^2}+\iint\limits_{\Omega_S} d\zeta_S d\overline{\zeta}_S  \dfrac{2if(\zeta_S,\overline{\zeta}_S)}{\left(1+\zeta_S\overline{\zeta}_S\right)^2}.
\label{integral12}
\end{align}
Thus, knowing the explicit form for these integrals, we are able to express the inner product of two functions that depends on the angular variables as
\begin{equation}
\langle f,g\rangle=\oiint\limits_{\Omega} d\Omega\overline{f}g.
\label{integral13}
\end{equation}
Thus, the inner product $\langle \ _0Y_{l'm'},\ _0Y_{lm}\rangle$, where $_0Y_{lm}=Y_{lm}$, can be computed in spherical coordinates as is usual
\begin{align}
\langle \ _0Y_{l'm'},\ _0Y_{lm}\rangle&=\int_0^{2\pi} d\phi \int_0^{\pi} d\theta \sin\theta \ _0\overline{Y}_{l'm'}(\theta,\phi) \ _0Y_{lm}(\theta,\phi),\nonumber\\
&=\delta_{ll'}\delta_{mm'}.
\label{integral14}
\end{align}
The explicit form of this inner product in stereographic coordinates $(q,p)$ is
\begin{align}
\langle \ _0Y_{l'm'},\ _0Y_{lm}\rangle&=\int_{-1}^{1} dq_N \int_{-\sqrt{1-q_N^2}}^{\sqrt{1-q_N^2}} dp_N  \dfrac{4\ _0\overline{Y_N}_{l'm'}(q_N,p_N) \ _0{Y_N}_{lm}(q_N,p_N)}{\left(1+q_N^2+p_N^2\right)^2}\nonumber\\
&+ \int_{-1}^{1} dq_S \int_{-\sqrt{1-q_S^2                                                                                                                   }}^{\sqrt{1-q_S^2}} dp_S  \dfrac{4\ _0\overline{Y_S}_{l'm'}(q_S,p_S) \ _0{Y_S}_{lm}(q_S,p_S)}{\left(1+q_S^2+p_S^2\right)^2},
\label{integral15}
\end{align}
which is completely analytic in $\Omega_N$ and $\Omega_S$. 
\\Now, observing that the $\eth$ and $\overline{\eth}$ operators can be written as
\begin{align}
\eth&=\dfrac{1+\zeta\overline{\zeta}}{2}\left(\partial_q+i\partial_p\right)+s\zeta, \nonumber\\
%&=\left(1+\zeta\overline{\zeta}\right)\partial_{\overline{\zeta}}+s\zeta \nonumber\\
%&=\left(1+\zeta\overline{\zeta}\right)^{1-s}\left(1+\zeta\overline{\zeta}\right)^{s-1}\left(\left(1+\zeta\overline{\zeta}\right)\partial_{\overline{\zeta}}+s\zeta\right)\\
&=\left(1+\zeta\overline{\zeta}\right)^{1-s}\left(\left(1+\zeta\overline{\zeta}\right)^{s}\partial_{\overline{\zeta}}+s\zeta\left(1+\zeta\overline{\zeta}\right)^{s-1}\right),\nonumber\\
&=\left(1+\zeta\overline{\zeta}\right)^{1-s}\partial_{\overline{\zeta}}\left(1+\zeta\overline{\zeta}\right)^{s}, \nonumber\\
&=P^{1-s}\partial_{\overline{\zeta}} P^{s},
\label{integral16}
\end{align}
and
\begin{align}
\overline{\eth}&=\dfrac{1+\zeta\overline{\zeta}}{2}\left(\partial_q-i\partial_p\right)-s\overline{\zeta}, \nonumber\\
&=\left(1+\zeta\overline{\zeta}\right)\partial_{{\zeta}}-s\overline{\zeta}, \nonumber\\
%&=\left(1+\zeta\overline{\zeta}\right)^{s+1}\left(1+\zeta\overline{\zeta}\right)^{-(s+1)}\left(\left(1+\zeta\overline{\zeta}\right)\partial_{{\zeta}}-s\overline{\zeta}\right) \nonumber\\
%&=\left(1+\zeta\overline{\zeta}\right)^{s+1}\left(\left(1+\zeta\overline{\zeta}\right)^{-s}\partial_{{\zeta}}-s\overline{\zeta}\left(1+\zeta\overline{\zeta}\right)^{-(s+1)}\right) \nonumber\\
&=\left(1+\zeta\overline{\zeta}\right)^{s+1}\partial_{{\zeta}}\left(1+\zeta\overline{\zeta}\right)^{-s}, \nonumber\\
&=P^{s+1}\partial_{{\zeta}}P^{-s},
\label{integral17}
\end{align}
where, we have defined the zero spin-weighted function
\begin{equation}
P=1+\zeta\overline{\zeta}.
\label{integral18}
\end{equation}
Observing that
\begin{align}
\eth \overline{\zeta}&=P\partial_{\overline{\zeta}}\overline{\zeta},\nonumber\\
&=P,
\label{integral19}
\end{align}
then
\begin{align}
\overline{\eth} P&=\overline{\eth}\eth\overline{\zeta},\nonumber\\
&=\eth\overline{\eth}\ \overline{\zeta},\nonumber\\
&=\eth P\partial_{\zeta}\overline{\zeta},\nonumber\\
&=0.
\label{integral20}
\end{align}
Also
\begin{align}
\overline{\eth} {\zeta}&=P\partial_{{\zeta}} {\zeta},\nonumber\\
&=P,
\label{integral21}
\end{align}
then
\begin{align}
{\eth} P&=\eth\overline{\eth}{\zeta},\nonumber\\
&=\overline{\eth}\eth {\zeta},\nonumber\\
&=\overline{\eth} P\partial_{\overline{\zeta}}{\zeta},\nonumber\\
&=0.
\label{integral22}
\end{align}
Thus, the equations \eqref{integral20} and \eqref{integral22} imply that
\begin{equation}
\eth(PA)=P\eth A, \hspace{1cm}\overline{\eth}(PA)=P\overline{\eth}A,
\label{integral23}
\end{equation}
for $A$, any spin-weight function.
\\Then, if it is consider two functions $f$ and $g$ with $s$ and $s-1$ spin-weight respectively, the inner product of $f$ and $\eth g$ is
\begin{align*}
\langle f,\eth g\rangle&=\oiint\limits_{\Omega} d\Omega \overline{f}\ \eth g,\\
&=\iint\limits_{\Omega} d\zeta d\overline{\zeta}\ \dfrac{2i}{P^2}\overline{f}\ P^{1-s}\partial_{\overline{\zeta}}\left(P^{s} g\right), \\
&=2i\iint\limits_{\Omega} d\zeta d\overline{\zeta}\ \overline{f}\ P^{-(1+s)}\partial_{\overline{\zeta}}\left(P^{s} g\right).
\end{align*}
The last equation can be written as
\begin{align}
\langle f,\eth g\rangle
=& 2i\iint\limits_{\Omega} d\zeta d\overline{\zeta} \left(\partial_{\overline{\zeta}} \left(\overline{f}\ P^{-(1+s)}P^{s} g\right) - P^{s} g\ \partial_{\overline{\zeta}} \left(\overline{f}\ P^{-(1+s)}\right)\right)\nonumber\\
=& 2i\left(\iint\limits_{\Omega} d\zeta d\overline{\zeta} \ \partial_{\overline{\zeta}} \left(\overline{f}\ P^{-(1+s)}P^{s} g\right) \right.\nonumber\\
&\left. - \iint\limits_{\Omega} d\zeta d\overline{\zeta} P^{s} g\ \partial_{\overline{\zeta}} \left(\overline{f}\ P^{-(1+s)}\right)\right) 
%&=2i\left(\iint\limits_{\Omega} d\zeta d\overline{\zeta} \ \partial_{\overline{\zeta}} \left(\overline{f}\ P^{-(1+s)}P^{s} g\right) - \iint\limits_{\Omega} d\zeta d\overline{\zeta} \ g P^{-1}P^{s+1}\ \partial_{\overline{\zeta}} \left(P^{-s}\overline{f}\ P^{-1}\right)\right)\\
%&=2i\left(\iint\limits_{\Omega} d\zeta d\overline{\zeta} \ \partial_{\overline{\zeta}} \left(\overline{f}\ P^{-(1+s)}P^{s} g\right) - \iint\limits_{\Omega}  d\overline{\zeta} d\zeta \ g P^{-1}P^{s+1}\ \partial_{\zeta} \left(P^{-s}\overline{f}\ P^{-1}\right)\right) 
\label{integral24}
\end{align}
The first term in this equation corresponds to
\begin{align*}
2i\iint\limits_{\Omega} d\zeta d\overline{\zeta} \ \partial_{\overline{\zeta}} \left(\overline{f}\ P^{-(1+s)}P^{s} g\right)&=2i\iint\limits_{\Omega} d\zeta d\overline{\zeta} P^{s-1} P^{1-s}\ \partial_{\overline{\zeta}} \left(P^{s}\overline{f}\ P^{-(1+s)} g\right),\nonumber\\
&=2i\iint\limits_{\Omega} d\zeta d\overline{\zeta} P^{s-1} \eth \left(\overline{f}\ P^{-(1+s)} g\right),\nonumber\\
&=2i\iint\limits_{\Omega} d\zeta d\overline{\zeta} P^{s-1} P^{-(1+s)}\eth \left(\overline{f}\  g\right),\nonumber\\
&=2i\iint\limits_{\Omega} d\zeta d\overline{\zeta} P^{-2} \eth \left(\overline{f}\  g\right),\nonumber\\
&=\left\langle 1,\eth(\overline{f} g)\right\rangle.
\end{align*}
Since $f$ is $s$ spin-weighted and $g$ has a spin-weight of $s-1$ then its product $\overline{f}g$ has $s=-1$, consequently $\eth(\overline{f} g)$ is a zero spin-weighted function, then it can be expanded in spherical harmonics in the form
\begin{equation*}
\eth(\overline{f} g)=\sum_{l,m}a_{lm}\ _0Y_{lm}.
\end{equation*}
Thus,
\begin{align}
\left\langle 1,\eth(\overline{f} g)\right\rangle&=\left\langle 1,\sum_{l,m}a_{lm}\ _0Y_{lm}\right\rangle,\nonumber\\
&=\sum_{l,m}a_{lm}\left\langle 1,\ _0Y_{lm}\right\rangle,\nonumber\\
&=0.
\label{integral25}
\end{align}
The second term in \eqref{integral24} is
\begin{align*}
2i\iint\limits_{\Omega} d\zeta d\overline{\zeta} P^{s} g\ \partial_{\overline{\zeta}} \left(\overline{f}\ P^{-(1+s)}\right)&=2i\iint\limits_{\Omega} d\zeta d\overline{\zeta} \ g P^{-1}P^{s+1}\ \partial_{\overline{\zeta}} \left(P^{-s}\overline{f}\ P^{-1}\right),\\
&=2i \iint\limits_{\Omega}  d\overline{\zeta} d\zeta \ g P^{-1}P^{s+1}\ \partial_{\zeta} \left(P^{-s}\overline{f}\ P^{-1}\right),
\end{align*}
where we have renamed the integration variables $\zeta$ and $\overline{\zeta}$. Thus
\begin{align}
2i\iint\limits_{\Omega} d\zeta d\overline{\zeta} P^{s} g\ \partial_{\overline{\zeta}} \left(\overline{f}\ P^{-(1+s)}\right)&=2i \iint\limits_{\Omega}  d\overline{\zeta} d\zeta \ g P^{-1}\overline{\eth} \left(\overline{f}\ P^{-1}\right), \nonumber\\
&=2i \iint\limits_{\Omega}  d\overline{\zeta} d\zeta \ g P^{-2}\overline{\eth} \left(\overline{f}\right), \nonumber\\
&=-\left\langle\overline{\eth}f,g\right\rangle.
\label{integral26}
\end{align}
Substituting \eqref{integral25} and \eqref{integral26} into \eqref{integral24} we obtain
\begin{equation}
\langle f,\eth g\rangle=-\left\langle\overline{\eth}f,g\right\rangle.
\label{integral27}
\end{equation}
Also, if is considered that $f$ and $g$ have $s$ and $s+1$ spin-weight respectively, then the inner product 
\begin{align*}
\left\langle f,\overline{\eth}g\right\rangle&=\oiint\limits_{\Omega}d\Omega\overline{f}\ \overline{\eth}g, \nonumber\\
&=\iint\limits_{\Omega}d\zeta d\overline{\zeta}\dfrac{2i}{P^2}\overline{f}P^{s+1}\partial_\zeta \left(P^{-s}g\right), \nonumber\\
&=2i\iint\limits_{\Omega}d\zeta d\overline{\zeta}\ \overline{f}P^{s-1}\partial_\zeta \left(P^{-s}g\right).
\end{align*}
The last can be written as
\begin{align}
\left\langle f,\overline{\eth}g\right\rangle&=2i\iint\limits_{\Omega}d\zeta d\overline{\zeta} \partial_\zeta \left(\overline{f}P^{s-1} P^{-s}g\right)-2i\iint\limits_{\Omega}d\zeta d\overline{\zeta}  P^{-s}g\partial_\zeta \left(\overline{f}P^{s-1}\right).
\label{integral28}
\end{align}
The first term is given by
\begin{align*}
2i\iint\limits_{\Omega}d\zeta d\overline{\zeta} \partial_\zeta \left(\overline{f}P^{s-1} P^{-s}g\right)&=2i\iint\limits_{\Omega}d\zeta d\overline{\zeta} P^{-(s+1)} P^{s+1}\partial_\zeta \left( P^{-s} \overline{f}P^{s-1} g\right),\\
&=2i\iint\limits_{\Omega}d\zeta d\overline{\zeta} P^{-(s+1)} \overline{\eth} \left( \overline{f}P^{s-1} g\right),
\end{align*}
i.e.,
\begin{align*}
2i\iint\limits_{\Omega}d\zeta d\overline{\zeta} \partial_\zeta \left(\overline{f}P^{s-1} P^{-s}g\right)&= 2i\iint\limits_{\Omega}d\zeta d\overline{\zeta}  P^{-2} \overline{\eth} \left( \overline{f} g\right),\\
&=\left\langle 1, \overline{\eth} \left( \overline{f} g\right)\right\rangle.
\end{align*}
Observing that
\begin{align*}
\overline{\eth} \left( \overline{f} g\right)=\sum_{l,m}a_{0lm}\ _0Y_{lm},
\end{align*}
then
\begin{align}
\left\langle 1, \overline{\eth} \left( \overline{f} g\right)\right\rangle &=\left\langle 1, \sum_{l,m}a_{0lm}\ _0Y_{lm}\right\rangle, \nonumber\\
&=\sum_{l,m}a_{0lm}\left\langle 1, \ _0Y_{lm}\right\rangle, \nonumber\\
&=0.
\label{integral29}
\end{align}
The second term in \eqref{integral28} is given by
\begin{align*}
2i\iint\limits_{\Omega}d\zeta d\overline{\zeta}  P^{-s}g\partial_\zeta \left(\overline{f}P^{s-1}\right)=2i\iint\limits_{\Omega} d\overline{\zeta} d\zeta P^{-s}g\partial_{\overline{\zeta}} \left(\overline{f}P^{s-1}\right),
\end{align*}
where, we interchange the variables $\zeta$ and $\overline{\zeta}$ in the integrals. Thus
\begin{align}
2i\iint\limits_{\Omega}d\zeta d\overline{\zeta}  P^{-s}g\partial_\zeta \left(\overline{f}P^{s-1}\right)&=2i\iint\limits_{\Omega} d\overline{\zeta} d\zeta \ g P^{-1} P^{1-s}\partial_{\overline{\zeta}} \left(P^s\overline{f}P^{-1}\right), \nonumber\\
&=2i\iint\limits_{\Omega} d\overline{\zeta} d\zeta g P^{-1} \eth \left(\overline{f}P^{-1}\right),  \nonumber\\
&=2i\iint\limits_{\Omega} d\overline{\zeta} d\zeta g P^{-2} \eth \overline{f}, \nonumber\\
&=\left\langle \eth f,g \right\rangle.
\label{integral30}
\end{align}
Thus, substituting \eqref{integral29} and \eqref{integral30} into \eqref{integral28} we obtain
\begin{equation}
\left\langle f,\overline{\eth}g\right\rangle=-\left\langle \eth f,g \right\rangle.
\label{integral31}
\end{equation}

==> docs/differential_operators.tex <==
\section{Transformation Rules for Vectors and One-forms}
In order to establish the transformation rules for the dyads, it is necessary to understand how the differential operators transform between one map to another. Thus, as $q_N:=q_N(q_S,p_S)$ and $p_N:=p_N(q_S,p_S)$ as is shown explicitly in \eqref{stereo11}, then the one-forms $\partial_{q_N}$ and $\partial_{q_S}$ transforms as
\begin{subequations}
\begin{align}
\partial_{q_N}&=(\partial_{q_N}q_S)\partial_{q_S}+(\partial_{q_N}p_S)\partial_{p_S},\label{diff3.1}\\
\partial_{p_N}&=(\partial_{p_N}q_S)\partial_{q_S}+(\partial_{p_N}p_S)\partial_{p_S}.\label{diff3.2}
\end{align}
\label{diff3}
\end{subequations}
%that corresponds to the transformation rule between one coordinate map and the other for vectors, i.e., if $\boldsymbol{S}$ is a vector, its components must transform as
%\begin{equation*}
%\dfrac{\partial S^A}{\partial x^B_N}=\dfrac{{\partial x_S^C}}{{\partial x_N^B}}\dfrac{\partial S^A}{\partial x_S^C}.
%\end{equation*}
Computing each coefficient in the equations \eqref{diff3} are obtained
%\begin{align*}
%\dfrac{\partial q_S}{\partial q_N}=\dfrac{p_N^2-q_N^2}{(q_N^2+p_N^2)^2},\hspace{1cm} \dfrac{\partial p_S}{\partial q_N}=\dfrac{2q_Np_N}{(q_N^2+p_N^2)^2},\\
%\dfrac{\partial q_S}{\partial p_N}=-\dfrac{2q_Np_N}{(q_N^2+p_N^2)^2},\hspace{1cm} \dfrac{\partial p_S}{\partial p_N}=\dfrac{p_N^2-q_N^2}{(q_N^2+p_N^2)^2}.
%\end{align*}
\begin{align*}
\partial_{q_N} q_S=\dfrac{p_N^2-q_N^2}{(q_N^2+p_N^2)^2},\hspace{1cm} \partial_{q_N} p_S=\dfrac{2q_Np_N}{(q_N^2+p_N^2)^2},\\
\partial_{p_N} q_S=-\dfrac{2q_Np_N}{(q_N^2+p_N^2)^2},\hspace{1cm} \partial_{p_N} p_S=\dfrac{p_N^2-q_N^2}{(q_N^2+p_N^2)^2}.
\end{align*}
It means that the differential operators \eqref{diff3} becomes as
\begin{subequations}
\begin{align}
\partial_{q_N}&=\dfrac{1}{\left(q_N^2+p_N^2\right)^2}\left(\left(p_N^2-q_N^2\right)\partial_{q_S}+2q_Np_N\partial_{p_S}\right), \label{diff4.1}\\
\partial_{p_N}&=\dfrac{1}{\left(q_N^2+p_N^2\right)^2}\left(-2q_Np_N\partial_{q_S} +\left(p_N^2-q_N^2\right)\partial_{p_S}\right).
\label{diff4.2}
\end{align}
\label{diff4}
\end{subequations}
Now, will be examined the transformation rule for the vectors
\begin{equation}
dx^A_N=\partial_{x^B_S} x^A_Ndx^B_S.
\end{equation}
Specifically, the transformation rules for the vectors $dq$ and $dp$ are given by
\begin{subequations}
\begin{align}
dq_N&=\partial_{q_{S}} q_{N} dq_S+ \partial_{p_{S}} q_{N} dp_S,\label{diff5.1}\\
dp_N&=\partial_{q_{S}} p_{N} dq_S+ \partial_{p_{S}} p_{N} dp_S.\label{diff5.2}
\end{align}
\label{diff5}
\end{subequations}
Here, it is important to appoint that the equations \eqref{stereo11} are symmetrical  with respect to the interchange of indices $N$ and $S$, i.e., the same expressions are obtained if $q_S$ and $p_S$ are considered as functions of $q_N$ and $p_S$, therefore
%\begin{align*}
%\dfrac{\partial q_N}{\partial q_S}=\dfrac{p_S^2-q_S^2}{(q_S^2+p_S^2)^2},\hspace{1cm} \dfrac{\partial p_N}{\partial q_S}=\dfrac{2q_Sp_S}{(q_S^2+p_S^2)^2},\\
%\dfrac{\partial q_N}{\partial p_S}=-\dfrac{2q_Sp_S}{(q_S^2+p_S^2)^2},\hspace{1cm} \dfrac{\partial p_N}{\partial p_S}=\dfrac{p_S^2-q_S^2}{(q_S^2+p_S^2)^2}.
%\end{align*}
\begin{align*}
\partial_{q_S} q_N=\dfrac{p_S^2-q_S^2}{(q_S^2+p_S^2)^2},\hspace{1cm} \partial_{q_S} p_N=\dfrac{2q_Sp_S}{(q_S^2+p_S^2)^2},\\
\partial_{p_S} q_N=-\dfrac{2q_Sp_S}{(q_S^2+p_S^2)^2},\hspace{1cm} \partial_{p_S} p_N=\dfrac{p_S^2-q_S^2}{(q_S^2+p_S^2)^2}.
\end{align*}
Then the vectors \eqref{diff5} transform as,
\begin{subequations}
\begin{align}
dq_N&=\dfrac{1}{\left(q_S^2+p_S^2\right)^2}\left(\left(p_S^2-q_S^2\right) dq_S - 2q_Sp_S dp_S\right),
\label{diff6.1}\\
dp_N&=\dfrac{1}{\left(q_S^2+p_S^2\right)^2}\left(2q_Sp_S dq_S+ \left(p_S^2-q_S^2\right) dp_S\right).
\label{diff6.2}
\end{align}
\label{diff6}
\end{subequations}
Notice that, by virtue of the interchangeability of the indices in \eqref{stereo11}, the relations \eqref{diff4} and \eqref{diff6} for one-forms and vectors are symmetrical with respect to the interchange of the indices $N$ and $S$. Therefore the same rules are applied to construct the inverse transformation from north to south. 

==> docs/eth_spherical.tex <==
\section{The $\eth$ and $\overline{\eth}$ in Spherical Coordinates}
A further generalisation of all the last results can be done, extending the operators $\eth$ and $\overline{\eth}$ to the case when are considered function with spin-weight different to zero. In order to do so, it is necessary consider the operators defined in the Equations \eqref{eth_spherical_7}, which can be written as
\begin{align}
\eth %&= \partial_\theta\ _s\Psi + i\csc\theta\partial_\phi\ _s\Psi - s\cot\theta\ _s\Psi,\\
&= \left(\sin\theta\right)^s \left(\sin\theta\right)^{-s}\left(\partial_\theta + i\csc\theta\partial_\phi - s\cot\theta\right), \nonumber\\
%&= \left(\sin\theta\right)^s \left(\left(\sin\theta\right)^{-s}\partial_\theta\ _s\Psi + i\csc\theta\left(\sin\theta\right)^{-s} \partial_\phi\ _s\Psi - s\cot\theta \left(\sin\theta\right)^{-s} \ _s\Psi\right)\\
&= \left(\sin\theta\right)^s \left(\partial_\theta\left(\sin\theta\right)^{-s} + i\csc\theta \partial_\phi \left(\sin\theta\right)^{-s}\right), \nonumber \\
&= \left(\sin\theta\right)^s \left(\partial_\theta + i\csc\theta \partial_\phi  \right) \left(\sin\theta\right)^{-s}, 
%\\
%&= \left[\left(\sin\theta\right)^s \left(\partial_\theta + i\csc\theta \partial_\phi  \right) \left(\sin\theta\right)^{-s}\right]  \ 
%_s\Psi
\label{eth_spherical_8}
\end{align}
and
\begin{align}
\overline{\eth} &= \left(\sin\theta\right)^s \left(\sin\theta\right)^{-s}\left(\partial_\theta - i\csc\theta\partial_\phi + s\cot\theta\right), \nonumber\\
&= \left(\sin\theta\right)^{-s} \left(\partial_\theta\left(\sin\theta\right)^{s}  - i\csc\theta \partial_\phi \left(\sin\theta\right)^{s} \right), \nonumber\\
&= \left(\sin\theta\right)^{-s} \left(\partial_\theta - i\csc\theta \partial_\phi  \right) \left(\sin\theta\right)^{s}.  
\label{eth_spherical_10}
\end{align}
It is worth stressing that the operations in \eqref{eth_spherical_8} are referred to operators, not to scalar functions.
\\From \eqref{eth_spherical_7}, one obtains the expressions for $\partial_\theta$ and $\partial_\phi$ 
%\begin{subequations}
\begin{equation}
\partial_{\theta}=\dfrac{\eth+\overline{\eth}}{2}, \hspace{1cm}
\partial_{\phi}=\dfrac{i\sin\theta}{2}\left(\overline{\eth}-\eth-2s\cot\theta\right). %\label{eth_spherical_16.2}
\label{eth_spherical_16}
\end{equation}
%\end{subequations}
And from the equations cited below, it is possible to obtain the expressions for $\eth^2$, $\overline{\eth}^2$, $\overline{\eth}\eth$ and $\eth\overline{\eth}$, which enable us to find the expressions for $\partial_{\theta\theta}$, $\partial_{\theta\phi}$ and $\partial_{\phi\phi}$. Thus, 
\begin{align}
\eth^2=&\left(\partial_\theta + i\csc\theta\partial_\phi - (s+1)\cot\theta\right) \left(\partial_\theta + i\csc\theta\partial_\phi - s\cot\theta\right), \nonumber\\
=&\left(\partial_\theta + i\csc\theta\partial_\phi - (s+1)\cot\theta\right)\partial_\theta + i\left(\partial_\theta + i\csc\theta\partial_\phi \right.\nonumber\\
&\left. - (s+1)\cot\theta\right)  \csc\theta\partial_\phi - s \left(\partial_\theta + i\csc\theta\partial_\phi - (s+1)\cot\theta\right)  \cot\theta.
\label{eth_spherical_17}
\end{align}
The first term in the last equation is
\begin{align}
\left(\partial_\theta + i\csc\theta\partial_\phi - (s+1)\cot\theta\right)\partial_\theta &= \partial_{\theta\theta} + i\csc\theta\partial_{\phi\theta} - (s+1)\cot\theta\partial_\theta.
\label{eth_spherical_18}
\end{align}
The second term in \eqref{eth_spherical_17} is given by
\begin{align}
&i\left(\partial_\theta + i\csc\theta\partial_\phi - (s+1)\cot\theta\right) \csc\theta\partial_\phi \nonumber\\
%&= i\left(\partial_\theta  \csc\theta\partial_\phi + i\csc\theta\partial_\phi  \csc\theta\partial_\phi - (s+1)\cot\theta \csc\theta\partial_\phi \right), \nonumber\\
=& i\big(-\csc\theta\cot\theta\partial_\phi + \csc\theta \partial_{\theta\phi} + i\csc^2\theta\partial_{\phi\phi} \nonumber\\
&- (s+1)\cot\theta  \csc\theta\partial_\phi \big).
\label{eth_spherical_19}
\end{align}
And the third term in \eqref{eth_spherical_17} is
\begin{align}
&- s\left(\partial_\theta + i\csc\theta\partial_\phi - (s+1)\cot\theta\right)  \cot\theta\nonumber\\
=& - s\left(\partial_\theta \cot\theta + i\csc\theta\partial_\phi  \cot\theta - (s+1)\cot^2\theta  \right), \nonumber\\
=& - s\left(-\csc^2\theta + \cot\theta \partial_\theta  + i\csc\theta\cot\theta\partial_\phi   - (s+1)\cot^2\theta  \right).
\label{eth_spherical_20}
\end{align}
Thus, the substitution of \eqref{eth_spherical_18}-\eqref{eth_spherical_20} into \eqref{eth_spherical_17} yields us to
\begin{align}
\eth^2
%&= \partial_{\theta\theta} + i\csc\theta\partial_{\phi\theta} - (s+1)\cot\theta\partial_\theta + i\big(-\csc\theta\cot\theta\partial_\phi + \csc\theta \partial_{\theta\phi} + i\csc^2\theta\partial_{\phi\phi} - (s+1)\cot\theta  \csc\theta\partial_\phi \big)\nonumber\\
%&- s\left(-\csc^2\theta + \cot\theta \partial_\theta  + i\csc\theta\cot\theta\partial_\phi   - (s+1)\cot^2\theta  \right),\nonumber\\
=& \partial_{\theta\theta} - \csc^2\theta\partial_{\phi\phi} + 2i\csc\theta\partial_{\phi\theta} - (2s+1)\cot\theta\partial_\theta  \nonumber\\
&- 2i (s+1)\cot\theta  \csc\theta\partial_\phi + s\left((s+1)\cot^2\theta + \csc^2\theta   \right).
\label{eth_spherical_21}
\end{align}
From \eqref{eth_spherical_7} we construct the $\overline{\eth}^2$ as
\begin{align}
\overline{\eth}^2 = &\left[\partial_\theta - i\csc\theta\partial_\phi + (s-1)\cot\theta\right]\left[\partial_\theta - i\csc\theta\partial_\phi + s\cot\theta\right],\nonumber\\
=&\partial_\theta\left[\partial_\theta - i\csc\theta\partial_\phi + s\cot\theta\right] - i\csc\theta\partial_\phi\left[\partial_\theta - i\csc\theta\partial_\phi + s\cot\theta\right]\nonumber\\
& + (s-1)\cot\theta\left[\partial_\theta - i\csc\theta\partial_\phi + s\cot\theta\right].
\label{eth_spherical_22}
\end{align}
The first term in the last equation corresponds to 
\begin{align}
\partial_\theta\left[\partial_\theta - i\csc\theta\partial_\phi + s\cot\theta\right]=& \partial_{\theta\theta} - i\partial_\theta\csc\theta\partial_\phi + s\partial_\theta\cot\theta, \nonumber\\
=&\partial_{\theta\theta} - i\csc\theta\partial_{\theta\phi} + i\csc\theta\cot\theta\partial_\phi  \nonumber\\
&- s\csc^2\theta + s\cot\theta\partial_\theta.
\label{eth_spherical_23}
\end{align}
The second term in \eqref{eth_spherical_22} is given by
\begin{align}
&- i\csc\theta\partial_\phi\left[\partial_\theta - i\csc\theta\partial_\phi + s\cot\theta\right]\nonumber\\
=& - i\left[\csc\theta\partial_{\phi\theta} - i\csc\theta\partial_\phi\csc\theta\partial_\phi + s\csc\theta\partial_\phi\cot\theta\right], \nonumber\\
=& - i\left[\csc\theta\partial_{\phi\theta} - i\csc^2\theta\partial_{\phi\phi} + s\csc\theta\cot\theta\partial_\phi\right].
\label{eth_spherical_24}
\end{align}
And the third term in \eqref{eth_spherical_22} is
\begin{align}
&(s-1)\cot\theta\left[\partial_\theta - i\csc\theta\partial_\phi + s\cot\theta\right]\nonumber\\
=&(s-1)\left[\cot\theta\partial_\theta - i\cot\theta\csc\theta\partial_\phi + s\cot^2\theta\right].
\label{eth_spherical_25}
\end{align}
Thus, substituting the \eqref{eth_spherical_23}-\eqref{eth_spherical_25} into \eqref{eth_spherical_22}
\begin{align}
\overline{\eth}^2&=\partial_{\theta\theta}-\csc^2\theta\partial_{\phi\phi}-2i\csc\theta\partial_{\theta\phi} + (2s-1)\cot\theta\partial_\theta  \nonumber\\
& - 2i(s-1)\cot\theta\csc\theta\partial_\phi + s\left((s-1)\cot^2\theta-\csc^2\theta\right).
\label{eth_spherical_26}
\end{align}
Also, from \eqref{eth_spherical_7} %and \eqref{eth_spherical_9}
\begin{align}
\eth\overline{\eth}=&\left[\partial_\theta + i\csc\theta\partial_\phi - (s-1)\cot\theta\right] \left[\partial_\theta - i\csc\theta\partial_\phi + s\cot\theta \right],\nonumber \\
=& \partial_\theta\left[\partial_\theta - i\csc\theta\partial_\phi + s\cot\theta \right] + i\csc\theta\partial_\phi\left[\partial_\theta - i\csc\theta\partial_\phi + s\cot\theta \right] \nonumber\\
& - (s-1)\cot\theta\left[\partial_\theta - i\csc\theta\partial_\phi + s\cot\theta \right], \nonumber\\
=&\partial_{\theta\theta}+\csc^2\theta\partial_{\phi\phi}+\cot\theta\partial_\theta+2is\csc\theta\cot\theta\partial_\phi-s\left(s\cot^2\theta+1\right),
\label{eth_spherical_27}
\end{align}
and
\begin{align}
\overline{\eth}\eth=&\left[\partial_\theta - i\csc\theta\partial_\phi + (s+1)\cot\theta\right]\left[\partial_\theta + i\csc\theta\partial_\phi - s\cot\theta\right],\nonumber\\
=&\partial_\theta\left[\partial_\theta + i\csc\theta\partial_\phi - s\cot\theta\right] - i\csc\theta\partial_\phi\left[\partial_\theta + i\csc\theta\partial_\phi - s\cot\theta\right] \nonumber\\
&+ (s+1)\cot\theta\left[\partial_\theta + i\csc\theta\partial_\phi - s\cot\theta\right],\nonumber\\
=&\partial_{\theta\theta}+\csc^2\theta\partial_{\phi\phi} + \cot\theta\partial_\theta + 2is\cot\theta\csc\theta\partial_\phi  - s \left[ (s+1) \cot^2\theta - \csc^2\theta\right], \nonumber\\
=&\partial_{\theta\theta}+\csc^2\theta\partial_{\phi\phi} + \cot\theta\partial_\theta + 2is\cot\theta\csc\theta\partial_\phi  - s \left( s \cot^2\theta - 1\right).
\label{eth_spherical_28}
\end{align}
In order to check the above expressions, the commutator $\left[\overline{\eth},\eth\right]$ is computed, resulting the known result 
\begin{equation*}
\left[\overline{\eth},\eth\right]= 2s,
\end{equation*}
and its anti-commutator yields us to
\begin{equation}
\left(\overline{\eth},\eth\right)= 2\left(\partial_{\theta\theta}+\csc^2\theta\partial_{\phi\phi} + \cot\theta\partial_\theta + 2is\cot\theta\csc\theta\partial_\phi  -  s^2 \cot^2\theta\right). 
\label{eth_spherical_29}
\end{equation}
Thus, from \eqref{eth_spherical_21}, \eqref{eth_spherical_26}, \eqref{eth_spherical_27}, \eqref{eth_spherical_28} we obtain the explicit form of the second order angular operators in terms of the spin-weighted  operators
\begin{subequations}
\begin{align}
\partial_{\theta\theta}=&\dfrac{{\eth}^2+\left(\overline{\eth},\eth\right)+\overline{\eth}^2}{4}, \label{eth_spherical_30.1}\\
\partial_{\phi\phi} =& -\dfrac{\sin^2\theta}{4} \left({\eth}^2 -\left(\overline{\eth},\eth\right) + \overline{\eth}^2 \right)  - s^2 \cos^2\theta\nonumber\\
& - \sin\theta\cos\theta\left(\left(s+\dfrac{1}{2}\right)\eth -\left(s-\dfrac{1}{2}\right)\overline{\eth}\right), \label{eth_spherical_30.2}\\
\partial_{\theta\phi} =&- \dfrac{i\sin\theta}{4}\left(\eth^2-\overline{\eth}^2\right) -is\cos\theta\dfrac{\eth+\overline{\eth}}{2}  \nonumber\\
& + \dfrac{i\cos\theta}{2}\left(\overline{\eth}-\eth-2s\cot\theta\right) + i\sin\theta\dfrac{s(\cot^2\theta+\csc^2\theta)}{2}. \label{eth_spherical_30.3}
\end{align}
\label{eth_spherical_30}
\end{subequations}
%\begin{align}
%\eth^2&=\eth\left[\left(\sin\theta\right)^s \left(\partial_\theta + i\csc\theta \partial_\phi  \right) \left(\sin\theta\right)^{-s}\right]\nonumber\\
%&=\left[\left(\sin\theta\right)^{s+1} \left(\partial_\theta + i\csc\theta \partial_\phi  \right) \left(\sin\theta\right)^{-(s+1)}\right] \left[\left(\sin\theta\right)^s \left(\partial_\theta + i\csc\theta \partial_\phi  \right) \left(\sin\theta\right)^{-s}\right]\nonumber\\
%&=\left(\sin\theta\right)^{s+1} \left(\partial_\theta + i\csc\theta \partial_\phi  \right) \left(\sin\theta\right)^{-s}  \left(\partial_\theta + i\csc\theta \partial_\phi  \right) \left(\sin\theta\right)^{-s}\nonumber\\
%&=\left(\left(\sin\theta\right)^{s+1} \left(\partial_\theta + i\csc\theta \partial_\phi  \right) \left(\sin\theta\right)^{-s} \partial_\theta + i\left(\sin\theta\right)^{s+1} \left(\partial_\theta + i\csc\theta \partial_\phi  \right) \left(\sin\theta\right)^{-s} \csc\theta \partial_\phi  \right) \left(\sin\theta\right)^{-s}
%\label{eth_spherical_15}
%\end{align}
%where, the first term in the parenthesis of the last equation is given by
%\begin{align}
%\left(\sin\theta\right)^{s+1} \left(\partial_\theta + i\csc\theta \partial_\phi  \right) \left(\sin\theta\right)^{-s} \partial_\theta&=  \left(\left(\sin\theta\right)^{s+1} \partial_\theta + i\left(\sin\theta\right)^{s+1} \csc\theta \partial_\phi  \right) \left(\sin\theta\right)^{-s} \partial_\theta \nonumber\\
%&=  \left(\left(\sin\theta\right)^{s+1} \partial_\theta + i\left(\sin\theta\right)^{s}  \partial_\phi  \right) \left(\sin\theta\right)^{-s} \partial_\theta \nonumber\\
%&=\left(\sin\theta\right)^{s+1} \partial_\theta \left(\sin\theta\right)^{-s} \partial_\theta + i\left(\sin\theta\right)^{s}  \partial_\phi \left(\sin\theta\right)^{-s} \partial_\theta  
%\label{eth_spherical_16}
%\end{align}
%The first term into \eqref{eth_spherical_16} is given by
%
%\begin{align*}
%\eth^2 %&= \eth \left[\left(\sin\theta\right)^s \left(\partial_\theta + i\csc\theta \partial_\phi  \right) \left(\sin\theta\right)^{-s}\right]\\
%&= \left[\left(\sin\theta\right)^{s+1} \left(\partial_\theta + i\csc\theta \partial_\phi  \right) \left(\sin\theta\right)^{-(s+1)}\right] \left[\left(\sin\theta\right)^s \left(\partial_\theta + i\csc\theta \partial_\phi  \right) \left(\sin\theta\right)^{-s}\right]\\
%&= \left(\sin\theta\right)^{s+1} \left(\partial_\theta + i\csc\theta \partial_\phi  \right) \left(\sin\theta\right)^{-1} \left(\partial_\theta + i\csc\theta \partial_\phi  \right) \left(\sin\theta\right)^{-s}\\
%&= \left(\sin\theta\right)^{s+1} \left(\partial_\theta + i\csc\theta \partial_\phi  \right) \left(\sin\theta\right)^{-1} \partial_\theta \left(\sin\theta\right)^{-s} + i \left(\sin\theta\right)^{s+1} \left(\partial_\theta + i\csc\theta \partial_\phi  \right) \left(\sin\theta\right)^{-2} \partial_\phi \left(\sin\theta\right)^{-s}\\
%&= \left(\sin\theta\right)^{s+1} \left(\partial_\theta + i\csc\theta \partial_\phi  \right) \left(\sin\theta\right)^{-1} \partial_\theta \left(\sin\theta\right)^{-s} + i \left(\sin\theta\right)^{s+1} \left(\partial_\theta + i\csc\theta \partial_\phi  \right) \left(\sin\theta\right)^{-(s+2)} \partial_\phi  
%\end{align*}
%The first term of the last equation is
%\begin{align*}
%& \left(\sin\theta\right)^{s+1} \left(\partial_\theta + i\csc\theta \partial_\phi  \right) \left(\sin\theta\right)^{-1} \partial_\theta \left(\sin\theta\right)^{-s}\\
%%& =   \left(\sin\theta\right)^{s+1} \partial_\theta \left(\sin\theta\right)^{-1} \partial_\theta \left(\sin\theta\right)^{-s} + i \left(\sin\theta\right)^{s+1} \csc\theta \partial_\phi \left(\sin\theta\right)^{-1} \partial_\theta \left(\sin\theta\right)^{-s} \\
%& =   \left(\sin\theta\right)^{s+1} \partial_\theta \left(\sin\theta\right)^{-1} \partial_\theta \left(\sin\theta\right)^{-s} + i \left(\sin\theta\right)^{s} \partial_\phi \left(\sin\theta\right)^{-1} \partial_\theta \left(\sin\theta\right)^{-s}
%\end{align*}
%but, just observing that
%\begin{align*}
%\left(\sin\theta\right)^{s+1} \partial_\theta \left(\sin\theta\right)^{-1} \partial_\theta \left(\sin\theta\right)^{-s}&= \left(\sin\theta\right)^{s+1} \partial_\theta \left(\sin\theta\right)^{-1} \left(-s\left(\sin\theta\right)^{-(s+1)}+\left(\sin\theta\right)^{-s}\partial_\theta \right) \\
%&= \left(\sin\theta\right)^{s+1} \partial_\theta  \left(-s  \left(\sin\theta\right)^{-(s+2)}+ \left(\sin\theta\right)^{-(s+1)}\partial_\theta \right)\\
%&= \left(\sin\theta\right)^{s+1} \partial_\theta  \left(-s  \left(\sin\theta\right)^{-(s+2)}\right)+ \left(\sin\theta\right)^{s+1} \partial_\theta \left(\sin\theta\right)^{-(s+1)}\partial_\theta 
%\end{align*}
%where
%\begin{align*}
%\left(\sin\theta\right)^{s+1} \partial_\theta  \left(-s  \left(\sin\theta\right)^{-(s+2)}\right)&= -s\left(\sin\theta\right)^{s+1} \partial_\theta    \left(\sin\theta\right)^{-(s+2)}\\
%&= -s\left(\csc\theta \partial_\theta  -(s+2) \csc\theta\cot\theta   \right)
%\end{align*}
%and
%\begin{align*}
%\left(\sin\theta\right)^{s+1} \partial_\theta \left(\sin\theta\right)^{-(s+1)}\partial_\theta &= \left(\sin\theta\right)^{s+1} \partial_\theta \left(\sin\theta\right)^{-(s+1)}\partial_\theta\\
%&= \left(\sin\theta\right)^{s+1} \left(\left(\sin\theta\right)^{-(s+1)}\partial_{\theta\theta} -(s+1) \left(\sin\theta\right)^{-(s+2)}\cos\theta\partial_\theta\right)\\
%&= \partial_{\theta\theta} -(s+1) \cot\theta\partial_\theta
%\end{align*}
%i.e.,
%\begin{align*}
%\left(\sin\theta\right)^{s+1} \partial_\theta \left(\sin\theta\right)^{-1} \partial_\theta \left(\sin\theta\right)^{-s}
%&= \left(\sin\theta\right)^{s+1} \partial_\theta  \left(-s  \left(\sin\theta\right)^{-(s+2)}\right)+ \left(\sin\theta\right)^{s+1} \partial_\theta \left(\sin\theta\right)^{-(s+1)}\partial_\theta 
%\end{align*}
%
%
%
%
%
%
%
%
%There are some important point to remark in this section. In first place, it is only with the introduction of two local charts, in this specific case spherical, that the scalar functions acquire spin-weight via the tangent vectors to the unitary sphere. Second, the nature of these last are complex in both cases spherical and stereographic. Third, the {\it eth} operators does not depend on the coordinate system selected and therefore its properties are still invariant for any coordinate system to be used. The last sentence has a certain relevance because we will use this fact to compute the left and the right side of the Einstein field equation in stereographic and spherical coordinates respectively in order to avoid unnecessary transformations. Fourth, a special careful must be taken into account in order to do these operator products, because they depend on the spin weight of the quantity in which are applied. 
%
%But $$
%Thus, from \eqref{abase1} and \eqref{abase2} we can to write the $\eth$ and $\overline{\eth}$ operators explicitly are
%\begin{subequations}
%\begin{align}
%\eth &=\dfrac{1+\zeta\overline{\zeta}}{2}\left(\partial_{q}+i\partial_{p}\right)+s\zeta \label{eth_spherical_1.1}\\
%\overline{\eth} &=\dfrac{1+\zeta\overline{\zeta}}{2}\left(\partial_{q}-i\partial_{p}\right)-s\overline{\zeta} \label{eth_spherical_1.2}
%\end{align}
%\label{eth_spherical_1}
%\end{subequations}
%Now, in order to obtain the $\partial_q$ and $\partial_p$ operators in terms of $\partial_{\theta}$ and $\partial_{\phi}$, we write the system formed by \eqref{legend12} and \eqref{legend32} as
%\begin{equation*}
%\begin{pmatrix}
%\partial_\theta \\
%\partial_\phi
%\end{pmatrix} = \begin{pmatrix}
%q_{,\theta} & p_{,\theta} \\
%q_{,\phi} & p_{,\phi} 
%\end{pmatrix}
%\begin{pmatrix}
%\partial_q \\
%\partial_p
%\end{pmatrix},
%\end{equation*}
%which allows us to write that
%\begin{equation*}
%\begin{pmatrix}
%\partial_q \\
%\partial_p
%\end{pmatrix}
%= \begin{pmatrix}
%q_{,\theta} & p_{,\theta} \\
%q_{,\phi} & p_{,\phi} 
%\end{pmatrix}^{-1}
%\begin{pmatrix}
%\partial_\theta \\
%\partial_\phi
%\end{pmatrix} ,
%\end{equation*}
%where
%\begin{equation*}
%\begin{pmatrix}
%q_{,\theta} & p_{,\theta} \\
%q_{,\phi} & p_{,\phi} 
%\end{pmatrix}^{-1}
%= \dfrac{1}{2q_{[,\theta}p_{,\phi]}}\begin{pmatrix}
%p_{,\phi}  & -p_{,\theta} \\
%-q_{,\phi} & q_{,\theta} 
%\end{pmatrix}.
%\end{equation*}
%It means that
%\begin{subequations}
%\begin{align}
%\partial_q&=\dfrac{ p_{,\phi}\partial_{\theta} - p_{,\theta}\partial_{\phi} }{2q_{[,\theta}p_{,\phi]}}, \label{eth_spherical_2.1}\\
%\partial_p&=\dfrac{ -q_{,\phi}\partial_{\theta} + q_{,\theta}\partial_{\phi} }{2q_{[,\theta}p_{,\phi]}}, \label{eth_spherical_2.2}
%\end{align}
%\label{eth_spherical_2}
%\end{subequations}
%where
%\begin{align*}
%2q_{[,\theta}p_{,\phi]} %&=q_{,\theta}p_{,\phi}-q_{,\phi}p_{,\theta}\\
%%&=\left(\dfrac{\left(\zeta+\overline{\zeta}\right)\left(1+\zeta\overline{\zeta}\right)}{4\left(\zeta\overline{\zeta}\right)^{1/2}}\right) \left(\dfrac{1}{2}(\overline{\zeta}+\zeta)\right) - \left(\dfrac{i}{2}(\zeta-\overline{\zeta})\right) \left(\dfrac{i\left(\overline{\zeta}-\zeta\right)\left(1+\zeta\overline{\zeta}\right)}{4\left(\zeta\overline{\zeta}\right)^{1/2}}\right)\\
%%&=\left(\dfrac{\left(\zeta+\overline{\zeta}\right)^2  \left(1+\zeta\overline{\zeta}\right)}{8\left(\zeta\overline{\zeta}\right)^{1/2}}\right)  -  \left(\dfrac{\left(\overline{\zeta}-\zeta\right)^2\left(1+\zeta\overline{\zeta}\right)}{8\left(\zeta\overline{\zeta}\right)^{1/2}}\right) \\
%%&=\dfrac{\left(1+\zeta\overline{\zeta}\right)}{8\left(\zeta\overline{\zeta}\right)^{1/2}}\left( \left(\zeta+\overline{\zeta}\right)^2  -  \left(\overline{\zeta}-\zeta\right)^2 \right)\\
%%&=\dfrac{4\zeta\overline{\zeta} \left(1+\zeta\overline{\zeta}\right)}{8\left(\zeta\overline{\zeta}\right)^{1/2}}\\
%&=\dfrac{\left(\zeta\overline{\zeta}\right)^{1/2} \left(1+\zeta\overline{\zeta}\right)}{2}
%\end{align*}
%Thus, \eqref{eth_spherical_1.1} takes the form
%\begin{align*}
%\eth %&=\dfrac{1+\zeta\overline{\zeta}}{2}\left(\partial_{q}+i\partial_{p}\right)+s\zeta \\
%%&=\dfrac{1+\zeta\overline{\zeta}}{4q_{[,\theta}p_{,\phi]}}\left( p_{,\phi}\partial_{\theta} - p_{\theta}\partial_{\phi} + i\left( -q_{,\phi}\partial_{\theta} + q_{\theta}\partial_{\phi} \right)\right) +s\zeta\\
%&=\dfrac{1+\zeta\overline{\zeta}}{4q_{[,\theta}p_{,\phi]}}\left( \left(p_{,\phi} -iq_{,\phi} \right)\partial_{\theta} +\left(iq_{,\theta}- p_{,\theta}\right)\partial_{\phi} \right)+s\zeta\\
%%\end{align*}
%%\begin{align*}
%\overline{\eth} %&=\dfrac{1+\zeta\overline{\zeta}}{2}\left(\partial_{q}-i\partial_{p}\right)-s\overline{\zeta} \\
%%&=\dfrac{1+\zeta\overline{\zeta}}{4q_{[,\theta}p_{,\phi]}}\left(p_{,\phi}\partial_{\theta} - p_{\theta}\partial_{\phi}-i\left(-q_{,\phi}\partial_{\theta} + q_{\theta}\partial_{\phi} \right)\right)-s\overline{\zeta}\\
%&=\dfrac{1+\zeta\overline{\zeta}}{4q_{[,\theta}p_{,\phi]}}\left(\left(p_{,\phi}+iq_{,\phi}\right)\partial_{\theta} - \left(p_{,\theta}+iq_{,\theta}\right)\partial_{\phi}\right)-s\overline{\zeta}
%\end{align*}
%also,
%\begin{align*}
%p_{,\phi} -iq_{,\phi} %&=\dfrac{1}{2}(\overline{\zeta}+\zeta) -i \left(\dfrac{i}{2}(\zeta-\overline{\zeta})\right) \\
%%&=\dfrac{1}{2}\left((\overline{\zeta}+\zeta) + \left(\zeta-\overline{\zeta}\right)\right)\\
%&= \zeta \\
%%\end{align*}
%%\begin{align*}
%p_{,\phi} +iq_{,\phi} %&=\dfrac{1}{2}(\overline{\zeta}+\zeta) +i \left(\dfrac{i}{2}(\zeta-\overline{\zeta})\right) \\
%%&=\dfrac{1}{2} \left((\overline{\zeta}+\zeta) - \left(\zeta-\overline{\zeta}\right)\right)\\ 
%&=\overline{\zeta}
%\end{align*}
%and
%\begin{align*}
%iq_{,\theta}- p_{,\theta}
%%&= i \left(\dfrac{\left(\zeta+\overline{\zeta}\right)\left(1+\zeta\overline{\zeta}\right)}{4\left(\zeta\overline{\zeta}\right)^{1/2}}\right) - \dfrac{i\left(\overline{\zeta}-\zeta\right)\left(1+\zeta\overline{\zeta}\right)}{4\left(\zeta\overline{\zeta}\right)^{1/2}} \\
%&= \dfrac{ 2 i \zeta \left(1+\zeta\overline{\zeta}\right)}{4\left(\zeta\overline{\zeta}\right)^{1/2}} \\
%%\end{align*}
%%\begin{align*}
%iq_{,\theta} + p_{,\theta} 
%%&= i \left(\dfrac{\left(\zeta+\overline{\zeta}\right)\left(1+\zeta\overline{\zeta}\right)}{4\left(\zeta\overline{\zeta}\right)^{1/2}}\right) + \dfrac{i\left(\overline{\zeta}-\zeta\right)\left(1+\zeta\overline{\zeta}\right)}{4\left(\zeta\overline{\zeta}\right)^{1/2}}\\
%&=\dfrac{2i \overline{\zeta}\left(1+\zeta\overline{\zeta}\right)}{4\left(\zeta\overline{\zeta}\right)^{1/2}} 
%\end{align*}
%%\begin{align*}
%%p_{,\phi}\partial_{\theta} - p_{\theta}\partial_{\phi} &= \dfrac{1}{2}(\overline{\zeta}+\zeta)\partial_{\theta} - \dfrac{i\left(\overline{\zeta}-\zeta\right)\left(1+\zeta\overline{\zeta}\right)}{4\left(\zeta\overline{\zeta}\right)^{1/2}}\partial_{\phi} \\
%%\end{align*}
%then
%\begin{align*}
%\eth &=\dfrac{1+\zeta\overline{\zeta}}{\left(\zeta\overline{\zeta}\right)^{1/2} \left(1+\zeta\overline{\zeta}\right)} \left( \zeta \partial_{\theta} +\left(\dfrac{ 2 i \zeta \left(1+\zeta\overline{\zeta}\right)}{4\left(\zeta\overline{\zeta}\right)^{1/2}}\right)\partial_{\phi} \right)+s\zeta\\
%%&=\dfrac{1}{\left(\zeta\overline{\zeta}\right)^{1/2}} \left( \zeta \partial_{\theta} +\left(\dfrac{ 2 i \zeta \left(1+\zeta\overline{\zeta}\right)}{4\left(\zeta\overline{\zeta}\right)^{1/2}}\right)\partial_{\phi} \right)+s\zeta \\
%%&= \dfrac{\zeta}{\left(\zeta\overline{\zeta}\right)^{1/2}}  \partial_{\theta} + \dfrac{ 2 i \zeta \left(1+\zeta\overline{\zeta}\right)}{4\zeta\overline{\zeta}} \partial_{\phi}  + s\zeta \\
%&= \left(\dfrac{\zeta}{\overline{\zeta}}\right)^{1/2}  \partial_{\theta} + \dfrac{ 2 i  \left(1+\zeta\overline{\zeta}\right)}{4\overline{\zeta}} \partial_{\phi}  + s\zeta
%\end{align*}
%then
%\begin{align*}
%\eth 
%%&= e^{i\phi}\partial_{\theta} + \dfrac{ 2 i  \left(1+\tan^2(\theta/2)\right)}{4\tan(\theta/2)e^{-i\phi}} \partial_{\phi}  + s\tan(\theta/2)e^{i\phi}\zeta \\
%&= e^{i\phi}\partial_{\theta} + \dfrac{ 2 i  \left(1+\tan^2(\theta/2)\right) e^{i\phi}}{4\tan(\theta/2)} \partial_{\phi}  + s\tan(\theta/2)e^{i\phi}
%\end{align*}
%now, using the fact that
%\begin{align*}
%\tan(\theta/2)
%%&=\dfrac{\sin(\theta/2)}{\cos(\theta/2)}\\
%%&=\dfrac{2\sin(\theta/2)\cos(\theta/2)}{2\cos^2(\theta/2)}\\
%%&=\dfrac{\sin \theta}{2\cos^2(\theta/2)}\\
%&=\dfrac{\sin \theta \left(1+\tan^2(\theta/2)\right)}{2}
%\end{align*}
%the eth operator can be written as
%\begin{align*}
%\eth %&= e^{i\phi}\partial_{\theta} + \dfrac{  i  e^{i\phi}}{\sin \theta } \partial_{\phi}  + s\tan(\theta/2)e^{i\phi} \\
%%&= e^{i\phi}\partial_{\theta} + i \csc\theta e^{i\phi} \partial_{\phi}  + s\tan(\theta/2)e^{i\phi} \\
%&= e^{i\phi}\left(\partial_{\theta} + i \csc\theta \partial_{\phi}  + s\tan(\theta/2)\right)
%\end{align*}
%Also, considering the identity
%\begin{align*}
%\tan(\theta/2)
%%&=\dfrac{\sin(\theta/2)}{\cos(\theta/2)}\\
%%&=\dfrac{2\sin^2(\theta/2)}{2\sin(\theta/2)\cos(\theta/2)}\\
%%&=\dfrac{2\sin^2(\theta/2)}{\sin \theta}\\
%&=\dfrac{1-\cos \theta}{\sin \theta}
%\end{align*}
%then,
%\begin{align*}
%\eth %&= e^{i\phi}\left(\partial_{\theta} + i \csc\theta \partial_{\phi}  + s\tan(\theta/2)\right) \\
%%&= e^{i\phi}\left(\partial_{\theta} + i \csc\theta \partial_{\phi}  + s\left(\dfrac{1}{\sin \theta} - \dfrac{\cos \theta}{\sin \theta} \right)\right)\\
%%&= e^{i\phi}\left(\partial_{\theta} + i \csc\theta \partial_{\phi}  + s\csc \theta - s\cot \theta \right)\\
%&= e^{i\phi}\left( i \csc\theta \partial_{\phi}  + s\csc \theta + \partial_{\theta} - s\cot \theta \right)
%\end{align*}
%When applied on an function it can be written as
%\begin{align*}
%\eth \ _s\Psi&= e^{i\phi}\left( i \csc\theta \partial_{\phi}  + s\csc \theta + \partial_{\theta} - s\cot \theta \right)\ _s\Psi
%\end{align*}
%Observing that
%\begin{align*}
%\left(\partial_{\theta} - s\cot \theta\right)\ _s\Psi &=\left(\sin\theta\right)^s \left(\sin\theta\right)^{-s}\left(\partial_{\theta} - s\cot \theta\right)\ _s\Psi\\
%&=\left(\sin\theta\right)^s \partial_{\theta}\left(\left(\sin\theta\right)^{-s} \ _s\Psi\right) 
%\end{align*}
%i.e.,
%\begin{align*}
%\eth \ _s\Psi&= e^{i\phi}\left[\left( i \csc\theta \partial_{\phi}  + s\csc \theta  \right)\ _s\Psi  + \left(\sin\theta\right)^s \partial_{\theta}\left(\left(\sin\theta\right)^{-s} \ _s\Psi\right)\right]\\
%&= \left[\csc\theta\left( i e^{i\phi}  \partial_{\phi}  + s e^{i\phi}  \right)\ _s\Psi  + \left(\sin\theta\right)^s \partial_{\theta}\left(e^{i\phi}\left(\sin\theta\right)^{-s} \ _s\Psi\right)\right]
%\end{align*}
%%\overline{\eth} &=\dfrac{1+\zeta\overline{\zeta}}{\left(\zeta\overline{\zeta}\right)^{1/2} \left(1+\zeta\overline{\zeta}\right)}\left(\left(p_{,\phi}+iq_{,\phi}\right)\partial_{\theta} - \left(p_{,\theta}+iq_{,\theta}\right)\partial_{\phi}\right)-s\overline{\zeta}

==> docs/first_order_perturbations.tex <==
\section{First Order Perturbations}
In this section, will be explored in full details the linear regime of the Einstein's field equations when an arbitrary background is considered. Despite the derivation for the wave equation at first order does not differs to those in which a Minkowski's background is taken into account, additional terms related with the background Riemann tensor and the correct interpretation of the D'Alembertian involving in this are shown.
\\As a starting point, perturbations to an arbitrary background $\overset{\hspace{-0.3cm}(0)}{g_{\mu\nu}}$ at first order are chosen, i.e.,
\begin{equation}
g_{\mu\nu}=\overset{\hspace{-0.3cm}(0)}{g_{\mu\nu}}+\epsilon \overset{\hspace{-0.3cm}(1)}{g_{\mu\nu}},
\label{eq2.1}
\end{equation}
where $\epsilon$ is a parameter that measures the perturbation, satisfying $\epsilon\ll 1$. It is worth stressing to notice that it guaranties that the second term is smaller than the first, because the characteristic length of such perturbations, $\lambda$, must be very small compared with the characteristic length of the radius of curvature of the background, $L$. This limit is known as the high frequency approximation \cite{I68_1}. 
\\Considering that the inverse metric $g^{\mu\nu}$ is given as a background term plus a first order perturbation with respect to the background, i.e.,
\begin{equation}
g^{\mu\nu}=\overset{\hspace{-0.3cm}(0)}{g^{\mu\nu}}+\epsilon\, \overset{\hspace{-0.3cm}(1)}{g^{\mu\nu}},
\label{eq2.2}
\end{equation}
and that $g_{\mu\nu}g^{\eta\nu}=\overset{\hspace{-0.3cm}(0)}{g_{\mu\nu}}\overset{\hspace{-0.3cm}(0)}{g^{\eta\nu}}=\delta_\mu^{~~\eta}$ then
\begin{align}
g_{\mu\sigma}g^{\sigma\nu}&= 
\overset{\hspace{-0.3cm}(0)}{g_{\mu\sigma}} \overset{\hspace{-0.3cm}(0)}{g^{\sigma\nu}}+ \epsilon\left(\, \overset{\hspace{-0.3cm}(1)}{g^{\sigma\nu}}\, \overset{\hspace{-0.3cm}(0)}{g_{\mu\sigma}} + \overset{\hspace{-0.3cm}(1)}{g_{\mu\sigma}} \overset{\hspace{-0.3cm}(0)}{g^{\sigma\nu}} \right)+O(\epsilon^2). 
\label{eq2.3}
\end{align}
Therefore, as the polynomial for $\epsilon$, \eqref{eq2.3}, is null term by term, then the perturbation in the metric inverse is given by
%\begin{equation}
%\overset{\hspace{-0.3cm}(1)}{L^{\eta\nu}} =- \overset{\hspace{-0.3cm}(1)}{g^{\eta\nu}},
%\label{eq2.4}
%\end{equation}
%where
\begin{equation}
\overset{\hspace{-0.3cm}(1)}{g^{\eta\nu}}=-\overset{\hspace{-0.3cm}(1)}{g_{\mu\sigma}} \overset{\hspace{-0.3cm}(0)}{g^{\mu\eta}}\overset{\hspace{-0.3cm}(0)}{g^{\sigma\nu}}.
\label{eq2.5}
\end{equation}
%Thus, the inverse metric \eqref{eq2.2} reads
%\begin{equation}
%g^{\mu\nu}=\overset{\hspace{-0.3cm}(0)}{g^{\mu\nu}}-\epsilon \overset{\hspace{-0.3cm}(1)}{g^{\mu\nu}}.
%\label{eq2.6}
%\end{equation}
With this, the Christoffel's symbols of the first kind, 
\begin{equation}
\Gamma_{\mu\nu\gamma}=\frac{1}{2}\left(g_{\mu\nu,\gamma}+g_{\gamma\mu,\nu}-g_{\nu\gamma,\mu}\right),
\label{eq2.7}
\end{equation}
where the comma indicating partial derivative, can be separated as a term referred to the background plus a perturbation
\begin{equation}
\Gamma_{\mu\nu\gamma}=\overset{\hspace{-0.6cm}(0)}{\Gamma_{\mu\nu\gamma}}+\epsilon \overset{\hspace{-0.6cm}(1)}{\Gamma_{\mu\nu\gamma}},%+O(\epsilon^2),
\label{eq2.8}
\end{equation}
where
\begin{equation}
\overset{\hspace{-0.6cm}(i)}{\Gamma_{\mu\nu\gamma}}=\frac{1}{2}\left(\,\overset{\hspace{-0.5cm}(i)}{g_{\mu\nu,\gamma}}+\overset{\hspace{-0.5cm}(i)}{g_{\gamma\mu,\nu}}
-
\overset{\hspace{-0.5cm}(i)}{g_{\nu\gamma,\mu}}\right),\hspace{0.5cm}i=0,1.
\label{eq2.9}
\end{equation}
Thus, the Christoffel's symbols of the second kind,
\begin{align}
\Gamma^\mu_{~\nu\gamma}&=g^{\mu\sigma}\Gamma_{\sigma\nu\gamma}, 
\label{eq2.10}
\end{align}
can also be separated as,
\begin{align}
\Gamma^\mu_{~\nu\gamma}&=
\overset{\hspace{-0.6cm}(0)}{\Gamma^\mu_{~\nu\gamma}} + \epsilon\overset{\hspace{-0.6cm}(1)}{\Gamma^\mu_{~\nu\gamma}}+O(\epsilon^2), 
\label{eq2.11}
\end{align}
where,
\begin{align}
\overset{\hspace{-0.6cm}(0)}{\Gamma^\mu_{~\nu\gamma}}=\overset{\hspace{-0.3cm}(0)}{g^{\mu\sigma}}\overset{\hspace{-0.6cm}(0)}{\Gamma_{\sigma\nu\gamma}}, 
\hspace{0.5cm}
\overset{\hspace{-0.6cm}(1)}{\Gamma^\mu_{~\nu\gamma}}= \overset{\hspace{-0.3cm}(0)}{g^{\mu\sigma}}\overset{\hspace{-0.6cm}(1)}{\Gamma_{\sigma\nu\gamma}}
%- 
+
\overset{\hspace{-0.3cm}(1)}{g^{\mu\sigma}}\overset{\hspace{-0.6cm}(0)}{\Gamma_{\sigma\nu\gamma}}.
\label{eq2.12}
\end{align}
In this manner the Riemann's tensor is written as a term associated to the background plus a term corresponding to the perturbation, i.e.,
\begin{align}
R^\mu_{~~\nu\gamma\delta}&= \overset{\hspace{-0.7cm}(0)}{R^\mu_{~~\nu\gamma\delta}}+\epsilon \overset{\hspace{-0.7cm}(1)}{R^\mu_{~~\nu\gamma\delta}},
\label{eq2.13}
\end{align}
where the background Riemann tensor is given by
%\begin{equation}
%\overset{\hspace{-0.7cm}(0)}{R^\mu_{~~\nu\gamma\delta}}=\overset{\hspace{-0.8cm}(0)}{\Gamma^\mu_{~\nu\delta,\gamma}}-\overset{\hspace{-0.8cm}(0)}{\Gamma^\mu_{~\nu\gamma,\delta}}
%+\overset{\hspace{-0.6cm}(0)}{\Gamma^\sigma_{~\nu\delta}}\overset{\hspace{-0.6cm}(0)}{\Gamma^\mu_{~\sigma\gamma}} 
%-\overset{\hspace{-0.6cm}(0)}{\Gamma^\sigma_{~\nu\gamma}}\overset{\hspace{-0.6cm}(0)}{\Gamma^\mu_{~\sigma\delta}},
%\label{eq2.14}
%\end{equation}
\begin{equation}
\overset{\hspace{-0.7cm}(0)}{R^\mu_{~~\nu\gamma\delta}}=
\overset{\hspace{-0.8cm}(0)}{\Gamma^\mu_{~\nu[\delta,\gamma]}}
+\overset{\hspace{-0.6cm}(0)}{\Gamma^\sigma_{~\nu[\delta}}\overset{\hspace{-0.6cm}(0)}{\Gamma^\mu_{~\gamma]\sigma}},
\label{eq2.14}
\end{equation}
and the term associated with the perturbation reads
\begin{align}
\overset{\hspace{-0.7cm}(1)}{R^\mu_{~~\nu\gamma\delta}}
%&=
%\overset{\hspace{-0.8cm}(1)}{\Gamma^\mu_{~\nu\delta,\gamma}}-\overset{\hspace{-0.8cm}(1)}{\Gamma^\mu_{~\nu\gamma,\delta}}
%+ \overset{\hspace{-0.5cm}(1)}{\Gamma^\mu_{~\sigma\gamma}}\overset{\hspace{-0.5cm}(0)}{\Gamma^\sigma_{~\nu\delta}}   
%+\overset{\hspace{-0.5cm}(1)}{\Gamma^\sigma_{~\nu\delta}}\overset{\hspace{-0.5cm}(0)}{\Gamma^\mu_{~\sigma\gamma}} 
%-\overset{\hspace{-0.5cm}(1)}{\Gamma^\mu_{~\sigma\delta}}\overset{\hspace{-0.5cm}(0)}{\Gamma^\sigma_{~\nu\gamma}} 
%-\overset{\hspace{-0.5cm}(1)}{\Gamma^\sigma_{~\nu\gamma}}\overset{\hspace{-0.5cm}(0)}{\Gamma^\mu_{~\sigma\delta}},\nonumber\\
&=
2\,\overset{\hspace{-0.8cm}(1)}{\Gamma^\mu_{~\nu[\delta,\gamma]}}
+ 2\, \overset{\hspace{-0.5cm}(1)}{\Gamma^\mu_{~\sigma[\gamma}}\overset{\hspace{-0.5cm}(0)}{\Gamma^\sigma_{~\delta]\nu}}   
+2\,\overset{\hspace{-0.5cm}(1)}{\Gamma^\sigma_{~\nu[\delta}}\overset{\hspace{-0.5cm}(0)}{\Gamma^\mu_{~\gamma]\sigma}}.
\label{eq2.15}
\end{align}
The square brackets indicates anti-symmetrisation as usual, i.e.,
\begin{equation}
A_{[\alpha_1\cdots\alpha_n]}=\frac{1}{n!}\epsilon_{\alpha_1\cdots\alpha_n}^{\hspace{0.9cm}\beta_1\cdots\beta_n}A_{\beta_1\cdots\beta_n},
\end{equation}
where $\epsilon_{\alpha_1\cdots\alpha_n}^{\hspace{0.9cm}\beta_1\cdots\beta_n}$ is the generalised Levi-Civita permutation symbol.\\
From $\overset{\hspace{-0.8cm}(1)}{\Gamma^\mu_{~\nu\delta:\gamma}}$, where the colon indicates covariant derivative  associated with the background metric $\overset{(0)}{g}_{\mu\nu}$, one obtains
\begin{equation}
\overset{\hspace{-0.7cm}(1)}{\Gamma^\mu_{~\nu[\delta,\gamma]}}= \overset{\hspace{-0.7cm}(1)}{\Gamma^\mu_{~\nu[\delta:\gamma]}} 
- \overset{\hspace{-0.5cm}(0)}{\Gamma^\mu_{~\sigma[\gamma}} \overset{\hspace{-0.5cm}(1)}{\Gamma^\sigma_{~\delta]\nu}}
+\overset{\hspace{-0.5cm}(0)}{\Gamma^\sigma_{~\nu[\gamma}}
\overset{\hspace{-0.5cm}(1)}{\Gamma^\mu_{~\delta]\sigma}}
+\overset{\hspace{-0.5cm}(0)}{\Gamma^\sigma_{~[\gamma\delta]}} \overset{\hspace{-0.5cm}(1)}{\Gamma^\mu_{~\nu\sigma}}.
\label{eq2.16}
\end{equation}
%\begin{equation}
%\overset{\hspace{-0.7cm}(1)}{\Gamma^\mu_{~\nu\gamma,\delta}}= \overset{\hspace{-0.7cm}(1)}{\Gamma^\mu_{~\nu\gamma:\delta}} 
%- \overset{\hspace{-0.5cm}(0)}{\Gamma^\mu_{~\delta\sigma}} \overset{\hspace{-0.5cm}(1)}{\Gamma^\sigma_{~\nu\gamma}}
%+\overset{\hspace{-0.5cm}(0)}{\Gamma^\sigma_{~\delta\nu}}
%\overset{\hspace{-0.5cm}(1)}{\Gamma^\mu_{~\sigma\gamma}}
%+\overset{\hspace{-0.5cm}(0)}{\Gamma^\sigma_{~\delta\gamma}} \overset{\hspace{-0.5cm}(1)}{\Gamma^\mu_{~\nu\sigma}}
%\end{equation}
%\begin{align}
%\overset{\hspace{-0.7cm}(1)}{\Gamma^\mu_{~\nu\delta,\gamma}}-\overset{\hspace{-0.7cm}(1)}{\Gamma^\mu_{~\nu\gamma,\delta}}&=
%\overset{\hspace{-0.7cm}(1)}{\Gamma^\mu_{~\nu\delta:\gamma}} 
%-\overset{\hspace{-0.7cm}(1)}{\Gamma^\mu_{~\nu\gamma:\delta}}
%- \overset{\hspace{-0.5cm}(0)}{\Gamma^\mu_{~\gamma\sigma}} \overset{\hspace{-0.5cm}(1)}{\Gamma^\sigma_{~\nu\delta}}
%+ \overset{\hspace{-0.5cm}(0)}{\Gamma^\mu_{~\delta\sigma}} \overset{\hspace{-0.5cm}(1)}{\Gamma^\sigma_{~\nu\gamma}}
%+\overset{\hspace{-0.5cm}(0)}{\Gamma^\sigma_{~\gamma\nu}}
%\overset{\hspace{-0.5cm}(1)}{\Gamma^\mu_{~\sigma\delta}}
%\nonumber\\
%&-
%\overset{\hspace{-0.5cm}(0)}{\Gamma^\sigma_{~\delta\nu}}
%\overset{\hspace{-0.5cm}(1)}{\Gamma^\mu_{~\sigma\gamma}}
%\end{align}
%\begin{align}
%\overset{\hspace{-0.7cm}(1)}{\Gamma^\mu_{~\nu[\delta,\gamma]}}&=
%\overset{\hspace{-0.7cm}(1)}{\Gamma^\mu_{~\nu[\delta:\gamma]}} 
%- \overset{\hspace{-0.5cm}(0)}{\Gamma^\mu_{~\sigma[\gamma}} \overset{\hspace{-0.5cm}(1)}{\Gamma^\sigma_{~\delta]\nu}}
%+\overset{\hspace{-0.5cm}(0)}{\Gamma^\sigma_{~\nu[\gamma}}
%\overset{\hspace{-0.5cm}(1)}{\Gamma^\mu_{~\delta]\sigma}}
%\end{align}
Thus, substituting it into the Riemann's tensor \eqref{eq2.15}, one obtains immediately
\begin{align}
\overset{\hspace{-0.7cm}(1)}{R^\mu_{~~\nu\gamma\delta}}&=
2\overset{\hspace{-0.9cm}(1)}{\Gamma^\mu_{~\nu[\delta:\gamma]}}.
\label{eq2.17}
\end{align}
From \eqref{eq2.10} it is observed that
\begin{align}
\overset{\hspace{-0.9cm}(1)}{\Gamma^\mu_{~\nu[\delta:\gamma]}}&= \overset{\hspace{-0.6cm}(1)}{\Gamma_{\sigma\nu[\delta}}\overset{\hspace{-0.8cm}(0)}{g^{\mu\sigma}_{~~~:\gamma]}} +\overset{\hspace{-0.3cm}(0)}{g^{\mu\sigma}}\overset{\hspace{-0.8cm}(1)}{\Gamma_{\sigma\nu[\delta:\gamma]}}
-\overset{\hspace{-0.6cm}(0)}{\Gamma_{\sigma\nu[\delta}}\overset{\hspace{-0.6cm}(1)}{g^{\mu\sigma}_{~~~:\gamma]}}
-\overset{\hspace{-0.3cm}(1)}{g^{\mu\sigma}}\overset{\hspace{-0.8cm}(0)}{\Gamma_{\sigma\nu[\delta:\gamma]}},\nonumber\\
&=\overset{\hspace{-0.3cm}(0)}{g^{\mu\sigma}}\overset{\hspace{-0.9cm}(1)}{\Gamma_{\sigma\nu[\delta:\gamma]}}
-\overset{\hspace{-0.6cm}(0)}{\Gamma_{\sigma\nu[\delta}}\overset{\hspace{-0.7cm}(1)}{g^{\mu\sigma}_{~~~:\gamma]}}
-\overset{\hspace{-0.3cm}(1)}{g^{\mu\sigma}}\overset{\hspace{-0.8cm}(0)}{\Gamma_{\sigma\nu[\delta:\gamma]}}.
\label{eq2.18}
\end{align}
Then, substituting \eqref{eq2.18} into \eqref{eq2.17}
\begin{align}
\overset{\hspace{-0.7cm}(1)}{R^\mu_{~~\nu\gamma\delta}} %=&
%2\overset{\hspace{-0.7cm}(1)}{\Gamma^\mu_{~\nu[\delta:\gamma]}}\\&=
%2\,\overset{\hspace{-0.3cm}(0)}{g^{\mu\sigma}}\overset{\hspace{-0.9cm}(1)}{\Gamma_{\sigma\nu[\delta:\gamma]}}
%-2\,\overset{\hspace{-0.6cm}(0)}{\Gamma_{\sigma\nu[\delta}}\overset{\hspace{-0.8cm}(1)}{g^{\mu\sigma}_{~~~:\gamma]}}
%-2\,\overset{\hspace{-0.3cm}(1)}{g^{\mu\sigma}}\overset{\hspace{-0.9cm}(0)}{\Gamma_{\sigma\nu[\delta:\gamma]}},\nonumber\\
=&\overset{\hspace{-0.3cm}(0)}{g^{\mu\sigma}}\overset{\hspace{-0.8cm}(1)}{\Gamma_{\sigma\nu\delta:\gamma}} - \overset{\hspace{-0.3cm}(0)}{g^{\mu\sigma}}\overset{\hspace{-0.8cm}(1)}{\Gamma_{\sigma\nu\gamma:\delta}}
-\overset{\hspace{-0.6cm}(0)}{\Gamma_{\sigma\nu\delta}}\overset{\hspace{-0.6cm}(1)}{g^{\mu\sigma}_{~~~:\gamma}}
+\overset{\hspace{-0.6cm}(0)}{\Gamma_{\sigma\nu\gamma}}\overset{\hspace{-0.6cm}(1)}{g^{\mu\sigma}_{~~~:\delta}}\nonumber\\
&-\overset{\hspace{-0.3cm}(1)}{g^{\mu\sigma}}\overset{\hspace{-0.7cm}(0)}{\Gamma_{\sigma\nu\delta:\gamma}}
+\overset{\hspace{-0.3cm}(1)}{g^{\mu\sigma}}\overset{\hspace{-0.7cm}(0)}{\Gamma_{\sigma\nu\gamma:\delta}}.
\label{eq2.19}
\end{align}
In order to compute the Riemann's tensor for the perturbation \eqref{eq2.19}, it is necessary to calculate
\begin{align}
\overset{\hspace{-0.8cm}(1)}{\Gamma_{\sigma\nu\delta:\gamma}}&=
\frac{1}{2}\left(\,\overset{\hspace{-0.7cm}(1)}{g_{\sigma\nu,\delta:\gamma}}+\overset{\hspace{-0.7cm}(1)}{g_{\delta\sigma,\nu:\gamma}}-\overset{\hspace{-0.7cm}(1)}{g_{\nu\delta,\sigma:\gamma}}\right),
\label{eq2.20}
\end{align}
%\begin{align}
%\overset{\hspace{-0.6cm}(1)}{\Gamma_{\sigma\nu\gamma:\delta}}&=
%\frac{1}{2}\left(\overset{(1)}{g_{\sigma\nu,\gamma:\delta}}+\overset{(1)}{g_{\gamma\sigma,\nu:\delta}}-\overset{(1)}{g_{\nu\gamma,\sigma:\delta}}\right)%_{:\gamma}
%\end{align}
%\begin{align}
%2\overset{\hspace{-0.6cm}(1)}{\Gamma_{\sigma\nu[\delta:\gamma]}}&=
%\overset{(1)}{g_{\sigma\nu,[\delta:\gamma]}}+\overset{(0)}{g_{\sigma\alpha}}\overset{(0)}{g_{\nu\beta}}\overset{(1)}{g^{~\,\alpha,\beta}_{[\delta~~\,:\gamma]}}-\overset{(0)}{g_{\alpha\nu}}\overset{(0)}{g_{\beta\sigma}}\overset{(1)}{g^{\alpha~\beta}_{~[\delta,~:\gamma]}}
%\end{align}
where
\begin{align}
\overset{\hspace{-0.7cm}(1)}{g_{\sigma\nu,\delta:\gamma}}&=\left(\overset{\hspace{-0.5cm}(1)}{g_{\sigma\nu:\delta}}+\overset{\hspace{-0.5cm}(0)}{\Gamma^{\lambda}_{~\sigma\delta}} \overset{\hspace{-0.3cm}(1)}{g_{\lambda\nu}}+\overset{\hspace{-0.7cm}(0)}{\Gamma^{\lambda}_{~~\delta\nu}}\overset{\hspace{-0.3cm}(1)}{g_{\sigma\lambda}}\right)_{:\gamma},\nonumber\\
&=
\overset{\hspace{-0.7cm}(1)}{g_{\sigma\nu:\delta\gamma}}
+\overset{\hspace{-0.7cm}(0)}{\Gamma^{\lambda}_{~\sigma\delta:\gamma}} \overset{\hspace{-0.3cm}(1)}{g_{\lambda\nu}}
+\overset{\hspace{-0.5cm}(0)}{\Gamma^{\lambda}_{~\sigma\delta}} \overset{\hspace{-0.5cm}(1)}{g_{\lambda\nu:\gamma}}
+\overset{\hspace{-0.8cm}(0)}{\Gamma^{\lambda}_{~~\delta\nu:\gamma}}\overset{\hspace{-0.3cm}(1)}{g_{\sigma\lambda}}
+\overset{\hspace{-0.5cm}(0)}{\Gamma^{\lambda}_{~~\delta\nu}}\overset{\hspace{-0.5cm}(1)}{g_{\sigma\lambda:\gamma}}.
\label{eq2.21}
\end{align}
Substituting \eqref{eq2.21} into \eqref{eq2.20} it is found that
\begin{align}
\overset{\hspace{-0.7cm}(1)}{\Gamma_{\sigma\nu\delta:\gamma}}=\frac{1}{2}\left(\,\overset{\hspace{-0.7cm}(1)}{g_{\sigma\nu:\delta\gamma}} + \overset{\hspace{-0.7cm}(1)}{g_{\delta\sigma:\nu\gamma}} - \overset{\hspace{-0.7cm}(1)}{g_{\nu\delta:\sigma\gamma}} \right)+\overset{\hspace{-0.8cm}(0)}{\Gamma^\lambda_{~\nu\delta:\gamma}}\overset{\hspace{-0.3cm}(1)}{g_{\sigma\lambda}}+\overset{\hspace{-0.5cm}(0)}{\Gamma^\lambda_{~\nu\delta}}\overset{\hspace{-0.6cm}(1)}{g_{\sigma\lambda:\gamma}}.
\label{eq2.22}
\end{align}
Therefore, substituting \eqref{eq2.22} into \eqref{eq2.19} one obtains that the Riemann tensor corresponding to the perturbations is given by
\begin{align}
\overset{\hspace{-0.7cm}(1)}{R^\mu_{~~\nu\gamma\delta}}
%=&\frac{1}{2}\,\overset{\hspace{-0.3cm}(0)}{g^{\mu\sigma}}\left(\,
%\overset{\hspace{-0.7cm}(1)}{g_{\sigma\nu:\delta\gamma}}
%+\overset{\hspace{-0.7cm}(1)}{g_{\delta\sigma:\nu\gamma}}
%+\overset{\hspace{-0.7cm}(1)}{g_{\nu\gamma:\sigma\delta}}
%-\overset{\hspace{-0.7cm}(1)}{g_{\nu\delta:\sigma\gamma}}
%-\overset{\hspace{-0.7cm}(1)}{g_{\sigma\nu:\gamma\delta}}
%-\overset{\hspace{-0.7cm}(1)}{g_{\gamma\sigma:\nu\delta}}
%\right),\nonumber\\
=&\frac{1}{2}\left(\,
\overset{\hspace{-0.6cm}(1)}{g^\mu_{~\nu:\delta\gamma}}
+\overset{\hspace{-0.6cm}(1)}{g^{~\mu}_{\delta~:\nu\gamma}}
+\overset{\hspace{-0.6cm}(1)}{g^{~~~\mu}_{\nu\gamma:~\delta}}
-\overset{\hspace{-0.6cm}(1)}{g^{~~~\mu}_{\nu\delta:~\gamma}}
-\overset{\hspace{-0.6cm}(1)}{g^{\mu}_{~\nu:\gamma\delta}}
-\overset{\hspace{-0.6cm}(1)}{g^{~\mu}_{\gamma~:\nu\delta}}
\right).
\label{eq2.23}
\end{align}
Now, writing the field equations as
\begin{equation}
R_{\mu\nu}=8\pi \left(T_{\mu\nu}-\frac{1}{2}g_{\mu\nu}T\right),
\label{eq2.24}
\end{equation}
where, $T_{\mu\nu}$ and $T$ are the energy-stress tensor and its trace respectively, and using \eqref{eq2.11} then
\begin{equation}
\overset{\hspace{-0.3cm}(0)}{R_{\mu\nu}}+\epsilon\overset{\hspace{-0.3cm}(1)}{R_{\mu\nu}}=8\pi \left(T_{\mu\nu}-\frac{1}{2}g_{\mu\nu}T\right).
\label{eq2.25}
\end{equation}
Assuming that the background satisfies the Einstein's field equations
\begin{equation}
\overset{\hspace{-0.3cm}(0)}{R_{\mu\nu}}=8\pi \left(T_{\mu\nu}-\frac{1}{2}g_{\mu\nu}T\right),
\label{eq2.26}
\end{equation}
we found that the perturbation to the Ricci's tensor satisfies
\begin{equation}
\overset{\hspace{-0.3cm}(1)}{R_{\mu\nu}}=0.
\label{eq2.27}
\end{equation}
Contracting \eqref{eq2.23}, and substituting in \eqref{eq2.27}
%\begin{align}
%\overset{\hspace{-0.3cm}(1)}{R_{\nu\delta}}=&\frac{1}{2}\left(
%\overset{(1)}{g^\mu_{~\nu:\delta\mu}}
%+\overset{(1)}{g^{~\mu}_{\delta~:\nu\mu}}
%+\overset{(1)}{g^{~~~\mu}_{\nu\mu:~\delta}}
%-\overset{(1)}{g^{~~~\mu}_{\nu\delta:~\mu}}
%-\overset{(1)}{g^{\mu}_{~\nu:\mu\delta}}
%-\overset{(1)}{g^{~\mu}_{\mu~:\nu\delta}}
%\right),\nonumber\\
%=&\frac{1}{2}\left(
%\overset{(1)}{g^\mu_{~\nu:\delta\mu}}
%+\overset{(1)}{g^{~\mu}_{\delta~:\nu\mu}}
%-\overset{(1)}{g^{~~~\mu}_{\nu\delta:~\mu}}
%-\overset{(1)}{g^{~\mu}_{\mu~:\nu\delta}}
%\right).
%\label{eq2.28}
%\end{align}
%i.e.,
\begin{equation}
\frac{1}{2}\left(
\overset{(1)}{g^\mu_{~\nu:\delta\mu}}
+\overset{(1)}{g^{~\mu}_{\delta~:\nu\mu}}
-\overset{(1)}{g^{~~~\mu}_{\nu\delta:~\mu}}
-\overset{(1)}{g^{~\mu}_{\mu~:\nu\delta}}
\right)=0
\label{eq2.28}
\end{equation}
which corresponds to the wave equation for the metric perturbations of the first order.
\\ It is worth stressing to note that \eqref{eq2.28} can be re-written as
\begin{equation}
\overset{\hspace{-0.3cm}(0)}{g^{\mu\sigma}}\left(
2\,\overset{\hspace{-0.8cm}(1)}{g_{\sigma\nu:[\delta\mu]}} +\overset{\hspace{-0.7cm}(1)}{g_{\sigma\nu:\mu\delta}}
+2\,\overset{\hspace{-0.8cm}(1)}{g_{\delta\sigma:[\nu\mu]}}
+\overset{\hspace{-0.7cm}(1)}{g_{\delta\sigma:\mu\nu}}
-\overset{\hspace{-0.7cm}(1)}{g_{\nu\delta:\sigma\mu}}
-\overset{\hspace{-0.7cm}(1)}{g_{\mu\sigma:\nu\delta}}\right)
=0,
\label{eq2.29}
\end{equation}
where
\begin{equation}
\overset{\hspace{-0.9cm}(1)}{g_{\sigma\nu:[\delta\mu]}}=
\overset{\hspace{-0.9cm}(1)}{g_{\sigma\nu,[\delta:\mu]}}
-\overset{\hspace{-0.9cm}(0)}{\Gamma^{\lambda}_{~\sigma[\delta:\mu]}}\overset{\hspace{-0.3cm}(1)}{g_{\nu\lambda}}
-\overset{\hspace{-0.5cm}(1)}{g_{\nu\lambda:[\mu}}\overset{\hspace{-0.6cm}(0)}{\Gamma^{\lambda}_{~\delta]\sigma}}
-\overset{\hspace{-0.9cm}(0)}{\Gamma^{\lambda}_{~\nu[\delta:\mu]}}\overset{\hspace{-0.3cm}(1)}{g_{\sigma\lambda}}
-\overset{\hspace{-0.5cm}(1)}{g_{\sigma\delta:[\mu}}\overset{\hspace{-0.6cm}(0)}{\Gamma^{\lambda}_{~\delta]\nu}}.
\label{eq2.30}
\end{equation}
Explicitly, \eqref{eq2.30} is
\begin{align*}
\overset{\hspace{-0.8cm}(1)}{g_{\sigma\nu:[\delta\mu]}}=&
\overset{\hspace{-0.8cm}(1)}{g_{\sigma\nu,[\delta\mu]}}-\overset{\hspace{-0.5cm}(1)}{g_{\lambda\nu,[\delta}}\overset{\hspace{-0.7cm}(0)}{\Gamma^{\lambda}_{~\mu]\sigma}}-\overset{\hspace{-0.5cm}(1)}{g_{\sigma\lambda,[\delta}}\overset{\hspace{-0.7cm}(0)}{\Gamma^\lambda_{~\mu]\nu}}-\overset{\hspace{-0.7cm}(0)}{\Gamma^\lambda_{~[\delta\mu]}}\overset{\hspace{-0.5cm}(0)}{g_{\sigma\nu,\lambda}}
\nonumber\\
&-\left(\,\overset{\hspace{-0.9cm}(0)}{\Gamma^\lambda_{~\sigma[\delta,\mu]}}+\overset{\hspace{-0.5cm}(0)}{\Gamma^\lambda_{~\epsilon[\mu}}\overset{\hspace{-0.5cm}(0)}{\Gamma^\epsilon_{~\delta]\sigma}}-\overset{\hspace{-0.5cm}(0)}{\Gamma^\epsilon_{~\sigma[\mu}}\overset{\hspace{-0.5cm}(0)}{\Gamma^\lambda_{~\delta]\epsilon}}-\overset{\hspace{-0.5cm}(0)}{\Gamma^\epsilon_{~[\delta\mu]}}\overset{\hspace{-0.5cm}(0)}{\Gamma^\lambda_{~\sigma\epsilon}}\right)\overset{\hspace{-0.3cm}(1)}{g_{\nu\lambda}}
\nonumber\\
&-\overset{\hspace{-0.6cm}(1)}{g_{\nu\lambda,[\mu}}\overset{\hspace{-0.6cm}(0)}{\Gamma^\lambda_{~\delta]\sigma}}+\overset{\hspace{-0.5cm}(0)}{\Gamma^\lambda_{~\sigma[\delta}}\overset{\hspace{-0.5cm}(0)}{\Gamma^\epsilon_{~\mu]\nu}}\overset{\hspace{-0.3cm}(1)}{g_{\epsilon\lambda}}+\overset{\hspace{-0.5cm}(0)}{\Gamma^\lambda_{~\sigma[\delta}}\overset{\hspace{-0.5cm}(0)}{\Gamma^\epsilon_{~\mu]\lambda}}\overset{\hspace{-0.3cm}(1)}{g_{\nu\epsilon}}
\nonumber\\
&-\left(\,\overset{\hspace{-0.9cm}(0)}{\Gamma^\lambda_{~\nu[\delta,\mu]}}+\overset{\hspace{-0.5cm}(0)}{\Gamma^\lambda_{~\epsilon[\mu}}\overset{\hspace{-0.5cm}(0)}{\Gamma^\epsilon_{~\delta]\nu}}-\overset{\hspace{-0.5cm}(0)}{\Gamma^\epsilon_{~\nu[\mu}}\overset{\hspace{-0.5cm}(0)}{\Gamma^\lambda_{~\delta]\epsilon}}-\overset{\hspace{-0.5cm}(0)}{\Gamma^\epsilon_{~[\delta\mu]}}\overset{\hspace{-0.5cm}(0)}{\Gamma^\lambda_{~\nu\epsilon}}\right)\overset{\hspace{-0.3cm}(1)}{g_{\sigma\lambda}}
\nonumber\\
&-\overset{\hspace{-0.6cm}(1)}{g_{\sigma\lambda,[\mu}}\overset{\hspace{-0.5cm}(0)}{\Gamma^\lambda_{~\delta]\nu}}+\overset{\hspace{-0.5cm}(0)}{\Gamma^\lambda_{~\nu[\delta}}\overset{\hspace{-0.5cm}(0)}{\Gamma^\epsilon_{~\mu]\sigma}}\overset{\hspace{-0.3cm}(1)}{g_{\epsilon\lambda}}+\overset{\hspace{-0.5cm}(0)}{\Gamma^\lambda_{~\nu[\delta}}\overset{\hspace{-0.5cm}(0)}{\Gamma^\epsilon_{~\mu]\lambda}}\overset{\hspace{-0.3cm}(1)}{g_{\sigma\epsilon}},
\end{align*}
or 
\begin{align}
\overset{\hspace{-0.8cm}(1)}{g_{\sigma\nu:[\delta\mu]}}
&=-\left(\,\overset{\hspace{-0.9cm}(0)}{\Gamma^\lambda_{~\sigma[\delta,\mu]}}+\overset{\hspace{-0.5cm}(0)}{\Gamma^\lambda_{~\epsilon[\mu}}\overset{\hspace{-0.5cm}(0)}{\Gamma^\epsilon_{~\delta]\sigma}}\right)\overset{\hspace{-0.3cm}(1)}{g_{\nu\lambda}}
-\left(\,\overset{\hspace{-0.9cm}(0)}{\Gamma^\lambda_{~\nu[\delta,\mu]}}+\overset{\hspace{-0.5cm}(0)}{\Gamma^\lambda_{~\epsilon[\mu}}\overset{\hspace{-0.5cm}(0)}{\Gamma^\epsilon_{~\delta]\nu}}\right)\overset{\hspace{-0.3cm}(1)}{g_{\sigma\lambda}},\nonumber\\
&=-\frac{1}{2}\left(
\overset{\hspace{-0.6cm}(0)}{R^\lambda_{~\sigma\mu\delta}}\overset{\hspace{-0.3cm}(1)}{g_{\nu\lambda}}
+\overset{\hspace{-0.6cm}(0)}{R^\lambda_{~\nu\mu\delta}}\overset{\hspace{-0.3cm}(1)}{g_{\sigma\lambda}}
\right).
\label{eq2.31}
\end{align}
Substituting \eqref{eq2.31} into \eqref{eq2.29}
%\begin{align}
%&\overset{\hspace{-0.3cm}(0)}{g^{\mu\sigma}}\bigg(
%-\overset{\hspace{-0.6cm}(0)}{R^\lambda_{~\sigma\mu\delta}}\overset{\hspace{-0.3cm}(1)}{g_{\nu\lambda}}-\overset{\hspace{-0.6cm}(0)}{R^\lambda_{~\nu\mu\delta}}\overset{\hspace{-0.3cm}(1)}{g_{\sigma\lambda}}
% -\overset{\hspace{-0.6cm}(0)}{R^\lambda_{~\delta\mu\nu}}\overset{\hspace{-0.3cm}(1)}{g_{\sigma\lambda}}-\overset{\hspace{-0.6cm}(0)}{R^\lambda_{~\sigma\mu\nu}}\overset{\hspace{-0.3cm}(1)}{g_{\delta\lambda}}
%  \nonumber\\
%& \hspace{1cm}
% +\overset{\hspace{-0.7cm}(1)}{g_{\sigma\nu:\mu\delta}}
%+\overset{\hspace{-0.7cm}(1)}{g_{\delta\sigma:\mu\nu}}
%-\overset{\hspace{-0.7cm}(1)}{g_{\nu\delta:\sigma\mu}}
%-\overset{\hspace{-0.7cm}(1)}{g_{\mu\sigma:\nu\delta}}\bigg)
%=0,
%\label{eq2.47}
%\end{align}
%or
\begin{align}
&%\bigg(
-\overset{\hspace{-0.6cm}(0)}{R^\lambda_{~\sigma\mu\delta}}\overset{\hspace{-0.3cm}(1)}{g_{\nu\lambda}}\overset{\hspace{-0.3cm}(0)}{g^{\mu\sigma}}
-\overset{\hspace{-0.6cm}(0)}{R^\lambda_{~\nu\mu\delta}}\overset{\hspace{-0.3cm}(1)}{g^\mu_{~\lambda}}
-\overset{\hspace{-0.6cm}(0)}{R^\lambda_{~\delta\mu\nu}}\overset{\hspace{-0.3cm}(1)}{g^\mu_{~\lambda}}-\overset{\hspace{-0.6cm}(0)}{R^\lambda_{~\sigma\mu\nu}}\overset{\hspace{-0.3cm}(1)}{g_{\delta\lambda}}\overset{\hspace{-0.3cm}(0)}{g^{\mu\sigma}}
\nonumber\\
& 
+\overset{\hspace{-0.7cm}(1)}{g^\mu_{~\nu:\mu\delta}}
+\overset{\hspace{-0.7cm}(1)}{g^\mu_{~\delta:\mu\nu}}
-\overset{\hspace{-0.7cm}(1)}{g^{~~~\mu}_{\nu\delta:~\mu}}
-\overset{\hspace{-0.7cm}(1)}{g^\mu_{~\mu:\nu\delta}}
%\bigg)
=0,
\label{eq2.32}
\end{align}
or
\begin{align}
&%\bigg(
2\overset{\hspace{-0.6cm}(0)}{R^{}_{\lambda\nu\delta\mu}}\overset{\hspace{-0.3cm}(1)}{g^{\mu\lambda}}
+\overset{\hspace{-0.3cm}(0)}{R^{}_{\lambda\nu}}\overset{\hspace{-0.3cm}(1)}{g^{~\lambda}_{\delta~}}
+\overset{\hspace{-0.3cm}(0)}{R^{}_{\lambda\delta}}\overset{\hspace{-0.3cm}(1)}{g^{~\lambda}_{\nu~}}
+\overset{\hspace{-0.7cm}(1)}{g^\mu_{~\nu:\mu\delta}}
+\overset{\hspace{-0.7cm}(1)}{g^\mu_{~\delta:\mu\nu}}
-\overset{\hspace{-0.7cm}(1)}{g^{~~~\mu}_{\nu\delta:~\mu}}
-\overset{\hspace{-0.7cm}(1)}{g^\mu_{~\mu:\nu\delta}}
=0,
\label{eq2.33}
\end{align}
that is just the wave equation satisfied by the perturbation for an arbitrary background. 
\\Defining now a reverse trace tensor $h_{\mu\nu}$ as
\begin{equation}
h_{\mu\nu}=\overset{\hspace{-0.3cm}(1)}{g_{\mu\nu}}-\frac{1}{2}\overset{(1)}{g}\,\overset{\hspace{-0.3cm}(0)}{g_{\mu\nu}},
\label{eq2.34}
\end{equation}
then
%\begin{equation}
%h^\mu_{~\nu}=\overset{\hspace{-0.3cm}(1)}{g^\mu_{~\nu}}-\frac{1}{2}\overset{(1)}{g}\,\overset{\hspace{-0.3cm}(0)}{\delta^\mu_{~\nu}}
%\label{eq2.50}
%\end{equation}
contracting \eqref{eq2.34} it is founded $h=-\overset{(1)}{g}$, therefore
\begin{equation}
\overset{\hspace{-0.3cm}(1)}{g_{\mu\nu}}=h_{\mu\nu}-\frac{1}{2}h\,\overset{\hspace{-0.3cm}(0)}{g_{\mu\nu}}.
\label{eq2.35}
\end{equation}
Substituting \eqref{eq2.35} into \eqref{eq2.33} one obtains for $h_{\mu\nu}$
%\begin{align}
%&
%2\overset{\hspace{-0.6cm}(0)}{R^{}_{\lambda\nu\delta\mu}}h^{\mu\lambda}+\overset{\hspace{-0.3cm}(0)}{R_{\nu\delta}}h
%+\overset{\hspace{-0.3cm}(0)}{R^{}_{\lambda\nu}}h^{~\lambda}_{\delta~}-\frac{1}{2}\,\overset{\hspace{-0.3cm}(0)}{R^{}_{\delta\nu}}h
%+\overset{\hspace{-0.3cm}(0)}{R^{}_{\lambda\delta}} h^{~\lambda}_{\nu~}-\frac{1}{2}\overset{\hspace{-0.3cm}(0)}{R^{}_{\nu\delta}}h
%+h^\mu_{~\nu:\mu\delta}-\frac{1}{2}h_{:\nu\delta}\nonumber\\
%&+h^\mu_{~\delta:\mu\nu}-\frac{1}{2}h_{:\delta\nu}
%-h_{\nu\delta:~\mu}^{~~~\mu}-\frac{1}{2}h_{:~\mu}^{\,\,\mu}\,\overset{\hspace{-0.3cm}(0)}{g_{\nu\delta}}
%+{h_{:\nu\delta}}
%=0,
%\label{eq2.36a}
%\end{align}
%and simplifying
\begin{align}
&
2\overset{\hspace{-0.6cm}(0)}{R^{}_{\lambda\nu\delta\mu}}h^{\mu\lambda}
+\overset{\hspace{-0.3cm}(0)}{R^{}_{\lambda\nu}}h^{~\lambda}_{\delta~}
+\overset{\hspace{-0.3cm}(0)}{R^{}_{\lambda\delta}} h^{~\lambda}_{\nu~}
+h^\mu_{~\nu:\mu\delta}+h^\mu_{~\delta:\mu\nu}
-h_{\nu\delta:~\mu}^{~~~\mu}-\frac{1}{2}h_{:~\mu}^{\,\,\mu}\,\overset{\hspace{-0.3cm}(0)}{g_{\nu\delta}}
=0.
\label{eq2.36}
\end{align}
Under the transformation of coordinates
\begin{align}
\overline{x}^{\alpha}:=\overline{x}^{\alpha} (x^\beta),
\label{eq2.37}
\end{align}
the metric transforms as
\begin{align}
g^{\overline{\mu}\,\overline{\nu}}=g^{\mu\nu}\Delta^{\overline{\mu}}_{~\mu} \Delta^{\overline{\nu}}_{~\nu},
\label{eq2.38}
\end{align}
where $g^{\overline{\mu}\,\overline{\nu}}$ ($g^{\mu\nu}$) are referred to the $\overline{x}^{\alpha}$, $x^{\alpha}$ coordinates respectively and the transformation matrix  $\Delta^{\overline{\mu}}_{~\mu}$ is given in terms of partial derivatives
\begin{equation}
\Delta^{\overline{\mu}}_{~\mu}=x^{\overline{\mu}}_{~,\mu}.
\label{eq2.39}
\end{equation}
Also, from the transformation \eqref{eq2.38} and the perturbation \eqref{eq2.1}, it is observed that
\begin{equation*}
\overset{(0)}{g_{\overline{\mu}\,\overline{\nu}}}+\epsilon\overset{(1)}{g_{\overline{\mu}\,\overline{\nu}}}=\Delta^\mu_{~\overline{\mu}}\Delta^\nu_{~\overline{\nu}}\left(\overset{(0)}{g_{\mu\nu}}+\epsilon\overset{(1)}{g_{\mu\nu}}\right), 
\end{equation*}
which implies that the perturbation obeys the transformation rules for tensor under Lorentz transformation.
\begin{equation}
\overset{(1)}{g_{\overline{\mu}\,\overline{\nu}}}= \Delta^\mu_{~\overline{\mu}}\Delta^\nu_{~\overline{\nu}} \overset{(1)}{g_{\mu\nu}}.
\label{eq2.40}
\end{equation}
In particular, if it is considered an infinitesimal boost,
\begin{equation}
\overline{x}^a=x^a+\epsilon\, \zeta^a,
\label{eq2.41}
\end{equation}
where $|\epsilon \zeta^a|\ll |x^a|$ are infinitesimal displacements, then the matrices \eqref{eq2.31} become
\begin{equation}
\overline{x}^{\alpha}_{~,\beta}=\delta^\alpha_{~,\beta}+\epsilon\,\zeta^\alpha_{~,\beta}.
\label{eq2.42}
\end{equation}
Thus, substituting \eqref{eq2.42} into \eqref{eq2.40},
\begin{align}
g^{\overline{\mu}\,\overline{\nu}}(\overline{x}^\beta)
%&=g^{\mu\nu}(x^\alpha)\left(\delta^{\overline{\mu}}_{~\mu}+\epsilon\,\zeta^{\overline{\mu}}_{~,\mu}\right) \left(\delta^{\overline{\nu}}_{~\nu}+\epsilon\,\zeta^{\overline{\nu}}_{~,\nu}\right), \nonumber\\
%&=g^{\mu\nu}(x^\alpha)\left(\delta^{\overline{\mu}}_{~\mu}\delta^{\overline{\nu}}_{~\nu}+\epsilon\left(\delta^{\overline{\mu}}_{~\mu}\zeta^{\overline{\nu}}_{~,\nu} + \delta^{\overline{\nu}}_{~\nu}\zeta^{\overline{\mu}}_{~,\mu}\right)+\epsilon^2\zeta^{\overline{\nu}}_{~,\nu}\zeta^{\overline{\mu}}_{~,\mu}\right) \nonumber\\
&=g^{\overline{\mu}\,\overline{\nu}}(x^\alpha)+\epsilon\left(\overset{(1)}{g^{\overline{\mu}\,\nu}}\zeta^{\overline{\nu}}_{~,\nu} + \overset{(1)}{g^{\mu\,\overline{\nu}}}\zeta^{\overline{\mu}}_{~,\mu}\right)+O(\zeta^2),
\label{eq2.43}
\end{align}
expanding the metric around $\zeta$,
\begin{equation}
g^{\overline{\mu}\,\overline{\nu}}(x^\alpha)\simeq g^{\overline{\mu}\,\overline{\nu}}-\epsilon\,\zeta^\sigma g^{\overline{\mu}\,\overline{\nu}}_{~~~,\sigma},
\label{eq2.44}
\end{equation}
and substituting it into \eqref{eq2.43}
\begin{align}
g^{\overline{\mu}\,\overline{\nu}}(\overline{x}^\beta)&\simeq g^{\overline{\mu}\,\overline{\nu}}-\epsilon\left(\zeta^\sigma g^{\overline{\mu}\,\overline{\nu}}_{~~~,\sigma} - g^{\overline{\mu}\,\nu}\zeta^{\overline{\nu}}_{~,\nu} - g^{\mu\,\overline{\nu}}\zeta^{\overline{\mu}}_{~,\mu}\right).
\label{eq2.45}
\end{align}
Now, from the covariant derivative of the inverse metric,
%\begin{equation*}
%g^{\mu\nu}_{~~~;\delta}=g^{\mu\nu}_{~~~,\delta}+g^{\sigma\nu}\Gamma^\mu_{~\sigma\delta}+g^{\mu\sigma}\Gamma^\nu_{~\sigma\delta}
%\end{equation*}
%we obtain
\begin{equation}
g^{\mu\nu}_{~~~,\delta}=-g^{\sigma\nu}\Gamma^\mu_{~\sigma\delta}-g^{\mu\sigma}\Gamma^\nu_{~\sigma\delta}.
\label{eq2.46}
\end{equation}
Substituting \eqref{eq2.46} into \eqref{eq2.45}, 
\begin{align}
g^{\overline{\mu}\,\overline{\nu}}(\overline{x}^\beta)&\simeq g^{\overline{\mu}\,\overline{\nu}}(x^\beta)
+\epsilon\left(\zeta^\sigma g^{\overline{\mu}\,\eta}\Gamma^{\overline{\nu}}_{~\sigma\eta}+\zeta^\sigma g^{\eta\,\overline{\nu}}\Gamma^{\overline{\mu}}_{~\sigma\eta} 
+g^{\overline{\mu}\,\nu}\zeta^{\overline{\nu}}_{~,\nu} 
+ g^{\mu\,\overline{\nu}}\zeta^{\overline{\mu}}_{~,\mu}\right),\nonumber\\
&\simeq g^{\overline{\mu}\,\overline{\nu}}(x^\beta)
+\epsilon\left(g^{\overline{\mu}\,\nu}\left(\zeta^{\overline{\nu}}_{~,\nu}
+\zeta^\sigma \Gamma^{\overline{\nu}}_{~\sigma\nu}\right)
+ g^{\mu\,\overline{\nu}}\left(\zeta^{\overline{\mu}}_{~,\mu}
+\zeta^\sigma \Gamma^{\overline{\mu}}_{~\sigma\mu}\right)\right),\nonumber\\
&\simeq g^{\overline{\mu}\,\overline{\nu}}(x^\beta)
+2\,\epsilon\,\zeta^{(\overline{\nu}:\overline{\mu})},
%+\zeta^{\overline{\mu};\overline{\nu}}
\label{eq2.47}
\end{align}
where, the round brackets indicates symmetrisation, as usual. The symmetrisation is defined as
\begin{equation}
A_{(\alpha_1\cdot\alpha_n)}=\frac{1}{n!}\sum_{n} A_{\alpha_{\sigma_1}\cdot\alpha_{\sigma_n}},
\end{equation}
where the sum is performed over all indices permutation.
\\Thus, the metric is invariant under such transformation always that
\begin{equation}
\zeta_{(\nu:\mu)}=0.
\label{eq2.48}
\end{equation}
In which case, the $\zeta^\alpha$ are just the killing vectors associated with the background space-time.
\\Lowering the indices of \eqref{eq2.47} with the metric, and using \eqref{eq2.1} immediately is obtained one gauge condition for the perturbations,
\begin{equation}
\overset{\hspace{-0.3cm}(1)}{g_{\mu\nu}}(\overline{x}^\beta)=\overset{\hspace{-0.3cm}(1)}{g_{\mu\nu}}(x^\beta)+2\zeta_{(\nu:\mu)}.
\label{eq2.49}
\end{equation}
From this, it is obtained immediately
\begin{equation}
\overset{\hspace{-0.7cm}(1)}{\overline{g}_{\mu\nu}^{~~~:\mu}}=\overset{\hspace{-0.7cm}(1)}{g_{\mu\nu}^{~~~:\mu}}+2\zeta_{(\nu:\mu)}^{~~~~~\mu},
\label{eq2.50}
\end{equation}
where the overline in this case indicate the metric in the new coordinate system, i.e., $\overset{\hspace{-0.3cm}(1)}{\overline{g}_{\mu\nu}}=\overset{\hspace{-0.3cm}(1)}{g_{\mu\nu}}(\overline{x}^\alpha)$ which allows to impose that
\begin{equation}
\overset{\hspace{-0.7cm}(1)}{\overline{g}_{\mu\nu}^{~~~:\mu}}=0.
\label{eq2.51}
\end{equation}
This gauge is known as De Donder or Hilbert gauge.
\\Using \eqref{eq2.34}, it is found from \eqref{eq2.49}, the form for the gauge for $h_{\mu\nu}$,
\begin{align}
\overline{h}_{\mu\nu}
%&=\overset{\hspace{-0.3cm}(1)}{\overline{g}_{\mu\nu}}-\frac{1}{2}\overset{(1)}{\overline{g}}\,\overset{\hspace{-0.3cm}(0)}{g_{\mu\nu}},\nonumber\\
&=\overset{\hspace{-0.3cm}(1)}{g_{\mu\nu}}-\frac{1}{2}\overset{(1)}{g}\,\overset{\hspace{-0.3cm}(0)}{g_{\mu\nu}}+2\zeta_{(\nu:\mu)}-\zeta^\sigma_{~:\sigma}\,\overset{\hspace{-0.3cm}(0)}{g_{\mu\nu}},\nonumber\\
&=h_{\mu\nu}+2\zeta_{(\nu:\mu)}-\zeta^\sigma_{~:\sigma}\,\overset{\hspace{-0.3cm}(0)}{g_{\mu\nu}},
\label{eq2.52}
\end{align}
which implies that its trace is given by
\begin{align}
\overline{h}&=h+2\zeta^\mu_{~:\mu}-\zeta^\sigma_{~:\sigma}\,\delta^\mu_{~\mu},\nonumber\\
&=h-2\zeta^\mu_{~:\mu}.
\label{eq2.53}
\end{align}
Therefore, computing the covariant derivative of \eqref{eq2.52}
\begin{align}
\overline{h}_{\mu\nu:}^{~~~\nu}&=h_{\mu\nu:}^{~~~\nu}+2\,\zeta_{(\nu:\mu)}^{~~~~\,\nu}-\zeta^{\sigma~\nu}_{~:\sigma}\,\overset{\hspace{-0.3cm}(0)}{g_{\mu\nu}},\nonumber\\
&=h_{\mu\nu:}^{~~~\nu}+2\,\zeta_{(\nu:\mu)}^{~~~~\,\nu}-\zeta^{\sigma}_{~:\sigma\mu},\nonumber\\
&=h_{\mu\nu:}^{~~~\nu}+\zeta_{\mu:~\nu}^{~\,\nu}+2\,\zeta^{\sigma}_{~:[\sigma\mu]}.
\label{eq2.54}
\end{align}
Taking into account that
\begin{align}
2\,\zeta^{\sigma}_{~:[\sigma\mu]}&=\overset{\hspace{-0.5cm}(0)}{R^\sigma_{\lambda\sigma\mu}}\zeta^\lambda,\nonumber\\
&=\overset{\hspace{-0.3cm}(0)}{R_{\lambda\mu}}\zeta^\lambda,
\label{eq2.55}
\end{align}
then,
\begin{align}
\overline{h}_{\mu\nu:}^{~~~\nu}
%&=h_{\mu\nu:}^{~~~\nu}+2\,\zeta_{(\nu:\mu)}^{~~~~\,\nu}-\zeta^{\sigma~\nu}_{~:\sigma}\,\overset{\hspace{-0.3cm}(0)}{g_{\mu\nu}}\nonumber\\
%&=h_{\mu\nu:}^{~~~\nu}+2\,\zeta_{(\nu:\mu)}^{~~~~\,\nu}-\zeta^{\sigma}_{~:\sigma\mu}\nonumber\\
&=h_{\mu\nu:}^{~~~\nu}+\zeta_{\mu:~\nu}^{~\,\nu}+\overset{\hspace{-0.3cm}(0)}{R_{\lambda\mu}}\zeta^\lambda.
\label{eq2.56}
\end{align}
Thus, \eqref{eq2.53} and \eqref{eq2.56} can be re-written as
\begin{equation}
h_{\mu\nu:}^{~~~\nu}=\overline{h}_{\mu\nu:}^{~~~\nu}-\zeta_{\mu:~\nu}^{~\,\nu}-\overset{\hspace{-0.3cm}(0)}{R_{\lambda\mu}}\zeta^\lambda,\hspace{0.5cm}h=\overline{h}+2\zeta^\mu_{~:\mu},
\label{eq2.57}
\end{equation}
meaning that the tensor field $h_{\mu\nu}$ can be recalibrated making the selection
\begin{align}
h=0, \hspace{0.5cm}h_{\mu\nu:}^{~~~\nu}=0,
\label{eq2.58}
\end{align}
if the following conditions are met,
\begin{align}
\overline{h}_{\mu\nu:}^{~~~\nu}=\zeta_{\mu:~\nu}^{~\,\nu}+\overset{\hspace{-0.3cm}(0)}{R_{\lambda\mu}}\zeta^\lambda, \hspace{0.5cm}\overline{h}=-2\zeta^\mu_{~:\mu}.
\label{eq2.59}
\end{align}
Substituting \eqref{eq2.58} into \eqref{eq2.36}, it is obtained
\begin{align}
&
2\overset{\hspace{-0.6cm}(0)}{R^{}_{\lambda\nu\delta\mu}}h^{\mu\lambda}
+\overset{\hspace{-0.3cm}(0)}{R^{}_{\lambda\nu}}h^{~\lambda}_{\delta~}
+\overset{\hspace{-0.3cm}(0)}{R^{}_{\lambda\delta}} h^{~\lambda}_{\nu~}
-h_{\nu\delta:~\mu}^{~~~\mu}
=0.
\label{eq2.60}
\end{align}
%
%
%
%
%
%
%
%
%
%\vspace{10cm}
%\\
% In that case, the wave equation \eqref{eq2.27} is reduced to
%\begin{equation}
%\overset{\hspace{-0.7cm}(1)}{g^{\mu}_{~~\delta|\nu\mu}} -\overset{\hspace{-0.7cm}(1)}{g^{~~~\mu}_{\nu\delta|~~\mu}}
%-\overset{\hspace{-0.7cm}(1)}{g^\mu_{~\mu|\nu\delta}}  =0,
%%\label{eq2.43}
%\end{equation}
%Also noting that
%\begin{align*}
%\overset{\hspace{-0.7cm}(1)}{g^{\mu}_{~~\delta|\nu\mu}}&=2\overset{\hspace{-0.9cm}(1)}{g^{\mu}_{~~\delta|[\nu\mu]}}-\overset{\hspace{-0.7cm}(1)}{g^{\mu}_{~~\delta|\mu\nu}}\nonumber\\
%&=2\overset{\hspace{-0.9cm}(1)}{g^{\mu}_{~~\delta|[\nu\mu]}}
%\end{align*}
%and that
%\begin{equation*}
%\overset{\hspace{-0.8cm}(1)}{g^{\mu}_{~~\delta|\nu\mu}}=\overset{\hspace{-0.3cm}(0)}{g_{\delta\sigma}}\overset{\hspace{-0.8cm}(1)}{g^{\mu\sigma}_{~~~|\nu\mu}}
%\end{equation*}
%then \eqref{eq2.43} takes the form
%\begin{equation}
%2\overset{\hspace{-0.3cm}(0)}{g_{\delta\sigma}}\overset{\hspace{-0.9cm}(1)}{g^{\mu\sigma}_{~~~|[\nu\mu]}} -\overset{\hspace{-0.7cm}(1)}{g^{~~~\mu}_{\nu\delta|~~\mu}}
%-\overset{\hspace{-0.7cm}(1)}{g^\mu_{~\mu|\nu\delta}}  =0.
%%\label{eq2.44}
%\end{equation}
%Now, observing that 
%\begin{align}
%\overset{\hspace{-0.9cm}(1)}{g^{\mu\sigma}_{~~~|[\nu\gamma]}}
%&=\overset{\hspace{-0.9cm}(1)}{g^{\mu\sigma}_{~~~,[\nu|\gamma]}}
%+2\overset{\hspace{-1.0cm}(0)}{\Gamma^{(\mu}_{~~\zeta[\nu|\gamma]}}\overset{\hspace{-0.4cm}(1)}{g^{\sigma)\zeta}}
%+2\overset{\hspace{-0.7cm}(0)}{\Gamma^{(\mu}_{~~\zeta[\nu}}\overset{\hspace{-0.7cm}(1)}{g^{\sigma)\zeta}_{~~~|\gamma]}}
%%+\overset{(0)}{\Gamma^\sigma_{~~\zeta[\nu|\gamma]}}\overset{(1)}{g^{\mu\zeta}}
%%+\overset{(0)}{\Gamma^\sigma_{~~\zeta[\nu}}\overset{(1)}{g^{\mu\zeta}_{~~~|\gamma]}}
%%\label{eq2.45}
%\end{align}
%where
%%\begin{align}
%%\overset{(1)}{g^{\mu\sigma}_{~~~,[\nu|\gamma]}}&=
%%\overset{(1)}{g^{\mu\sigma}_{~~~,[\nu\gamma]}}
%%+\overset{(0)}{\Gamma^\mu_{~~\zeta[\gamma}}\overset{(1)}{g^{\zeta\sigma}_{~~~,\nu]}} +\overset{(0)}{\Gamma^\sigma_{~~\zeta[\gamma}}\overset{(1)}{g^{\mu\zeta}_{~~~,\nu]}}
%%-\overset{(0)}{\Gamma^\zeta_{~~[\nu\gamma]}}g^{\mu\sigma}_{~~~,\zeta}\nonumber\\
%%&=\overset{(0)}{\Gamma^\mu_{~~\zeta[\gamma}}\overset{(1)}{g^{\zeta\sigma}_{~~~,\nu]}} +\overset{(0)}{\Gamma^\sigma_{~~\zeta[\gamma}} \overset{(1)}{g^{\mu\zeta}_{~~~,\nu]}},
%%\end{align}
%\begin{align}
%\overset{\hspace{-0.9cm}(1)}{g^{\mu\sigma}_{~~,[\nu|\gamma]}}&=
%\overset{\hspace{-0.9cm}(1)}{g^{\mu\sigma}_{~~,[\nu\gamma]}}
%+2\overset{\hspace{-0.7cm}(0)}{\Gamma^{(\mu}_{~~\zeta[\gamma}}\overset{\hspace{-0.7cm}(1)}{g^{\sigma)\zeta}_{~~~,\nu]}} 
%-\overset{\hspace{-0.7cm}(0)}{\Gamma^\zeta_{~[\nu\gamma]}}\overset{\hspace{-0.5cm}(1)}{g^{\mu\sigma}_{~~,\zeta}}\nonumber\\
%&=2\overset{\hspace{-0.7cm}(0)}{\Gamma^{(\mu}_{~~\zeta[\gamma}}\overset{\hspace{-0.7cm}(1)}{g^{\sigma)\zeta}_{~~~,\nu]}},
%%\label{eq2.46}
%\end{align}
%and
%%\begin{align}
%%\overset{(0)}{\Gamma^\mu_{~~\zeta[\nu|\gamma]}}\overset{(1)}{g^{\zeta\sigma}}&=\left(\overset{(0)}{\Gamma^\mu_{~~\zeta[\nu,\gamma]}}+\overset{(0)}{\Gamma^\mu_{~~\eta[\gamma}}\overset{(0)}{\Gamma^\eta_{~~\nu]\zeta}}-\overset{(0)}{\Gamma^\eta_{~~\zeta[\gamma}}\overset{(0)}{\Gamma^\mu_{~~\nu]\eta}}-\overset{(0)}{\Gamma^\eta_{~~[\nu\gamma]}}\overset{(0)}{\Gamma^\mu_{~~\zeta\eta}}\right)\overset{(1)}{g^{\zeta\sigma}}\nonumber\\
%%&=\left(\overset{(0)}{R^\mu_{~~\zeta\gamma\nu}}-\overset{(0)}{\Gamma^\eta_{~~\zeta[\gamma}}\overset{(0)}{\Gamma^\mu_{~~\nu]\eta}}\right)\overset{(1)}{g^{\zeta\sigma}}
%%\end{align}
%\begin{align}
%\overset{\hspace{-1cm}(0)}{\Gamma^{(\mu}_{~~\zeta[\nu|\gamma]}}\overset{\hspace{-0.5cm}(1)}{g^{\sigma)\zeta}}&=
%\overset{\hspace{-1cm}(0)}{\Gamma^{(\mu}_{~~\zeta[\nu,\gamma]}}\overset{\hspace{-0.5cm}(1)}{g^{\sigma)\zeta}}
%+\overset{\hspace{-0.5cm}(1)}{g^{\zeta(\sigma}}\overset{\hspace{-0.8cm}(0)}{\Gamma^{\mu)}_{~~\eta[\gamma}}\overset{\hspace{-0.7cm}(0)}{\Gamma^\eta_{~\nu]\zeta}}
%-\overset{\hspace{-0.7cm}(0)}{\Gamma^\eta_{~\zeta[\gamma}}\overset{\hspace{-0.8cm}(0)}{\Gamma^{(\mu}_{~~\nu]\eta}}\overset{\hspace{-0.5cm}(1)}{g^{\sigma)\zeta}}
%-\overset{\hspace{-0.9cm}(0)}{\Gamma^\eta_{~[\nu\gamma]}}\overset{\hspace{-0.7cm}(0)}{\Gamma^{(\mu}_{~~\zeta\eta}}\overset{\hspace{-0.5cm}(1)}{g^{\sigma)\zeta}}\nonumber\\
%&=\overset{\hspace{-0.7cm}(0)}{R^{(\mu}_{~~\zeta\gamma\nu}}\overset{\hspace{-0.5cm}(1)}{g^{\sigma)\zeta}}
%-\overset{\hspace{-0.7cm}(0)}{\Gamma^\eta_{~\zeta[\gamma}}\overset{\hspace{-0.7cm}(0)}{\Gamma^{(\mu}_{~\nu]\eta}}\overset{\hspace{-0.5cm}(1)}{g^{\sigma)\zeta}}
%%\label{eq2.47}
%\end{align}
%and
%\begin{align}
%\overset{\hspace{-0.7cm}(0)}{\Gamma^{(\mu}_{~~\zeta[\nu}}\overset{\hspace{-0.7cm}(1)}{g^{\sigma)\zeta}_{~~~|\gamma]}}=
%\overset{\hspace{-0.7cm}(0)}{\Gamma^{(\mu}_{~~\zeta[\nu}}\overset{\hspace{-0.7cm}(1)}{g^{\sigma)\zeta}_{~~~,\gamma]}}
%+\overset{\hspace{-0.7cm}(0)}{\Gamma^{(\mu}_{~~\zeta[\nu}}\overset{\hspace{-0.7cm}(0)}{\Gamma^{\sigma)}_{~~\gamma]\eta}}\overset{\hspace{-0.3cm}(1)}{g^{\eta\zeta}}
%+\overset{\hspace{-0.5cm}(0)}{\Gamma^{\zeta}_{~\eta[\gamma}}\overset{\hspace{-0.7cm}(0)}{\Gamma^{(\mu}_{~~\nu]\zeta}}\overset{\hspace{-0.5cm}(1)}{g^{\sigma)\eta}}
%%\label{eq2.48}
%\end{align}
%%\begin{align}
%%\overset{(0)}{\Gamma^\mu_{~~\zeta[\nu}}\overset{(1)}{g^{\zeta\sigma}_{~~~|\gamma]}}&=\overset{(0)}{\Gamma^\mu_{~~\zeta[\nu}}\overset{(1)}{g^{\zeta\sigma}_{~~~,\gamma]}}+\overset{(0)}{\Gamma^\mu_{~~\zeta[\nu}}\overset{(0)}{\Gamma^{\zeta}_{~~\gamma]\eta}}\overset{(1)}{g^{\eta\sigma}}+\overset{(0)}{\Gamma^\mu_{~~\zeta[\nu}}\overset{(0)}{\Gamma^{\sigma}_{~~\gamma]\eta}}\overset{(1)}{g^{\zeta\eta}}
%%\end{align}
%Substituting, \eqref{eq2.46}-\eqref{eq2.48} into \eqref{eq2.45}
%\begin{align*}
%\overset{(1)}{g^{\mu\sigma}_{~~~|[\nu\gamma]}}=& 2\overset{\hspace{-0.7cm}(0)}{\Gamma^{(\mu}_{~~\zeta[\gamma}}\overset{\hspace{-0.7cm}(1)}{g^{\sigma)\zeta}_{~~~,\nu]}} 
%+ 2\overset{\hspace{-0.7cm}(0)}{R^{(\mu}_{~~\zeta\gamma\nu}}\overset{\hspace{-0.5cm}(1)}{g^{\sigma)\zeta}}
%-2\overset{\hspace{-0.7cm}(0)}{\Gamma^\eta_{~\zeta[\gamma}}\overset{\hspace{-0.7cm}(0)}{\Gamma^{(\mu}_{~\nu]\eta}}\overset{\hspace{-0.5cm}(1)}{g^{\sigma)\zeta}}\\
%&+2\overset{\hspace{-0.7cm}(0)}{\Gamma^{(\mu}_{~~\zeta[\nu}}\overset{\hspace{-0.7cm}(1)}{g^{\sigma)\zeta}_{~~~,\gamma]}}
%+2\overset{\hspace{-0.7cm}(0)}{\Gamma^{(\mu}_{~~\zeta[\nu}}\overset{\hspace{-0.7cm}(0)}{\Gamma^{\sigma)}_{~~\gamma]\eta}}\overset{\hspace{-0.3cm}(1)}{g^{\eta\zeta}}
%+2\overset{\hspace{-0.5cm}(0)}{\Gamma^{\zeta}_{~\eta[\gamma}}\overset{\hspace{-0.7cm}(0)}{\Gamma^{(\mu}_{~~\nu]\zeta}}\overset{\hspace{-0.5cm}(1)}{g^{\sigma)\eta}}\\
%=&  
%2\overset{\hspace{-0.7cm}(0)}{R^{(\mu}_{~~\zeta\gamma\nu}}\overset{\hspace{-0.5cm}(1)}{g^{\sigma)\zeta}}
%+2\overset{\hspace{-0.7cm}(0)}{\Gamma^{(\mu}_{~~\zeta[\nu}}\overset{\hspace{-0.7cm}(0)}{\Gamma^{\sigma)}_{~~\gamma]\eta}}\overset{\hspace{-0.3cm}(1)}{g^{\eta\zeta}}
%\end{align*}
%where, 
%\begin{align*}
%\overset{\hspace{-0.7cm}(0)}{\Gamma^{(\mu}_{~~\zeta[\nu}}\overset{\hspace{-0.7cm}(0)}{\Gamma^{\sigma)}_{~~\gamma]\eta}}\overset{\hspace{-0.3cm}(1)}{g^{\eta\zeta}}&=
%\frac{1}{4}\left(\overset{\hspace{-0.7cm}(0)}{\Gamma^{\mu}_{~~\zeta\nu}}\overset{\hspace{-0.7cm}(0)}{\Gamma^{\sigma}_{~~\gamma\eta}}\overset{\hspace{-0.3cm}(1)}{g^{\eta\zeta}}
%-\overset{\hspace{-0.7cm}(0)}{\Gamma^{\mu}_{~~\zeta\gamma}}\overset{\hspace{-0.7cm}(0)}{\Gamma^{\sigma}_{~~\nu\eta}}\overset{\hspace{-0.3cm}(1)}{g^{\eta\zeta}}\right.\\
%&\left.\hspace{1cm}+\overset{\hspace{-0.7cm}(0)}{\Gamma^{\sigma}_{~~\zeta\nu}}\overset{\hspace{-0.7cm}(0)}{\Gamma^{\mu}_{~~\gamma\eta}}\overset{\hspace{-0.3cm}(1)}{g^{\eta\zeta}}
%-\overset{\hspace{-0.7cm}(0)}{\Gamma^{\sigma}_{~~\zeta\gamma}}\overset{\hspace{-0.7cm}(0)}{\Gamma^{\mu}_{~~\nu\eta}}\overset{\hspace{-0.3cm}(1)}{g^{\eta\zeta}}\right)\\
%&=0
%\end{align*}
%Therefore, \eqref{eq2.44} 
%\begin{equation}
%4\overset{\hspace{-0.3cm}(0)}{g_{\delta\sigma}}\overset{\hspace{-0.7cm}(0)}{R^{(\mu}_{~~\zeta\mu\nu}}\overset{\hspace{-0.5cm}(1)}{g^{\sigma)\zeta}} -\overset{\hspace{-0.7cm}(1)}{g^{~~~\mu}_{\nu\delta|~~\mu}}
%-\overset{\hspace{-0.7cm}(1)}{g^\mu_{~\mu|\nu\delta}}  =0.
%%\label{eq2.49}
%\end{equation}
%Defining now
%\begin{equation}
%\overline{g}_{\mu\nu}=\overset{\hspace{-0.3cm}(1)}{g_{\mu\nu}}-\frac{1}{2}\overset{\hspace{-0.3cm}(0)}{g_{\mu\nu}}\overset{(1)}{g}
%\end{equation}
%then
%\begin{equation}
%\overline{g}^{\mu}_{~\nu}=\overset{\hspace{-0.3cm}(1)}{g^{\mu}_{~\nu}}-\frac{1}{2}{\delta^{\mu}_{~\nu}}\overset{(1)}{g}
%\end{equation}
%contracting
%\begin{align}
%\overline{g}%&=\overset{(1)}{g}-2\overset{(1)}{g}\nonumber\\
%&=-\overset{(1)}{g}
%\end{align}
%Thus,
%\begin{equation}
%\overset{\hspace{-0.3cm}(1)}{g_{\mu\nu}}=\overline{g}_{\mu\nu}-\frac{1}{2}\overset{\hspace{-0.3cm}(0)}{g_{\mu\nu}}\overline{g}
%\end{equation}
%Observing that \eqref{eq2.49} is
%\begin{align*}
%\overset{\hspace{-0.7cm}(1)}{g^{~~~\mu}_{\nu\delta|~~\mu}}
%+\overset{\hspace{-0.7cm}(1)}{g^\mu_{~\mu|\nu\delta}}  &=
%2\overset{\hspace{-0.3cm}(0)}{g_{\delta\sigma}}\overset{\hspace{-0.7cm}(0)}{R^{\mu}_{~\zeta\mu\nu}}\overset{\hspace{-0.3cm}(1)}{g^{\sigma\zeta}}
%+2\overset{\hspace{-0.3cm}(0)}{g_{\delta\sigma}}\overset{\hspace{-0.7cm}(0)}{R^{\sigma}_{~\zeta\mu\nu}}\overset{\hspace{-0.3cm}(1)}{g^{\mu\zeta}}\\
%&=
%2\overset{\hspace{-0.3cm}(0)}{g_{\delta\sigma}}\overset{\hspace{-0.3cm}(0)}{R_{\zeta\nu}}\overset{\hspace{-0.3cm}(1)}{g^{\sigma\zeta}}
%+2\overset{\hspace{-0.7cm}(0)}{R_{\delta\zeta\mu\nu}}\overset{\hspace{-0.3cm}(1)}{g^{\mu\zeta}}.
%%\label{eq2.50}
%\end{align*}
%Substituting it into \eqref{eq2.49}
%\begin{equation}
%\overline{g}^{~~~\mu}_{\nu\delta|~~\mu}-\frac{1}{2}\,\overset{\hspace{-0.3cm}(0)}{g_{\nu\delta}}\,\overline{g}^{~\mu}_{|~~\mu}
%+\overline{g}_{|\nu\delta}  = 2\overset{\hspace{-0.3cm}(0)}{g_{\delta\sigma}}\overset{\hspace{-0.3cm}(0)}{R_{\zeta\nu}}\overline{g}^{\sigma\zeta}
%-\overset{\hspace{-0.3cm}(0)}{R_{\delta\nu}}\overline{g}
%+2\overset{\hspace{-0.5cm}(0)}{R_{\delta\zeta\mu\nu}}\overline{g}^{\mu\zeta}
%-\overset{\hspace{-0.5cm}(0)}{R_{\delta\zeta\mu\nu}}\overline{g}\overset{\hspace{-0.3cm}(0)}{g^{\mu\zeta}}.
%%\label{eq2.50}
%\end{equation}
%and assuming that the $\overline{g}_{\mu\nu}$ is trace-free, i.e., $\overline{g}=0$, then
%\begin{equation}
%\overline{g}^{~~~\mu}_{\nu\delta|~~\mu}
%%-\frac{1}{2}\,\overset{\hspace{-0.3cm}(0)}{g_{\nu\delta}}\,\overline{g}^{~\mu}_{|~~\mu}
%%+\overline{g}_{|\nu\delta}  
%= 2\overset{\hspace{-0.3cm}(0)}{g_{\delta\sigma}}\overset{\hspace{-0.3cm}(0)}{R_{\zeta\nu}}\overline{g}^{\sigma\zeta}
%%-\overset{\hspace{-0.3cm}(0)}{R_{\delta\nu}}\overline{g}
%+2\overset{\hspace{-0.5cm}(0)}{R_{\delta\zeta\mu\nu}}\overline{g}^{\mu\zeta}
%%-\overset{\hspace{-0.5cm}(0)}{R_{\delta\zeta\mu\nu}}\overline{g}\overset{\hspace{-0.3cm}(0)}{g^{\mu\zeta}}.
%%\label{eq2.50}
%\end{equation}
%%\\The relation \eqref{eq2.40} is a gauge transformation for which the Riemann tensor and consequently the field equations still invariant. From \eqref{eq2.22},
%%\begin{align}
%%\overset{(1)}{R^\mu_{~~\nu\gamma\delta}}(\overline{x}^\alpha)=
%%&\frac{1}{2}\left(
%%\left(g^\mu_{~\delta}+\zeta^\mu_{~~|\delta}+\zeta_{\delta|}^{~~\mu}\right)_{|\nu\gamma} -\left(g_{\nu\delta}+\zeta_{\nu|\delta}+\zeta_{\delta|\nu}\right)^{~\mu}_{|~~\gamma} \right.\nonumber\\
%%&\left.-\left(g^\mu_{~\gamma}+\zeta^\mu_{~~|\gamma}+\zeta_{\gamma|}^{~~\mu}\right)_{|\nu\delta} 
%%+\left(g_{\nu\gamma}+\zeta_{\nu|\gamma}+\zeta_{\gamma|\nu}\right)^{~\mu}_{|~~\delta}
%%\right)\nonumber\\
%%=
%%&\frac{1}{2}\left(
%%g^\mu_{~\delta|\nu\gamma} -g_{\nu\delta|~~\gamma}^{~~~\mu} -g^\mu_{~\gamma|\nu\delta} +g_{\nu\gamma|~~\delta}^{~~~\mu}
%%\right)\nonumber\\
%%&+\frac{1}{2}\left(
%%\zeta^\mu_{~~|\delta\nu\gamma}+\zeta_{\delta|~~\nu\gamma}^{~~\mu} -\zeta_{\nu|\delta~~\gamma}^{~~~\mu}-\zeta_{\delta|\nu~~\gamma}^{~~~\mu} \right.\nonumber\\
%%&\left.-\left(\zeta^\mu_{~~|\gamma\nu\delta}+\zeta_{\gamma|~~\nu\delta}^{~~\mu}\right)
%%+\left(\zeta_{\nu|\gamma~~\delta}^{~~~\mu}+\zeta_{\gamma|\nu~~\delta}^{~~~\mu}\right)
%%\right)%\nonumber\\
%%\label{eq2.41}
%%\end{align}
%%\begin{align}
%%\overset{(1)}{R^\mu_{~~\nu\gamma\delta}}=
%%&\frac{1}{2}\left(
%%\overset{(1)}{g^\mu_{~\delta|\nu\gamma}} -\overset{(1)}{g^{~~~\mu}_{\nu\delta|~~\gamma}}
%%-
%%\overset{(1)}{g^\mu_{~\gamma|\nu\delta}} 
%%+\overset{(1)}{g^{~~~\mu}_{\nu\gamma|~~\delta}}
%%\right).
%%%\label{eq2.22}
%%\end{align}
%%We must note that
%%\begin{equation}
%%\zeta_{\mu|\nu}=\zeta_{\mu,\nu}-\Gamma^\sigma_{~\mu\nu}\zeta_\sigma
%%\end{equation}
%%then
%%\begin{align*}
%%\zeta_{\mu|\nu\delta}=&\zeta_{\mu,\nu|\delta}-\left(\Gamma^\sigma_{~\mu\nu}\zeta_\sigma\right)_{|\delta}\\
%%=&\zeta_{\mu,\nu\delta}-\zeta_{\mu,\sigma}\Gamma^\sigma_{~\nu\delta}-\zeta_{\sigma,\nu}\Gamma^\sigma_{~\mu\delta}-\left(\Gamma^\sigma_{~\mu\nu}\zeta_\sigma\right)_{|\delta}\\
%%=&\zeta_{\mu,\nu\delta}-\zeta_{\mu,\sigma}\Gamma^\sigma_{~\nu\delta}-\zeta_{\sigma,\nu}\Gamma^\sigma_{~\mu\delta}-\Gamma^\sigma_{~\mu\nu|\delta}\zeta_{\sigma}-\Gamma^\sigma_{~\mu\nu}\zeta_{\sigma|\delta}\\
%%=&\zeta_{\mu,\nu\delta}-\zeta_{\mu,\sigma}\Gamma^\sigma_{~\nu\delta}-\zeta_{\sigma,\nu}\Gamma^\sigma_{~\mu\delta}-\left(\Gamma^\sigma_{~\mu\nu,\delta}+\Gamma^\epsilon_{~\mu\nu}\Gamma^\sigma_{~\epsilon\delta}-\Gamma^\sigma_{~\epsilon\nu}\Gamma^\epsilon_{~\mu\delta}-\Gamma^\sigma_{~\mu\epsilon}\Gamma^\epsilon_{~\nu\delta}\right)\zeta_{\sigma}\\
%%&-\Gamma^\sigma_{~\mu\nu}\left(\zeta_{\sigma,\delta}-\zeta_{\eta}\Gamma^\eta_{~\sigma\delta }\right)
%%\end{align*}
%%Thus,
%%\begin{align*}
%%\zeta_{\mu|\delta\nu}=&\zeta_{\mu,\delta\nu}-\zeta_{\mu,\sigma}\Gamma^\sigma_{~\delta\nu}-\zeta_{\sigma,\delta}\Gamma^\sigma_{~\mu\nu}-\left(\Gamma^\sigma_{~\mu\delta,\nu}+\Gamma^\epsilon_{~\mu\delta}\Gamma^\sigma_{~\epsilon\nu}-\Gamma^\sigma_{~\epsilon\delta}\Gamma^\epsilon_{~\mu\nu}-\Gamma^\sigma_{~\mu\epsilon}\Gamma^\epsilon_{~\delta\nu}\right)\zeta_{\sigma}\\
%%&-\Gamma^\sigma_{~\mu\delta}\left(\zeta_{\sigma,\nu}-\zeta_{\eta}\Gamma^\eta_{~\sigma\nu }\right)
%%\end{align*}
%%\begin{align*}
%%\zeta_{\mu|\nu\delta}-\zeta_{\mu|\delta\nu}=&-\left(\zeta_{\sigma,\nu}\Gamma^\sigma_{~\mu\delta}-\zeta_{\sigma,\delta}\Gamma^\sigma_{~\mu\nu}\right)
%%\end{align*}
%
%%\\Defining now the quantity
%%\begin{equation}
%%\overset{(1)}{g_{\mu\nu}}^{TT}=\overset{(1)}{g_{\mu\nu}}-\frac{1}{2}\overset{(0)}{g_{\mu\nu}}\overset{(1)}{g}
%%\label{eq2.41}
%%\end{equation}

==> docs/high_order_perturbations.tex <==
\section{Higher Order Perturbations}
In this point, the question on how is the form of the higher order perturbations to the Ricci's tensor is raised. Different approximations can be made considering different expansions for the metric $g_{\mu\nu}$ or for the inverse metric $g^{\mu\nu}$. The perturbation method can vary depending on which quantity is expanded and how it is done. In particular \citeonline{I68_1} shows the Ricci's tensor for higher order perturbation, expanding only the inverse metric $g^{\mu\nu}$; however, other perturbation schemes were explored with interesting results, for example \citeonline{B69}, expands the metric and its inverse supposing {\it ab initio} that both quantities depends on two parameters, a frequency and a phase, which leaves to different versions of the perturbed Ricci tensor. 
As a starting point, the procedure exposed by \citeonline{I68_1} is followed. Thus, the metric is expanded as 
\begin{equation}
g_{\mu\nu}=\overset{\hspace{-0.3cm}(0)}{g_{\mu\nu}}
+\epsilon\, \overset{\hspace{-0.3cm}(1)}{g_{\mu\nu}},
%+\sum_{i=1}^n \epsilon^i\,\overset{\hspace{-0.3cm}(i)}{g_{\mu\nu}}+O(\epsilon^{n+1}),
\label{eq2.2.1}
\end{equation}
%in \eqref{eq2.1} 
whereas its inverse metric, $g^{\mu\nu}$, is expanded as%in a power series containing perturbation of different orders, 
%where $\epsilon\ll 1$. Whereas, it is considered the inverse metric as
\begin{equation}
g^{\mu\nu}=\overset{\hspace{-0.3cm}(0)}{g^{\mu\nu}}+\sum_{i=1}^{n}\epsilon^i\,\overset{\hspace{-0.3cm}(i)}{g^{\mu\nu}}+O(\epsilon^{n+1}).
\label{eq2.2.2}
\end{equation}
Thus, from \eqref{eq2.2.1} and \eqref{eq2.2.2} 
\begin{equation}
g_{\mu\nu}g^{\nu\delta}=\overset{\hspace{-0.3cm}(0)}{g_{\mu\nu}}\overset{\hspace{-0.3cm}(0)}{g^{\nu\delta}}+\sum_{i=1}^{n}\epsilon^i\left(\,\overset{\hspace{-0.3cm}(0)}{g_{\mu\nu}}\overset{\hspace{-0.3cm}(i)}{g^{\nu\delta}}+\overset{\hspace{-0.3cm}(1)}{g_{\mu\nu}} \ \overset{\hspace{-0.1cm}(i-1)}{g^{\nu\delta}}\right)+O(\epsilon^{n+1}),
\label{eq2.2.3}
\end{equation}
which implies 
\begin{equation}
\overset{\hspace{-0.3cm}(i)}{g^{\zeta\delta}}=-\overset{\hspace{-0.3cm}(1)}{g_{\mu\nu}}\ \overset{\hspace{-0.3cm}(0)}{g^{\mu\zeta}}\ \overset{\hspace{-0.1cm}(i-1)}{g^{\nu\delta}},\hspace{1cm}i=1,2,\cdots
\label{eq2.2.4}
\end{equation}
Then, 
\begin{equation}
\overset{\hspace{-0.3cm}(1)}{g^{\zeta\delta}}=-\overset{\hspace{-0.3cm}(1)}{g_{\mu\nu}}\ \overset{\hspace{-0.3cm}(0)}{g^{\mu\zeta}}\ \overset{\hspace{-0.3cm}(0)}{g^{\nu\delta}},\hspace{0.5cm}
\overset{\hspace{-0.3cm}(2)}{g^{\zeta\delta}}=-\overset{\hspace{-0.3cm}(1)}{g_{\mu\nu}}\ \overset{\hspace{-0.3cm}(0)}{g^{\mu\zeta}}\ \overset{\hspace{-0.3cm}(1)}{g^{\nu\delta}},\hspace{0.5cm}\overset{\hspace{-0.3cm}(3)}{g^{\zeta\delta}}=-\overset{\hspace{-0.3cm}(1)}{g_{\mu\nu}}\ \overset{\hspace{-0.3cm}(0)}{g^{\mu\zeta}}\ \overset{\hspace{-0.3cm}(2)}{g^{\nu\delta}}, \hspace{0.5cm}\cdots
\label{eq2.2.5}
\end{equation}
Substituting recursively the last equations, it is found
\begin{align}
&\overset{\hspace{-0.3cm}(1)}{g^{\zeta\delta}}=-\overset{\hspace{-0.3cm}(1)}{g_{\mu\nu}}\ \overset{\hspace{-0.3cm}(0)}{g^{\mu\zeta}}\ \overset{\hspace{-0.3cm}(0)}{g^{\nu\delta}},
\hspace{1cm}
\overset{\hspace{-0.3cm}(2)}{g^{\zeta\delta}}=\overset{\hspace{-0.3cm}(1)}{g_{\mu\nu}} \ \overset{\hspace{-0.3cm}(1)}{g_{\alpha\beta}}\ \overset{\hspace{-0.3cm}(0)}{g^{\mu\zeta}}\ \overset{\hspace{-0.3cm}(0)}{g^{\alpha\nu}} \overset{\hspace{-0.3cm}(0)}{g^{\beta\delta}},
\hspace{1cm}\nonumber
\\
&\overset{\hspace{-0.3cm}(3)}{g^{\zeta\delta}}=-\overset{\hspace{-0.3cm}(1)}{g_{\mu\nu}}\ \overset{\hspace{-0.3cm}(1)}{g_{\alpha\beta}}\ \overset{\hspace{-0.3cm}(1)}{g_{\gamma\eta}}\ \overset{\hspace{-0.3cm}(0)}{g^{\mu\zeta}}\ \overset{\hspace{-0.3cm}(0)}{g^{\alpha\nu}}\ \overset{\hspace{-0.3cm}(0)}{g^{\gamma\beta}}\ \overset{\hspace{-0.3cm}(0)}{g^{\eta\delta}},
\hspace{1cm}\cdots
\label{eq2.2.6}
\end{align}
In this approximation, the Christoffel symbols of the first kind can be separated just as in \eqref{eq2.8}, i.e.,
\begin{equation}
\Gamma_{\alpha\beta\gamma}=\overset{(0)}{\Gamma}_{\alpha\beta\gamma}+\epsilon\,\overset{(1)}{\Gamma}_{\alpha\beta\gamma},
%%\sum_{i=1}^{n}\epsilon^i\,\overset{(i)}{\Gamma}_{\alpha\beta\gamma}+O(\epsilon^{n+1})
\label{eq2.2.7}
\end{equation}
where each summand is given by \eqref{eq2.9}. Using \eqref{eq2.2.2} for rise its first index, it is found
\begin{equation}
\Gamma^{\alpha}_{~\beta\gamma}=\overset{\hspace{-0.6cm}(0)}{\Gamma^{\alpha}_{~\beta\gamma}}+\sum_{i=1}^{n}\epsilon^i\,\overset{\hspace{-0.6cm}(i)}{\Gamma^{\alpha}_{~\beta\gamma}}+O(\epsilon^{n+1}),
\label{eq2.2.8}
\end{equation}
where
\begin{equation}
\overset{\hspace{-0.6cm}(0)}{\Gamma^{\alpha}_{~\beta\gamma}}=\overset{\hspace{-0.3cm}(0)}{g^{\alpha\eta}}\ \overset{\hspace{-0.6cm}(0)}{\Gamma^{}_{\eta\beta\gamma}},
\hspace{1cm}\overset{\hspace{-0.6cm}(k)}{\Gamma^{\alpha}_{~\beta\gamma}}=\ 
 \overset{\hspace{-0.3cm}(k-1)}{g^{\alpha\eta}}\ \overset{\hspace{-0.6cm}(1)}{\Gamma^{}_{\eta\beta\gamma}}+\overset{\hspace{-0.3cm}(k)}{g^{\alpha\eta}}\overset{\hspace{-0.6cm}(0)}{\Gamma^{}_{\eta\beta\gamma}}, \hspace{1cm}k=1,2,\cdots,
\label{eq2.2.9}
\end{equation}
which is just one of the possibilities for generalise \eqref{eq2.12}. The separation for the Christoffel's symbols of the second kind allows that the Riemann's tensor can be written as
\begin{equation}
R^\mu_{~\nu\gamma\delta}=\overset{\hspace{-0.6cm}(0)}{R^\mu_{~\nu\gamma\delta}}+\sum_{i=1}^{n}\epsilon^i\,\overset{\hspace{-0.6cm}(i)}{R^\mu_{~\nu\gamma\delta}}+O(\epsilon^{n+1}),
\label{eq2.2.10}
\end{equation}
where $\overset{\hspace{-0.6cm}(0)}{R^{\mu}_{~\nu\gamma\delta}}$ is given in \eqref{eq2.14} and $\overset{\hspace{-0.6cm}(i)}{R^{\mu}_{~\nu\gamma\delta}}$ corresponds to
\begin{equation}
\overset{\hspace{-0.6cm}(k)}{R^{\mu}_{~\nu\gamma\delta}}=2\,\overset{\hspace{-0.9cm}(k)}{\Gamma^{\mu}_{~\nu[\delta:\gamma]}}+2\,\sum_{i=1}^{k}\ \ \overset{\hspace{-0.7cm}(k-i)}{\Gamma^{\mu}_{~\sigma[\gamma}} \ \overset{\hspace{-0.6cm}(i)}{\Gamma^{\sigma}_{~\delta]\nu}}.
\label{eq2.2.11}
\end{equation}
Deriving \eqref{eq2.2.9} and anti-symmetrising is obtained
\begin{equation}
\overset{\hspace{-0.9cm}(k)}{\Gamma^{\alpha}_{~\beta[\gamma:\delta]}}=\ 
 \overset{\hspace{-0.7cm}(1)}{\Gamma^{}_{\eta\beta[\gamma}}\,\overset{\hspace{-0.5cm}(k-1)}{g^{\alpha\eta}_{~~~:\delta]}} 
 +\ \overset{\hspace{-0.3cm}(k-1)}{g^{\alpha\eta}}\ \overset{\hspace{-0.9cm}(1)}{\Gamma^{}_{\eta\beta[\gamma:\delta]}}
 +\overset{\hspace{-0.7cm}(0)}{\Gamma^{}_{\eta\beta[\gamma}}\,\overset{\hspace{-0.6cm}(k)}{g^{\alpha\eta}_{~~~:\delta]}}+\overset{\hspace{-0.3cm}(k)}{g^{\alpha\eta}}\,\,\overset{\hspace{-1cm}(0)}{\Gamma^{}_{\eta\beta[\gamma:\delta]}}. 
\label{eq2.2.12}
\end{equation}
Observing that
\begin{align}
\overset{\hspace{-0.6cm}(1)}{\Gamma^{}_{\eta\beta\gamma}}&=
\overset{\hspace{-0.6cm}(1)}{g_{\eta\beta:\gamma}}
+\overset{\hspace{-0.6cm}(1)}{g_{\gamma\eta:\beta}}
-\overset{\hspace{-0.6cm}(1)}{g_{\beta\gamma:\eta}}
+2\,\overset{\hspace{-0.6cm}(0)}{\Gamma^\sigma_{~\gamma\beta}}\,\overset{\hspace{-0.3cm}(1)}{g_{\sigma\eta}},
\label{eq2.2.13}
\end{align}
then
\begin{align}
\overset{\hspace{-0.7cm}(1)}{\Gamma^{}_{\eta\beta\gamma:\delta}}&=
\overset{\hspace{-0.7cm}(1)}{g_{\eta\beta:\gamma\delta}}
+\overset{\hspace{-0.7cm}(1)}{g_{\gamma\eta:\beta\delta}}
-\overset{\hspace{-0.7cm}(1)}{g_{\beta\gamma:\eta\delta}}
+2\,\overset{\hspace{-0.6cm}(0)}{\Gamma^\sigma_{~\gamma\beta:\delta}}\,\overset{\hspace{-0.3cm}(1)}{g_{\sigma\eta}}+2\,\overset{\hspace{-0.6cm}(0)}{\Gamma^\sigma_{~\gamma\beta}}\,\overset{\hspace{-0.5cm}(1)}{g_{\sigma\eta:\delta}}.
\label{eq2.2.14}
\end{align}
With this,
\begin{align}
2\,\overset{\hspace{-0.9cm}(1)}{\Gamma^{}_{\eta\beta[\gamma:\delta]}}=&
2\,\overset{\hspace{-0.7cm}(1)}{g_{\eta\beta:[\gamma\delta]}}
+\overset{\hspace{-0.7cm}(1)}{g_{\gamma\eta:\beta\delta}}-\overset{\hspace{-0.7cm}(1)}{g_{\delta\eta:\beta\gamma}}
-\overset{\hspace{-0.7cm}(1)}{g_{\beta\gamma:\eta\delta}}+\overset{\hspace{-0.7cm}(1)}{g_{\beta\delta:\eta\gamma}}\nonumber\\
&+4\,\overset{\hspace{-0.6cm}(0)}{\Gamma^\sigma_{~\beta[\gamma:\delta]}}\,\overset{\hspace{-0.3cm}(1)}{g_{\sigma\eta}}+4\,\overset{\hspace{-0.5cm}(1)}{g_{\sigma\eta:[\delta}}\,\overset{\hspace{-0.6cm}(0)}{\Gamma^\sigma_{~\gamma]\beta}}.
\label{eq2.2.15}
\end{align}
The first term in \eqref{eq2.2.12} is
\begin{align}
\overset{\hspace{-0.7cm}(1)}{\Gamma^{}_{\eta\beta[\gamma}}\,\overset{\hspace{-0.5cm}(k-1)}{g^{\alpha\eta}_{~~~:\delta]}}
&=
\overset{\hspace{-0.6cm}(1)}{g_{\eta\beta:[\gamma}}\,\overset{\hspace{-0.5cm}(k-1)}{g^{\alpha\eta}_{~~~:\delta]}}
+\overset{\hspace{-0.5cm}(k-1)}{g^{\alpha\eta}_{~~~:[\delta}}\,\overset{\hspace{-0.6cm}(1)}{g_{\gamma]\eta:\beta}}
-\overset{\hspace{-0.5cm}(k-1)}{g^{\alpha\eta}_{~~~:[\delta}}\,\overset{\hspace{-0.6cm}(1)}{g_{\gamma]\beta:\eta}}
+2\,\overset{\hspace{-0.5cm}(k-1)}{g^{\alpha\eta}_{~~~:[\delta}}\,\overset{\hspace{-0.6cm}(0)}{\Gamma^\sigma_{~\gamma]\beta}}\,\overset{\hspace{-0.3cm}(1)}{g_{\sigma\eta}},
\end{align}
the second term in \eqref{eq2.2.12} is
\begin{align}
\overset{\hspace{-0.3cm}(k-1)}{g^{\alpha\eta}}\ \overset{\hspace{-0.9cm}(1)}{\Gamma^{}_{\eta\beta[\gamma:\delta]}}&= 
\ \ \overset{\hspace{-0.3cm}(k-1)}{g^{\alpha\eta}}\ \left(
\,\overset{\hspace{-0.7cm}(1)}{g_{\eta\beta:[\gamma\delta]}}
+\,\overset{\hspace{-0.6cm}(0)}{\Gamma^\sigma_{~\gamma\beta:\delta}}\,\overset{\hspace{-0.3cm}(1)}{g_{\sigma\eta}}
-\,\overset{\hspace{-0.6cm}(0)}{\Gamma^\sigma_{~\delta\beta:\gamma}}\,\overset{\hspace{-0.3cm}(1)}{g_{\sigma\eta}}
+2\,\overset{\hspace{-0.5cm}(1)}{g_{\sigma\eta:[\delta}}\,\overset{\hspace{-0.6cm}(0)}{\Gamma^\sigma_{~\gamma]\beta}}
\right)\nonumber\\
&+ \frac{1}{2}\ \ \overset{\hspace{-0.3cm}(k-1)}{g^{\alpha\eta}}\ \left(
\overset{\hspace{-0.7cm}(1)}{g_{\gamma\eta:\beta\delta}}
-\overset{\hspace{-0.7cm}(1)}{g_{\delta\eta:\beta\gamma}}
+\overset{\hspace{-0.7cm}(1)}{g_{\beta\delta:\eta\gamma}}
-\overset{\hspace{-0.7cm}(1)}{g_{\beta\gamma:\eta\delta}}
\right). 
\end{align}
%Notice that \eqref{eq2.14} and \eqref{eq2.15} are particular cases of \eqref{eq2.2.7}. Using the fact that
%\begin{equation}
%\overset{\hspace{-1.0cm}(k)}{\Gamma^{\mu}_{~\nu[\delta,\gamma]}}=\overset{\hspace{-1.0cm}(k)}{\Gamma^{\mu}_{~\nu[\delta:\gamma]}}-\overset{\hspace{-0.7cm}(0)}{\Gamma^{\mu}_{~\sigma[\gamma}}\overset{\hspace{-0.7cm}(k)}{\Gamma^{\sigma}_{~\delta]\nu}}+\overset{\hspace{-0.6cm}(0)}{\Gamma^{\sigma}_{~\nu[\gamma}}\overset{\hspace{-0.6cm}(k)}{\Gamma^{\mu}_{~\delta]\sigma}}
%\label{eq2.2.8}
%\end{equation}
%then
%\begin{equation}
%\overset{\hspace{-0.6cm}(k)}{R^\mu_{~\nu\gamma\delta}}=2\, \overset{\hspace{-1cm}(k)}{\Gamma^{\mu}_{~\nu[\delta:\gamma]}}+2\,\sum_{i=1}^{k-1}\ \ \ \overset{\hspace{-0.7cm}(k-i)}{\Gamma^{\sigma}_{~\nu[\delta}}\, \overset{\hspace{-0.7cm}(i)}{\Gamma^{\mu}_{~\gamma]\sigma}},\hspace{1cm}k=1,2,\cdots
%\label{eq2.2.9}
%\end{equation}
%which constitutes a slight extension of \eqref{eq2.17}. For example, for perturbations of second order, one obtains
%\begin{equation}
%\overset{\hspace{-0.6cm}(2)}{R^\mu_{~\nu\gamma\delta}}=2\, \overset{\hspace{-1cm}(2)}{\Gamma^{\mu}_{~\nu[\delta:\gamma]}}+  2\,\overset{\hspace{-0.6cm}(1)}{\Gamma^{\sigma}_{~\nu[\delta}}\, \overset{\hspace{-0.6cm}(1)}{\Gamma^{\mu}_{~\gamma]\sigma}}
%\label{eq2.2.10}
%\end{equation}
%Notice that From \eqref{eq2.2.5}
%\begin{equation}
%\overset{\hspace{-1cm}(k)}{\Gamma^{\mu}_{~\nu[\delta:\gamma]}}=\sum_{i=0}^{k}\left(\,\,\overset{\hspace{-0.7cm}(i)}{\Gamma_{\eta\nu[\delta}}\ \ \overset{\hspace{-0.5cm}(k-i)}{g^{\mu\eta}_{~~:\gamma]}} + \overset{\hspace{-0.3cm}(k-i)}{g^{\mu\eta}}\ \overset{\hspace{-0.9cm}(i)}{\Gamma_{\eta\nu[\delta:\gamma]}}\right)
%\end{equation}












%From \eqref{eq2.10} it is possible to write
%\begin{equation}
%\overset{\hspace{-1cm}(k)}{\Gamma^{\mu}_{~\nu[\delta:\gamma]}}=\overset{\hspace{-0.7cm}(k)}{\Gamma^{}_{\sigma\nu[\gamma}}g^{\mu\sigma}_{~~:\delta]}+g^{\mu\sigma}\,\overset{\hspace{-1cm}(k)}{\Gamma_{\sigma\nu[\gamma:\delta]}}
%\label{eq2.2.11}
%\end{equation}
%in particular, for this approximation (in agreement with \eqref{eq2.2.5})
%\begin{equation}
%\overset{\hspace{-1cm}(k)}{\Gamma^{\mu}_{~\nu[\delta:\gamma]}}=\overset{\hspace{-0.3cm}(0)}{g^{\mu\sigma}}\,\overset{\hspace{-1cm}(k)}{\Gamma_{\sigma\nu[\gamma:\delta]}}
%\label{eq2.2.12}
%\end{equation}
%
%In order to start this, it is proposed that the metric $g_{\mu\nu}$ can be expressed as a series of small perturbations of the background metric in the form
%%\begin{equation}
%%g_{\mu\nu}=\overset{\hspace{-0.3cm}(0)}{g_{\mu\nu}}+\epsilon\,\overset{\hspace{-0.3cm}(1)}{g_{\mu\nu}}+\epsilon^2\,\overset{\hspace{-0.3cm}(2)}{g_{\mu\nu}}+\epsilon^3\,\overset{\hspace{-0.3cm}(3)}{g_{\mu\nu}}+\cdots
%%%\label{eq2.2.1}
%%\end{equation}
%\begin{equation}
%g_{\mu\nu}=\overset{\hspace{-0.3cm}(0)}{g_{\mu\nu}}+\sum_{i=1}^n \epsilon^i\,\overset{\hspace{-0.3cm}(i)}{g_{\mu\nu}}+O(\epsilon^{n+1})
%\label{eq2.2.1}
%\end{equation}
%where, $|\epsilon|\ll 1$. The inverse metric is then proposed, just as 
%%\begin{equation}
%%g^{\mu\nu}=\overset{\hspace{-0.3cm}(0)}{g^{\mu\nu}}+\epsilon\,\overset{\hspace{-0.3cm}(1)}{L^{\mu\nu}}+\epsilon^2\,\overset{\hspace{-0.3cm}(2)}{L^{\mu\nu}}+\epsilon^3\,\overset{\hspace{-0.3cm}(3)}{L^{\mu\nu}}+\cdots
%%\label{eq2.2.2}
%%\end{equation}
%\begin{equation}
%g^{\mu\nu}=\overset{\hspace{-0.3cm}(0)}{g^{\mu\nu}}+\sum_{i=1}^{n}\epsilon^i\,\overset{\hspace{-0.3cm}(i)}{g^{\mu\nu}}+O(\epsilon^{n+1})
%\label{eq2.2.2}
%\end{equation}
%where, the terms $\overset{\hspace{-0.3cm}(i)}{g^{\mu\nu}}$ are unknown and will be determined. Thus, making the product between \eqref{eq2.2.1} and \eqref{eq2.2.2} and reorganising,
%%\begin{align}
%%&\epsilon\left(\overset{\hspace{-0.3cm}(1)}{g_{\mu\nu}}\,\overset{\hspace{-0.3cm}(0)}{g^{\nu\delta}}+
%%\overset{\hspace{-0.3cm}(0)}{g_{\mu\nu}}\,\overset{\hspace{-0.3cm}(1)}{L^{\nu\delta}}
%%\right)+\epsilon^2\left(\overset{\hspace{-0.3cm}(2)}{g_{\mu\nu}}\,\overset{\hspace{-0.3cm}(0)}{g^{\nu\delta}}+
%%\overset{\hspace{-0.3cm}(1)}{g_{\mu\nu}}\,\overset{\hspace{-0.3cm}(1)}{L^{\nu\delta}}
%%+
%%\overset{\hspace{-0.3cm}(0)}{g_{\mu\nu}}\,\overset{\hspace{-0.3cm}(2)}{L^{\nu\delta}}
%%\right)\nonumber\\
%%&
%%+\epsilon^3\left(\overset{\hspace{-0.3cm}(3)}{g_{\mu\nu}}\,\overset{\hspace{-0.3cm}(0)}{g^{\nu\delta}}+
%%\overset{\hspace{-0.3cm}(2)}{g_{\mu\nu}}\,\overset{\hspace{-0.3cm}(1)}{L^{\nu\delta}}
%%+
%%\overset{\hspace{-0.3cm}(1)}{g_{\mu\nu}}\,\overset{\hspace{-0.3cm}(2)}{L^{\nu\delta}}
%%+
%%\overset{\hspace{-0.3cm}(0)}{g_{\mu\nu}}\,\overset{\hspace{-0.3cm}(3)}{L^{\nu\delta}}
%%\right)+\cdots=0.
%%\label{eq2.2.3}
%%\end{align}
%\begin{align}
%\sum_{k=1}^n\epsilon^k\sum_{j=0}^{k}\ \ \overset{\hspace{-0.3cm}(k-j)}{g_{\mu\nu}}\ \ \overset{\hspace{-0.3cm}(j)}{g^{\nu\delta}}=0
%\end{align}
%This polynomial for $\epsilon$ is null for each coefficient, which implies
%\begin{subequations}
%\begin{align}
%%\overset{\hspace{-0.3cm}(1)}{L^{\gamma\delta}}&=-\overset{\hspace{-0.3cm}(1)}{g_{\mu\nu}}\,\overset{\hspace{-0.3cm}(0)}{g^{\mu\gamma}}\,\overset{\hspace{-0.3cm}(0)}{g^{\nu\delta}} \label{eq2.2.4.1}\\
%%\overset{\hspace{-0.3cm}(2)}{L^{\gamma\delta}}&=-\overset{\hspace{-0.3cm}(2)}{g_{\mu\nu}}\,\overset{\hspace{-0.3cm}(0)}{g^{\mu\gamma}}\,\overset{\hspace{-0.3cm}(0)}{g^{\nu\delta}}-\overset{\hspace{-0.3cm}(1)}{g_{\mu\nu}}\,\overset{\hspace{-0.3cm}(0)}{g^{\mu\gamma}}\,\overset{\hspace{-0.3cm}(1)}{L^{\nu\delta}} \label{eq2.2.4.2}\\
%%\overset{\hspace{-0.3cm}(3)}{L^{\gamma\delta}}&=-\overset{\hspace{-0.3cm}(3)}{g_{\mu\nu}}\,\overset{\hspace{-0.3cm}(0)}{g^{\mu\gamma}}\,\overset{\hspace{-0.3cm}(0)}{g^{\nu\delta}}-\overset{\hspace{-0.3cm}(2)}{g_{\mu\nu}}\,\overset{\hspace{-0.3cm}(0)}{g^{\mu\gamma}}\,\overset{\hspace{-0.3cm}(1)}{L^{\nu\delta}}-\overset{\hspace{-0.3cm}(1)}{g_{\mu\nu}}\,\overset{\hspace{-0.3cm}(0)}{g^{\mu\gamma}}\,\overset{\hspace{-0.3cm}(2)}{L^{\nu\delta}} \label{eq2.2.4.3}\\
%%\vdots\nonumber\\
%\overset{\hspace{-0.3cm}(k)}{g^{\gamma\delta}}&=-\sum_{i=0}^{k-1}\ \ \overset{\hspace{-0.3cm}(k-i)}{g_{\mu\nu}}\ \overset{\hspace{-0.3cm}(0)}{g^{\mu\gamma}}\  \overset{\hspace{-0.3cm}(i)}{g^{\nu\delta}},\hspace{1cm}k=1,2,\cdots
%\end{align}
%\label{eq2.2.4}
%\end{subequations}
%Substituting recursively the equations \eqref{eq2.2.4} it is found that
%%\begin{subequations}
%%	\begin{align}
%%	\overset{\hspace{-0.3cm}(1)}{L^{\gamma\delta}}&=-\overset{\hspace{-0.3cm}(1)}{g_{\mu\nu}}\,\overset{\hspace{-0.3cm}(0)}{g^{\mu\gamma}}\,\overset{\hspace{-0.3cm}(0)}{g^{\nu\delta}} %\label{eq2.2.4.1}
%%	\\
%%	\overset{\hspace{-0.3cm}(2)}{L^{\gamma\delta}}&=-\overset{\hspace{-0.3cm}(2)}{g_{\mu\nu}}\,\overset{\hspace{-0.3cm}(0)}{g^{\mu\gamma}}\,\overset{\hspace{-0.3cm}(0)}{g^{\nu\delta}}+\overset{\hspace{-0.3cm}(1)}{g_{\mu\nu}}\,\overset{\hspace{-0.3cm}(1)}{g_{\alpha\beta}}\,\overset{\hspace{-0.3cm}(0)}{g^{\mu\gamma}}\,\overset{\hspace{-0.3cm}(0)}{g^{\alpha\nu}}\,\overset{\hspace{-0.3cm}(0)}{g^{\beta\delta}}
%%	%\label{eq2.2.4.2}
%%	\\
%%	\overset{\hspace{-0.3cm}(3)}{L^{\gamma\delta}}&=-\overset{\hspace{-0.3cm}(3)}{g_{\mu\nu}}\,\overset{\hspace{-0.3cm}(0)}{g^{\mu\gamma}}\,\overset{\hspace{-0.3cm}(0)}{g^{\nu\delta}}+\overset{\hspace{-0.3cm}(2)}{g_{\mu\nu}}\,\overset{\hspace{-0.3cm}(1)}{g_{\alpha\beta}}\,\overset{\hspace{-0.3cm}(0)}{g^{\mu\gamma}}\,\overset{\hspace{-0.3cm}(0)}{g^{\alpha\nu}}\,\overset{\hspace{-0.3cm}(0)}{g^{\beta\delta}}+\,\overset{\hspace{-0.3cm}(1)}{g_{\mu\nu}}\,\overset{\hspace{-0.3cm}(2)}{g_{\alpha\beta}}\,\overset{\hspace{-0.3cm}(0)}{g^{\mu\gamma}}\,\overset{\hspace{-0.3cm}(0)}{g^{\alpha\nu}}\,\overset{\hspace{-0.3cm}(0)}{g^{\beta\delta}}\nonumber\\
%%	&\hspace{0.45cm}-\overset{\hspace{-0.3cm}(1)}{g_{\mu\nu}}\,\overset{\hspace{-0.3cm}(1)}{g_{\theta\sigma}}\,\overset{\hspace{-0.3cm}(1)}{g_{\alpha\beta}}\,\overset{\hspace{-0.3cm}(0)}{g^{\mu\gamma}}\,\overset{\hspace{-0.3cm}(0)}{g^{\theta\nu}}\,\overset{\hspace{-0.3cm}(0)}{g^{\alpha\sigma}}\,\overset{\hspace{-0.3cm}(0)}{g^{\beta\delta}}
%%	%\label{eq2.2.4.3}
%%	\\
%%	\vdots\nonumber
%%	\end{align}
%%	\label{eq2.2.5}
%%\end{subequations}
%\begin{subequations}
%	\begin{align}
%	\overset{\hspace{-0.3cm}(1)}{g^{\gamma\delta}}&=-\overset{\hspace{-0.3cm}(1)}{g_{\mu\nu}}\,\overset{\hspace{-0.3cm}(0)}{g^{\mu\gamma}}\,\overset{\hspace{-0.3cm}(0)}{g^{\nu\delta}} %\label{eq2.2.4.1}
%	\\
%	\overset{\hspace{-0.3cm}(2)}{g^{\gamma\delta}}&=-\overset{\hspace{-0.3cm}(2)}{g_{\mu\nu}}\,\overset{\hspace{-0.3cm}(0)}{g^{\mu\gamma}}\,\overset{\hspace{-0.3cm}(0)}{g^{\nu\delta}}+\overset{\hspace{-0.3cm}(1)}{g_{\mu\nu}}\,\overset{\hspace{-0.3cm}(1)}{g_{\alpha\beta}}\,\overset{\hspace{-0.3cm}(0)}{g^{\mu\gamma}}\,\overset{\hspace{-0.3cm}(0)}{g^{\alpha\nu}}\,\overset{\hspace{-0.3cm}(0)}{g^{\beta\delta}}
%	%\label{eq2.2.4.2}
%	\\
%	\overset{\hspace{-0.3cm}(3)}{g^{\gamma\delta}}&=-\overset{\hspace{-0.3cm}(3)}{g_{\mu\nu}}\,\overset{\hspace{-0.3cm}(0)}{g^{\mu\gamma}}\,\overset{\hspace{-0.3cm}(0)}{g^{\nu\delta}}+\overset{\hspace{-0.3cm}(2)}{g_{\mu\nu}}\,\overset{\hspace{-0.3cm}(1)}{g_{\alpha\beta}}\,\overset{\hspace{-0.3cm}(0)}{g^{\mu\gamma}}\,\overset{\hspace{-0.3cm}(0)}{g^{\alpha\nu}}\,\overset{\hspace{-0.3cm}(0)}{g^{\beta\delta}}+\,\overset{\hspace{-0.3cm}(1)}{g_{\mu\nu}}\,\overset{\hspace{-0.3cm}(2)}{g_{\alpha\beta}}\,\overset{\hspace{-0.3cm}(0)}{g^{\mu\gamma}}\,\overset{\hspace{-0.3cm}(0)}{g^{\alpha\nu}}\,\overset{\hspace{-0.3cm}(0)}{g^{\beta\delta}}\nonumber\\
%	&\hspace{0.45cm}-\overset{\hspace{-0.3cm}(1)}{g_{\mu\nu}}\,\overset{\hspace{-0.3cm}(1)}{g_{\theta\sigma}}\,\overset{\hspace{-0.3cm}(1)}{g_{\alpha\beta}}\,\overset{\hspace{-0.3cm}(0)}{g^{\mu\gamma}}\,\overset{\hspace{-0.3cm}(0)}{g^{\theta\nu}}\,\overset{\hspace{-0.3cm}(0)}{g^{\alpha\sigma}}\,\overset{\hspace{-0.3cm}(0)}{g^{\beta\delta}}
%	%\label{eq2.2.4.3}
%	\\
%	\vdots\nonumber
%	\end{align}
%	\label{eq2.2.5}
%\end{subequations}
%Thus, 
%%\begin{equation}
%%\Gamma_{\mu\nu\gamma}=\overset{\hspace{-0.6cm}(0)}{\Gamma_{\mu\nu\gamma}}+\epsilon\, \overset{\hspace{-0.6cm}(1)}{\Gamma_{\mu\nu\gamma}}+\epsilon^2\, \overset{\hspace{-0.6cm}(2)}{\Gamma_{\mu\nu\gamma}}+\epsilon^3\, \overset{\hspace{-0.6cm}(3)}{\Gamma_{\mu\nu\gamma}}+\cdots,
%%%\label{eq2.8}
%%\end{equation}
%\begin{equation}
%\Gamma_{\mu\nu\gamma}=\overset{\hspace{-0.6cm}(0)}{\Gamma_{\mu\nu\gamma}}+\sum_{i=1}^{n}\epsilon^i\, \overset{\hspace{-0.6cm}(i)}{\Gamma_{\mu\nu\gamma}}+O(n+1),
%%\label{eq2.8}
%\end{equation}
%where
%\begin{equation}
%\overset{\hspace{-0.6cm}(i)}{\Gamma_{\mu\nu\gamma}}=\frac{1}{2}\left(\,\overset{\hspace{-0.5cm}(i)}{g_{\mu\nu,\gamma}}+\overset{\hspace{-0.5cm}(i)}{g_{\gamma\mu,\nu}}-\overset{\hspace{-0.5cm}(i)}{g_{\nu\gamma,\mu}}\right),\hspace{0.5cm}i=0,1,2\cdots.
%%\label{eq2.9}
%\end{equation}
%and
%%\begin{align}
%%\Gamma^\mu_{~\nu\gamma}&=
%%\overset{\hspace{-0.6cm}(0)}{\Gamma^\mu_{~\nu\gamma}} + \epsilon\,\overset{\hspace{-0.6cm}(1)}{\Gamma^\mu_{~\nu\gamma}}+ \epsilon^2\,\overset{\hspace{-0.6cm}(2)}{\Gamma^\mu_{~\nu\gamma}}+ \epsilon^3\,\overset{\hspace{-0.6cm}(3)}{\Gamma^\mu_{~\nu\gamma}}+\cdots, 
%%%\label{eq2.11}
%%\end{align}
%\begin{align}
%\Gamma^\mu_{~\nu\gamma}&=
%\overset{\hspace{-0.6cm}(0)}{\Gamma^\mu_{~\nu\gamma}} +  \sum_{i=1}^{n}\epsilon^i\,\overset{\hspace{-0.6cm}(i)}{\Gamma^\mu_{~\nu\gamma}}+\cdots, 
%%\label{eq2.11}
%\end{align}
%where
%\begin{align*}
%%\overset{\hspace{-0.6cm}(0)}{\Gamma^\mu_{~\nu\gamma}}&=\overset{\hspace{-0.3cm}(0)}{g^{\mu\sigma}}\overset{\hspace{-0.6cm}(0)}{\Gamma_{\sigma\nu\gamma}}, \\
%%\overset{\hspace{-0.6cm}(1)}{\Gamma^\mu_{~\nu\gamma}}&= \overset{\hspace{-0.3cm}(0)}{g^{\mu\sigma}}\overset{\hspace{-0.6cm}(1)}{\Gamma_{\sigma\nu\gamma}}+ \overset{\hspace{-0.3cm}(1)}{g^{\mu\sigma}}\overset{\hspace{-0.6cm}(0)}{\Gamma_{\sigma\nu\gamma}}\\.
%%\overset{\hspace{-0.6cm}(2)}{\Gamma^\mu_{~\nu\gamma}}&= \overset{\hspace{-0.3cm}(0)}{g^{\mu\sigma}}\overset{\hspace{-0.6cm}(2)}{\Gamma_{\sigma\nu\gamma}}+ \overset{\hspace{-0.3cm}(1)}{g^{\mu\sigma}}\overset{\hspace{-0.6cm}(1)}{\Gamma_{\sigma\nu\gamma}}+
%%\overset{\hspace{-0.3cm}(2)}{g^{\mu\sigma}}\overset{\hspace{-0.6cm}(0)}{\Gamma_{\sigma\nu\gamma}}\\
%\overset{\hspace{-0.6cm}(k)}{\Gamma^\mu_{~\nu\gamma}}&=\sum_{i=0}^{k}\overset{\hspace{-0.3cm}(i)}{g^{\mu\sigma}}\ \ \overset{\hspace{-0.6cm}(k-i)}{\Gamma_{\sigma\nu\gamma}}
%%\label{eq2.12}
%\end{align*}

==> docs/ladder_operators.tex <==
\section{Rising and Lowering Operators}
Here it will be shown the action of the differential operators induced by the projection of the covariant derivative of the tensor field defined in \eqref{spinscalars10}. In order to do this, it is useful to compact the notation in the form,
\begin{equation}
\tilde{\Lambda}_{\tilde{A}_{ab}}=\prod\limits_{i=a}^{b}\Lambda_{A_i},\hspace{1cm}\tilde{\Lambda}^{\tilde{A}_{ab}}=\prod\limits_{i=a}^{b}\Lambda^{A_i},
\label{ladder1}
\end{equation}
and for the tensor field
\begin{equation}
\Psi^{\tilde{B}_{1m}}_{\hspace{0.6cm}\tilde{A}_{1n}}=\Psi^{B_{1}\cdots B_{m}}_{\hspace{1.1cm}A_{1}\cdots A_{n}}.
\label{ladder2}
\end{equation}
Thus, \eqref{spinscalars10} will be written as
\begin{equation}
_s\Psi=\tilde{\Lambda}_{\tilde{B}_{1m}} \tilde{\Lambda}^{\tilde{A}_{1n}}\Psi^{\tilde{B}_{1m}}_{\hspace{0.6cm}\tilde{A}_{1n}}.
\label{ladder3}
\end{equation}
The {\it eth} operator $\eth$ is defined through the projection of the covariant derivative of $\Psi^{B_1\cdots B_m}_{\hspace{1.1cm}A_1\cdots A_n}$ associated with $q_{AB}$ noted by
\begin{equation}
\triangle_A\Psi^{B_1\cdots B_m}_{\hspace{1.1cm}A_1\cdots A_n}=\Psi^{B_1\cdots B_m}_{\hspace{1.1cm}A_1\cdots A_n|A},
\end{equation} 
onto the dyads $\boldsymbol{q}$, i.e.,
\begin{align}
\eth \ _s\Psi&=q^D\ _s\Psi_{|D},\nonumber\\
&=q^D\tilde{\Lambda}_{\tilde{B}_{1m}}\tilde{\Lambda}^{\tilde{A}_{1n}}  \Psi^{\tilde{B}_{1m}}_{\hspace{0.65cm}\tilde{A}_{1n}|D},
\label{ladder4}
%\label{ethgen1_v2}
\end{align}
where the symbols $\Lambda_{B_i}$ and the $\Lambda^{A_j}$ are defined as
\begin{subequations}
	\begin{equation}
	\Lambda_{B_i}=\begin{cases}
	q_{B_i} & \text{if} \hspace{0.5cm} i\le x\\
	\overline{q}_{B_i} & \text{if} \hspace{0.5cm} i> x
	\end{cases},
	\label{ethgen2.1}
	\end{equation}
	and
	\begin{equation}
	\Lambda^{A_j}=\begin{cases}
	q^{A_j} & \text{if}\hspace{0.5cm} j\le y\\
	\overline{q}^{A_j} & \text{if} \hspace{0.5cm} j> y\\
	\end{cases},
	\label{ethgen2.2}
	\end{equation}
	\label{ethgen2}
\end{subequations}
for $1\le x\le m$ and $1\le y \le n$. In this case, the spin-weight of this function, in agreement with \eqref{spinscalars11}, will be
\begin{equation}
s=2(x+y)-(m+n).
\end{equation}
Considering that the covariant derivative $\Psi^{\tilde{B}_{1m}}_{\hspace{0.65cm}\tilde{A}_{1n}|D}$ associated to $q_{AB}$ is
\begin{align}
\Psi^{\tilde{B}_{1m}}_{\hspace{0.65cm}\tilde{A}_{1n}|D}=&\Psi^{\tilde{B}_{1m}}_{\hspace{0.65cm}\tilde{A}_{1n},D}+\Omega^{B_{1}}_{~~~DC}\Psi^{C \tilde{B}_{2m}}_{\hspace{0.75cm}\tilde{A}_{1n}}+\cdots
+\Omega^{B_{m}}_{~~~DC}\Psi^{\tilde{B}_{1(m-1)}C}_{\hspace{1.3cm}\tilde{A}_{1n}}\nonumber\\ &-\Omega^C_{~~A_1D}\Psi^{\tilde{B}_{1m}}_{\hspace{0.6cm}C\tilde{A}_{2m}}
%\nonumber\\&
-\cdots -\Omega^C_{~~A_mD}\Psi^{\tilde{B}_{1m}}_{\hspace{0.6cm}\tilde{A}_{1(m-1)}C},
\label{ethgen3_v2}
\end{align}
then, when substituted into \eqref{ladder4} yields to
\begin{align}
\eth \ _s\Psi=& q^D\tilde{\Lambda}_{\tilde{B}_{1m}}\tilde{\Lambda}^{\tilde{A}_{1n}} \Psi^{\tilde{B}_{1m}}_{\hspace{0.6cm}\tilde{A}_{1n},D} 
%\nonumber\\&
+ q^D \tilde{\Lambda}_{\tilde{B}_{1m}} \tilde{\Lambda}^{\tilde{A}_{1n}} \Omega^{B_{1}}_{~~~DC}\Psi^{C \tilde{B}_{2m}}_{\hspace{0.8cm}\tilde{A}_{1n}} +\cdots\nonumber\\
&+q^D\tilde{\Lambda}_{\tilde{B}_{1m}}\tilde{\Lambda}^{\tilde{A}_{1n}}\Omega^{B_{m}}_{~~~DC}\Psi^{\tilde{B}_{1(m-1)C}}_{\hspace{1.3cm}\tilde{A}_{1n}} - q^D\tilde{\Lambda}_{\tilde{B}_{1m}} \tilde{\Lambda}^{\tilde{A}_{1n}}\Omega^C_{~~A_1D} \Psi^{\tilde{B}_{1m}}_{\hspace{0.6cm}C\tilde{A}_{2n}} \nonumber
\\&-\cdots-q^D\tilde{\Lambda}_{\tilde{B}_{1m}}\tilde{\Lambda}^{\tilde{A}_{1n}}\Omega^C_{~~A_mD}\Psi^{\tilde{B}_{1m}}_{\hspace{0.6cm}\tilde{A}_{1(n-1)}C}.
\label{ethgen4_v2}
\end{align}
Notice that the first term of the last equation can be written as
\begin{align}
q^D\tilde{\Lambda}_{\tilde{B}_{1m}}\tilde{\Lambda}^{\tilde{A}_{1n}}\Psi^{\tilde{B}_{1m}}_{\hspace{0.6cm}\tilde{A}_{1n,D}}%\nonumber\\
=& q^D\left(_s\Psi\right)_{,D} %\\
- q^D\Lambda_{B_1,D}\tilde{\Lambda}_{\tilde{B}_{2m}} \tilde{\Lambda}^{\tilde{A}_{1n}} \Psi^{\tilde{B}_{1m}}_{\hspace{0.6cm}\tilde{A}_{1n}}-\cdots\nonumber\\
&-q^D\Lambda_{B_{m},D}\tilde{\Lambda}_{\tilde{B}_{1(m-1)}} \tilde{\Lambda}^{\tilde{A}_{1n}} \Psi^{\tilde{B}_{1m}}_{\hspace{0.6cm}\tilde{A}_{1n}}-\cdots \nonumber\\
&-q^D\Lambda^{A_{1}}_{~~~,D} \tilde{\Lambda}_{\tilde{B}_{1m}} \tilde{\Lambda}^{\tilde{A}_{2n}} \Psi^{\tilde{B}_{1m}}_{\hspace{0.6cm}\tilde{A}_{1n}}\nonumber\\
&-\cdots-q^D \Lambda^{A_n}_{~~~,D} \tilde{\Lambda}_{\tilde{B}_{1m}} \tilde{\Lambda}^{\tilde{A}_{1(n-1)}} \Psi^{\tilde{B}_{1m}}_{\hspace{0.6cm}\tilde{A}_{1n}}.
\label{ethgen5_v2}
\end{align}
Thus, substituting \eqref{ethgen5_v2} into \eqref{ethgen4_v2}, reorganising the sums and changing the name of some indices  one obtains
\begin{align}
\eth \ _s\Psi=& q^D\left(_s\Psi\right)_{,D} - q^D\left(\Lambda_{B_1,D}-\Lambda_{C}\Omega^{C}_{~~~B_1 D}\right) \tilde{\Lambda}_{\tilde{B}_{2m}} \tilde{\Lambda}^{\tilde{A}_{1n}}\Psi^{\tilde{B}_{1m}}_{\hspace{0.6cm}\tilde{A}_{1n}}  -\cdots\nonumber\\
&-q^D\left(\Lambda_{B_m,D}-\Lambda_{C}\Omega^{C}_{~~~B_{m}D}\right) \tilde{\Lambda}_{\tilde{B}_{1(m-1)}} \tilde{\Lambda}^{\tilde{A}_{1n}}\Psi^{\tilde{B}_{1m}}_{\hspace{0.6cm}\tilde{A}_{1n}} \nonumber\\
&- q^D\left(\Lambda^{A_1}_{~~~,D}+\Lambda^{C}\Omega^{A_1}_{~~~CD}\right)  \tilde{\Lambda}_{\tilde{B}_{1m}} \tilde{\Lambda}^{\tilde{A}_{2n}}\Psi^{\tilde{B}_{1m}}_{\hspace{0.6cm}\tilde{A}_{1n}}-\cdots \nonumber\\
&-q^D\left(\Lambda^{A_n}_{~~~,D}+\Lambda^{C}\Omega^{A_n}_{~~CD}\right) \tilde{\Lambda}_{\tilde{B}_{1m}} \tilde{\Lambda}^{\tilde{A}_{1(n-1)}}\Psi^{\tilde{B}_{1m}}_{\hspace{0.6cm}\tilde{A}_{1n}}.
\label{ethgen7_v2}
\end{align}
Recognising the covariant derivatives for the lambda symbols in the brackets, one obtains,
\begin{align}
\eth \ _s\Psi=& q^D\left(_s\Psi\right)_{,D} - q^D \Lambda_{B_1|D} \tilde{\Lambda}_{\tilde{B}_{2m}} \tilde{\Lambda}^{\tilde{A}_{1n}}\Psi^{\tilde{B}_{1m}}_{\hspace{0.6cm}\tilde{A}_{1n}}  -\cdots
\nonumber\\&
-q^D\Lambda_{B_m|D} \tilde{\Lambda}_{\tilde{B}_{1(m-1)}} \tilde{\Lambda}^{\tilde{A}_{1n}}\Psi^{\tilde{B}_{1m}}_{\hspace{0.6cm}\tilde{A}_{1n}} 
- q^D\Lambda^{A_1}_{~~~|D} \tilde{\Lambda}_{\tilde{B}_{1m}} \tilde{\Lambda}^{\tilde{A}_{2n}}\Psi^{\tilde{B}_{1m}}_{\hspace{0.6cm}\tilde{A}_{1n}}-\cdots \nonumber\\
&-q^D\Lambda^{A_n}_{~~~|D} \tilde{\Lambda}_{\tilde{B}_{1m}} \tilde{\Lambda}^{\tilde{A}_{1(n-1)}}\Psi^{\tilde{B}_{1m}}_{\hspace{0.6cm}\tilde{A}_{1n}}.
\label{ethgen8_v2}
\end{align}
Now, it is important to observe that %for each $1\le k\le n$,
\begin{align}
q^D\Lambda^{A_k}_{~~~|D}&=\dfrac{q^{A_k}q^D\overline{q}^{C}\Lambda_{C|D}+\overline{q}^{A_k}q^D{q}^{C}\Lambda_{C|D}}{2}.
\label{ethgen9}
\end{align}
Since,
\begin{align}
q^Aq^{C}q_{C|A}&=\dfrac{q^Aq^{C}q_{C|A}+q^Aq^{C}q_{C|A}}{2},\nonumber\\
&=\dfrac{q^A\left(q^{C}q_{C|A}+q_{C}q^{C}_{~~|A}\right)}{2},\nonumber\\
&=0.
\label{ethgen10}
\end{align}
Then, \eqref{ethgen9} reads
\begin{align}
q^D\Lambda^{A_k}_{~~~|D}&=\begin{cases}
\dfrac{q^{A_k}q^D\overline{q}^{C}q_{C|D}}{2} & \text{for} \hspace{0.5cm}\Lambda^{A_k}=q^{A_k}\\[.4cm]
-\dfrac{\overline{q}^{A_k}q^D\overline{q}^{C}q_{C|D}}{2} & \text{for} \hspace{0.5cm} \Lambda^{A_k}=\overline{q}^{A_k}
\end{cases},
\label{ethgen13}
\end{align}
Also, since in stereographic coordinates
\begin{align}
q^A\overline{q}^{C}q_{C|A}&=q^A\overline{q}^{C}q_{C,A}-q^A\overline{q}^{C}q_D\Omega^D_{~~CA},\nonumber\\
&=-2\zeta,
\label{ethgen11}
\end{align}
where
\begin{equation}
q^A\overline{q}^{C}q_D\Omega^D_{~~CA}=0,
\label{ethgen12}
\end{equation}
then, \eqref{ethgen13} is simplified to
\begin{align}
q^D\Lambda^{A_k}_{~~~|D}&=\begin{cases}
q^{A_k}\zeta & \text{for} \hspace{0.5cm}\Lambda^{A_k}=q^{A_k}\\[.4cm]
-\overline{q}^{A_k}\zeta & \text{for} \hspace{0.5cm} \Lambda^{A_k}=\overline{q}^{A_k}
\end{cases}.
\label{ethgen14}
\end{align}
Thus, from \eqref{ethgen14}, lowering the index with the metric $q_{AB}$, it is obtained that
\begin{align}
q^D\Lambda^{}_{A_k|D}&=\begin{cases}
q_{A_k}\zeta & \text{for} \hspace{0.5cm}\Lambda_{A_k}=q_{A_k}\\[.4cm]
-\overline{q}_{A_k}\zeta & \text{for} \hspace{0.5cm} \Lambda_{A_k}=\overline{q}_{A_k}
\end{cases}.
\label{ethgen15}
\end{align}
Writing \eqref{ethgen8_v2} in the form, 
\begin{align}
\eth \ _s\Psi=& q^D\left(_s\Psi\right)_{,D} - \left(q^D \Lambda_{B_1|D} \tilde{\Lambda}_{\tilde{B}_{2m}} +\cdots + q^D\Lambda_{B_m|D} \tilde{\Lambda}_{\tilde{B}_{1(m-1)}} \right)\tilde{\Lambda}^{\tilde{A}_{1n}} \Psi^{\tilde{B}_{1m}}_{\hspace{0.6cm}\tilde{A}_{1n}}  
\nonumber\\&
- \left(q^D\Lambda^{A_1}_{~~~|D}  \tilde{\Lambda}^{\tilde{A}_{2n}}+\cdots 
+q^D\Lambda^{A_n}_{~~~|D}  \tilde{\Lambda}^{\tilde{A}_{1(n-1)}}\right) \tilde{\Lambda}_{\tilde{B}_{1m}} \Psi^{\tilde{B}_{1m}}_{\hspace{0.6cm}\tilde{A}_{1n}},
\label{ethgen16}
\end{align}
it is observed that the first bracket corresponds to
\begin{align*}
& q^D \Lambda_{B_1|D}\tilde{\Lambda}_{\tilde{B}_{2m}}  +\cdots+q^D\Lambda_{B_m|D}\tilde{\Lambda}_{\tilde{B}_{1(m-1)}}\\
=& q^D \Lambda_{B_1|D}\tilde{\Lambda}_{\tilde{B}_{2x}} \tilde{\Lambda}_{\tilde{B}_{(x+1)m}}+\cdots+q^D\Lambda_{B_x|D} \tilde{\Lambda}_{\tilde{B}_{1(x-1)}} \tilde{\Lambda}_{\tilde{B}_{(x+1)m}}  \nonumber\\
&+q^D\Lambda_{B_{x+1}|D} \tilde{\Lambda}_{\tilde{B}_{1x}} \tilde{\Lambda}_{\tilde{B}_{(x+2)m}} +\cdots+q^D\Lambda_{B_m|D} \tilde{\Lambda}_{\tilde{B}_{1x}} \tilde{\Lambda}_{\tilde{B}_{(x+1)(m-1)}},\\
&=\zeta\Bigg(\underbrace{- \tilde{q}_{\tilde{B}_{1x}} \tilde{\overline{q}}_{\tilde{B}_{(x+1)m}}-\cdots- \tilde{q}_{\tilde{B}_{1x}} \tilde{\overline{q}}_{\tilde{B}_{(x+1)m}}}_{x \ \text{terms}}\\
&\hspace{1cm} +\underbrace{ \tilde{q}_{\tilde{B}_{1x}} \tilde{\overline{q}}_{\tilde{B}_{(x+1)m}} 
	+\cdots+ \tilde{q}_{\tilde{B}_{1x}} \tilde{\overline{q}}_{\tilde{B}_{(x+1)m}}}_{m-x \ \text{terms}}\Bigg), 
\end{align*}
i.e.,
\begin{align}
 q^D \Lambda_{B_1|D} \tilde{\Lambda}_{\tilde{B}_{2m}}  +\cdots+q^D\Lambda_{B_m|D} \tilde{\Lambda}_{\tilde{B}_{1(m-1)}}
=\zeta(m-2x) \tilde{\Lambda}_{\tilde{B}_{1m}}.
\label{ethgen17}
\end{align}
Whereas the second bracket is
\begin{align*}
& q^D\Lambda^{A_1}_{~~~|D} \tilde{\Lambda}^{\tilde{A}_{2n}}+\cdots + q^D\Lambda^{A_n}_{~~~|D}\tilde{\Lambda}^{\tilde{A}_{1(n-1)}}\nonumber\\
&= -q^{A_1}\zeta \tilde{q}^{\tilde{A}_{2y}} \tilde{\overline{q}}^{\tilde{A}_{(y+1)n}}
\Psi^{\tilde{B}_{1m}}_{\hspace{0.6cm}\tilde{A}_{1n}}
-\cdots-q^{A_y}\zeta \tilde{q}^{\tilde{A}_{1(y-1)}} \tilde{\overline{q}}^{\tilde{A}_{(y+1)n}}
\nonumber\\
&\hspace{0.5cm}+\overline{q}^{A_{y+1}}\zeta \tilde{q}^{\tilde{A}_{1y}} \tilde{\overline{q}}^{\tilde{A}_{(y+2)n}}\Psi^{\tilde{B}_{1m}}_{\hspace{0.6cm}\tilde{A}_{1n}} +\cdots +\overline{q}^{A_{n}}\zeta \tilde{q}^{\tilde{A}_{1y}} \tilde{\overline{q}}^{\tilde{A}_{(y+1)(n-1)}},\nonumber\\
&=\zeta\Bigg(\underbrace{-\tilde{q}^{\tilde{A}_{1y}} \tilde{\overline{q}}^{\tilde{A}_{(y+1)n}} -\cdots- \tilde{q}^{\tilde{A}_{1y}} \tilde{\overline{q}}^{\tilde{A}_{(y+1)n}}}_{y \ \text{terms}}\nonumber\\
&\hspace{1cm}+ \underbrace{\tilde{q}^{\tilde{A}_{1y}} \tilde{\overline{q}}^{\tilde{A}_{(y+1)n}} +\cdots + \tilde{q}^{\tilde{A}_{1y}} \tilde{\overline{q}}^{\tilde{A}_{(y+1)n}}}_{n-y\ \text{terms}}\Bigg),
\end{align*}
or
\begin{align}
q^D\Lambda^{A_1}_{~~~|D} \tilde{\Lambda}^{\tilde{A}_{2n}}+\cdots + q^D\Lambda^{A_n}_{~~~|D}\tilde{\Lambda}^{\tilde{A}_{1(n-1)}}
=\zeta(n-2y)\tilde{\Lambda}^{\tilde{A}_{1n}}.
\label{ethgen18}
\end{align}
Thus, substituting \eqref{ethgen17} and \eqref{ethgen18} into \eqref{ethgen16} is obtained a simple expression in stereographic coordinates
\begin{align}
\eth \ _s\Psi=& q^D\left(_s\Psi\right)_{,D} - \zeta(m-2x+n-2y) \tilde{\Lambda}_{\tilde{B}_{1m}} \tilde{\Lambda}^{\tilde{A}_{1n}} \Psi^{\tilde{B}_{1m}}_{\hspace{0.6cm}\tilde{A}_{1n}},\nonumber\\
=& q^D\left(_s\Psi\right)_{,D} + s\, \zeta \ _s\Psi.
\label{ethgen19}
\end{align}
The {\it eth bar} operator is defined as
\begin{equation}
\overline{\eth} \ _s\Psi=\overline{q}^D \tilde{\Lambda}_{\tilde{B}_{1m}} \tilde{\Lambda}^{\tilde{A}_{1n}}  \Psi^{\tilde{B}_{1m}}_{\hspace{0.6cm}\tilde{A}_{1n}|D},
\label{ethgen18_v2}
\end{equation} 
and using \eqref{ethgen3_v2} one obtains that
%\begin{align}
%\overline{\eth} \ _s\Psi&=\overline{q}^D\left(_s\Psi\right)_{,D} - \overline{q}^D \Lambda_{B_1|D}\prod_{i=2}^m \Lambda_{B_i}\prod_{j=1}^n \Lambda^{A_j}\Psi^{B_1 \cdots B_m}_{\hspace{1.1cm}A_1\cdots A_n}  -\cdots\nonumber\\
%&-\overline{q}^D\Lambda_{B_m|D}\prod_{i=1}^{m-1} \Lambda_{B_i}\prod_{j=1}^n \Lambda^{A_j}\Psi^{B_1 \cdots B_{m}}_{\hspace{1.1cm}A_1\cdots A_n} \nonumber
%\\
%&- \overline{q}^D\Lambda^{A_1}_{~~~|D} \prod_{i=1}^m \Lambda_{B_i}\prod_{j=2}^n \Lambda^{A_j}\Psi^{B_1\cdots B_m}_{\hspace{1.1cm}A_1\cdots A_{n}}-\cdots \nonumber\\
%&-\overline{q}^D\Lambda^{A_n}_{~~~|D}\prod_{i=1}^m \Lambda_{B_i}\prod_{j=1}^{n-1} \Lambda^{A_j}\Psi^{B_1\cdots B_m}_{\hspace{1.1cm}A_1\cdots A_{n}}.
%\label{ethgen19}
%\end{align}
\begin{align}
\overline{\eth} \ _s\Psi&=\overline{q}^D\left(_s\Psi\right)_{,D} - \overline{q}^D \Lambda_{B_1|D} \tilde{\Lambda}_{\tilde{B}_{2m}} \tilde{\Lambda}^{\tilde{A}_{1n}}\Psi^{\tilde{B}_{1m}}_{\hspace{0.6cm}\tilde{A}_{1n}}  -\cdots\nonumber\\
&-\overline{q}^D\Lambda_{B_m|D} \tilde{\Lambda}_{\tilde{B}_{1(m-1)}} \tilde{\Lambda}^{\tilde{A}_{1n}}\Psi^{\tilde{B}_{1m}}_{\hspace{0.6cm}\tilde{A}_{1n}} %\nonumber
%\\&
- \overline{q}^D\Lambda^{A_1}_{~~~|D} \tilde{\Lambda}_{\tilde{B}_{1m}} \tilde{\Lambda}^{\tilde{A}_{2n}} \Psi^{\tilde{B}_{1m}}_{\hspace{0.6cm}\tilde{A}_{1n}} -\cdots \nonumber\\
&-\overline{q}^D\Lambda^{A_n}_{~~~|D} \tilde{\Lambda}_{\tilde{B}_{1m}} \tilde{\Lambda}^{\tilde{A}_{1(n-1)}}\Psi^{\tilde{B}_{1m}}_{\hspace{0.6cm}\tilde{A}_{1n}}.
\label{ethgen19_v2}
\end{align}
where
\begin{align}
\overline{q}^D\Lambda^{A_k}_{~~~|D}&=\dfrac{q^{A_k}\overline{q}^D\overline{q}^{C}\Lambda_{C|D}+\overline{q}^{A_k}\overline{q}^D{q}^{C}\Lambda_{C|D}}{2},
\label{ethgen20}
\end{align}
and
\begin{align}
\overline{q}^D\Lambda_{B_k|D}&=\dfrac{q_{B_k}\overline{q}^D\overline{q}^{C}\Lambda_{C|D}+\overline{q}^D\overline{q}_{B_k}{q}^{C}\Lambda_{C|D}}{2}.
\label{ethgen21}
\end{align}
Since the two last equations results as
\begin{align}
\overline{q}^D\Lambda^{A_k}_{~~~|D}&=\begin{cases}
q^{A_k}\overline{\zeta} & \text{if} \hspace{0.5cm}\Lambda^{A_k}=q^{A_k}\\ %[.4cm]
-\overline{q}^{A_k}\overline{\zeta} & \text{if} \hspace{0.5cm} \Lambda^{A_k}=\overline{q}^{A_k}
\end{cases},
\label{ethgen22}
\end{align}
and
\begin{align}
\overline{q}^D\Lambda_{B_k|D}&=\begin{cases}
q_{B_k}\overline{\zeta} & \text{for} \hspace{0.5cm} \Lambda_{B_k}=q_{B_k}\\ %[.4cm]
-\overline{q}_{B_k}\overline{\zeta}  & \text{for} \hspace{0.5cm} \Lambda_{B_k}=\overline{q}_{B_k}
\end{cases}.
\label{ethgen23}
\end{align}
Then, the expression for associated with the $\overline{\eth}$ operator actuating on the $_s\Psi$ becomes as
\begin{align}
\overline{\eth} \ _s\Psi&=\overline{q}^D\left(_s\Psi\right)_{,D} -\overline{\zeta}(2x-m)\ _s\Psi -\overline{\zeta}(2y-n)\ _s\Psi,\nonumber\\
%&=\overline{q}^D\ _s\Psi_{,D} -\overline{\zeta}(2x-m+2y-n)\ _s\Psi,\nonumber\\
&=\overline{q}^D\ _s\Psi_{,D} -s\overline{\zeta} \ _s\Psi.
\label{ethgen24}
\end{align}
It is worth stressing that from \eqref{ethgen19} and \eqref{ethgen24} the $\eth$ and $\overline{\eth}$ operators can be written in general, as
%\begin{align}
%\eth \ _s\Psi= q^D\left(_s\Psi\right)_{,D} + s\, \Omega \ _s\Psi,\hspace{0.5cm} \overline{\eth} \ _s\Psi= \overline{q}^D\left(_s\Psi\right)_{,D} - s\, \overline{\Omega} \ _s\Psi
%\label{ethgen25}
%\end{align}
\begin{align}
\eth = q^D\partial_D + s\, \Omega ,\hspace{0.5cm} \overline{\eth} = \overline{q}^D\partial_D - s\, \overline{\Omega}.
\label{ethgen251}
\end{align}
where $\Omega$ is defined from \eqref{ethgen11}, by
\begin{equation}
\Omega=\frac{1}{2}q^A\overline{q}^Bq_{AB}.
\label{ethgen26}
\end{equation}
Note that, \eqref{ethgen19} and \eqref{ethgen24}, or equivalently \eqref{ethgen26}, allows operate directly on the spin-weighted functions. Furthermore, they put in evidence their character to rise and lowering the spin-weight of the function $_s\Psi$. Under a transformation of coordinates between north and south hemispheres, 
\begin{align*}
\left(\eth \ _s\Psi\right)_N&=q^D_N\left(_s\Psi_N\right)_{,D} + s\, \zeta_N \ _s\Psi_N,\\
&=e^{i\alpha}q^D_S\left(e^{i\alpha s}\ _s\Psi_S\right)_{,D} + s\, e^{i\alpha}\zeta_S e^{i\alpha s}\ _s\Psi_S,\\
&=e^{i\alpha(s+1)}\left(q^D_S\left( _s\Psi_S\right)_{,D} + s\, \zeta_S \ _s\Psi_S\right),\\
&=e^{i\alpha(s+1)}\left(\eth \ _s\Psi\right)_S,
\end{align*}
and in analogy,
\begin{align*}
\left(\overline{\eth} \ _s\Psi\right)_N&=\overline{q}^D_N\left( _s\Psi_N\right)_{,D} -s\overline{\zeta}_N \ _s\Psi_N,\\
&=e^{i\alpha(s-1)}\left(\overline{q}^D_N\left( _s\Psi_N\right)_{,D} -s\overline{\zeta}_N \ _s\Psi_N\right),\\
&=e^{i\alpha(s-1)}\left(\overline{\eth} \ _s\Psi\right)_S.
%\\
%&=e^{i\alpha}q^D_S\left(e^{i\alpha s}\ _s\Psi_S\right)_{,D} + s\, e^{i\alpha}\zeta_S e^{i\alpha s}\ _s\Psi_S\\
%&=e^{i\alpha(s+1)}\left(q^D_S\left( _s\Psi_S\right)_{,D} + s\, \zeta_S \ _s\Psi_S\right)\\
%&=e^{i\alpha(s+1)}\left(\eth \ _s\Psi\right)_S
\end{align*}
Despite, it was used the stereographic coordinates in each chart, this property does not depend on the coordinates chosen to be used in each coordinate map.
The last equations show that $\eth\ _{s}\Psi$ and $\overline{\eth}\ _{s}\Psi$ are function with $s+1$ and $s-1$ spin-weight. Then,
%\\Thus, the remarkable points here are:
%\\ First operators defined in the equations \eqref{ethgen17} and \eqref{ethgen24} can be interpreted as raising and lowering operators, named $\eth$ and $\overline{\eth}$ respectively, for the spin-weighted functions. Thus,
\begin{equation}
\eth\ _s\Psi=A_{s+1}\ _{s+1}\Psi, \hspace{1cm} \overline{\eth}\ _s\Psi=A_{s-1}\ _{s-1}\Psi,
\label{ethgen27}
\end{equation}
where $A_{s+1}$ and $A_{s-1}$ are multiplicative constants. 
\\The explicit form of the $\eth$ and $\bar{\eth}$ operators in spherical coordinates is
\begin{equation}
\eth= \partial_\theta + i\csc\theta\partial_\phi - s\cot\theta, \hspace{0.5cm} \overline{\eth}= \partial_\theta - i\csc\theta\partial_\phi + s\cot\theta.
\label{eth_spherical_7}
\end{equation}
where were used \eqref{eth_spherical_1} and \eqref{eth_spherical_2}, and \eqref{ethgen26} results as
\begin{equation}
\Omega=-\cot\theta.
\label{ethgen28}
\end{equation}

%Second we can use them to re-express the basis $\partial_q$ and $\partial_p$ in terms of $\eth$ and $\overline{\eth}$ operators.
%Substituting \eqref{ethgen14_v2} and \eqref{ethgen16_v2} into \eqref{ethgen8_v2} one obtains
%\begin{align}
%\eth \ _s\Psi&=q^D\left(_s\Psi\right)_{,D} +\zeta(2x-m)\ _s\Psi +\zeta(2y-n)\ _s\Psi,\nonumber\\
%%&=q^D\ _s\Psi_{,D} +\zeta(2x-m+2y-n)\ _s\Psi,\nonumber\\
%&=q^D\ _s\Psi_{,D} +s\zeta \ _s\Psi.
%\label{ethgen17}
%\end{align}
%Now, we are able to construct the correspondent expression for the application of the $\overline{\eth}$ operator on the function $_s\Psi$. Thus from,
%%\begin{equation}
%%\overline{\eth} \ _s\Psi=\overline{q}^D\prod_{i=1}^m \Lambda_{B_i}\prod_{j=1}^n \Lambda^{A_j}  \Psi^{B_1\cdots B_m}_{\hspace{1.1cm}A_1\cdots A_n|D},
%%\label{ethgen18}
%%\end{equation} 
%\begin{equation}
%\overline{\eth} \ _s\Psi=\overline{q}^D \tilde{\Lambda}_{\tilde{B}_{1m}} \tilde{\Lambda}^{\tilde{A}_{1n}}  \Psi^{\tilde{B}_{1m}}_{\hspace{0.6cm}\tilde{A}_{1n}|D},
%\label{ethgen18_v2}
%\end{equation} 
%and using \eqref{ethgen3_v2} one obtains that
%%\begin{align}
%%\overline{\eth} \ _s\Psi&=\overline{q}^D\left(_s\Psi\right)_{,D} - \overline{q}^D \Lambda_{B_1|D}\prod_{i=2}^m \Lambda_{B_i}\prod_{j=1}^n \Lambda^{A_j}\Psi^{B_1 \cdots B_m}_{\hspace{1.1cm}A_1\cdots A_n}  -\cdots\nonumber\\
%%&-\overline{q}^D\Lambda_{B_m|D}\prod_{i=1}^{m-1} \Lambda_{B_i}\prod_{j=1}^n \Lambda^{A_j}\Psi^{B_1 \cdots B_{m}}_{\hspace{1.1cm}A_1\cdots A_n} \nonumber
%%\\
%%&- \overline{q}^D\Lambda^{A_1}_{~~~|D} \prod_{i=1}^m \Lambda_{B_i}\prod_{j=2}^n \Lambda^{A_j}\Psi^{B_1\cdots B_m}_{\hspace{1.1cm}A_1\cdots A_{n}}-\cdots \nonumber\\
%%&-\overline{q}^D\Lambda^{A_n}_{~~~|D}\prod_{i=1}^m \Lambda_{B_i}\prod_{j=1}^{n-1} \Lambda^{A_j}\Psi^{B_1\cdots B_m}_{\hspace{1.1cm}A_1\cdots A_{n}}.
%%\label{ethgen19}
%%\end{align}
%\begin{align}
%\overline{\eth} \ _s\Psi&=\overline{q}^D\left(_s\Psi\right)_{,D} - \overline{q}^D \Lambda_{B_1|D} \tilde{\Lambda}_{\tilde{B}_{2m}} \tilde{\Lambda}^{\tilde{A}_{1n}}\Psi^{\tilde{B}_{1m}}_{\hspace{0.6cm}\tilde{A}_{1n}}  -\cdots\nonumber\\
%&-\overline{q}^D\Lambda_{B_m|D} \tilde{\Lambda}_{\tilde{B}_{1(m-1)}} \tilde{\Lambda}^{\tilde{A}_{1n}}\Psi^{\tilde{B}_{1m}}_{\hspace{0.6cm}\tilde{A}_{1n}} %\nonumber
%%\\&
%- \overline{q}^D\Lambda^{A_1}_{~~~|D} \tilde{\Lambda}_{\tilde{B}_{1m}} \tilde{\Lambda}^{\tilde{A}_{2n}} \Psi^{\tilde{B}_{1m}}_{\hspace{0.6cm}\tilde{A}_{1n}} -\cdots \nonumber\\
%&-\overline{q}^D\Lambda^{A_n}_{~~~|D} \tilde{\Lambda}_{\tilde{B}_{1m}} \tilde{\Lambda}^{\tilde{A}_{1(n-1)}}\Psi^{\tilde{B}_{1m}}_{\hspace{0.6cm}\tilde{A}_{1n}}.
%\label{ethgen19_v2}
%\end{align}
%where
%\begin{align}
%\overline{q}^D\Lambda^{A_k}_{~~~|D}&=\dfrac{q^{A_k}\overline{q}^D\overline{q}^{C}\Lambda_{C|D}+\overline{q}^{A_k}\overline{q}^D{q}^{C}\Lambda_{C|D}}{2},
%\label{ethgen20}
%\end{align}
%and
%\begin{align}
%\overline{q}^D\Lambda_{B_k|D}&=\dfrac{q_{B_k}\overline{q}^D\overline{q}^{C}\Lambda_{C|D}+\overline{q}^D\overline{q}_{B_k}{q}^{C}\Lambda_{C|D}}{2}.
%\label{ethgen21}
%\end{align}
%Since the two last equations results as
%\begin{align}
%\overline{q}^D\Lambda^{A_k}_{~~~|D}&=\begin{cases}
%q^{A_k}\overline{\zeta} & \text{if} \hspace{0.5cm}\Lambda^{A_k}=q^{A_k}\\ %[.4cm]
%-\overline{q}^{A_k}\overline{\zeta} & \text{if} \hspace{0.5cm} \Lambda^{A_k}=\overline{q}^{A_k}
%\end{cases},
%\label{ethgen22}
%\end{align}
%and
%\begin{align}
%\overline{q}^D\Lambda_{B_k|D}&=\begin{cases}
%q_{B_k}\overline{\zeta} & \text{for} \hspace{0.5cm} \Lambda_{B_k}=q_{B_k}\\ %[.4cm]
%-\overline{q}_{B_k}\overline{\zeta}  & \text{for} \hspace{0.5cm} \Lambda_{B_k}=\overline{q}_{B_k}
%\end{cases}.
%\label{ethgen23}
%\end{align}
%Then, the expression for associated with the $\overline{\eth}$ operator actuating on the $_s\Psi$ becomes as
%\begin{align}
%\overline{\eth} \ _s\Psi&=\overline{q}^D\left(_s\Psi\right)_{,D} -\overline{\zeta}(2x-m)\ _s\Psi -\overline{\zeta}(2y-n)\ _s\Psi,\nonumber\\
%%&=\overline{q}^D\ _s\Psi_{,D} -\overline{\zeta}(2x-m+2y-n)\ _s\Psi,\nonumber\\
%&=\overline{q}^D\ _s\Psi_{,D} -s\overline{\zeta} \ _s\Psi.
%\label{ethgen24}
%\end{align}
%Thus, the remarkable points here are:
%\\ First operators defined in the equations \eqref{ethgen17} and \eqref{ethgen24} can be interpreted as raising and lowering operators, named $\eth$ and $\overline{\eth}$ respectively, for the spin-weighted functions. Thus,
%\begin{equation}
%\eth\ _s\Psi=A_{s+1}\ _{s+1}\Psi, \hspace{1cm} \overline{\eth}\ _s\Psi=A_{s-1}\ _{s-1}\Psi,
%\label{ethgen25}
%\end{equation}
%where $A_{s+1}$ and $A_{s-1}$ multiplicative constants. Second we can use them to re-express the basis $\partial_q$ and $\partial_p$ in terms of $\eth$ and $\overline{\eth}$ operators.
%%Also, when is used the metric to rising and lowering the indices, 
%%\begin{align}
%%q^D\Lambda_{B_k|D}&=\dfrac{q_{B_k}q^D\overline{q}_{C}\Lambda^{C}_{~~|D}+\overline{q}_{B_k}q^D{q}_{C}\Lambda^{C}_{~~|D}}{2},\nonumber\\
%%&=\dfrac{q_{B_k}q^D\overline{q}^{C}\Lambda_{C|D}+\overline{q}_{B_k}q^D{q}^{C}\Lambda_{C|D}}{2}.
%%\label{ethgen11}
%%\end{align}
%%Thus, the last equation becomes as
%%\begin{align*}
%%q^D\Lambda_{B_k|D}&=\begin{cases}
%%\dfrac{q_{B_k}q^D\overline{q}^{C}q_{C|D}
%%	%+\overline{m}_{B_k}m^D{m}^{C}m_{C|D}
%%}{2} & \text{for} \hspace{0.5cm} \Lambda_{B_k}=q_{B_k}\\[.4cm]
%%\dfrac{
%%	%m_{B_k}m^D\overline{m}^{C}\overline{m}_{C|D}+
%%	\overline{q}_{B_k}q^D{q}^{C}\overline{q}_{C|D}}{2} & \text{for} \hspace{0.5cm} \Lambda_{B_k}=\overline{q}_{B_k}
%%\end{cases},
%%\end{align*}
%%which, can be written as
%%\begin{align}
%%q^D\Lambda_{B_k|D}&=\begin{cases}
%%-q_{B_k}\zeta & \text{for} \hspace{0.5cm} \Lambda_{B_k}=q_{B_k}\\ %[.4cm]
%%\overline{q}_{B_k}\zeta  & \text{for} \hspace{0.5cm} \Lambda_{B_k}=\overline{q}_{B_k}
%%\end{cases},
%%\label{ethgen12}
%%\end{align}
%%In order to start this derivation, is useful to consider first a simple scalar field $\Psi$ with spin-weight zero. %We denote as $\Psi$ meaning $_0\Psi$. 
%
%%Thus,
%%\begin{equation}
%%\Psi_N=\Psi_S.
%%\label{eth1}
%%\end{equation}
%%Its covariant derivatives is reduced to partial derivatives,
%%\begin{equation}
%%\Psi_{|A}=\Psi_{,A},
%%\label{eth2}
%%\end{equation}
%%where here $|$ denotes covariant differentiation referred to the unit sphere metric $q_{AB}$, i.e., $\Psi_{|A}=\triangle_A \Psi$. Then, we define the $\eth$ and $\overline{\eth}$ operators, from
%%\begin{equation*}
%%\eth\ \Psi=q^A\Psi_{|A},\hspace{1cm}\overline{\eth}\ \Psi=\overline{q}^A\Psi_{|A}.
%%%\label{eth3}
%%\end{equation*}
%%Thus, from \eqref{eth2} for this scalar field, one obtains
%%\begin{equation}
%%\eth\ \Psi=q^A\Psi_{,A},\hspace{1cm}\overline{\eth}\ \Psi=\overline{q}^A\Psi_{,A}.
%%\label{eth3}
%%\end{equation}
%%Therefore, from the transformation between north and south regions given in \eqref{spin7},
%%\begin{equation}
%%\eth_N\ \Psi_N%&=q^A_N{\Psi_N}_{,A},\nonumber\\
%%=e^{i\alpha}q^A_S{\Psi_S}_{,A}, \hspace{1cm}
%%%\label{eth4}
%%%\end{equation}
%%%also,
%%%\begin{equation}
%%\overline{\eth}_N\ \Psi_N%&=\overline{q}^A_N{\Psi_N}_{,A},\nonumber\\
%%=e^{-i\alpha}\overline{q}^A_S{\Psi_S}_{,A}.
%%\label{eth4}
%%\end{equation}
%%A remarkable point here is the fact that whereas $\Psi$ is a spin zero scalar function, $\eth \Psi$ and $\overline{\eth} \Psi$ are 1 and -1 spin-weighted functions respectively. This is natural considering that the $\eth$ or conversely $\overline{\eth}$ operators are constructed from the projection of the covariant derivative on the dyads $\boldsymbol{q}$.
%%\\A further generalisation of this becomes when is considered a spin-weighted function $_s\Psi$ rather those of spin-weight zero. In order to do that, we will need to compute the covariant derivative of a tensor field. Then, the calculus of the explicit form of the connexion coefficients, 
%%\begin{equation}
%%\Omega^C_{~~AB}=\dfrac{q^{CD}}{2}\left(q_{DA,B}+q_{DB,A}-q_{AB,D}\right),
%%\label{eth5.aux}
%%\end{equation}
%%becomes unavoidable.
%%\\Thus, the non-null components of the Christoffel's symbols of the second kind in the stereographic coordinates are explicitly
%%\begin{subequations}
%%	\begin{align}
%%	\Omega^3_{~~33}=\dfrac{-2q}{1+\zeta\overline{\zeta}}, \hspace{0.5cm}\Omega^3_{~~34}=\dfrac{-2p}{1+\zeta\overline{\zeta}}, \hspace{0.5cm}\Omega^3_{~~44}=\dfrac{2q}{1+\zeta\overline{\zeta}}, \label{eth6.1}\\
%%	\Omega^4_{~~33}=\dfrac{2p}{1+\zeta\overline{\zeta}}, \hspace{0.5cm}\Omega^4_{~~34}=\dfrac{-2q}{1+\zeta\overline{\zeta}},\hspace{0.5cm} \Omega^4_{~~44}=\dfrac{-2p}{1+\zeta\overline{\zeta}}.\label{eth6.2}
%%	\end{align}
%%	\label{eth6}
%%\end{subequations}
%%In order to do this calculus simple, we will start considering a vector field $\Psi_B$, thus
%%\begin{align}
%%\eth \ _1\Psi&=q^Aq^B \triangle_A\Psi_{B},\nonumber\\
%%&=q^Aq^B\Psi_{B|A}.
%%\label{eth7}
%%\end{align} 
%%From the covariant derivative for a vector field,
%%\begin{subequations}
%%	\begin{align}
%%	\Psi_{B|A}&=\Psi_{B,A}-\Omega^C_{~~AB}\Psi_{C},\label{eth8.1}\\
%%	\Psi^{B}_{~~|A}&=\Psi^{B}_{~~,A}+\Omega^B_{~~AC}\Psi^{C},\label{eth8.2}
%%	\end{align} 
%%	\label{eth8}
%%\end{subequations}
%%Then, substituting \eqref{eth8.1} into \eqref{eth7},
%%\begin{align}
%%\eth \ _1\Psi%&=q^Aq^B\left(\Psi_{B,A}-\Omega^C_{~~AB}\Psi_{C}\right),\nonumber\\
%%&=q^A\left(q^B\Psi_{B,A}-q^B\Omega^C_{~~AB}\Psi_{C}\right),\nonumber\\
%%&=q^A\left(\left(q^B\Psi_{B}\right)_{,A}-\Psi_{B}{q^B}_{,A}-q^B\Omega^C_{~~AB}\Psi_{C}\right),\nonumber\\
%%&=q^A\left(\left(q^B\Psi_{B}\right)_{,A}-\left({q^B}_{,A}+q^D\Omega^B_{~~AD}\right)\Psi_{B}\right),\nonumber\\
%%&=q^A\left(q^B\Psi_{B}\right)_{,A}-q^A{q^B}_{|A}\Psi_{B}.
%%\label{eth9}
%%\end{align} 
%%Taking into account that,
%%\begin{align}
%%q^B_{~~|A}&=\left(q^{BC}q_C\right)_{|A},\nonumber\\
%%%&=q^{BC}_{~~~~|A}q_C + q^{BC}q_{C|A},\nonumber\\
%%&=q^{BC}q_{C|A},
%%\label{eth10}
%%\end{align}
%%%because the covariant derivative for the metric is null, i.e.,
%%%\begin{equation*}
%%%q_{BC|A}=0.
%%%\end{equation*}
%%then,  \eqref{eth9} becomes
%%\begin{align}
%%\eth \ _1\Psi&=q^A\left(q^B\Psi_{B}\right)_{,A}-q^Aq^{BC}q_{C|A}\Psi_{B},\nonumber\\
%%&=q^A\left(q^B\Psi_{B}\right)_{,A}-q^Aq^{(B}\overline{q}^{C)}q_{C|A}\Psi_{B},\nonumber\\
%%&=q^A\left(q^B\Psi_{B}\right)_{,A}-\left(\dfrac{q^A\overline{q}^{C}q_{C|A}}{2}\right)q^{B}\Psi_{B}-\left(\dfrac{q^Aq^{C}q_{C|A}}{2}\right)\overline{q}^{B}\Psi_{B}.
%%\label{eth11}
%%\end{align}
%%The factor in brackets in the third term of the last equation is
%%\begin{align}
%%\dfrac{q^Aq^{C}q_{C|A}}{2}&=\dfrac{q^Aq^{C}q_{C|A}+q^Aq^{C}q_{C|A}}{4},\nonumber\\
%%%&=\dfrac{q^Aq^{C}q_{C|A}+q^Aq^{C}\left(q_{CD}q^{D}\right)_{|A}}{4},\nonumber\\
%%%&=\dfrac{q^Aq^{C}q_{C|A}+q^Aq_{D}q^{D}_{~~|A}}{4},\nonumber\\
%%&=\dfrac{q^A\left(q^{C}q_{C|A}+q_{C}q^{C}_{~~|A}\right)}{4}.
%%\label{eth12}
%%\end{align}
%%Taking the covariant derivative of \eqref{decomposition4}, 
%%\begin{equation*}
%%\left(q^Cq_C\right)_{|A}=0,
%%\end{equation*}
%%results,
%%\begin{equation}
%%q^Cq_{C|A}=-q_Cq^C_{~~|A}.
%%\label{eth12aux}
%%\end{equation}
%Thus, it implies that \eqref{eth12} is null
%\begin{equation*}
%\dfrac{q^Aq^{C}q_{C|A}}{2}=0,
%\end{equation*}
%In this manner, \eqref{eth11} is immediately simplified to
%\begin{align}
%\eth \ _1\Psi &=q^A\left(q^B\Psi_{B}\right)_{,A}-\left(\dfrac{q^A\overline{q}^{C}q_{C|A}}{2}\right)q^{B}\Psi_{B},\nonumber\\
%&=q^A\ _1\Psi_{,A}+\Omega\ _1\Psi.
%\label{eth13}
%\end{align}
%where
%\begin{equation}
%\Omega=-\dfrac{q^A\overline{q}^{C}q_{C|A}}{2},
%\label{eth14}
%\end{equation}
%and $_1\Psi$ is defined as the 1-spin-weighted scalar
%\begin{equation}
%_1\Psi=q^{B}\Psi_{B}.
%\label{eth15}
%\end{equation}
%Now, it is possible to compute explicitly $\Omega$ from \eqref{eth14}, that is
%\begin{align}
%\Omega&=-\dfrac{1}{2}q^A\overline{q}^{C}\left(q_{C,A}-\Omega^D_{~~CA}q_D\right),\nonumber\\
%&=-\dfrac{1}{2}\left(q^A\overline{q}^{C}q_{C,A}-q^A\overline{q}^{C}\Omega^D_{~~CA}q_D\right).
%\label{eth16}
%\end{align}
%The first term in the brackets of the last equation can be computed using \eqref{decomposition8} and  %\eqref{decomposition9}, 
%\eqref{decomposition10} 
%%and \eqref{decomposition11}
%, thus
%%\begin{equation}
%%q^A\overline{q}^{C}q_{C,A}=q^3\overline{q}^{3}q_{3,3}+q^3\overline{q}^{4}q_{4,3}+q^4\overline{q}^{3}q_{3,4}+q^4\overline{q}^{4}q_{4,4},
%%\label{eth17}
%%\end{equation}
%%where
%%\begin{align*}
%%q^3\overline{m}^{3}m_{3,3}=-q, \hspace{0.5cm} m^3\overline{m}^{4}m_{4,3}=-q, \\
%%q^4\overline{m}^{3}m_{3,4}=-ip, \hspace{0.5cm} m^4\overline{m}^{4}m_{4,4}=-ip.
%%\end{align*}
%%Thus \eqref{eth17} results as
%\begin{align}
%q^A\overline{q}^{C}q_{C,A}&=-2(q+ip),\nonumber\\
%&=-2\zeta.
%\label{eth18}
%\end{align}
%The second term in the brackets of \eqref{eth16} is computing with the help of the explicit form for the cmponents of the Christoffel's symbols \eqref{eth6}. Developing the sums and computing each term
%\begin{align}
%q^A\overline{q}^{C}\Omega^D_{~~CA}q_D=& q^3\overline{q}^{3}\Omega^3_{~~33}q_3 + q^3\overline{q}^{4}\Omega^3_{~~43}q_3 + q^4\overline{q}^{3}\Omega^3_{~~34}q_3
%\nonumber\\
%&\hspace{0.1cm} +q^4\overline{q}^{4}\Omega^3_{~~44}q_3
%+q^3\overline{q}^{3}\Omega^4_{~~33}q_4 + q^3\overline{q}^{4}\Omega^4_{~~43}q_4 
%\nonumber\\
%&\hspace{0.1cm}  + q^4\overline{q}^{3}\Omega^4_{~~34}q_4
%+q^4\overline{q}^{4}\Omega^4_{~~44}q_4,
%\label{eth19}
%\end{align}
%%where each term is computing, these terms yield to
%%\begin{align*}
%%m^3\overline{m}^{3}\Omega^3_{~~33}m_3=-q, \hspace{0.5cm} m^3\overline{m}^{4}\Omega^3_{~~43}m_3=ip, \hspace{0.5cm} m^4\overline{m}^{3}\Omega^3_{~~34}m_3=-ip, \hspace{0.5cm} m^4\overline{m}^{4}\Omega^3_{~~44}m_3=q, \nonumber\\
%%m^3\overline{m}^{3}\Omega^4_{~~33}m_4=ip, \hspace{0.5cm} m^3\overline{m}^{4}\Omega^4_{~~43}m_4=-q, \hspace{0.5cm} m^4\overline{m}^{3}\Omega^4_{~~34}m_4=q, \hspace{0.5cm}m^4\overline{m}^{4}\Omega^4_{~~44}m_4=-ip.
%%\end{align*}
%%In this form, \eqref{eth19} results as
%\begin{align}
%q^A\overline{q}^{C}\Omega^D_{~~CA}q_D%&%=-q + ip -ip +q +ip -q +q -ip,\nonumber\\
%&=0.
%\label{eth20}
%\end{align}
%Substituting \eqref{eth18} and \eqref{eth20} into \eqref{eth16} we found that
%\begin{equation}
%\Omega=\zeta.
%\label{eth21}
%\end{equation}
%Then, when the last equation is used into \eqref{eth13}, it is obtained
%\begin{align}
%\eth \ _1\Psi &=q^A\ _1\Psi_{,A}+\zeta\ _1\Psi.
%\label{eth22}
%\end{align}
%Now, for the case of the $\overline{\eth}$ operator, we start from
%\begin{align}
%\overline{\eth} \ _1\Psi&=\overline{q}^Aq^B\Psi_{B|A},
%\label{eth23}
%\end{align}
%which in analogy with \eqref{eth11} immediately yields to
%\begin{align}
%\overline{\eth} \ _1\Psi&=
%\overline{q}^A\left(q^B\Psi_{B}\right)_{,A}-\left(\dfrac{\overline{q}^A\overline{q}^{C}q_{C|A}}{2}\right)q^{B}\Psi_{B}-\left(\dfrac{\overline{q}^Aq^{C}q_{C|A}}{2}\right)\overline{q}^{B}\Psi_{B}.
%\label{eth24}
%\end{align}
%Taking into account that
%\begin{align}
%\overline{q}^Aq^{C}q_{C|A}&=\dfrac{\overline{q}^Aq^{C}q_{C|A}+\overline{q}^Aq^{C}q_{C|A}}{2},\nonumber\\
%%&=\dfrac{\overline{q}^Aq^{C}q_{C|A}+\overline{q}^Aq_{C}q^{C}_{~~|A}}{2},\nonumber\\
%&=\dfrac{\overline{q}^Aq^{C}q_{C|A}-\overline{q}^Aq^{C}q_{C|A}}{2},\nonumber\\
%&=0.
%\label{eth24aux}
%\end{align}
%where we have used \eqref{eth12aux}. Then \eqref{eth24} is reduced to
%\begin{align}
%\overline{\eth} \ _1\Psi&=
%\overline{q}^A\left(q^B\Psi_{B}\right)_{,A}-\left(\dfrac{\overline{q}^A\overline{q}^{C}q_{C|A}}{2}\right)q^{B}\Psi_{B},\nonumber\\
%&=\overline{q}^A\ _1\Psi_{,A}+\Theta\ _1\Psi,
%\label{eth25}
%\end{align}
%where
%\begin{equation*}
%\Theta=-\left(\dfrac{\overline{m}^A\overline{m}^{C}m_{C|A}}{2}\right).
%\end{equation*}
%Taking the conjugate of the last expression, one looks
%\begin{align*}
%\overline{\Theta}&=-\overline{\left(\dfrac{\overline{m}^A\overline{m}^{C}m_{C|A}}{2}\right)},\nonumber\\
%&=-\left(\dfrac{m^Am^{C}\overline{m}_{C|A}}{2}\right).
%\end{align*}
%Since from \eqref{decomposition4}, 
%\begin{equation*}
%\left(m^C\overline{m_C}\right)_{|A}=0,
%\end{equation*}
%then
%\begin{equation}
%m^C\overline{m}_{C|A}=-m^C_{~~|A}\overline{m}_C.
%\label{eth25.aux}
%\end{equation}
%It implies that 
%\begin{align}
%\overline{\Theta}&=\left(\dfrac{m^A\overline{m}_C m^C_{~~|A}}{2}\right),\nonumber\\
%&=-\zeta.
%\label{eth26}
%\end{align}
%where was used \eqref{eth14}. Substituting \eqref{eth26} into \eqref{eth25}, it is immediately obtained
%\begin{align}
%\overline{\eth} \ _1\Psi&=\overline{m}^A\ _1\Psi_{,A}-\overline{\zeta}\ _1\Psi,
%\label{eth27}
%\end{align}
%Here, the most important points to leave into account is that we obtain two simple expressions for the $\eth$ and $\overline{\eth}$ operators, as showed in the expression \eqref{eth22} and \eqref{eth27}. These results can be generalised for function with spin-weight $s$.

==> docs/legendrian.tex <==
\section{Legendrian Operator}
This section is dedicated to the treatment of the Legendrian operator and its relationship with the spherical harmonics $_0Y_{lm}$. Here this operator is expressed in terms on the raise and lowering spin-weighted operators $\eth$ and $\overline{\eth}$. 
\\As is well known, the Laplace equation 
%when is referred only to the angular variables is given by  , 
\begin{equation}
\nabla^2\Psi=0,
\label{legend1}
\end{equation}
can be written as
\begin{equation}
\dfrac{1}{r}\partial_{rr}\left(r\Psi\right)+\dfrac{1}{r^2}\mathcal{L}^2\Psi=0,
\label{legend2}
\end{equation}
where the Legendrian operator $\mathcal L^2$ is given by,
\begin{equation}
\mathcal L^2=\dfrac{1}{\sin\theta}\partial_\theta\left(\sin\theta\partial_\theta\right)+\dfrac{1}{\sin^2\theta}\partial_{\phi\phi}.
\label{legend3}
\end{equation}
The partial differential equation \eqref{legend1} is hyperbolic and hence their solutions can be written as,
\begin{equation}
\Psi(\theta,\phi)=\dfrac{R(r)}{r}P(\theta)Q(\phi).
\label{legend4}
\end{equation}
It yields to a set of ordinary differential equations for the functions $R(r)$, $P(\theta)$ and $Q(\phi)$, 
\begin{subequations}
	\begin{align}
	&\dfrac{d^2R(r)}{dr^2}+\dfrac{l(l+1)R(r)}{r^2}=0, \label{legend5.1}\\
	&\dfrac{d^2Q(\phi)}{d\phi^2}+m^2Q(\phi)=0, \label{legend5.2}\\
	&\dfrac{1}{\sin\theta}\dfrac{d}{d\theta}\left(\sin\theta\dfrac{dP(\theta)}{d\theta}\right)+\left(l(l+1)-\dfrac{m^2}{\sin^2\theta}\right)P(\theta)=0. \label{legend5.3}
	\end{align}
	\label{legend5}
\end{subequations}
The solutions for \eqref{legend5.3} for any $l\in \mathbb{Z^+}$ and $m\in \mathbb{Z}$ in which   $-\left(l+1\right)\le m\le l+1$, are the associated Legendre polynomials which satisfy the orthogonality relation
\begin{equation}
\int_{-1}^{1}dxP^m_{l'}(x)P^m_{l}(x)=\dfrac{2}{2l+1}\dfrac{\left(l+m\right)!}{\left(l-m\right)!}\delta_{ll'}.
\label{legend6}
\end{equation}
With these polynomials and with the solution of \eqref{legend5.2}, i.e., 
\begin{equation}
Q(\phi)=e^{im\phi},
\end{equation}
a base for all angular functions are constructed. Such base is called as spherical harmonics, which reads
\begin{equation}
Y_{lm}(\theta,\phi)=\sqrt{\dfrac{2l+1}{4\pi}\dfrac{(l-m)!}{(l+m)!}}P^m_l(\cos\theta)e^{im\phi}.
\label{legend7}
\end{equation}
Thus, particular solutions for the Laplace equation can be constructed, in the form
\begin{equation*}
\Psi_{lm}=\dfrac{R_{l}(r)}{r}Y_{lm}(\theta,\phi).
\end{equation*}
Substituting the last into \eqref{legend2} and using \eqref{legend5.1}, one obtains that the spherical harmonics are the eigenfunctions to the Legendrian operator, corresponding to the eigenvalues $-l(l+1)$, i.e.,
\begin{equation}
\mathcal{L}^2Y_{lm}=-l(l+1)Y_{lm}.
\label{legend8}
\end{equation}
Now, it is possible to write \eqref{legend3}, in the form
\begin{align}
\mathcal L^2&=\dfrac{1}{\tan\theta}\partial_\theta +\partial_{\theta\theta}+\dfrac{1}{\sin^2\theta}\partial_{\phi\phi}, \nonumber\\
%&=\dfrac{1-\tan^2\left(\theta/2\right)}{2\tan\left(\theta/2\right)}\partial_\theta +\partial^2_\theta+\left(\dfrac{1}{\sin\theta}\right)^2\partial^2_\phi \nonumber\\
&=\dfrac{1-\tan^2\left(\theta/2\right)}{2\tan\left(\theta/2\right)}\partial_\theta +\partial_{\theta\theta}+\left(\dfrac{1}{2\tan\left(\theta/2\right)\cos^2\left(\theta/2\right)}\right)^2\partial_{\phi\phi},
\label{legend9}
\end{align}
where,
\begin{equation}
\dfrac{1-\tan^2\left(\theta/2\right)}{2\tan\left(\theta/2\right)}=\dfrac{1-\zeta\overline{\zeta}}{2\left(\zeta\overline{\zeta}\right)^{1/2}},
\label{legend10}
\end{equation}
and
\begin{equation}
\left(\dfrac{1}{2\tan\left(\theta/2\right)\cos^2\left(\theta/2\right)}\right)^2=\dfrac{\left(1+\zeta\overline{\zeta}\right)^2}{4\zeta\overline{\zeta}}.
\label{legend11}
\end{equation}
The operator $\partial_\theta$ can be developed as
\begin{align}
\partial_\theta&=q_{,\theta}\partial_q+p_{,\theta}\partial_p, 
\label{legend12}
\end{align}
where the factors $q_{,\theta}$ and $p_{,\theta}$ are computed using \eqref{stereo1}, 
\begin{align}
q_{,\theta}&=\dfrac{1}{2}(\zeta+\overline{\zeta})_{,\theta},\nonumber\\
&=\dfrac{1+\tan^2\left(\theta/2\right)}{4}(e^{i\phi}+e^{-i\phi}),
%&=\dfrac{\left(\zeta+\overline{\zeta}\right)\left(1+\zeta\overline{\zeta}\right)}{4\left(\zeta\overline{\zeta}\right)^{1/2}},
\label{legend13}
\end{align}
and
\begin{align}
p_{,\theta}&=\dfrac{i}{2}\left(\overline{\zeta}-\zeta\right)_{,\theta},\nonumber\\
&=-i\dfrac{1+\tan^2\left(\theta/2\right)}{4}(e^{i\phi}-e^{-i\phi}).
%&=\dfrac{i\left(\overline{\zeta}-\zeta\right)\left(1+\zeta\overline{\zeta}\right)}{4\left(\zeta\overline{\zeta}\right)^{1/2}}.
\label{legend14}
\end{align}
Thus, in terms of $\zeta$ and $\overline{\zeta}$ the equations \eqref{legend13} and \eqref{legend14} take the form
\begin{align}
q_{,\theta}&=\dfrac{\left(\zeta+\overline{\zeta}\right)\left(1+\zeta\overline{\zeta}\right)}{4\left(\zeta\overline{\zeta}\right)^{1/2}},
\label{legend15}
\end{align}
and
\begin{align}
p_{,\theta}&=\dfrac{i\left(\overline{\zeta}-\zeta\right)\left(1+\zeta\overline{\zeta}\right)}{4\left(\zeta\overline{\zeta}\right)^{1/2}}.
\label{legend16}
\end{align}
Under the substitution of \eqref{legend15} and \eqref{legend16}, the equation \eqref{legend12} immediately takes the form
\begin{align}
\partial_\theta&=\dfrac{\left(1+\zeta\overline{\zeta}\right)}{4\left(\zeta\overline{\zeta}\right)^{1/2}}\left(\left(\zeta+\overline{\zeta}\right)\partial_q + i\left(\overline{\zeta}-\zeta\right)\partial_p\right). 
\label{legend17}
\end{align}
Since the spherical harmonics defined in \eqref{legend7} have spin-weight $s$ zero, then the operators $\partial_q$ and $\partial_p$  given in \eqref{abase5} are reduced to
\begin{subequations}
	\begin{align}
	\partial_{q}&=\dfrac{1}{1+\zeta\overline{\zeta}}\left(\eth +\overline{\eth}  \right), \label{legend16.1}\\
	\partial_{p}&=\dfrac{i}{1+\zeta\overline{\zeta}}\left(\overline{\eth}  - \eth \right).\label{legend16.2}
	\end{align}
	\label{legend18}
\end{subequations}
Then, the operators given in \eqref{legend18}, yields us to re-express \eqref{legend17} as
\begin{align}
\partial_\theta
%&=\dfrac{1}{4\left(\zeta\overline{\zeta}\right)^{1/2}}\left(\left(\zeta+\overline{\zeta}\right)\left(\eth+\overline{\eth}\right) + \left(\zeta-\overline{\zeta}\right)\left(\overline{\eth}-\eth\right)\right),\nonumber\\
&=\dfrac{ \overline{\zeta}\ \eth+ \zeta\ \overline{\eth} }{2\left(\zeta\overline{\zeta}\right)^{1/2}}.
\label{legend19}
\end{align}
In order to compute the second order derivative $\partial_{\theta\theta}$, is necessary make the calculation of the quantities $q_{,\theta\theta}$ and $p_{,\theta\theta}$.  Thus from \eqref{legend13},
\begin{align}
q_{,\theta\theta}&=\dfrac{\left(1+\tan^2\left(\theta/2\right)\right)_{,\theta}}{4}(e^{i\phi}+e^{-i\phi}), \nonumber\\
&=\dfrac{\tan\left(\theta/2\right)\left(1+\tan^2\left(\theta/2\right)\right)}{4}(e^{i\phi}+e^{-i\phi}),\nonumber\\
&=\dfrac{\left(\zeta+\overline{\zeta}\right)\left(1+\zeta\overline{\zeta}\right)}{4},
\label{legend20}
\end{align}
and from \eqref{legend14},
\begin{align}
p_{,\theta\theta}&=-i\dfrac{\left(1+\tan^2\left(\theta/2\right)\right)_{,\theta}}{4}(e^{i\phi}-e^{-i\phi}), \nonumber\\
&=-i\dfrac{\left(\zeta-\overline{\zeta}\right)\left(1+\zeta\overline{\zeta}\right)}{4}.
\label{legend21}
\end{align}
The second order operator $\partial_{\theta\theta}$ is computed directly, using for this \eqref{legend12}, thus
\begin{align*}
\partial_{\theta\theta} &= \partial_\theta\left(q_{,\theta}\partial_q+p_{,\theta}\partial_p\right),\\
&= q_{,\theta\theta}\partial_q + p_{,\theta\theta}\partial_p + q_{,\theta}\partial_{\theta q}  +p_{,\theta}\partial_{\theta p},
\end{align*}
where
\begin{align*}
q_{,\theta}\partial_\theta\partial_q &= q_{,\theta}\left(q_{,\theta}\partial_q+p_{,\theta}\partial_p\right)\partial_q,\\
&= q_{,\theta}^2 \partial_{qq} + q_{,\theta}p_{,\theta} \partial_{pq}, 
\end{align*}
and
\begin{align*}
p_{,\theta}\partial_\theta\partial_p&=p_{,\theta}\left(q_{,\theta}\partial_q+p_{,\theta}\partial_p\right)\partial_p,\\
&=p_{,\theta}q_{,\theta}\partial_{qp}+p_{,\theta}^2\partial_{pp}.
\end{align*}
In this form, the second order operator $\partial_{\theta\theta}$ is,
\begin{align}
\partial_{\theta\theta}&= q_{,\theta\theta}\partial_q + p_{,\theta\theta}\partial_p + q_{,\theta}^2 \partial_{qq} + 2q_{,\theta}p_{,\theta} \partial_{qp}   +p_{,\theta}^2\partial_{pp}.
\label{legend22}
\end{align}
The commutator for the $\overline{\eth}$ and $\eth$ given in \eqref{abase31} becomes for zero spin-weighted functions as
\begin{equation}
\left[\overline{\eth},\eth\right]\ _0\Psi=0,
\label{legend23}
\end{equation}
then the anti-commutator for these functions takes the form
\begin{equation}
\left(\overline{\eth},\eth\right)\ _0\Psi=2\overline{\eth}\eth\ _0\Psi.
\label{legend24}
\end{equation}
For functions of these type, the second order differential operators $\partial_{qq}$, $\partial_{pp}$ and $\partial_{qp}$, given in \eqref{abase13.2}, \eqref{abase20.2} and \eqref{abase25.2} respectively, are strongly simplified to
\begin{subequations}
	\begin{align}
	\partial_{,qq}
	&=\dfrac{1}{\left(1+\zeta\overline{\zeta}\right)^2}\left(\eth^2\  + \overline{\eth}^2 + 2\overline{\eth}\eth -2\zeta \ \eth  -2\overline{\zeta}\ \overline{\eth}  \right), \label{legend25.1} \\
	\partial_{,pp}
	&=-\dfrac{1}{\left(1+\zeta\overline{\zeta}\right)^2}\left( \eth^2 + \overline{\eth}^2 - 2\overline{\eth}\eth -2\overline{\zeta}\ \overline{\eth} -2\zeta\ \eth   \right), \label{legend25.2} \\
	\partial_{,qp} 
	&=\dfrac{i}{\left(1+\zeta\overline{\zeta}\right)^2}\left( \overline{\eth}^2 - \eth^2 + 2\zeta \ \eth - 2\overline{\zeta} \ \overline{\eth} \right). \label{legend25.3}
	\end{align}
	\label{legend25}
\end{subequations}
Thus, the two first terms in \eqref{legend22} are obtained using \eqref{legend20}, \eqref{legend21} and \eqref{legend18}, 
\begin{align}
q_{,\theta\theta}\partial_q + p_{,\theta\theta}\partial_p 
%&= \dfrac{\left(1+\zeta\overline{\zeta}\right)}{4} \left( \left(\zeta+\overline{\zeta}\right) \dfrac{1}{1+\zeta\overline{\zeta}}\left(\eth +\overline{\eth}  \right) + i\left(\overline{\zeta}-\zeta\right)\dfrac{i}{1+\zeta\overline{\zeta}}\left(\overline{\eth}  - \eth \right)\right)\\
% &= \dfrac{1}{4} \left( \left(\zeta+\overline{\zeta}\right) \left(\eth +\overline{\eth}  \right) - \left(\overline{\zeta}-\zeta\right)\left(\overline{\eth}  - \eth \right)\right),\nonumber\\
% &= \dfrac{1}{4} \left( \left(\zeta+\overline{\zeta}\right) \eth  + \left(\zeta+\overline{\zeta}\right) \overline{\eth}  - \left(\overline{\zeta}-\zeta\right) \overline{\eth}  + \left(\overline{\zeta}-\zeta\right)  \eth  \right), \nonumber\\
&= \dfrac{1}{2} \left(  \overline{\zeta}\ \eth  + \zeta \ \overline{\eth}   \right).
\label{legend26}
\end{align}
The third term in \eqref{legend22} will be obtained when \eqref{legend15} and \eqref{legend25.1} are used,
\begin{align}
q_{,\theta}^2 \partial_{qq} 
%&= \left(\dfrac{\left(\zeta+\overline{\zeta}\right)\left(1+\zeta\overline{\zeta}\right)}{4\left(\zeta\overline{\zeta}\right)^{1/2}}\right)^2 \dfrac{1}{\left(1+\zeta\overline{\zeta}\right)^2}\left(\eth^2\  + \overline{\eth}^2 + 2\overline{\eth}\eth -2\zeta \ \eth  -2\overline{\zeta}\ \overline{\eth}  \right)\\
%&= \dfrac{\zeta^2+\overline{\zeta}^2+2\zeta\overline{\zeta}}{16\zeta\overline{\zeta}} \left(\eth^2\  + \overline{\eth}^2 + 2\overline{\eth}\eth -2\zeta \ \eth  -2\overline{\zeta}\ \overline{\eth}  \right),\nonumber\\
&= \dfrac{\left(\zeta+\overline{\zeta}\right)^2}{16\zeta\overline{\zeta}} \left(\eth^2\  + \overline{\eth}^2 + 2\overline{\eth}\eth -2\zeta \ \eth  -2\overline{\zeta}\ \overline{\eth}  \right).
\label{legend27}
\end{align}
The fourth term in \eqref{legend22} is obtained when \eqref{legend15}, \eqref{legend16} and \eqref{legend25.3} are employed
\begin{align}
2q_{,\theta}p_{,\theta} \partial_{qp}
%&=2\left(\dfrac{\left(\zeta+\overline{\zeta}\right)\left(1+\zeta\overline{\zeta}\right)}{4\left(\zeta\overline{\zeta}\right)^{1/2}}\right) \left(\dfrac{i\left(\overline{\zeta}-\zeta\right)\left(1+\zeta\overline{\zeta}\right)}{4\left(\zeta\overline{\zeta}\right)^{1/2}}\right) \dfrac{i}{\left(1+\zeta\overline{\zeta}\right)^2}\left( \overline{\eth}^2 - \eth^2 + 2\zeta \ \eth - 2\overline{\zeta} \ \overline{\eth} \right)\\
%&=-\dfrac{2\left( \overline{\zeta}^2-\zeta^2 \right)}{16 \zeta\overline{\zeta}} \left( \overline{\eth}^2 - \eth^2 + 2\zeta \ \eth - 2\overline{\zeta} \ \overline{\eth} \right),\nonumber\\
&=\dfrac{2 \left( \zeta+\overline{\zeta} \right) \left( \zeta-\overline{\zeta} \right)}{16 \zeta\overline{\zeta}} \left( \overline{\eth}^2 - \eth^2 + 2\zeta \ \eth - 2\overline{\zeta} \ \overline{\eth} \right).
\label{legend28}
\end{align}
After the substitution of \eqref{legend25.2} and \eqref{legend16}, the fifth term in \eqref{legend22} results as,
\begin{align}
p_{,\theta}^2\partial_{pp}
%&=\left(\dfrac{i\left(\overline{\zeta}-\zeta\right)\left(1+\zeta\overline{\zeta}\right)}{4\left(\zeta\overline{\zeta}\right)^{1/2}}\right)^2\left(-\dfrac{1}{\left(1+\zeta\overline{\zeta}\right)^2}\left( \eth^2 + \overline{\eth}^2 - 2\overline{\eth}\eth -2\overline{\zeta}\ \overline{\eth} -2\zeta\ \eth   \right)\right) \\
%&= \dfrac{ \overline{\zeta}^2 +\zeta^2 -2\zeta\overline{\zeta} }{16 \zeta\overline{\zeta} } \left( \eth^2 + \overline{\eth}^2 - 2\overline{\eth}\eth -2\overline{\zeta}\ \overline{\eth} -2\zeta\ \eth   \right),\\
&= \dfrac{ \left( \zeta - \overline{\zeta} \right)^2 }{16 \zeta\overline{\zeta} } \left( \eth^2 + \overline{\eth}^2 - 2\overline{\eth}\eth -2\overline{\zeta}\ \overline{\eth} -2\zeta\ \eth   \right).
\label{legend29}
\end{align}
Thus, adding \eqref{legend27} and \eqref{legend29}
\begin{align*}
q_{,\theta}^2 \partial_{qq}+p_{,\theta}^2\partial_{pp}&=\dfrac{1}{16\zeta\overline{\zeta}}\Big(\left(\left(\zeta+\overline{\zeta}\right)^2+\left(\zeta-\overline{\zeta}\right)^2\right)\left(\eth^2+\overline{\eth}^2-2\zeta\ \eth -2\overline{\zeta}\ \overline{\eth}\right)\nonumber\\
&\hspace{1cm}+2\left(\left(\zeta+\overline{\zeta}\right)^2-\left(\zeta-\overline{\zeta}\right)^2\right)\eth\overline{\eth}\Big).
\end{align*}
Using the last equation and \eqref{legend28}, we obtain
\begin{align}
& q_{,\theta}^2 \partial_{qq}+p_{,\theta}^2\partial_{pp}+2q_{,\theta}p_{,\theta} \partial_{qp} \nonumber\\
%&=\dfrac{1}{16\zeta\overline{\zeta}}\Big(\left(\left(\zeta+\overline{\zeta}\right)^2+\left(\zeta-\overline{\zeta}\right)^2\right)\left(\eth^2+\overline{\eth}^2-2\zeta\ \eth -2\overline{\zeta}\ \overline{\eth}\right)\nonumber\\
%&+2\left(\left(\zeta+\overline{\zeta}\right)^2-\left(\zeta-\overline{\zeta}\right)^2\right)\eth\overline{\eth}\Big)+\dfrac{2 \left( \zeta+\overline{\zeta} \right) \left( \zeta-\overline{\zeta} \right)}{16 \zeta\overline{\zeta}} \left( \overline{\eth}^2 - \eth^2 + 2\zeta \ \eth - 2\overline{\zeta} \ \overline{\eth} \right)\\
%&=\dfrac{1}{16\zeta\overline{\zeta}}\Bigg( \left(\left(\zeta+\overline{\zeta}\right)^2+\left(\zeta-\overline{\zeta}\right)^2\right)\left(\eth^2+\overline{\eth}^2-2\zeta\ \eth -2\overline{\zeta}\ \overline{\eth}\right)\nonumber\\
%&+ 2 \left( \zeta+\overline{\zeta} \right) \left( \zeta-\overline{\zeta} \right) \left( \overline{\eth}^2 - \eth^2 + 2\zeta \ \eth - 2\overline{\zeta} \ \overline{\eth} \right) +2\left(\left(\zeta+\overline{\zeta}\right)^2-\left(\zeta-\overline{\zeta}\right)^2\right)\eth\overline{\eth}  \Bigg) \\
%&=\dfrac{1}{16\zeta\overline{\zeta}}\Bigg( \left(\left(\zeta+\overline{\zeta}\right)^2 + 2 \left( \zeta+\overline{\zeta} \right) \left( \zeta-\overline{\zeta} \right) + \left(\zeta-\overline{\zeta}\right)^2\right)\left(\overline{\eth}^2  - 2\overline{\zeta}\ \overline{\eth}\right)\nonumber\\
%&+\left( \left(\zeta+\overline{\zeta}\right)^2 - 2 \left( \zeta+\overline{\zeta} \right) \left( \zeta-\overline{\zeta} \right) + \left(\zeta-\overline{\zeta}\right)^2 \right) \left( \eth^2 - 2\zeta \ \eth \right)\\ &+2\left(\left(\zeta+\overline{\zeta}\right)^2-\left(\zeta-\overline{\zeta}\right)^2\right)\eth\overline{\eth}  \Bigg) \\
%&=\dfrac{1}{16\zeta\overline{\zeta}}\Bigg( \left(\left(\zeta+\overline{\zeta}\right) + \left(\zeta-\overline{\zeta}\right)\right)^2\left(\overline{\eth}^2  - 2\overline{\zeta}\ \overline{\eth}\right)\nonumber\\
%&+\left( \left(\zeta+\overline{\zeta}\right) - \left(\zeta-\overline{\zeta}\right) \right)^2 \left( \eth^2 - 2\zeta \ \eth \right)\\ &+2\left(\left(\zeta+\overline{\zeta}\right)^2-\left(\zeta-\overline{\zeta}\right)^2\right)\eth\overline{\eth}  \Bigg) \\
% \dfrac{1}{16\zeta\overline{\zeta}}\Bigg( 4 \zeta^2\left(\overline{\eth}^2  - 2\overline{\zeta}\ \overline{\eth}\right) +4 \overline{\zeta}^2 \left( \eth^2 - 2\zeta \ \eth \right) %\\ &
%+2\left(\left(\zeta+\overline{\zeta}\right)^2-\left(\zeta-\overline{\zeta}\right)^2\right)\eth\overline{\eth}  \Bigg) 
%\nonumber\\
%& 
=& \dfrac{1}{16\zeta\overline{\zeta}}\Bigg( 4 \zeta^2\left(\overline{\eth}^2  - 2\overline{\zeta}\ \overline{\eth}\right) +4 \overline{\zeta}^2 \left( \eth^2 - 2\zeta \ \eth \right) %\\ &
+8  \zeta\overline{\zeta} \eth\overline{\eth}  \Bigg).
\label{legend30}
\end{align}
Then, using \eqref{legend30} and \eqref{legend26}, it is obtained that \eqref{legend22} takes the explicit form
\begin{align}
\partial_{\theta\theta} 
%& \dfrac{1}{16\zeta\overline{\zeta}}\Bigg( 4 \zeta^2\left(\overline{\eth}^2  - 2\overline{\zeta}\ \overline{\eth}\right) +4 \overline{\zeta}^2 \left( \eth^2 - 2\zeta \ \eth \right) %\\ &
%+2\left(\left(\zeta+\overline{\zeta}\right)^2-\left(\zeta-\overline{\zeta}\right)^2\right)\eth\overline{\eth}  \Bigg) + \dfrac{1}{2} \left(  \overline{\zeta}\ \eth  + \zeta \ \overline{\eth}   \right) = \nonumber \\
%& \dfrac{1}{16\zeta\overline{\zeta}}\Bigg( 4 \zeta^2\left(\overline{\eth}^2  - 2\overline{\zeta}\ \overline{\eth}\right) +4 \overline{\zeta}^2 \left( \eth^2 - 2\zeta \ \eth \right) %\\ &
%+2\left(\left(\zeta+\overline{\zeta}\right)^2-\left(\zeta-\overline{\zeta}\right)^2\right)\eth\overline{\eth} + 8\zeta\overline{\zeta}  \left(  \overline{\zeta}\ \eth  + \zeta \ \overline{\eth}   \right) \Bigg) = \\
%& \dfrac{1}{16\zeta\overline{\zeta}}\Bigg( 4 \zeta^2 \overline{\eth}^2 +4 \overline{\zeta}^2   \eth^2  %\\ &
%+2\left(\left(\zeta+\overline{\zeta}\right)^2-\left(\zeta-\overline{\zeta}\right)^2\right)\eth\overline{\eth}  \Bigg) =\\
= \dfrac{1}{16\zeta\overline{\zeta}}\Bigg( 4 \zeta^2 \overline{\eth}^2 +4 \overline{\zeta}^2   \eth^2  %\\ &
+8 \zeta\overline{\zeta}  \eth\overline{\eth}  \Bigg). 
%& \dfrac{1}{16\zeta\overline{\zeta}} \left(4\overline{\zeta}^2\eth^2+4{\zeta}^2\overline{\eth}^2 + 16\left(\zeta^3\overline{\zeta} + \overline{\zeta}^3\zeta\right)\eth\overline{\eth} \right).
\label{legend31}
\end{align}
Now, the differential operator $\partial_{\phi}$ can be developed as
\begin{align}
\partial_\phi&=q_{,\phi}\partial_q+p_{,\phi}\partial_p, 
\label{legend32}
\end{align}
where the coefficients $q_{,\phi}$ and $p_{,\phi}$ are
\begin{align}
q_{,\phi}&=\dfrac{1}{2}(\zeta+\overline{\zeta})_{,\phi},\nonumber\\
%&=\dfrac{\tan\left(\theta/2\right)}{2}(ie^{i\phi}-ie^{-i\phi}),\nonumber\\
&=\dfrac{i}{2}(\zeta-\overline{\zeta}),
\label{legend33}
\end{align}
and
\begin{align}
p_{,\phi}&=\dfrac{i}{2}\left(\overline{\zeta}-\zeta\right)_{,\phi},\nonumber\\
&=\dfrac{1}{2}(\overline{\zeta}+\zeta).
\label{legend34}
\end{align}
Then, using the two last relations and \eqref{legend18}
\begin{align}
\partial_\phi&=\dfrac{i(\zeta-\overline{\zeta})}{2\left(1+\zeta\overline{\zeta}\right)}\left(\eth +\overline{\eth}  \right) +  \dfrac{i(\zeta+\overline{\zeta})}{2\left(1+\zeta\overline{\zeta}\right)}\left(\overline{\eth}  - \eth \right),\nonumber\\
%&=\dfrac{i}{2\left(1+\zeta\overline{\zeta}\right)}\left((\zeta-\overline{\zeta}) \left(\eth +\overline{\eth}  \right) +  (\zeta+\overline{\zeta})\left(\overline{\eth}  - \eth \right)\right),\nonumber\\
&=i\dfrac{-\overline{\zeta}\eth +  \zeta\eth }{\left(1+\zeta\overline{\zeta}\right)}. 
\label{legend35}
\end{align}
The second order partial derivative $\partial_{\phi\phi}$ can be computed as
\begin{align*}
\partial_{\phi\phi} %&=\partial_\phi\left(\partial_\phi\right)\\
&= \partial_\phi\left(q_{,\phi}\partial_q+p_{,\phi}\partial_p\right),\\
&= q_{,\phi\phi}\partial_q + p_{,\phi\phi}\partial_p + q_{,\phi}\partial_{\phi q}  +p_{,\phi}\partial_{\phi p},
\end{align*}
where
\begin{align*}
q_{,\phi}\partial_\phi\partial_q &= q_{,\phi}\left(q_{,\phi}\partial_q+p_{,\phi}\partial_p\right)\partial_q,\\
&= q_{,\phi}^2 \partial_{qq} + q_{,\phi}p_{,\phi} \partial_{pq},
\end{align*}
and
\begin{align*}
p_{,\phi}\partial_\phi\partial_p&=p_{,\phi}\left(q_{,\phi}\partial_q+p_{,\phi}\partial_p\right)\partial_p,\\
&=p_{,\phi}q_{,\phi}\partial_{qp}+p_{,\phi}^2\partial_{pp}.
\end{align*}
Then, for this reason
\begin{align}
\partial_{\phi\phi}&= q_{,\phi\phi}\partial_q + p_{,\phi\phi}\partial_p + q_{,\phi}^2 \partial_{qq} + 2q_{,\phi}p_{,\phi} \partial_{pq} + p_{,\phi}^2\partial_{pp}.
\label{legend36}
\end{align}
The factor $q_{,\phi\phi}$ is computed from \eqref{legend33} and with the help of \eqref{legend34}. Thus
\begin{align}
q_{\phi\phi}&=\dfrac{i}{2}(\zeta-\overline{\zeta})_{,\phi},\nonumber\\
&=-\dfrac{1}{2}(\overline{\zeta}+\zeta).
\label{legend37}
\end{align}
The factor $p_{,\phi\phi}$ is calculated from \eqref{legend34}
\begin{align}
p_{,\phi\phi}&=\dfrac{1}{2}(\overline{\zeta}+\zeta)_{,\phi},\nonumber\\
&=\dfrac{i}{2}(\zeta-\overline{\zeta}),
\label{legend38}
\end{align}
where we have used \eqref{legend33}. Thus, when \eqref{legend37}, \eqref{legend38} and \eqref{legend18} are substituted into the two first terms of \eqref{legend36} one obtains
\begin{align}
q_{,\phi\phi}\partial_q + p_{,\phi\phi}\partial_p&=- \dfrac{1}{2\left(1+\zeta\overline{\zeta}\right)}\left(\left(\overline{\zeta}+\zeta\right)\left(\eth +\overline{\eth}  \right) + \left(\zeta-\overline{\zeta}\right)\left(\overline{\eth}  - \eth \right)\right),\nonumber\\
%&=- \dfrac{1}{2\left(1+\zeta\overline{\zeta}\right)}\left(\left(\overline{\zeta}+\zeta\right)\eth +\left(\overline{\zeta}+\zeta\right)\overline{\eth}   + \left(\zeta-\overline{\zeta}\right)\overline{\eth}  - \left(\zeta-\overline{\zeta}\right)\eth \right),\nonumber\\
&=- \dfrac{ \overline{\zeta}\ \eth + \zeta\ \overline{\eth} }{\left(1+\zeta\overline{\zeta}\right)}. %,\nonumber\\
\label{legend39}
\end{align} 
The third term in \eqref{legend36} is computed using \eqref{legend25.1} and \eqref{legend33}, 
\begin{align}
q_{,\phi}^2 \partial_{qq}
%&=\left(\dfrac{i}{2}(\zeta-\overline{\zeta})\right)^2\dfrac{1}{\left(1+\zeta\overline{\zeta}\right)^2}\left(\eth^2\  + \overline{\eth}^2 + 2\overline{\eth}\eth -2\zeta \ \eth  -2\overline{\zeta}\ \overline{\eth}  \right) \\
&=-\dfrac{\left(\zeta-\overline{\zeta}\right)^2}{4\left(1+\zeta\overline{\zeta}\right)^2}\left(\eth^2\  + \overline{\eth}^2 + 2\overline{\eth}\eth -2\zeta \ \eth  -2\overline{\zeta}\ \overline{\eth}  \right).
\label{legend40}
\end{align}
The fourth term in \eqref{legend36} is obtained from \eqref{legend25.3}, \eqref{legend33} and \eqref{legend34}
\begin{align}
2q_{,\phi}p_{,\phi} \partial_{pq}
%&=2\left(\dfrac{i}{2}(\zeta-\overline{\zeta})\right)\left(\dfrac{1}{2}(\overline{\zeta}+\zeta)\right) \dfrac{i}{\left(1+\zeta\overline{\zeta}\right)^2}\left( \overline{\eth}^2 - \eth^2 + 2\zeta \ \eth - 2\overline{\zeta} \ \overline{\eth} \right)\\
&=- \dfrac{2\left(\zeta-\overline{\zeta}\right)\left(\overline{\zeta}+\zeta\right)}{4\left(1+\zeta\overline{\zeta}\right)^2}\left( \overline{\eth}^2 - \eth^2 + 2\zeta \ \eth - 2\overline{\zeta} \ \overline{\eth} \right).
\label{legend41}
\end{align}
The last term in \eqref{legend36} is computed from \eqref{legend25.2} and \eqref{legend34}
\begin{align}
p_{,\phi}^2\partial_{pp}&=-\dfrac{\left(\overline{\zeta}+\zeta\right)^2}{4\left(1+\zeta\overline{\zeta}\right)^2}\left( \eth^2 + \overline{\eth}^2 - 2\overline{\eth}\eth -2\overline{\zeta}\ \overline{\eth} -2\zeta\ \eth   \right).
\label{legend42}
\end{align}
The addition of \eqref{legend40} and \eqref{legend42} yields us to
\begin{align*}
q_{,\phi}^2 \partial_{qq}+p_{,\phi}^2\partial_{pp}
%&=-\dfrac{\left(\zeta-\overline{\zeta}\right)^2}{4\left(1+\zeta\overline{\zeta}\right)^2}\left(\eth^2\  + \overline{\eth}^2 + 2\overline{\eth}\eth -2\zeta \ \eth  -2\overline{\zeta}\ \overline{\eth}  \right)\\
%&-\dfrac{\left(\overline{\zeta}+\zeta\right)^2}{4\left(1+\zeta\overline{\zeta}\right)^2}\left( \eth^2 + \overline{\eth}^2 - 2\overline{\eth}\eth -2\overline{\zeta}\ \overline{\eth} -2\zeta\ \eth   \right)\\
%&=-\dfrac{1}{4\left(1+\zeta\overline{\zeta}\right)^2}\Bigg( \left(\zeta-\overline{\zeta}\right)^2 \left(\eth^2\  + \overline{\eth}^2 + 2\overline{\eth}\eth -2\zeta \ \eth  -2\overline{\zeta}\ \overline{\eth}  \right)\\
%&+\left(\overline{\zeta}+\zeta\right)^2\left( \eth^2 + \overline{\eth}^2 - 2\overline{\eth}\eth -2\overline{\zeta}\ \overline{\eth} -2\zeta\ \eth   \right)\Bigg)\\
=& -\dfrac{1}{4\left(1+\zeta\overline{\zeta}\right)^2}\Bigg( \left(\left(\zeta-\overline{\zeta}\right)^2 + \left(\overline{\zeta}+\zeta\right)^2 \right) \left(\eth^2\  + \overline{\eth}^2 -2\zeta \ \eth  -2\overline{\zeta}\ \overline{\eth}  \right)\\
&+2\left(\left(\zeta-\overline{\zeta}\right)^2 - \left(\overline{\zeta}+\zeta\right)^2 \right) \overline{\eth}\eth \Bigg),
\end{align*}
and summing to the last result \eqref{legend41} one obtains
\begin{align}
& q_{,\phi}^2 \partial_{qq}+p_{,\phi}^2\partial_{pp}+2q_{,\phi}p_{,\phi} \partial_{pq} \nonumber\\
%&=-\dfrac{1}{4\left(1+\zeta\overline{\zeta}\right)^2}\Bigg( \left(\left(\zeta-\overline{\zeta}\right)^2 + \left(\overline{\zeta}+\zeta\right)^2 \right) \left(\eth^2\  + \overline{\eth}^2 -2\zeta \ \eth  -2\overline{\zeta}\ \overline{\eth}  \right)\\
%& + 2\left(\zeta-\overline{\zeta}\right)\left(\overline{\zeta}+\zeta\right)\left( \overline{\eth}^2 - \eth^2 + 2\zeta \ \eth - 2\overline{\zeta} \ \overline{\eth} \right) +2\left(\left(\zeta-\overline{\zeta}\right)^2 - \left(\overline{\zeta}+\zeta\right)^2 \right) \overline{\eth}\eth \Bigg), \\
%&=-\dfrac{1}{4\left(1+\zeta\overline{\zeta}\right)^2}\Bigg( \left(\left(\zeta-\overline{\zeta}\right)^2 +2\left(\zeta-\overline{\zeta}\right)\left(\overline{\zeta}+\zeta\right) + \left(\overline{\zeta}+\zeta\right)^2 \right) \left(\overline{\eth}^2 -2\overline{\zeta}\ \overline{\eth}  \right)\\
%&+ \left( \left(\zeta-\overline{\zeta}\right)^2 - 2\left(\zeta-\overline{\zeta}\right)\left(\overline{\zeta}+\zeta\right) + \left(\overline{\zeta}+\zeta\right)^2\right)\left( \eth^2 - 2\zeta \ \eth  \right) \\
%&+2\left(\left(\zeta-\overline{\zeta}\right)^2 - \left(\overline{\zeta}+\zeta\right)^2 \right) \overline{\eth}\eth \Bigg)\\
%&=-\dfrac{1}{4\left(1+\zeta\overline{\zeta}\right)^2}\bigg( 4\zeta^2 \left(\overline{\eth}^2 -2\overline{\zeta}\ \overline{\eth}  \right) + 4\overline{\zeta}^2\left( \eth^2 - 2\zeta \ \eth  \right) -2\left(4\zeta\overline{\zeta} \right) \overline{\eth}\eth \bigg)\\
=&-\dfrac{\zeta^2 \left(\overline{\eth}^2 -2\overline{\zeta}\ \overline{\eth}  \right) + \overline{\zeta}^2\left( \eth^2 - 2\zeta \ \eth  \right) -2 \zeta\ \overline{\zeta}\   \overline{\eth}\eth}{\left(1+\zeta\overline{\zeta}\right)^2}.
\label{legend43}
\end{align}
Thus, substituting \eqref{legend39} and \eqref{legend43} into \eqref{legend36} is obtained
\begin{align}
\partial_{\phi\phi}
%&= q_{,\phi\phi}\partial_q + p_{,\phi\phi}\partial_p + q_{,\phi}^2 \partial_{qq} + 2q_{,\phi}p_{,\phi} \partial_{pq} + p_{,\phi}^2\partial_{pp},\nonumber\\
%&=- \dfrac{ \left(\overline{\zeta}\ \eth + \zeta\ \overline{\eth}\right) \left(1+\zeta\overline{\zeta}\right)}{\left(1+\zeta\overline{\zeta}\right)^2} -\dfrac{1}{\left(1+\zeta\overline{\zeta}\right)^2}\bigg( \zeta^2 \left(\overline{\eth}^2 -2\overline{\zeta}\ \overline{\eth}  \right) + \overline{\zeta}^2\left( \eth^2 - 2\zeta \ \eth  \right) -2 \zeta\ \overline{\zeta}\   \overline{\eth}\eth \bigg)\\
%&=-\dfrac{1}{\left(1+\zeta\overline{\zeta}\right)^2}\left( \left(\overline{\zeta}\ \eth + \zeta\ \overline{\eth}\right) \left(1+\zeta\overline{\zeta}\right) +\bigg( \zeta^2 \left(\overline{\eth}^2 -2\overline{\zeta}\ \overline{\eth}  \right) + \overline{\zeta}^2\left( \eth^2 - 2\zeta \ \eth  \right) -2 \zeta\ \overline{\zeta}\   \overline{\eth}\eth \bigg)\right),\nonumber \\
&=-\dfrac{\overline{\zeta}\ \eth + \zeta\ \overline{\eth}  +  \zeta^2 \left(\overline{\eth}^2 -\overline{\zeta}\ \overline{\eth}  \right) + \overline{\zeta}^2\left( \eth^2 - \zeta \ \eth  \right) -2 \zeta\ \overline{\zeta}\   \overline{\eth}\eth}{\left(1+\zeta\overline{\zeta}\right)^2}.
\label{legend44}
\end{align}
With these results we will compute the explicit form, in terms of the $\overline{\eth}$ and $\eth$ operators, of the Legendrian given in \eqref{legend9}. Thus its first term is computed directly from \eqref{legend10} and \eqref{legend19}
\begin{align}
\dfrac{1}{\tan\theta}\partial_\theta
%&=\dfrac{1-\zeta\overline{\zeta}}{8 \left(\zeta\overline{\zeta}\right)} \left(\left(\zeta+\overline{\zeta}\right)\left(\eth+\overline{\eth}\right) + \left(\zeta-\overline{\zeta}\right)\left(\overline{\eth}-\eth\right)\right) \\
%&=\dfrac{1-\zeta\overline{\zeta}}{8 \left(\zeta\overline{\zeta}\right)} \left( \left(\zeta+\overline{\zeta}\right)\eth+\left(\zeta+\overline{\zeta}\right)\overline{\eth}  +  \left(\zeta-\overline{\zeta}\right)\overline{\eth}-\left(\zeta-\overline{\zeta}\right)\eth \right) \\
&=\dfrac{4 \left( \overline{\zeta}\ \eth-\zeta\overline{\zeta}^2\ \eth + \zeta\ \overline{\eth}-\zeta^2\overline{\zeta} \ \overline{\eth}  \right)}{16  \zeta\overline{\zeta} }. 
\label{legend45}
\end{align}
Also, using \eqref{legend11} and \eqref{legend44}, the third term in \eqref{legend9} is
\begin{align}
\dfrac{1}{\sin^2\theta}\partial_{\phi\phi}
%&=  \left(- \dfrac{\left(1+\zeta\overline{\zeta}\right)^2}{4\zeta\overline{\zeta}} \dfrac{1}{\left(1+\zeta\overline{\zeta}\right)^2}\left(    \overline{\zeta}\ \eth + \zeta\ \overline{\eth}  +  \zeta^2 \left(\overline{\eth}^2 -\overline{\zeta}\ \overline{\eth}  \right) + \overline{\zeta}^2\left( \eth^2 - \zeta \ \eth  \right) -2 \zeta\ \overline{\zeta}\   \overline{\eth}\eth  \right)\right) \\
&= - \dfrac{\overline{\zeta}\ \eth + \zeta\ \overline{\eth}  +  \zeta^2 \left(\overline{\eth}^2 -\overline{\zeta}\ \overline{\eth}  \right) + \overline{\zeta}^2\left( \eth^2 - \zeta \ \eth  \right) -2 \zeta\ \overline{\zeta}\   \overline{\eth}\eth }{4\zeta\overline{\zeta}} .
\label{legend46}
\end{align}
Then substituting \eqref{legend31}, \eqref{legend45} and \eqref{legend46},
\begin{align}
\mathcal L^2 %&=\dfrac{1}{\tan\theta}\partial_\theta +\partial_{\theta\theta}+\dfrac{1}{\sin^2\theta}\partial_{\phi\phi}, \nonumber\\
%&=\dfrac{4 \left( \overline{\zeta}\ \eth-\zeta\overline{\zeta}^2\ \eth + \zeta\ \overline{\eth}-\zeta^2\overline{\zeta} \ \overline{\eth}  \right)}{16  \zeta\overline{\zeta} } + \dfrac{1}{16\zeta\overline{\zeta}}\Bigg( 4 \zeta^2 \overline{\eth}^2 +4 \overline{\zeta}^2   \eth^2  %\\ &
%+8 \zeta\overline{\zeta}  \eth\overline{\eth}  \Bigg) \nonumber\\
%& - \dfrac{4}{16\zeta\overline{\zeta}} \left(    \overline{\zeta}\ \eth + \zeta\ \overline{\eth}  +  \zeta^2 \left(\overline{\eth}^2 -\overline{\zeta}\ \overline{\eth}  \right) + \overline{\zeta}^2\left( \eth^2 - \zeta \ \eth  \right) -2 \zeta\ \overline{\zeta}\   \overline{\eth}\eth  \right) \\
&=\dfrac{4}{16\zeta\overline{\zeta}} \left( \overline{\zeta}\ \eth-\zeta\overline{\zeta}^2\ \eth + \zeta\ \overline{\eth}-\zeta^2\overline{\zeta} \ \overline{\eth}  \right)  + \dfrac{1}{16\zeta\overline{\zeta}}\Bigg( 4 \zeta^2 \overline{\eth}^2 +4 \overline{\zeta}^2   \eth^2  %\\ &
+8 \zeta\overline{\zeta}  \eth\overline{\eth}  \Bigg) \nonumber\\
& - \dfrac{4}{16\zeta\overline{\zeta}} \left(    \overline{\zeta}\ \eth + \zeta\ \overline{\eth}  +  \zeta^2 \left(\overline{\eth}^2 -\overline{\zeta}\ \overline{\eth}  \right) + \overline{\zeta}^2\left( \eth^2 - \zeta \ \eth  \right) -2 \zeta\ \overline{\zeta}\   \overline{\eth}\eth  \right), \nonumber\\
&=  \eth\overline{\eth}.  
\label{legend47}
\end{align}
The last implies that, the eigenvalue equation \eqref{legend8} can be written as
\begin{equation}
\eth\overline{\eth}Y_{lm}=-l(l+1)Y_{lm}.
\label{legend48}
\end{equation}
We appoint here that the functional dependence of the spherical harmonics was not written. This was made intentionally because the last is valid independently of the coordinate system selected. But, there are two ways to make this completely consistent. One of these is expressing the operators $\eth$ and $\overline{\eth}$ in spherical coordinates in which case the operator $\eth\overline{\eth}$ would act in those coordinate system. The other way is to express the spherical harmonics in stereographic coordinates. The last implies compute the explicit form for the associated Legendre polynomials which enable us to make this kind of transformation.
%then, multiplying at the left in both sides of the equation by the matrix inverse,  are obtained that
%\begin{equation}
%\begin{pmatrix}
%\partial_q \\
%\partial_p
%\end{pmatrix} = \dfrac{1}{q_{,\theta}p_{,\phi}-q_{,\phi}p_{,\theta}}\begin{pmatrix}
%p_{,\phi} & -p_{,\theta} \\
%-q_{,\phi} & q_{,\theta}  
%\end{pmatrix}
%\begin{pmatrix}
%\partial_\theta \\
%\partial_\phi
%\end{pmatrix}
%\end{equation}
%with this, \eqref{legend48} takes the form
%\begin{align*}
%\eth %&=\dfrac{1+\zeta\overline{\zeta}}{2}\left(\partial_{q}+i\partial_{p}\right)+s\zeta %\\
%%&= \dfrac{1+\tan^2\left(\theta/2\right)}{2\left(q_{,\theta}p_{,\phi}-q_{,\phi}p_{,\theta}\right)}\left(\left(p_{,\phi}\partial_{\theta}-p_{\theta}\partial_{\phi}\right)+i\left(-q_{,\phi}\partial_{\theta}+q_{\theta}\partial_{\phi}\right)\right) +s\tan(\theta/2)e^{i\phi}\\
%&= \dfrac{1+\tan^2\left(\theta/2\right)}{2\left(q_{,\theta}p_{,\phi}-q_{,\phi}p_{,\theta}\right)}\left(\left(p_{,\phi}-iq_{,\phi}\right)\partial_{\theta}  +\left(-p_{,\theta}+iq_{,\theta}\right)\partial_{\phi}\right) +s\tan(\theta/2)e^{i\phi}
%%\label{legend48}
%\end{align*}
%%where
%%\begin{align*}
%%q_{,\theta}p_{,\phi}-q_{,\phi}p_{,\theta}
%%%\\
%%%&= \left(\dfrac{\sec^2(\theta/2)\tan(\theta/2) \left(e^{i\phi}+e^{-i\phi}\right)^2}{2(4)}\right)  - \left(\dfrac{\tan(\theta/2)\sec^2(\theta/2) \left(e^{i\phi} - e^{-i\phi}\right)^2}{2(4)}\right) \\
%%%&=  \dfrac{\sec^2(\theta/2)\tan(\theta/2) }{2(4)} \left(\left(e^{i\phi}+e^{-i\phi}\right)^2  - \left(e^{i\phi} - e^{-i\phi}\right)^2\right) \\
%%&=  \dfrac{\sec^2(\theta/2)\tan(\theta/2) }{2 }  
%%\end{align*}
%%\begin{equation*}
%%p_{,\phi}-iq_{,\phi}=\tan(\theta/2)
%%\end{equation*}
%%and
%%\begin{align*}
%%-p_{,\theta}+iq_{,\theta}&=\left(\dfrac{i}{4}\sec^2(\theta/2)(e^{i\phi}-e^{-i\phi})\right)+i\left(\dfrac{1}{4}\sec^2(\theta/2)(e^{i\phi}+e^{-i\phi})\right) \\
%%&=\dfrac{i}{2}\sec^2(\theta/2) e^{i\phi} 
%%\end{align*}
%%then
%%\begin{align*}
%%\eth &= \dfrac{1}{ \tan(\theta/2) }\left(\tan(\theta/2)\partial_{\theta}  +i\left(\dfrac{1}{2}\sec^2(\theta/2) e^{i\phi}\right)\partial_{\phi}\right) +s\tan(\theta/2)e^{i\phi} \\
%%&= \left(\partial_{\theta}  +i \dfrac{\sec^2(\theta/2) e^{i\phi}}{2\tan(\theta/2)}\partial_{\phi}\right) +s\tan(\theta/2)e^{i\phi}\\
%%&= \partial_{\theta}  +i \dfrac{e^{i\phi}}{\sin \theta }\partial_{\phi} +s\tan(\theta/2)e^{i\phi}
%%%\label{legend48}
%%\end{align*}
%
%%\begin{equation}
%%\partial_q=\dfrac{\left(p_{,\phi}\partial_{\theta}-p_{\theta}\partial_{\phi}\right)}{q_{,\theta}p_{,\phi}-q_{,\phi}p_{,\theta}}
%%\end{equation}
%%\begin{equation}
%%\partial_p=\dfrac{\left(-q_{,\phi}\partial_{\theta}+q_{\theta}\partial_{\phi}\right)}{q_{,\theta}p_{,\phi}-q_{,\phi}p_{,\theta}}
%%\end{equation}
%%where
%%\begin{equation}
%%\begin{pmatrix}
%%q_{,\theta} & p_{,\theta} \\
%%q_{,\phi} & p_{,\phi} 
%%\end{pmatrix}^{-1}=\dfrac{1}{q_{,\theta}p_{,\phi}-q_{,\phi}p_{,\theta}}\begin{pmatrix}
%%p_{,\phi} & -p_{,\theta} \\
%%-q_{,\phi} & q_{,\theta}  
%%\end{pmatrix}
%%\end{equation} 
%%Thus, the eigenvalue equation for the usual spherical harmonics \eqref{legend8} can be rewritten as
%%\begin{equation}
%%\eth\overline{\eth}Y_{lm}=-l(l+1)Y_{lm}
%%\end{equation}

==> docs/linear_regime.tex <==
\chapter{LINEAR REGIME OF THE EINSTEIN'S FIELD EQUATIONS AND GRAVITATIONAL WAVES}
This chapter is dedicated to explore the linear regime of the Einstein's field equations and the prediction of the gravitational waves. Commonly, the linearisation of the Einstein's field equations is performed assuming a flat background which allow to make good estimative on the source features \cite{B07,C101,C102,C103}. However, it turns inapplicable to the cases in which strong fields are involved. Eisenhart in 1926 and Komar in 1957 make perturbations to the metric tensor at the first order showing how the gravitational waves are propagated away to the sources \cite{RW57}. \citeonline{RW57} performed slight perturbations in a spherical symmetric space-time to explore the stability of the Schwarzschild's solution,  obtaining a radial wave equation in presence of an effective gravitational potential, namely the {\it Reege-Wheeler equation}, which appears for odd-parity perturbations. \citeonline{Z70} made even-parity perturbations obtaining a different radial wave equation, namely the {\it Zerilli equation} obeying a different effective potential. After this, by using the vector and tensor harmonics, Moncrief extend the Zerilli works to the Reissner-Nordstr\"om exterior space-time and to stellar models by using a perfect fluid stress-energy tensor \cite{M74_I,M74_II,M74_III,M74_IV}. \citeonline{BH64} explored the stability of the {\it Geons}, which are objects composed by electromagnetic fields held together by gravitational attraction, in the linear regime of the field equations, off the flat assumption, but considering spherical symmetry and an asymptotically flat space-time.  Isaacson found a generalisation to the gravitational wave equation when an arbitrary background is considered. He proved that the gravitational waves for high an lower frequencies are founded by performing perturbation to distinct orders in the metric tensor \cite{I68_1,I68_2}. Here some of the aspects in the linearisation approximation to first and higher order are examined. Through the Wentzel-Kramers-Brillouin approximation (WKB) the eikonal equation is founded relating the tensor of amplitudes for the metric perturbations with its propagation vector. %Some simple questions related to the eikonal equation are raised. 
After this, in the Minkowski's background the gravitational waves are expressed in terms of the Green's functions. Using this, a multipolar expansion is made as usual. Finally, the quadrupole radiation formula is treated with some detail.  
\input{./docs/first_order_perturbations}
\input{./docs/high_order_perturbations}
%\section{Green Functions}
%\section{Multipolar Expansion}
%\section{Quadrupole Radiation Formula}










==> docs/non_linear_regime.tex <==
\chapter{THE INITIAL VALUE PROBLEM AND THE NONLINEAR REGIME OF THE EINSTEIN'S FIELD EQUATIONS}
Here will be shown briefly the meaning of the initial value problem (IVP) in the context of the general relativity and the different formulations that there are in the literature to study this. In essence there are two distinct formulation, the first of them the ADM formulations or $3+1$ are characterised by a decomposition of the space-time in space-like hypersurfaces, whereas in the other are used the characteristic hypersurfaces to the differential partial equations which result in null cones. These cones can be oriented to the past, to the future or in both directions. In particular, special attention will be given to the characteristic formulation based in null cones oriented to the future. 
\\This chapter will be present as follows, first it be shown the initial value problem, after this, some of the ADM formulations will be presented briefly and finally some of the principal aspects of the outgoing characteristic formulation will be recast in this presentation. 
\section{The Initial Value Problem}
The initial value problem (IVP) consist essentially in the evolution of a metric $g_{\mu\nu}$ and its first derivatives $g_{\mu\nu,\gamma}$ which are specified in an initial ($t=t_0$) three dimensional hypersurface. The evolution of the space-time is then performed using the field equations;  in some cases the matter sources are evolved from the conservation laws.  
\input{./docs/ADM}
\input{./docs/Characteristic}


==> docs/non_linear_regime_eth.tex <==
\section{The Einstein's field equations using the eth formalism}
When the eth formalism is used, the field equations taken the following form
\begin{subequations}
\begin{align}
\beta_{,r}&=N_\beta,\\
U_{,r}&=r^{-2}e^{2\beta}Q+N_U,\\
\left(r^2Q\right)_{,r}&=-r^2\left(\overline{\eth}J+\eth K\right)_{,r}+2r^4\eth\left(r^{-2}\beta\right)_{,r}+N_Q,\\
w_{,r}&=\dfrac{e^{2\beta}}{2}\mathcal{R}-1-e^{\beta}\eth \overline{\eth}e^{\beta}+\dfrac{r^{-2}}{4}\left(r^4\left(\eth \overline{U}+\overline{\eth} U\right)\right)_{,r}+N_w,
\end{align}
\end{subequations}
where the Ricci's scalar associated to $h_{AB}$ take the form
\begin{equation}
\mathcal{R}=2K-\eth\overline{\eth}K+\dfrac{\overline{\eth}^2J+\eth^2\overline{J}}{2}+\dfrac{\overline{\eth}\overline{J}\eth J -\overline{\eth}J\eth \overline{J} }{4K}.
\end{equation}
The evolution equation reads
\begin{align}
 2\left(rJ\right)_{,ur}-\left(r^{-1}(r+W)\left(rJ\right)_{,r}\right)_{,r}=&-r^{-1}\left(r^2\eth U\right)_{,r} + 2r^{-1}e^\beta\eth^2e^{\beta} \nonumber\\
&-\left(r^{-1}w\right)_{,r}J+N_J,
\end{align}
where
\begin{subequations}
	\begin{align}
N_\beta&=\dfrac{r\left(J_{,r}\overline{J}_{,r}-K_{,r}^2\right)}{8},\\
N_U&=\dfrac{e^{2\beta}\left(KQ-Q-J\overline{Q}\right)}{r^2},\\
N_Q&=r^2\left((1-K)\left(\eth K_{,r}+\overline{\eth}J_{,r}\right)+\eth\left(\overline{J}J_{,r}\right)+\overline{\eth}\left(JK_{,r}\right)-J_{,r}\overline{\eth}K\right)\nonumber\\
&+\dfrac{r^2}{2K^2}\left(\eth \overline{J}\left(J_{,r}-J^2\overline{J}_{,r}\right)+\overline{\eth}J\left(\overline{J}_{,r}-\overline{J}^2J_{,r}\right)\right),\\
N_w&=e^{2\beta}\left((1-K)\left(\eth\overline{\eth}\beta+\eth\beta\overline{\beta}\right)+\dfrac{J\left(\overline{\eth}\beta\right)^2+\overline{J}\left(\eth\beta\right)^2}{2}\right)\nonumber\\
&-\dfrac{e^{2\beta}}{2}\left(\eth\beta\left(\overline{\eth}K-\eth\overline{J}\right)+\overline{\eth}\beta\left(\eth K-\overline{\eth}J\right)\right)+\dfrac{e^{2\beta}}{2}\left(J\overline{\eth}^2\beta+\overline{J}\eth^2\beta\right)\nonumber\\
&-\dfrac{e^{-2\beta}r^4}{8}\left(2KU_{,r}\overline{U}_{,r}+J\overline{U}^2_{,r}+\overline{J}U^2_{,r}\right),\\
N_J&=\sum_{i=1}^{7}N_{Ji}+\dfrac{J\sum_{n=1}^{4}P_n}{r},
\end{align}
\end{subequations}
where
\begin{subequations}
\begin{align}
N_{J1}=&-\dfrac{e^{2\beta}}{r}\left(K\left(\eth J \overline{\eth}\beta+2\eth K \eth\beta-\overline{\eth}J\eth\beta\right)+J\left(\overline{\eth}J-2\eth K\right)\overline{\eth}\beta\right.\nonumber\\
&-\left.\overline{J}\eth J \eth\beta\right),\\
N_{J2}=&-\dfrac{\left(\eth J\left(r^2\overline{U}\right)_{,r}+\overline{\eth} J\left(r^2U\right)_{,r}\right)}{2r},\\
N_{J3}=&\dfrac{\left(1-K\right)\eth\left(r^2U\right)_{,r}-J\eth\left(r^2\overline{U}\right)_{,r}}{r},\\
N_{J4}=&\dfrac{r^3e^{-2\beta}\left(K^2U^2_{,r}+2JKU_{,r}\overline{U}_{,r}+J^2\overline{U}^2_{,r}\right)}{2},\\
N_{J5}=&-\dfrac{rJ_{,r}\left(\overline{\eth}U+\eth\overline{U}\right)}{2},\\
N_{J6}=&\dfrac{r\left(\overline{U}\eth J + U\overline{\eth}J\right)\left(J\overline{J}_{,r}-\overline{J}J_{,r}\right)}{2} +r\left(JK_{,r}-KJ_{,r}\right)\overline{U}\overline{\eth}J\nonumber\\
&-r\overline{U}\left(\eth J_{,r}-2K\eth H J_{,r}+2J\eth K K_{,r}\right)-rU\left(\overline{\eth}J_{,r}-K\eth \overline{J} J_{,r}+J\eth \overline{J}K_{,r}\right),\\
N_{J7}=&r\left(J_{,r}K-JK_{,r}\right)\left(\overline{U}\left(\overline{\eth}J-\eth K\right)+U\left(\overline{\eth}K-\eth\overline{J}\right)\right.\nonumber\\
&\left.+K\left(\overline{\eth}U-\eth\overline{U}\right)+\left(J\overline{\eth}\overline{U}-\overline{J}\eth U\right)\right),
\end{align}
\end{subequations}
\begin{subequations}
\begin{align}
P_1&=\dfrac{r^2\left(J_{,u}\left(\overline{J}K\right)_{,r}+\overline{J}_{,u}\left(JK\right)_{,r}\right)}{K}-8V\beta_{,r},\\
P_2&=e^{2\beta}\left(-2K\left(\eth\overline{\eth}\beta+\overline{\eth}\beta\eth\beta\right)-\left(\overline{\eth}\beta\eth K+\eth\beta\overline{\eth}K\right)\right.\nonumber\\
&\left.+J\left(\overline{\eth}^2\beta+(\overline{\eth}\beta)^2\right)+\overline{J}\left(\eth^2\beta+(\overline{\eth}\beta)^2\right)+\overline{\eth}J\overline{\eth}\beta+\eth \overline{J}\eth\beta\right),\\
P_3&=\dfrac{\overline{\eth}\left(r^2U\right)_{,r}+\eth\left(r^2\overline{U}\right)_{,r}}{2},\\
P_4&=-\dfrac{r^4e^{-2\beta}\left(2KU_{,r}\overline{U}_{,r}+J\overline{U}^2_{,r}+\overline{J}U^2_{,r}\right)}{4},
\end{align}
\end{subequations}



==> docs/simbolos.tex <==
\begin{simbolos}
\hypertarget{estilo:simbolos}{}
\\
Greek indices $\alpha,\beta,\gamma,\cdots$ &--& run from 1 to 4\\
Capital Latin indices $A,B,C,\cdots$ &--& run from 3 to 4\\
Upper indices $(i),\ i=0,1,2,\cdots$ &--& Indicates the perturbation order\\
$G_{\mu\nu}$   &--& Einstein's tensor \\
$T_{\mu\nu}$   &--& Stress-energy tensor \\
$R_{\mu\nu}$   &--& Ricci's tensor \\
$R_{\mu\nu\gamma\delta}$  &--& Riemann's tensor of type $(0,4)$\\
$R^\mu_{~\nu\delta\gamma}$  &--& Riemann's tensor of type $(1,3)$\\
$_{,\alpha}$ or $\partial_\alpha$   &--& Partial derivative\\
$_{;\alpha}$ or $\nabla_\alpha$  &--& Covariant derivative\\
$_{:\alpha}$ or $\overset{\hspace{-0.2cm}(0)}{\nabla_\alpha}$  &--& Covariant derivative referred to the background\\
$\Gamma_{\alpha\beta\gamma}$ &--& Christoffel's symbols of the first kind\\
$\Gamma^\alpha_{~\beta\gamma}$ &--& Christoffel's symbols of the second kind\\
$_{|A}$ or $\triangle_A$  &--& Covariant derivative referred to $q_{AB}$\\
$_{\|A}$ or $\nabla_A$&--& Covariant derivative referred to $h_{AB}$\\
$q^A$ &--& Dyads related to the vectors in $T_p\mathcal{S}$\\
$\mathcal{L}$ &--& Legendrian operator\\
$\eth$ &--& Eth operator\\
$\overline{\eth}$ &--& Eth bar operator\\
$_sY_{lm}$ &--& Spin-weighted spherical harmonic\\
$_sZ_{lm}$ &--& Spin-weighted spherical harmonic\\
\end{simbolos}


==> docs/spin_weighted_scalars.tex <==
\section{Spin-weighted Scalars and Spin-weight}
Here, will be shown that any tensor field of rank $2$ of type $(0,2)$, namely $\omega_{AB}$, in the tangent space of the unit sphere admits a irreducible decomposition in spin-weighted functions. In order to show that, it is first considered that $\omega_{AB}$, can be decomposed into its symmetric and anti-symmetric part, i.e.,
\begin{equation}
\omega_{AB}=\omega_{(AB)}+ \omega_{[AB]}.
\label{spinscalars1}
\end{equation}
The symmetric part can be separated in two parts, one trace-free and other corresponding to its trace, 
\begin{equation}
\omega_{(AB)}=t_{AB}+\dfrac{q_{AB}}{2}\omega,
\label{spinscalars2}
\end{equation}
where $t=q^{AB}t_{AB}=0$, i.e., $t_{AB}$ is the trace-free symmetric part of $\omega_{AB}$, and the second term is its trace, i.e., 
\begin{align}
\omega&=\omega_{AB}q^{AB},\nonumber\\
&=2\omega_{AB}q^{(A}\overline{q}^{B)}. 
\label{spinscalars3}
\end{align}
In this manner, $\omega_{AB}$ can be written as
\begin{equation}
\omega_{AB}=t_{AB}+\dfrac{q_{AB}}{2}\omega+ \omega_{[AB]}.
\label{spinscalars4}
\end{equation}
The anti-symmetric part can be expressed as
\begin{align*}
\omega_{[AB]}&=\omega_{CD}\delta^C_{~~[A}\delta^D_{~~B]},\nonumber\\
&=\dfrac{\omega_{CD}}{2}\left(\delta^C_{~~A}\delta^D_{~~B}-\delta^C_{~~B}\delta^D_{~~A}\right),\nonumber
\end{align*}
where using \eqref{decomposition5}
\begin{align*}
\omega_{[AB]}
&=\dfrac{\omega_{CD}}{2}\left(\overline{q}^{(C}q_{A)}\overline{q}^{(D}q_{B)}-\overline{q}^{(C}q_{B)}\overline{q}^{(D}q_{A)}\right),\nonumber\\
&=\dfrac{1}{4}\dfrac{\omega_{CD}}{2}\Bigg(\left(\overline{q}_{A}q_{B}-q_{A}\overline{q}_{B}\right)\left(q^{C}\overline{q}^{D}-\overline{q}^{C}q^{D}\right)\Bigg),\nonumber
\label{spinscalars5}
\end{align*}
i.e.,
\begin{equation}
\omega_{[AB]}=\dfrac{1}{2}\overline{q}_{[A}q_{B]}u,
\label{spinscalars6}
\end{equation}
where,
\begin{equation}
u=\omega_{CD}q^{[C}\overline{q}^{D]}.
\label{spinscalars7}
\end{equation}
For this reason, \eqref{spinscalars4} can be written as
\begin{equation}
\omega_{AB}=t_{AB}+\dfrac{\omega}{2}q_{AB}+ \dfrac{1}{2}\overline{q}_{[A}q_{B]}u.
\label{spinscalars8}
\end{equation}
Here, it is important to notice that $\omega$ and $u$ are scalar functions with spin weight zero, as given in \eqref{spinscalars3} and \eqref{spinscalars7} respectively. The symmetric traceless part, $t_{AB}$ admit a irreducible decomposition in scalar spin-weighted functions as follow,
\begin{equation}
I=t_{AB}q^Aq^B, \hspace{1cm} L=t_{AB}\overline{q}^A\overline{q}^B, \hspace{1cm} S=t_{AB}\overline{q}^Aq^B,
\label{spinscalars9}
\end{equation}
where, if is considered that $t_{AB} \in \mathbb{R}$, then $L=\overline{I}$, and $S=\overline{S}$.
\\In this form, any tensor field of type $(0,2)$, saying $\omega_{AB}$, is completely determined by a linear combination of spin-weighted scalar fields of weight $0$, $2$ and $-2$. In general, it is possible to construct spin-weighted scalars from tensor fields into the tangent space to the unitary sphere, in the form
\begin{equation}
_s\Psi=\prod_{i=1}^{n}q_{A_i} \prod_{j=n+1}^{r}\overline{q}_{A_{j}}\prod_{k=1}^{m}q^{B_k}\prod_{l=m+1}^{\tilde{s}}\overline{q}^{B_l} \Psi^{A_1\cdots A_n A_{n+1}\cdots A_r}_{\hspace{2.3cm}B_1\cdots B_m B_{m+1}\cdots B_{\tilde{s}}}.
\label{spinscalars10}
\end{equation}
Then, it is possible to compute the spin-weight of $_s\Psi$ taking advantage of \eqref{spin12}. Considering the above expression for the north or south hemisphere, and making the transformation from one region to the another, one obtains that the spin-weight for the $_s\Psi$ function is,
\begin{equation}
s=2(n+m)-r-\tilde{s}.
\label{spinscalars11}
\end{equation}

==> docs/stereo_coordinates.tex <==
\section{Stereographic Coordinates}
This section starts with the description of the construction of the stereographic atlas which covers the entire sphere. As an example, a point (in green) in the equatorial plane is projected to the north hemisphere from the south pole as sketched in the Figure \ref{fstereo1}
\begin{figure}[h!]
\begin{center}		
	\vspace{-1.5cm}
\begin{tabular}{cc}
\includegraphics[height=10cm]{./Figuras/stereographic/stereo1}&\begin{minipage}{10cm}
\vspace{-11cm}\hspace{-1cm}\includegraphics[height=6cm]{./Figuras/stereographic/stereo2}
\end{minipage}	
\end{tabular}
\end{center}
\vspace{-1.5cm}
\caption{Stereographic coordinates construction: The equatorial plane is projected from the south pole to the unit sphere surface. The interior points to the equator are projected to the north hemisphere, whereas the exterior points are projected to the south.}
\label{fstereo1}
\end{figure}
The coordinates in the equatorial plane (the green point) have been represented as having coordinates $(q,p)$ and the point to be represented in the sphere $P$ as having coordinates $(x,y,z)$. From the Figure \ref{fstereo1},
\begin{equation}
\rho=\tan\left(\frac{\theta}{2}\right), \hspace{1cm} q=\rho\cos\phi,\hspace{1cm} p=\rho\sin\phi.
\label{stereo1}
\end{equation}
Then, it is possible to represent the coordinates through a complex quantity $\zeta$, in the form
\begin{equation}
\zeta=\tan\left(\dfrac{\theta}{2}\right)e^{i\phi}.
\label{stereo2}
\end{equation}
In this manner, $\Re(\zeta)=q$ and $\Im(\zeta)=p$. It is worth stressing to note that it is not possible to map the all points in the sphere surface into the equatorial plane, even if the plane is extended to the infinity. Thus it is necessary to appeal to almost two coordinate charts. One possible way to do this, is by selecting one for each hemisphere, north $(N)$ and south $(S)$ as
\begin{equation}
\zeta_N=\tan\left(\dfrac{\theta}{2}\right)e^{i\phi}, \hspace{1cm}\zeta_S=\cot\left(\dfrac{\theta}{2}\right)e^{-i\phi}, \hspace{1cm} \zeta_{N\atop S}=q_{N\atop S}+ip_{N\atop S}.
\label{stereo3}
\end{equation}
such that
\begin{equation}
|q_{N}|\le 1, \hspace{1cm} |p_{N}|\le 1. 
\label{stereo4}
\end{equation}
which defines a rectangular domain in the plane to be mapped  into the sphere.
\\From the definition \eqref{stereo1}, it is observed immediately that
\begin{equation}
q=\tan\left(\frac{\theta}{2}\right)\cos\phi,\hspace{1cm} p=\tan\left(\frac{\theta}{2}\right)\sin\phi,
\label{stereo5}
\end{equation}
and taken into account
\begin{align}
\tan\left(\frac{\theta}{2}\right)&=\frac{\sin\theta}{2}\left(1+\tan^2\left(\frac{\theta}{2}\right)\right),
\label{stereo6}
\end{align}
then, the relationship between the rectangular and the $q,p$ is established
\begin{equation}
x=\frac{2q}{1+q^2+p^2},\hspace{1cm}y=\frac{2p}{1+q^2+p^2}.
\label{stereo7}
\end{equation}
This allows to write the $z$ coordinate as
\begin{align}
z&=\cos\theta,\nonumber\\
&=\cos^2\left(\frac{\theta}{2}\right)\left(1-\tan^2\left(\frac{\theta}{2}\right)\right),\nonumber\\
&=\frac{1-q^2-p^2}{1+q^2+p^2}.
\label{stereo8}
\end{align} 
With the equations \eqref{stereo7} and \eqref{stereo8} the coordinate lines $(q,p)$ into the sphere surface are constructed, as shown in the figure \ref{fig:stereo1}.
\begin{figure}[h!]
\begin{center}
\vspace{-1.5cm}
\includegraphics[height=10cm]{./Figuras/stereographic/stereo3}
\vspace{-1.5cm}
\end{center}	
\caption{Coordinate atlas in the sphere. Coordinate lines as result of the mapping of the plane maps contructed from the equator of the sphere.}
\label{fstereo2}
\end{figure}
\\It shows how is constructed the atlas $\{\{q_N,p_N\},\{q_S,p_S\}\}$ for the unit sphere. 
\\From \eqref{stereo3}, for all points except the poles,
\begin{align}
\zeta_N % %&=\dfrac{1}{\cot\left(\dfrac{\theta}{2}\right)e^{-i\phi}}\nonumber\\
&=\dfrac{1}{\zeta_S},
\label{stereo9}
\end{align}
or,
\begin{align}
\zeta_N&=\dfrac{\bar{\zeta_S}}{\zeta_S\bar{\zeta_S}}.
\label{stereo10}
\end{align}
In terms of the $q$ and $p$ coordinates, the \eqref{stereo10} yield us to
\begin{align}
q_N=\dfrac{q_S}{q_S^2+p_S^2}, \hspace{1cm} p_N=\dfrac{-p_S}{q_S^2+p_S^2},
\label{stereo11}
\end{align}
which defines the relationship between the north and south coordinates. This corresponds to the transformation between the coordinate maps, north and south. Thus, the form of the coordinate lines $(q_N,p_N)$, corresponding to the north map when $p_S$ or $q_S$ are considered as constant, can be traced. It is particularly useful when a discretisation scheme of the angular operators in the sphere is implemented, because it shows clearly that a bi-dimensional interpolation is needed to pass information from one to the another coordinate map. We make a simple plot to show the behaviour of these coordinate lines for  different values. It draws how to the lines for $q_S$ or $p_S$ constants in the north hemisphere are mapped.
\begin{figure}[h!]
	\begin{center}
			\includegraphics[height=8cm]{./Figuras/stereographic/stereo4}
	\end{center}
	\caption{Coordinate lines of north hemisphere into the south region. The equatorial line is indicated as a circle in black.
		}
	\label{fig:stereo1}
\end{figure}

==> docs/tangent_vectors_spin_weight.tex <==
\section{Transformation Rules for the Dyads and Spin-weigth}
Any vector field $\boldsymbol{v}$ can be expanded in terms a basis of one-forms $\boldsymbol{e}_A$, explicitly $\boldsymbol{v}=v^A\boldsymbol{e}_A$. Thus, for each hemisphere
\begin{equation}
\boldsymbol{v}_N=v^A_N\boldsymbol{e}_{A_N}, \hspace{1cm}\boldsymbol{v}_S=v^A_S\boldsymbol{e}_{A_S}.
\label{spin1}
\end{equation}
In particular for a local coordinate basis $\{\partial_{A_N}\}$ and $\{\partial_{A_S}\}$, the complex vectors $\boldsymbol{q}_N$ and $\boldsymbol{q}_S$ can be expressed as the linear combinations
\begin{equation}
\boldsymbol{q}_N=q^A_N\partial_{A_N}, \hspace{1cm}\boldsymbol{q}_S=q^A_S\partial_{A_S}.
\label{spin2}
\end{equation}
Using the explicit expression for the dyads components $q_N^A$ given in \eqref{decomposition10}, \eqref{spin2} take the explicit form
\begin{align}
\boldsymbol{q}_N&=\dfrac{\left(1+\zeta\overline{\zeta}\right)}{2}\left(\delta^A_{~~3}+i\delta^A_{~~4}\right)\partial_{A_N},\nonumber\\
&=\dfrac{\left(1+\zeta_N\overline{\zeta}_N\right)}{2}\left(\partial_{q_N}+i\partial_{p_N}\right).
\label{spin3}
\end{align}
Then, transforming the basis in \eqref{spin3}, using for this \eqref{diff4}, leads to
\begin{align}
\boldsymbol{q}_N&=\dfrac{\left(1+\zeta_N\overline{\zeta}_N\right)}{2\left(q_N^2+p_N^2\right)^2}\left(\left(\left(p_N^2-q_N^2\right)\partial_{q_S}+2q_Np_N\partial_{p_S}\right)+i\left(-2q_Np_N\partial_{q_S} +\left(p_N^2-q_N^2\right)\partial_{p_S}\right)\right),\nonumber\\
&=-\dfrac{\left(1+\zeta_N\overline{\zeta}_N\right)}{2\overline{\zeta}_N^2}\left(\partial_{q_S}+i\partial_{p_S}\right),\nonumber\\
&=-\dfrac{\overline{\zeta}_S}{\zeta_S}\dfrac{\left(1+\zeta_S\overline{\zeta}_S\right)}{2}\left(\partial_{q_S}+i\partial_{p_S}\right),\nonumber\\
&=-\dfrac{\overline{\zeta}_S}{\zeta_S}\boldsymbol{q}_S,
\label{spin4}
\end{align}
which is the transformation's rule for the dyads. It is worth stressing that, apparently this transformation appears as induced by the stereographic mapping used to make the finite coverage to the unit sphere, however it is a vector property that appears by the fact that the atlas is constructed from two local charts, whose centres are diametrically opposed. This result can be written in terms of components, as
\begin{equation}
q^A_N=e^{i \alpha}q^A_S,
\label{spin5}
\end{equation}
where the complex factor,
\begin{equation}
e^{i \alpha}=-\dfrac{\overline{\zeta}_S}{\zeta_S},
\label{spin6}
\end{equation}
is the spin-weight associated with the transformation of coordinates.\\
From \eqref{spin5} immediately is obtained the rule for the complex conjugate dyads components, 
\begin{equation}
\overline{q}^A_N=e^{-i \alpha}\overline{q}^A_S.
\label{spin7}
\end{equation}
In order to complete this description, it is necessary to examine the transformation rules of the covariant components of the dyads. Thus, expressing the dyads as linear combinations of the vectors,
 \begin{align}
\boldsymbol{q}_N=q_{A_N}\boldsymbol{e}^{A_N}, \hspace{1cm}\boldsymbol{q}_S=q_{A_S}\boldsymbol{e}^{A_S}.
\label{spin8}
 \end{align}
Then, using a local coordinate basis,
 \begin{align}
\boldsymbol{q}_N&=\dfrac{2}{\left(1+\zeta_N\overline{\zeta}_N\right)}\left(\delta^3_{~~A}+i\delta^4_{~~A}\right)dx^{A_N},\nonumber\\
&=\dfrac{2}{\left(1+\zeta_N\overline{\zeta}_N\right)}\left(dq_N+idp_N\right).
\label{spin9}
 \end{align}
Using the transformation rules \eqref{diff6}, it is obtained
 \begin{align*}
\boldsymbol{q}_N&=\dfrac{2}{\left(1+\zeta_N\overline{\zeta}_N\right)}\dfrac{1}{\left(q_S^2+p_S^2\right)^2}\left(\left(p_S^2-q_S^2\right) dq_S - 2q_Sp_S dp_S\right.\nonumber\\
&\hspace{0.5cm}+\left.i\left(2q_Sp_S dq_S+ \left(p_S^2-q_S^2\right) dp_S\right)\right),\\
&=-\dfrac{\overline{\zeta}_S}{\zeta_S}\dfrac{2}{\left(1+\zeta_S\overline{\zeta}_S\right)}\left( dq_S +i dp_S\right),
 \end{align*} 
or simply
 \begin{align*}
\boldsymbol{q}_N&=-\dfrac{\overline{\zeta}_S}{\zeta_S}\boldsymbol{q}_S.
 \end{align*} 
It shows that these transformation rules are completely consistent. Thus, we are enable to low the index with the metric of the unit sphere, from \eqref{spin5} and \eqref{spin7},
\begin{equation}
q_{A_N}=e^{i\alpha}q_{A_S}, \hspace{1cm} \overline{q}_{A_N}=e^{-i\alpha}\overline{q}_{A_S}.
\label{spin10}
\end{equation} 
It is worth mentioning that the metric of the unit sphere \eqref{decomposition1} has spin-weight zero, 
\begin{align*}
{q_N}_{(A}{\overline{q}_N}_{B)}&=e^{i\alpha}{q_S}_{(A}e^{-i\alpha}{\overline{q}_S}_{B)},\\
&={q_S}_{(A}{\overline{q}_S}_{B)}.
\end{align*}
The spin-weight of a finite product of these tangent vectors, depends on the number of $q_A$, $\overline{q}_A$, $q^A$ and $\overline{q}^A$ considered. For example, if is considered the product $\prod_{i=1}^n {q}_{Ai}$ of tangent vectors, then its transformation from north to south hemisphere is given by
\begin{align}
\prod_{i=1}^n {q_N}_{Ai}&=\prod_{i=1}^n e^{i\alpha}{q_S}_{Ai},\nonumber\\
&=\left(e^{i\alpha}\right)^n\prod_{i=1}^n {q_S}_{Ai}.
\label{spin11}
\end{align}
then, this implies that this product has a spin-weight of $s=n$. As an another example, if is considered the product $\prod_{i=1}^n {q}_{Ai} \prod_{j=n+1}^m {\overline{q}}_{Aj}$, then it transforms as
\begin{align}
\prod_{i=1}^n {q_N}_{Ai} \prod_{j=n+1}^m {\overline{q}_N}_{Aj}&=\prod_{i=1}^n e^{i\alpha}{q_S}_{Ai} \prod_{j=n+1}^m e^{-i\alpha}{\overline{q}_S}_{Aj},\nonumber\\
&=e^{i n\alpha}e^{-i(m-n)\alpha}\prod_{i=1}^n {q_S}_{Ai} \prod_{j=n+1}^m {\overline{q}_S}_{Aj},\nonumber\\
&=\left(e^{i \alpha}\right)^{(2n-m)}\prod_{i=1}^n {q_S}_{Ai} \prod_{j=n+1}^m {\overline{q}_S}_{Aj}.
\label{spin12}
\end{align}
which implies that its spin-weight is $s=2n-m$. Therefore, if is considered scalar quantities involving products like those given above, then these scalars must have spin-weight induced by these products. Thus, the scalar functions constructed trough the projection of the tensors onto these dyads, inherits the spin-weight carried by these dyads. This crucial point will be clarified in the next section.

==> docs/transforming_basis.tex <==
\section{Transforming the Coordinate Basis}
Developing explicitly \eqref{ethgen19} it is obtained
\begin{align*}
\eth\ _s\Psi&=q^3\ _s\Psi_{,x^3}+q^4\ _s\Psi_{,x^4}+s\zeta\ _s\Psi,
\end{align*}
and substituting the tangent vector components \eqref{decomposition10},
\begin{align}
\eth\ _s\Psi &=\dfrac{1+\zeta\overline{\zeta}}{2}\left(\ _s\Psi_{,q}+i\ _s\Psi_{,p}\right)+s\zeta\ _s\Psi.
\label{abase1}
\end{align}
Also, the explicit form for \eqref{ethgen24} is
\begin{align*}
\overline{\eth}\ _s\Psi&=\overline{q}^3\ _s\Psi_{,x^3}+\overline{q}^4\ _s\Psi_{,x^4}-s\overline{\zeta}\ _s\Psi,
\end{align*}
thus, making the replacement of the conjugates $\overline{q}^A$ 
\begin{align}
\overline{\eth}\ _s\Psi&= \dfrac{1+\zeta\overline{\zeta}}{2} \left(\ _s\Psi_{,q}-i \ _s\Psi_{,p}\right)-s\overline{\zeta}\ _s\Psi.
\label{abase2}
\end{align}
Then, from \eqref{abase1} and \eqref{abase2} 
\begin{subequations}
\begin{align}
_s\Psi_{,q}=\dfrac{\eth\ _s\Psi+\overline{\eth}\ _s\Psi -s(\zeta-\overline{\zeta}) \ _s\Psi}{1+\zeta\overline{\zeta}}
\label{abase3.1},\\
_s\Psi_{,p}=i\dfrac{\overline{\eth}\ _s\Psi - \eth\ _s\Psi+ s(\zeta+\overline{\zeta}) \ _s\Psi}{1+\zeta\overline{\zeta}}
\label{abase3.2}.
\end{align}
\label{abase3}
\end{subequations}
Or in terms of $q$ and $p$ they result as
\begin{subequations}
\begin{align}
_s\Psi_{,q}=\dfrac{\eth\ _s\Psi+\overline{\eth}\ _s\Psi -2isp \ _s\Psi}{1+q^2+p^2}
\label{abase4.1},\\
_s\Psi_{,p}=i\dfrac{\overline{\eth}\ _s\Psi - \eth\ _s\Psi+ 2sq \ _s\Psi}{1+q^2+p^2}
\label{abase4.2}.
\end{align}
\label{abase4}
\end{subequations}
Thus it implies that, the base vectors (or conversely the differential operators) $\partial_q$ and $\partial_p$ can be written as
\begin{subequations}
\begin{align}
\partial_{q}&=\dfrac{1}{1+\zeta\overline{\zeta}}\left(\eth +\overline{\eth} -s(\zeta-\overline{\zeta}) \right), \label{abase5.1}\\
\partial_{p}&=\dfrac{i}{1+\zeta\overline{\zeta}}\left(\overline{\eth}  - \eth + s(\zeta+\overline{\zeta})  \right).\label{abase5.2}
\end{align}
\label{abase5}
\end{subequations}
It worth stressing that, in these expression appear the spin-weight $s$ associated with the functions. Consequently these operators must be applied carefully in future computations, in order to avoid errors.  
\\Immediately from \eqref{abase1}, \eqref{abase2} and \eqref{abase3} it is possible to obtain the expressions for $_s\Psi_{,qq}$, $_s\Psi_{,qp}$ and $_s\Psi_{,pp}$. Here, will be started with $_s\Psi_{,qq}$. There are almost two forms to do it. We follows both in order to check the expressions. Thus, first will be considered the action of the derivative respect to $q$ on $ _s\Psi_{,q}$. Thus, using \eqref{abase3.1} one obtains
\begin{align}
_s\Psi_{,qq}=&\left(_s\Psi_{,q}\right)_{,q},\nonumber\\
=&\left(\dfrac{\eth\ _s\Psi+\overline{\eth}\ _s\Psi -s(\zeta-\overline{\zeta}) \ _s\Psi}{1+\zeta\overline{\zeta}}\right)_{,q},\nonumber\\
=&\left(\dfrac{1}{1+\zeta\overline{\zeta}}\right)_{,q}\left(\eth\ _s\Psi+\overline{\eth}\ _s\Psi -s(\zeta-\overline{\zeta}) \ _s\Psi\right)\nonumber\\
&+\left(\dfrac{1}{1+\zeta\overline{\zeta}}\right)\left(\eth\ _s\Psi+\overline{\eth}\ _s\Psi -s(\zeta-\overline{\zeta})\ _s\Psi\right)_{,q},
\label{abase6}
\end{align}
where 
\begin{align}
\left(\dfrac{1}{1+\zeta\overline{\zeta}}\right)_{,q}=-\dfrac{\zeta+\overline{\zeta}}{\left(1+\zeta\overline{\zeta}\right)^2},
\label{abase7}
\end{align}
and
\begin{align}
\left(\eth\ _s\Psi+\overline{\eth}\ _s\Psi -s(\zeta-\overline{\zeta})\ _s\Psi\right)_{,q}
&=\left(\eth\ _s\Psi\right)_{,q}+\left(\overline{\eth}\ _s\Psi\right)_{,q} -s (\zeta-\overline{\zeta})\ _s\Psi_{,q},
\label{abase8}
\end{align}
because $(\zeta-\overline{\zeta})_{,q}=0$.
The first term in \eqref{abase6} is
\begin{align}
&\left(\dfrac{1}{1+\zeta\overline{\zeta}}\right)_{,q}\left(\eth\ _s\Psi+\overline{\eth}\ _s\Psi -s(\zeta-\overline{\zeta}) \ _s\Psi\right)\nonumber\\
&=-\dfrac{\left(\zeta+\overline{\zeta}\right)\eth\ _s\Psi+\left(\zeta+\overline{\zeta}\right)\overline{\eth}\ _s\Psi
-s\left(\zeta^2-\overline{\zeta}^2\right) \ _s\Psi}{\left(1+\zeta\overline{\zeta}\right)^2}.
\label{abase9}
\end{align}
\\Each derivative in \eqref{abase8} is computed considering \eqref{ethgen27} and \eqref{abase3.1}. Then
\begin{subequations}
\begin{align}
\left(\eth\ _s\Psi\right)_{,q}&=\left(A_{s+1} \ _{s+1}\Psi\right)_{,q},\nonumber\\
&=\dfrac{\eth\left( _{s+1}\Psi\right)+\overline{\eth}\left(_{s+1}\Psi\right) -(s+1)(\zeta-\overline{\zeta}) \ _{s+1}\Psi}{1+\zeta\overline{\zeta}},\nonumber\\
&=\dfrac{\eth\left(\eth\ _s\Psi\right)+\overline{\eth}\left(\eth\ _s\Psi\right) -(s+1)(\zeta-\overline{\zeta}) \eth\ _s\Psi}{1+\zeta\overline{\zeta}},\nonumber\\
&=\dfrac{\eth^2\ _s\Psi+\overline{\eth}\eth\ _s\Psi -(s+1)(\zeta-\overline{\zeta}) \eth\ _s\Psi}{1+\zeta\overline{\zeta}},
\label{abase10.1}
\end{align}
and
\begin{align}
\left(\overline{\eth}\ _s\Psi\right)_{,q}&=\left(A_{s-1}\ _{s-1}\Psi\right)_{,q},\nonumber\\
&=\dfrac{\eth \left(_{s-1}\Psi\right)+\overline{\eth}\left(_{s-1}\Psi\right) -(s-1)(\zeta-\overline{\zeta}) \ _{s-1}\Psi}{1+\zeta\overline{\zeta}},\nonumber\\
&=\dfrac{\eth\left(\overline{\eth}\ _{s}\Psi\right)+\overline{\eth}\left(\overline{\eth}\ _{s}\Psi\right) -(s-1)(\zeta-\overline{\zeta}) \overline{\eth} _{s}\Psi}{1+\zeta\overline{\zeta}},\nonumber\\
&=\dfrac{\eth\overline{\eth}\ _{s}\Psi+\overline{\eth}^2\ _{s}\Psi -(s-1)(\zeta-\overline{\zeta}) \overline{\eth} _{s}\Psi}{1+\zeta\overline{\zeta}}.
\label{abase10.2}
\end{align}
\label{abase10}
\end{subequations}
Thus, substituting the relations \eqref{abase10} into \eqref{abase8} is obtained
\begin{align}
&\left(\eth\ _s\Psi+\overline{\eth}\ _s\Psi -s(\zeta-\overline{\zeta})\ _s\Psi\right)_{,q}\nonumber\\
=&\dfrac{1}{1+\zeta\overline{\zeta}}\left(\eth^2\ _s\Psi + \overline{\eth}^2\ _{s}\Psi + (\overline{\eth},\eth)\ _s\Psi -(2s+1)(\zeta-\overline{\zeta}) \eth\ _s\Psi  \right. \nonumber\\
&\left.-(2s-1)(\zeta-\overline{\zeta}) \overline{\eth} _{s}\Psi + s^2(\zeta-\overline{\zeta})^2  \ _s\Psi\right),
\label{abase11}
\end{align}
where were used the anti-commutator
\begin{equation}
\left(\overline{\eth},\eth\right)\ _s\Psi=\overline{\eth} \eth\ _s\Psi+ \eth\overline{\eth} \ _s\Psi.
\label{abase12}
\end{equation}
Then, \eqref{abase6} takes the form
\begin{subequations}
\begin{align}
_s\Psi_{,qq}
&=\dfrac{1}{\left(1+\zeta\overline{\zeta}\right)^2}\Bigg(\eth^2\ _s\Psi + \overline{\eth}^2\ _{s}\Psi + (\overline{\eth},\eth)\ _s\Psi +2\left(s\overline{\zeta}-(s+1)\zeta\right) \eth\ _s\Psi   \nonumber\\
&-2\left(s\zeta-(s-1)\overline{\zeta}\right)\overline{\eth}\ _s\Psi+ s\left(s(\zeta-\overline{\zeta})^2  \ _s\Psi +\left(\zeta^2-\overline{\zeta}^2\right) \ _s\Psi\right)\Bigg).
\label{abase13.1}
\end{align}
Then, the second order differential operator $\partial_{qq}$ can be written as
\begin{align}
\partial_{,qq}
&=\dfrac{1}{\left(1+\zeta\overline{\zeta}\right)^2}\Bigg(\eth^2\  + \overline{\eth}^2 + (\overline{\eth},\eth) +2\left(s\overline{\zeta}-(s+1)\zeta\right) \eth    \nonumber\\
&-2\left(s\zeta-(s-1)\overline{\zeta}\right)\overline{\eth}+ s\left(s(\zeta-\overline{\zeta})^2   +\left(\zeta^2-\overline{\zeta}^2\right) \right)\Bigg).
\label{abase13.2}
\end{align}
\label{abase13}
\end{subequations}
After of this,  $_s\Psi_{,pp}$ is computed using for this \eqref{abase3.2}. Thus
\begin{align}
_s\Psi_{,pp}&=\left( _s\Psi_{,p}\right)_{,p},\nonumber\\
=&\left( i\dfrac{\overline{\eth}\ _s\Psi-\eth\ _s\Psi +s(\zeta+\overline{\zeta})\ _s\Psi}{1+\zeta\overline{\zeta}}\right)_{,p},\nonumber\\
=&i\left(\left(\dfrac{1}{1+\zeta\overline{\zeta}}\right)_{,p}(\overline{\eth}\ _s\Psi-\eth\ _s\Psi +s(\zeta+\overline{\zeta})\ _s\Psi)\right.\nonumber\\
&\left.+\left(\dfrac{1}{1+\zeta\overline{\zeta}}\right)(\overline{\eth}\ _s\Psi-\eth\ _s\Psi +s(\zeta+\overline{\zeta})\ _s\Psi)_{,p}\right),
\label{abase14}
\end{align}
where
\begin{equation}
\left(\dfrac{1}{1+\zeta\overline{\zeta}}\right)_{,p}=\dfrac{i(\zeta-\overline{\zeta})}{\left(1+\zeta\overline{\zeta}\right)^2}.
\label{abase15}
\end{equation}
Then the first term in \eqref{abase14} is
\begin{align}
&\left(\dfrac{1}{1+\zeta\overline{\zeta}}\right)_{,p}(\overline{\eth}\ _s\Psi-\eth\ _s\Psi +s(\zeta+\overline{\zeta})\ _s\Psi)
\nonumber\\
=&i\dfrac{(\zeta-\overline{\zeta})\overline{\eth}\ _s\Psi-(\zeta-\overline{\zeta})\eth\ _s\Psi +s(\zeta^2-\overline{\zeta}^2)\ _s\Psi}{\left(1+\zeta\overline{\zeta}\right)^2}.
\label{abase16}
\end{align}
The second term can be spanned as
\begin{align}
(\overline{\eth}\ _s\Psi-\eth\ _s\Psi +s(\zeta+\overline{\zeta})\ _s\Psi)_{,p}
&=(\overline{\eth}\ _s\Psi)_{,p}-(\eth\ _s\Psi)_{,p} +s(\zeta+\overline{\zeta})\ _s\Psi_{,p},
\label{abase17}
\end{align}
where it is considered that $(\zeta+\overline{\zeta})_{,p}=0$.
\\Each term in the last equation can be computed, using for this \eqref{ethgen27} and \eqref{abase3.2}. They result as, 
\begin{subequations}
\begin{align}
\left(\overline{\eth}\ _s\Psi\right)_{,p}&=\left(A_{s-1}\ _{s-1}\Psi\right)_{,p},\nonumber\\
&=i\dfrac{\overline{\eth}\ _{s-1}\Psi-\eth\ _{s-1}\Psi +(s-1)(\zeta+\overline{\zeta})\ _{s-1}\Psi}{1+\zeta\overline{\zeta}},\nonumber\\
&=i\dfrac{\overline{\eth}\left(\overline{\eth}\ _{s}\Psi\right)-\eth\left(\overline{\eth}\ _{s}\Psi\right) +(s-1)(\zeta+\overline{\zeta})\overline{\eth}\ _{s}\Psi}{1+\zeta\overline{\zeta}},\nonumber\\
&=i\dfrac{\overline{\eth}^2\ _{s}\Psi-\eth\overline{\eth}\ _{s}\Psi +(s-1)(\zeta+\overline{\zeta})\overline{\eth}\ _{s}\Psi}{1+\zeta\overline{\zeta}},
\label{abase18.1}
\end{align}
and
\begin{align}
\left(\eth\ _s\Psi\right)_{,p}&=\left(A_{s+1}\ _{s+1}\Psi\right)_{,p},\nonumber\\
&=i\dfrac{\overline{\eth}\ _{s+1}\Psi-\eth\ _{s+1}\Psi +(s+1)(\zeta+\overline{\zeta})\ _{s+1}\Psi}{1+\zeta\overline{\zeta}},\nonumber\\
&=i\dfrac{\overline{\eth}\left(\eth\ _s\Psi\right)-\eth\left(\eth\ _s\Psi\right) +(s+1)(\zeta+\overline{\zeta})\eth\ _s\Psi}{1+\zeta\overline{\zeta}},\nonumber\\
&=i\dfrac{\overline{\eth}\eth\ _s\Psi-\eth^2\ _s\Psi +(s+1)(\zeta+\overline{\zeta})\eth\ _s\Psi}{1+\zeta\overline{\zeta}}.
\label{abase18.2}
\end{align}
\label{abase18}
\end{subequations}
The substitution of the relations \eqref{abase18} into \eqref{abase17} yields us to
\begin{align}
&(\overline{\eth}\ _s\Psi-\eth\ _s\Psi +s(\zeta+\overline{\zeta})\ _s\Psi)_{,p}\nonumber\\
=&\dfrac{i}{1+\zeta\overline{\zeta}}\Bigg(\eth^2\ _s\Psi + \overline{\eth}^2\ _{s}\Psi-(\eth,\overline{\eth})\ _{s}\Psi +(s-1)(\zeta+\overline{\zeta})\overline{\eth}\ _{s}\Psi    \nonumber\\
&-(s+1)(\zeta+\overline{\zeta})\eth\ _s\Psi+ s(\zeta+\overline{\zeta})\overline{\eth}\ _s\Psi-s(\zeta+\overline{\zeta}){\eth}\ _s\Psi+s^2(\zeta+\overline{\zeta})^2\ _s\Psi \Bigg).
\label{abase19}
\end{align}
Thus, substituting \eqref{abase16} and \eqref{abase19} into \eqref{abase14}
\begin{subequations}
\begin{align}
_s\Psi_{,pp}
&=-\dfrac{1}{\left(1+\zeta\overline{\zeta}\right)^2}\Bigg( \eth^2\ _s\Psi + \overline{\eth}^2\ _{s}\Psi-(\eth,\overline{\eth})\ _{s}\Psi +2(s\zeta +(s-1)\overline{\zeta})\overline{\eth}\ _{s}\Psi   \nonumber\\
& -2(s\overline{\zeta}+(s+1)\zeta)\eth\ _s\Psi +s\left(s\left(\zeta+\overline{\zeta}\right)^2  +\left(\zeta^2-\overline{\zeta}^2\right)\right)\ _s\Psi\Bigg),
\label{abase20.1}
\end{align}
i.e, the second order operator $\partial_{pp}$ is given by
\begin{align}
\partial_{,pp}
&=-\dfrac{1}{\left(1+\zeta\overline{\zeta}\right)^2}\Bigg( \eth^2 + \overline{\eth}^2 - (\eth,\overline{\eth}) +2(s\zeta +(s-1)\overline{\zeta})\overline{\eth}   
\nonumber\\
& -2(s\overline{\zeta}+(s+1)\zeta)\eth  +s\left(s\left(\zeta+\overline{\zeta}\right)^2  +\left(\zeta^2-\overline{\zeta}^2\right)\right)\Bigg).
\label{abase20.2}
\end{align}
\label{abase20}
\end{subequations}
Now, we will compute the mixed derivative $_s\Psi_{,qp}$ using for this \eqref{ethgen27} and \eqref{abase3}. In this form
\begin{align*}
_s\Psi_{,qp} =\left(_s\Psi_{,q}\right)_{,p},
\end{align*}
thus, using \eqref{abase3.1}
\begin{align}
_s\Psi_{,qp} =&\left(\dfrac{\eth\ _s\Psi+\overline{\eth}\ _s\Psi -s(\zeta-\overline{\zeta}) \ _s\Psi}{1+\zeta\overline{\zeta}}\right)_{,p},\nonumber\\
=&\left(\dfrac{1}{1+\zeta\overline{\zeta}}\right)_{,p}\left(\eth\ _s\Psi+\overline{\eth}\ _s\Psi -s(\zeta-\overline{\zeta}) \ _s\Psi\right)\nonumber\\
&+\dfrac{1}{1+\zeta\overline{\zeta}}\left(\eth\ _s\Psi+\overline{\eth}\ _s\Psi -s(\zeta-\overline{\zeta}) \ _s\Psi\right)_{,p}.
\label{abase21}
\end{align}
The first term in the last equation is given by
\begin{align}
&\left(\dfrac{1}{1+\zeta\overline{\zeta}}\right)_{,p}\left(\eth\ _s\Psi+\overline{\eth}\ _s\Psi -s(\zeta-\overline{\zeta}) \ _s\Psi\right)\nonumber\\
=&\dfrac{i}{\left(1+\zeta\overline{\zeta}\right)^2}\left((\zeta-\overline{\zeta})\eth\ _s\Psi+(\zeta-\overline{\zeta})\overline{\eth}\ _s\Psi -s(\zeta-\overline{\zeta})^2 \ _s\Psi\right),
\label{abase22}
\end{align}
where we have use \eqref{abase15}. The second term is computed using the equations \eqref{abase3} and \eqref{abase18}, thus
\begin{align}
&\dfrac{1}{1+\zeta\overline{\zeta}}\left(\eth\ _s\Psi+\overline{\eth}\ _s\Psi -s(\zeta-\overline{\zeta}) \ _s\Psi\right)_{,p}\nonumber\\
&=\dfrac{i}{\left(1+\zeta\overline{\zeta}\right)^2}\Bigg( \overline{\eth}^2\ _{s}\Psi - \eth^2\ _s\Psi + [\overline{\eth},\eth]\ _s\Psi  + \left((2s+1)\zeta + \overline{\zeta}\right)\eth\ _s\Psi  \nonumber\\
& +\left((2s-1)\overline{\zeta} -\zeta\right)\overline{\eth}\ _{s}\Psi  - s\left(2(1+\zeta\overline{\zeta}) + s (\zeta^2-\overline{\zeta}^2) \right)\ _s\Psi \Bigg),
\label{abase23}
\end{align}
where we have used the commutator
\begin{equation}
\left[\overline{\eth},\eth\right]=\overline{\eth}\eth - \eth\overline{\eth}.
\label{abase24}
\end{equation}
Then, the substitution of  \eqref{abase22} and \eqref{abase23} into \eqref{abase21} yields us to
\begin{subequations}
\begin{align}
_s\Psi_{,qp} 
&=\dfrac{i}{\left(1+\zeta\overline{\zeta}\right)^2}\Bigg( \overline{\eth}^2\ _{s}\Psi - \eth^2\ _s\Psi + [\overline{\eth},\eth]\ _s\Psi  + 2(s+1)\zeta \ \eth\ _s\Psi  \nonumber\\
& + 2(s-1)\overline{\zeta} \ \overline{\eth}\ _{s}\Psi  - s\left(2 + \zeta^2 +\overline{\zeta}^2 + s (\zeta^2-\overline{\zeta}^2)   \right)\ _s\Psi  
\Bigg).
\label{abase25.1}
\end{align}
it allows us to write that
\begin{align}
\partial_{,qp} 
&=\dfrac{i}{\left(1+\zeta\overline{\zeta}\right)^2}\Bigg( \overline{\eth}^2 - \eth^2 + [\overline{\eth},\eth]  + 2(s+1)\zeta \ \eth + 2(s-1)\overline{\zeta} \ \overline{\eth} \nonumber\\
&   - s\left(2 + \zeta^2 +\overline{\zeta}^2 + s (\zeta^2-\overline{\zeta}^2)   \right)  
\Bigg).
\label{abase25.2}
\end{align}
\label{abase25}
\end{subequations}
In order to test the consistency of this formalism, and with the goal to confirm \eqref{abase25}, we will compute the mixed derivative $_s\Psi_{,pq}$.
\\Thus,
\begin{equation*}
_s\Psi_{,pq}=\left(s\Psi_{,p}\right)_{,q}.
\end{equation*}
Then, using \eqref{abase3.2} is obtained
\begin{align}
_s\Psi_{,pq}=&\left(i\dfrac{\overline{\eth}\ _s\Psi - \eth\ _s\Psi+ s(\zeta+\overline{\zeta}) \ _s\Psi}{1+\zeta\overline{\zeta}}\right)_{,q},\nonumber\\
=&i\left(\left(\dfrac{1}{1+\zeta\overline{\zeta}}\right)_{,q} \left(\overline{\eth}\ _s\Psi - \eth\ _s\Psi+ s(\zeta+\overline{\zeta}) \ _s\Psi\right)\right. \nonumber\\
&\left. + 
\dfrac{1}{1+\zeta\overline{\zeta}} \left(\overline{\eth}\ _s\Psi - \eth\ _s\Psi+ s(\zeta+\overline{\zeta}) \ _s\Psi\right)_{,q}\right).
\label{abase26}
\end{align}
The first term in the last equation is given by
\begin{align}
&\left(\dfrac{1}{1+\zeta\overline{\zeta}}\right)_{,q} \left(\overline{\eth}\ _s\Psi - \eth\ _s\Psi+ s(\zeta+\overline{\zeta}) \ _s\Psi\right)
\nonumber\\
&=-\dfrac{1}{\left(1+\zeta\overline{\zeta}\right)^2} \left(\left(\zeta+\overline{\zeta}\right)\overline{\eth}\ _s\Psi - \left(\zeta+\overline{\zeta}\right)\eth\ _s\Psi+ s\left(\zeta+\overline{\zeta}\right)^2 \ _s\Psi\right),
\label{abase27}
\end{align}
where we have used \eqref{abase7}. The second term in \eqref{abase26} is computed taking into account the equations \eqref{abase3.1} and \eqref{abase10} 
\begin{align}
&\dfrac{1}{1+\zeta\overline{\zeta}} \left(\overline{\eth}\ _s\Psi - \eth\ _s\Psi+ s(\zeta+\overline{\zeta}) \ _s\Psi\right)_{,q}\nonumber\\
=&\dfrac{1}{1+\zeta\overline{\zeta}} \left(\left(\overline{\eth}\ _s\Psi\right)_{,q} - \left(\eth\ _s\Psi\right)_{,q}+ s(\zeta+\overline{\zeta}) \ _s\Psi\right)_{,q},\nonumber\\
=&\dfrac{1}{\left(1+\zeta\overline{\zeta}\right)^2}\Bigg(\overline{\eth}^2\ _{s}\Psi - \eth^2\ _s\Psi + [\eth,\overline{\eth}]\ _{s}\Psi  +((2s-1)\overline{\zeta}+\zeta) \overline{\eth} _{s}\Psi  \nonumber\\
& +((2s+1)\zeta-\overline{\zeta}) \eth\ _s\Psi +s\left(2(1+\zeta\overline{\zeta}) -s\left(\zeta^2-\overline{\zeta}^2\right)\right) \ _s\Psi \Bigg).
\label{abase28}
\end{align}
Then, substituting \eqref{abase27} and \eqref{abase28} into \eqref{abase26}
\begin{subequations}
\begin{align}
 _s\Psi_{,pq}
&= \dfrac{i}{\left(1+\zeta\overline{\zeta}\right)^2}\Bigg( \overline{\eth}^2\ _{s}\Psi - \eth^2\ _s\Psi + \left[\eth,\overline{\eth}\right]\ _{s}\Psi  +2(s-1)\overline{\zeta}\ \overline{\eth} _{s}\Psi   \nonumber\\
&+2(s+1)\zeta \eth\ _s\Psi +s\left(2- \zeta^2 - \overline{\zeta}^2 -s\left(\zeta^2-\overline{\zeta}^2\right) \right)\ _s\Psi \Bigg),
\label{abase29.1}
\end{align}
which allows to write that
\begin{align}
\partial_{,pq}
&= \dfrac{i}{\left(1+\zeta\overline{\zeta}\right)^2}\Bigg( \overline{\eth}^2 - \eth^2  + \left[\eth,\overline{\eth}\right]  +2(s-1)\overline{\zeta}\ \overline{\eth}  +2(s+1)\zeta \eth   \nonumber\\
& +s\left(2- \zeta^2 - \overline{\zeta}^2 -s\left(\zeta^2-\overline{\zeta}^2\right) \right) \Bigg),
\label{abase29.2}
\end{align}
\label{abase29}
\end{subequations}
Now, observing that
\begin{equation}
\left[\partial_q,\partial_p\right]\ _s\Psi=0,
\label{abase30}
\end{equation}
because $_s\Psi$ is supposed as a complex function with almost second derivative continuous. Then,  using \eqref{abase25} and \eqref{abase29}
\begin{align*}
_s\Psi_{,qp}-_s\Psi_{,pq}&=\dfrac{i}{\left(1+\zeta\overline{\zeta}\right)^2}\left(\left[\overline{\eth},\eth\right]-\left[\eth,\overline{\eth}\right]-4s\right)\ _s\Psi.
\end{align*}
It implies that
\begin{align*}
\left(\left[\overline{\eth},\eth\right]-\left[\eth,\overline{\eth}\right]-4s\right)\ _s\Psi&=\left(\left[\overline{\eth},\eth\right]+\left[\overline{\eth},\eth\right]-4s\right)\ _s\Psi, \nonumber\\
&=\left(2\left[\overline{\eth},\eth\right]-4s\right)\ _s\Psi,\nonumber\\
&=0,
\end{align*}
i.e., that the commutator of the $\eth$ and $\overline{\eth}$ satisfy an eigenvalue equation,
\begin{equation}
\left[\overline{\eth},\eth\right]\ _s\Psi=2s\ _s\Psi.
\label{abase31}
\end{equation}
It is worth stressing that, by using \eqref{ethgen27} it is obtained
\begin{align}
\left[\overline{\eth},\eth\right]\ _s\Psi&= \overline{\eth}\eth \ _s\Psi - \eth\overline{\eth} \ _s\Psi, \nonumber\\
&= \overline{\eth}\left(A_{s+1} \ _{s+1}\Psi\right) - \eth \left(A_{s-1} \ _{s-1}\Psi\right), \nonumber\\
&= A_{s+1}\overline{\eth}\left(  _{s+1}\Psi\right) - A_{s-1} \eth \left(  _{s-1}\Psi\right), \nonumber\\
&= A_{s}\left(A_{s+1}    - A_{s-1} \right) \ _{s}\Psi,
\label{abase32}
\end{align}
which defines the constant of structure for the group of function that satisfies \eqref{abase31}, i.e., 
\begin{equation}
A_{s}\left(A_{s+1} - A_{s-1} \right)=2s.
\label{abase33}
\end{equation}
Thus, was obtained the explicit form for the partial derivatives $\partial_q\ _s\Psi$ and $\partial_p \ _s\Psi$ as expressed in the equations \eqref{abase3}. With these expressions the mixed derivatives $\partial_{qq}\ _s\Psi$, $\partial_{pp}\ _s\Psi$, $\partial_{qp}\ _s\Psi$ and $\partial_{pq}\ _s\Psi$ were expressed as in \eqref{abase13.1}, \eqref{abase20.1}, \eqref{abase25.1} and \eqref{abase29.1} respectively. These equations allow us to write the explicit form of the second order operators $\partial_{qq}$, $\partial_{qp}$, $\partial_{pq}$ and $\partial_{pp}$ as given by \eqref{abase13.2}, \eqref{abase20.2}, \eqref{abase25.2} and \eqref{abase29.2} respectively, but it is important to highlight that $\partial_q$ and $\partial_p$ are commutable. With this last fact was derived the commutation rule for $\eth$ and $\overline{\eth}$, which is given in \eqref{abase31}. The last relation is particularly important because from this, are constructed the eigenfunctions for this eigenvalue equation. 

==> docs/unit_metric_decomposition.tex <==
\section{Decomposition for the Metric of the Unit Sphere}
The square of the line element that describes the $S^2$ manifold (the unit sphere) in spherical coordinates is given by
\begin{equation}
ds^2=d\theta^2+\sin^2\theta d\phi^2.
\label{angular1}
\end{equation}
Now, from \eqref{stereo2} the total differential of $\zeta$ and $\overline{\zeta}$ is computed i.e.,
\begin{subequations}
	\begin{align}
	d\zeta&=\zeta_{,\theta}d\theta+\zeta_{,\phi}d\phi, \label{angular2.1}\\
	d\overline{\zeta}&=\overline{\zeta}_{,\theta}d\theta+\overline{\zeta}_{,\phi}d\phi. \label{angular2.2}
	\end{align}
	\label{angular2}
\end{subequations}
Here the absence of the indices $N$ or $S$ means that the results are equal for the north and south hemispheres.
Thus, from \eqref{angular2} one obtains that
\begin{align*}
d\zeta d\overline{\zeta} &= \zeta_{,\theta}\overline{\zeta}_{,\theta}d\theta^2 +  \left(\zeta_{,\theta} \overline{\zeta}_{,\phi} + \zeta_{,\phi} \overline{\zeta}_{,\theta}\right) d\phi d\theta + \zeta_{,\phi} \overline{\zeta}_{,\phi}d\phi^2, \\
%&= \dfrac{1}{4}\sec^4\left(\dfrac{\theta}{2}\right) d\theta^2 + \tan^2\left(\dfrac{\theta}{2}\right) d\phi^2,\\
&= \dfrac{1}{4}\sec^4\left(\dfrac{\theta}{2}\right) \left(d\theta^2 + \sin^2\theta d\phi^2\right),\\
%&= \dfrac{1}{4}\left(1+\tan^2\left(\dfrac{\theta}{2}\right)\right)^2 \left(d\theta^2 + \sin^2\theta d\phi^2\right),\\
&= \dfrac{1}{4}\left(1+\zeta\overline{\zeta}\right)^2 \left(d\theta^2 + \sin^2\theta d\phi^2\right).
\end{align*}
Therefore, the unit sphere metric in terms of $\zeta,\overline{\zeta}$ takes the non-diagonal form,
\begin{equation}
d\theta^2 + \sin^2\theta d\phi^2=\dfrac{4}{\left(1+\zeta\overline{\zeta}\right)^2}d\zeta d\overline{\zeta}.
\label{angular3}
\end{equation}
Expressing the total derivatives $d\zeta$ and $d\overline{\zeta}$ as
\begin{equation}
d\zeta=dq+i dp, \hspace{1cm}d\overline{\zeta}=dq-i dp,
\label{angular4}
\end{equation}
then
\begin{equation}
d\zeta d\overline{\zeta}=dq^2+dp^2.
\label{angular5}
\end{equation}
For this reason, the element of line \eqref{angular3} can be written as,
\begin{equation}
d\theta^2 + \sin^2\theta d\phi^2=\dfrac{4}{\left(1+\zeta\overline{\zeta}\right)^2}\left(dq^2+dp^2\right).
\label{angular6}
\end{equation}
\\Now, it is admitted that the metric \eqref{angular6} can be decomposed in terms of a new complex vector $q_A$ in the form 
\begin{equation}
q_{AB}=q_{(A}\overline{q}_{B)}.
\label{decomposition1}
\end{equation}
%where the over-line indicates complex conjugation. 
This vector is related to the tangent vectors to the unit sphere along the coordinate lines. 
%It becomes directly from the line-element definition when expressed as linear combination of these tangent vectors. 
These two vectors $q_A$ and $\overline{q}_A$ that allow decompose the unit sphere metric, are knowing as dyads and it is said that the metric is written in terms of dyadic products. The metric and its inverse are related as
\begin{equation}
q_{AB}q^{BC}=\delta_A^{~~C},
\label{decomposition2}
\end{equation}
then,  in terms of these dyads one obtains
\begin{align}
\delta_A^{~~C}&=(q_{(A}\overline{q}_{B)})(q^{(B}\overline{q}^{C)}),\nonumber\\
&=\dfrac{1}{4}\left(q_{A}\overline{q}^{C}\overline{q}_{B}q^{B} +\overline{q}_{A}q^{C}q_{B}\overline{q}^{B} +\overline{q}_{A}\overline{q}^{C}q_{B}q^{B}+q_{A}q^{C}\overline{q}_{B}\overline{q}^{B}\right).
\label{decomposition3}
\end{align}
Imposing that,
\begin{equation}
\overline{q}_{B}q^{B}=2, \hspace{1cm}\overline{q}_{B}\overline{q}^{B}=0,
\label{decomposition4}
\end{equation}
the expression \eqref{decomposition3} is reduced to
\begin{align}
\delta_A^{~~C}&=\dfrac{1}{2}\left(q_{A}\overline{q}^{C} +\overline{q}_{A}q^{C}\right),\nonumber\\
&=q_{(A}\overline{q}^{C)}. 
\label{decomposition5}
\end{align}
From \eqref{angular6} and \eqref{decomposition1},
\begin{equation}
\dfrac{4}{\left(1+\zeta\overline{\zeta}\right)^2}\delta_{AB}=q_{(A}\overline{q}_{B)},
\label{decomposition7}
\end{equation}
it is obtained
\begin{equation*}
|q_{3}|^2=\dfrac{4}{\left(1+\zeta\overline{\zeta}\right)^2}, \hspace{1cm}|q_{4}|^2=\dfrac{4}{\left(1+\zeta\overline{\zeta}\right)^2}.
\end{equation*}
Thus, it is possible to make the choice
\begin{equation*}
q_{3}=\dfrac{2}{\left(1+\zeta\overline{\zeta}\right)}, \hspace{1cm}q_{4}=\dfrac{2i}{\left(1+\zeta\overline{\zeta}\right)}.
\end{equation*}
For this reason, the complex vectors $q_A$ can be written as,
\begin{equation}
q_{A}=\dfrac{2}{\left(1+\zeta\overline{\zeta}\right)}\left(\delta^3_{~A}+i\delta^4_{~A}\right), \hspace{1cm} \overline{q}_{A}=\dfrac{2}{\left(1+\zeta\overline{\zeta}\right)}\left(\delta^3_{~A}-i\delta^4_{~A}\right).
\label{decomposition8}
\end{equation}
Raising the index of $q_A$ with the metric $q^{AB}$ one obtains
\begin{equation}
q^{A}
=\dfrac{\left(1+\zeta\overline{\zeta}\right)}{2}\left(\delta^A_{~~3}+i\delta^A_{~~4}\right),\hspace{1cm}
\overline{q}^{A}=\dfrac{\left(1+\zeta\overline{\zeta}\right)}{2}\left(\delta^A_{~~3}-i\delta^A_{~~4}\right).
\label{decomposition10}
\end{equation}
It is worth stressing that, if the spherical coordinates are used, then \eqref{decomposition1} can be written as,
\begin{equation}
\begin{pmatrix}
1 & 0 \\
0 & \sin^2\theta
\end{pmatrix}=\begin{pmatrix}
q_3\overline{q}_3 & q_3\overline{q}_4 + \overline{q}_3q_4 \\
q_3\overline{q}_4 + \overline{q}_3q_4 & q_4\overline{q_4}
\end{pmatrix},
\label{eth_spherical_1}
\end{equation}
which implies that the spherical dyads take the form
\begin{subequations}
\begin{align}
q_A=\delta^{~~3}_A+i\sin\theta\delta^{~~4}_A, \hspace{1cm} \overline{q}_A=\delta^{~~3}_A-i\sin\theta\delta^{~~4}_A,\\
q^A=\delta^A_{~~3}+i\csc\theta\delta^A_{~~4}, \hspace{1cm} \overline{q}^A=\delta^A_{~~3}-i\csc\theta\delta^A_{~~4}. 
\label{eth_spherical_2}
\end{align}
\end{subequations} 

==> pdftohtmlB <==
#!/usr/bin/perl
#########################################################3
print "Script \t\"pdftohtmlB \" \n\t(Convert: PDF -> HTML)\n\nAuthor: Bruno Roth (roth\@lit.inpe.br)\n\n\n";

print "USE:\n\tpdftohtmlB PDF DEVICE RESOLUTION PAGE_SIZE_HTML [IMG|NOIMG]\n\n";
print "OPTIONS:\n";
print "\tPDF: \t\tfile\n";
print "\tDEVICE: \tpngmono pnggray png16 png256 png16m jpeg jpeggray \n";
print "\tRESOLUTION: \tpixels/inch resolution\n";
print "\tPAGE_SIZE_HTML: page (HTML) size in pixels\n";
print "\tIMG | NOIMG: \"Create/Not create\" device image\n";
#print "\tUPDATE_DEVICE_IMG: update device image#\n";

print "\n\nEX:\n\tpdftohtmlB file.pdf jpeg 100 500x0 IMG \n\n\n";


if(@ARGV != 5){
	exit;
}
########################################################3
#Configure

$namepdf="../@ARGV[0]";
$basenamefig = "./p";

if (grep(/png/,@ARGV[1])){
	$fig="png";
}
else{
	$fig="jpg";
}
@reshtml = split(/x/,@ARGV[3]);
$width=@reshtml[0];#842;
$height=@reshtml[1];#595;

$dpi=@ARGV[2];

@namepdfTMPL =  split(/\./,@ARGV[0]);
$namepdfTMP = @namepdfTMPL[0];
$dirhtml="html$namepdfTMP";

#print @ARGV[0],$namepdf,$basenamefig,$fig,$width,$height,$dirhtml;
#exit;


###########################################################################

mkdir($dirhtml,0777);
chdir($dirhtml);

####################
if (!@ARGV[5]=="0"){
	system("/usr/bin/gs -r$dpi -dNOPAUSE -dBATCH -sDEVICE=@ARGV[1] -sOutputFile=$basenamefig@ARGV[5].$fig -dFirstPage=@ARGV[5] -dLastPage=@ARGV[5] $namepdf");
	exit();
}
######################

$cont = -1;
$beginHtml="
<!DOCTYPE html PUBLIC \"-//W3C//DTD HTML 4.01 Transitional//EN\">
<html>
<head>
  <meta http-equiv=\"content-type\" content=\"text/html; charset=ISO-8859-1\">
  <link href=\"./html.css\" rel=\"stylesheet\" type=\"text/css\">
</head>
<body bgcolor=\"#FFFFFF\">
<table border=1 width=\"100%\" >
<tr align=\"center\" valign=\"top\" >
";
$endHtml="
</tr>
</table>
</body>
</html>
";

$beginFigure = "<div align=\"center\"><img src=\"";
$endFigure= "\"";

if(!$width=="0"){
        $endFigure = "$endFigure width=\"$width\"";
}

if(!$height=="0"){
	$endFigure = "$endFigure height=\"$height\"";
}

$endFigure= "$endFigure border=\"0\" align=\"middle\"></div>";
#$endFigure= "\" border=\"0\" align=\"middle\"></div>";

$htmlcss="
body {
        background-color: white;
}
";
####################
system("/bin/echo \"$htmlcss\" > html.css");
######################

####################
#system("/usr/bin/gs -r$dpi -dNOPAUSE -dBATCH -sDEVICE=@ARGV[1] -sOutputFile=$basenamefig\%d.$fig $namepdf");
if (!grep(/NOIMG/,@ARGV[4])){
	system("/usr/bin/gs -r$dpi -dNOPAUSE -dBATCH -sDEVICE=@ARGV[1] -sOutputFile=$basenamefig\%d.$fig $namepdf");
}
######################


@filespng = qx!ls *.$fig!;
$firstpage = -1; 
$lastpage = scalar(@filespng)-2; 
while($line = <@filespng>){
print "PAGE: $cont\n";

open(OUT,">$basenamefig$cont.html");
print OUT $beginHtml,"\n";
print OUT "<td>";
print OUT "<B>PAG: $cont</B><br><HR>";
#print OUT "<B>NAVEGAÇÃO:</B><br>";
print OUT "<a href=\"./$basenamefig$firstpage.html\">[INICIO]</A><BR>";
$tmp = scalar($cont) + 50;
if ($tmp>$lastpage){$tmp=$lastpage;}
print OUT "<a href=\"./$basenamefig$tmp.html\">[+50]</A><BR>";
$tmp = scalar($cont) + 10;
if ($tmp>$lastpage){$tmp=$lastpage;}
print OUT "<a href=\"./$basenamefig$tmp.html\">[+10]</A><BR>";
$tmp = scalar($cont) + 5;
if ($tmp>$lastpage){$tmp=$lastpage;}
print OUT "<a href=\"./$basenamefig$tmp.html\">[+05]</A><BR>";
$tmp = scalar($cont) + 1;
if ($tmp>$lastpage){$tmp=$lastpage;}
print OUT "<a href=\"./$basenamefig$tmp.html\">[+01]</A><BR>";
$tmp = scalar($cont) - 1;
if ($tmp<$firstpage){$tmp=$firstpage;}
print OUT "<a href=\"./$basenamefig$tmp.html\">[-01]</A><BR>";
$tmp = scalar($cont) - 5;
if ($tmp<$firstpage){$tmp=$firstpage;}
print OUT "<a href=\"./$basenamefig$tmp.html\">[-05]</A><BR>";
$tmp = scalar($cont) - 10;
if ($tmp<$firstpage){$tmp=$firstpage;}
print OUT "<a href=\"./$basenamefig$tmp.html\">[-10]</A><BR>";
$tmp = scalar($cont) - 50;
if ($tmp<$firstpage){$tmp=$firstpage;}
print OUT "<a href=\"./$basenamefig$tmp.html\">[-50]</A><BR>";

print OUT "<a href=\"./$basenamefig$lastpage.html\">[FIM]</A><BR>";

print OUT "<HR>";
#print OUT "<a href=\"./@ARGV[0]\">[@ARGV[0]]</a><BR>";
print OUT "<a href=\"../@ARGV[0]\">[PDF]</a><BR>";


#for($cont2=1 ; $cont2 <= scalar(@filespng) ; $cont2++){
#	print OUT "<a href=\"./$basenamefig$cont2.html\">[$cont2]</a> ";
#}
$contAux = $cont+2;
print OUT "</td>";
	print OUT "<td><a href=$basenamefig$contAux.$fig>",$beginFigure,$basenamefig,$contAux,".",$fig,$endFigure,"</a></td>","\n",; 	
	print OUT $endHtml;
close(OUT);
	$cont = $cont + 1;


}

exit;

